Applications of QR-based Vector-Valued Rational Approximation

Several applications of the QR-AAA algorithm, a greedy scheme for vector-valued rational approximation, are presented. The focus is on demonstrating the flexibility and practical effectiveness of QR-AAA in a variety of computational settings, including Stokes flow computation, multivariate rational approximation, function extension, the development of novel quadrature methods and near-field approximation in the boundary element method.

==> aaaErr.tex <==
0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,1.5133e-07,0,1.4822e-05,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,1.0068e-05,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,2.8701e-08,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,6.7976e-06,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0,0
0.0052632,2.5015e-05,5.0756e-06,1.4559e-06,2.4665e-07,3.8602e-08,1.6435e-07,5.4598e-06,4.0838e-05,1.2861e-06,6.0436e-06,1.1031e-07,5.8869e-08,3.1074e-07,4.2091e-06,9.7366e-06,2.3728e-05,2.6062e-05,6.6298e-06,7.8463e-07,2.0089e-07,4.1624e-08,4.5196e-07,4.3886e-07,4.3039e-06,1.6189e-06,8.3751e-07,1.4074e-07,4.1315e-08,1.0223e-07,1.266e-06,1.1766e-05,2.6235e-05,2.1794e-05,1.0411e-05,1.0949e-05,9.7046e-08,9.2331e-08,1.066e-06,1.1633e-06,3.5952e-06,2.1654e-06,3.0753e-06,1.498e-07,7.4961e-08,1.7106e-07,8.7947e-07,1.0952e-05,5.456e-05,2.5923e-05,1.6034e-06,7.2224e-07,2.6257e-07,5.1397e-08,1.1934e-07,2.5157e-07,4.571e-07,6.3696e-07,1.9002e-07,2.0137e-07,5.6869e-08,1.6186e-07,4.0985e-06,4.8286e-06,1.6002e-05,1.9428e-05,1.5419e-05,6.6645e-07,3.5349e-07,3.0626e-08,1.0118e-07,1.6801e-07,1.1909e-06,3.0866e-07,1.3648e-07,4.4266e-08,2.2767e-08,1.6652e-07,4.416e-07,3.8815e-06,1.9069e-05,1.9886e-05,5.9498e-06,2.9384e-07,2.895e-07,4.5916e-08,2.8499e-08,3.7764e-07,3.5075e-07,1.3458e-07,1.2828e-07,1.9296e-08,2.242e-07,2.782e-07,4.4412e-07,1.2539e-06,2.358e-05,1.447e-05,1.6647e-06,3.3197e-07,5.5561e-07,3.4884e-07,1.4454e-08,3.9065e-08,3.2836e-07,7.2627e-08,4.2837e-08,1.878e-08,9.8768e-08,2.6044e-07,3.7973e-07,3.1772e-06,1.6028e-05,1.3898e-05,1.427e-06,1.8324e-07,1.0093e-07,1.4396e-07,1.1561e-08,2.4819e-08,1.2155e-07,2.766e-07,1.2749e-08,2.1622e-08,2.8053e-07,1.1433e-07,1.4397e-07,9.3423e-07,1.0048e-05,1.2325e-05,4.8519e-07,3.499e-07,3.838e-08,8.2152e-08,5.347e-09,6.1996e-08,2.3384e-06,1.1995e-07,5.9154e-08,1.2827e-08,8.6582e-08,4.2574e-08,3.8594e-07,6.535e-07,1.1962e-05,2.6755e-05,1.2082e-06,2.9437e-07,2.9512e-07,2.8994e-08,3.5238e-08,1.5794e-07,2.1148e-07,3.9567e-07,7.4812e-08,2.6471e-08,3.1867e-08,1.5095e-07,2.4177e-07,4.0041e-07,1.0132e-05,1.4951e-05,4.5563e-07,1.3171e-07,1.1103e-07,1.878e-07,3.7711e-07,1.8604e-07,4.471e-07,2.5271e-06,2.0266e-07,3.4448e-07,3.8911e-08,1.8703e-07,1.7449e-07,4.8513e-07,8.8545e-06,8.3878e-06,1.3759e-06,1.3022e-07,1.5187e-07,6.0764e-09,1.2854e-07,7.1968e-07,2.124e-05,1.3116e-05,7.3113e-07,1.0297e-07,6.1034e-09,1.6182e-07,1.2824e-07,3.8879e-07,7.0858e-06,7.1274e-06,6.7274e-07,1.6275e-08,1.9804e-08,1.2866e-08,1.0824e-08,3.5736e-07,1.8367e-06,2.2387e-06,3.6718e-08,2.427e-08,3.1077e-08,1.9647e-07,8.8235e-08,3.7739e-07,6.8684e-06,6.5582e-06,3.5122e-07,5.1261e-08,3.2167e-08,5.0895e-09,1.5345e-08,1.1675e-07,4.8826e-07,6.1923e-07,1.399e-07,7.0013e-09,6.308e-09,4.5314e-08,5.3536e-08,2.2808e-07,8.1662e-06,6.2884e-06,9.0151e-07,2.3522e-08,4.5697e-09,3.8088e-09,6.7318e-09,8.4649e-08,4.9824e-07,2.1742e-07,1.5418e-07,8.466e-09,1.0462e-07,6.0463e-08,2.902e-08,5.8552e-07,6.5356e-06,5.1179e-06,1.2034e-07,2.3442e-08,6.6199e-09,3.9857e-09,6.1679e-09,3.5624e-07,1.5457e-07,7.8997e-08,6.2276e-08,8.0296e-08,1.5487e-08,1.2956e-08,2.4285e-08,1.2087e-06,6.3971e-06,6.6499e-06,1.5755e-07,2.8989e-08,4.9096e-09,8.7883e-09,7.3621e-09,7.7742e-08,3.6553e-07,1.1428e-07,1.0055e-07,8.3876e-09,1.1861e-08,7.2259e-09,2.8332e-08,5.9368e-07,6.5811e-06,6.8208e-06,2.3336e-07,5.0657e-08,1.9602e-08,3.8886e-09,1.7521e-07,1.1143e-07,2.8631e-07,3.4802e-07,1.3614e-07,8.5998e-09,7.0754e-09,3.8469e-08,5.5096e-08,2.0421e-07,6.4202e-06,6.9705e-06,4.5679e-07,7.8039e-08,2.3804e-07,1.0653e-08,5.5703e-08,8.9943e-07,5.6151e-07,1.2736e-06,6.0767e-08,2.3819e-07,4.9854e-09,2.0025e-08,9.2937e-08,2.5928e-07,7.6364e-06,8.1233e-06,3.4822e-07,1.1894e-07,3.9678e-08,2.8903e-09,7.8751e-08,4.1375e-06,8.1596e-06,9.1248e-06,7.678e-07,1.6931e-07,3.1307e-08,5.9091e-08,1.1997e-07,4.2419e-07,9.1567e-06,1.0057e-05,3.9026e-07,1.1954e-07,1.5777e-07,2.8396e-08,4.9984e-07,1.4183e-07,4.7226e-07,4.7752e-07,2.0911e-07,2.0779e-07,1.4121e-07,1.6124e-07,1.615e-07,4.9215e-07,8.7966e-06,1.6132e-05,7.5125e-07,2.1917e-07,3.7748e-07,6.1179e-08,2.3861e-08,9.9962e-08,1.6096e-07,2.0416e-07,2.7124e-07,1.88e-08,2.9638e-08,1.1136e-07,1.792e-07,1.2275e-06,9.1198e-06,1.0332e-05,2.8125e-07,3.741e-07,3.9794e-07,9.3572e-08,2.8439e-08,1.0698e-07,4.03e-07,3.9149e-07,5.7799e-08,8.75e-09,9.7445e-08,3.5632e-08,3.8624e-07,7.933e-07,1.2562e-05,1.0844e-05,9.0896e-07,6.4402e-08,1.1153e-07,3.4409e-07,1.3994e-08,4.1135e-08,2.1541e-07,5.0841e-07,4.8358e-08,1.2083e-08,3.2349e-07,3.3394e-08,2.941e-07,5.8255e-07,1.2514e-05,1.8379e-05,9.2561e-06,3.2359e-07,3.7893e-07,9.0563e-08,1.8196e-08,4.5399e-08,7.5099e-07,1.8788e-07,1.4854e-07,1.3953e-08,3.1302e-07,2.7591e-07,3.9594e-07,1.3574e-06,2.7439e-05,2.0494e-05,2.3337e-06,1.3683e-06,2.1408e-07,6.3463e-08,2.3569e-08,1.267e-07,3.767e-07,6.0674e-07,1.1632e-07,3.3586e-08,1.3495e-07,1.8755e-07,4.0847e-07,2.8637e-06,2.0069e-05,1.7419e-05,2.3551e-06,1.2876e-06,2.2783e-07,6.8147e-08,7.044e-08,1.2852e-07,1.5085e-07,4.8002e-07,1.088e-07,9.2891e-08,3.235e-07,1.619e-07,3.6397e-07,3.2489e-06,1.6128e-05,2.1195e-05,2.1917e-06,2.8455e-06,4.5569e-07,4.7071e-08,2.5756e-07,2.4386e-07,7.8724e-06,1.5595e-06,2.7375e-07,4.056e-07,5.8653e-08,3.884e-07,1.48e-06,5.1985e-06,5.5273e-06,2.5285e-05,3.3723e-06,2.423e-06,1.1741e-07,7.2497e-08,4.8852e-08,1.2289e-06,1.3041e-06,2.5007e-06,1.1675e-06,1.054e-07,2.177e-07,9.7142e-08,1.9744e-06,2.5899e-06,3.1752e-05,3.2668e-05,2.3938e-05,1.4173e-06,1.0334e-06,3.9714e-08,1.655e-07,4.6687e-07,1.5273e-06,2.645e-06,5.6249e-07,2.4361e-07,6.797e-08,4.7362e-07,1.4881e-06,1.9367e-05,2.9281e-05,2.2202e-05,2.7211e-05,2.6525e-06,2.1587e-07,5.2585e-08,8.1246e-08,4.0062e-07,4.4668e-06,1.214e-05,1.1102e-06,1.1764e-07,6.7597e-08,3.3589e-07,2.3562e-06,2.8663e-05,2.8686e-05,1.338e-05,3.2224e-05,1.074e-05,1.8076e-07,1.7681e-07,1.2464e-07,7.8541e-07,1.0817e-05,5.7688e-06,3.9743e-05,2.5744e-06,2.9543e-07,8.5911e-08,9.6201e-07,2.1683e-05,1.0504e-05
0.010526,1.9469e-05,6.9392e-06,1.7335e-06,3.1862e-07,5.1195e-08,2.2238e-07,6.2942e-06,3.6866e-05,1.6298e-06,8.3831e-06,1.4713e-07,7.9925e-08,4.0855e-07,4.3942e-06,1.0594e-05,1.7942e-05,1.7554e-05,1.1021e-05,1.0383e-06,2.5844e-07,5.6684e-08,6.4647e-07,5.7282e-07,5.2854e-06,1.926e-06,1.1019e-06,1.9183e-07,5.0395e-08,1.3176e-07,1.4719e-06,6.2036e-06,1.7881e-05,1.7228e-05,1.1896e-05,5.8515e-06,1.2639e-07,1.3363e-07,1.7065e-06,1.4601e-06,1.5227e-06,2.339e-06,3.7021e-06,1.9626e-07,1.0599e-07,1.5612e-07,1.07e-06,6.6812e-06,1.9634e-05,2.6529e-05,2.7593e-06,9.1821e-07,3.7308e-07,7.1739e-08,1.4637e-07,3.3471e-07,5.3057e-07,7.5315e-07,2.473e-07,2.6616e-07,7.7068e-08,2.1562e-07,4.6509e-06,6.3951e-06,1.3834e-05,1.484e-05,8.2585e-06,8.9208e-07,5.1878e-07,4.1119e-08,1.431e-07,2.2742e-07,1.0471e-07,3.6292e-07,1.804e-07,5.9102e-08,3.0835e-08,2.2026e-07,5.4971e-07,4.9412e-06,1.4823e-05,1.6925e-05,4.5558e-06,3.5839e-07,3.5505e-07,5.9916e-08,4.0497e-08,4.7881e-07,4.5896e-07,1.5905e-07,1.6814e-07,2.6814e-08,2.57e-07,3.4392e-07,5.6953e-07,1.5599e-06,1.7929e-05,8.9965e-06,1.9324e-06,4.2447e-07,9.4445e-07,1.2428e-07,2.0231e-08,4.5091e-08,3.7055e-07,8.8345e-08,5.6642e-08,2.6355e-08,1.3817e-07,3.656e-07,4.7984e-07,2.5394e-06,1.6182e-05,1.0731e-05,1.4761e-06,2.1418e-07,1.1378e-07,1.9062e-07,1.5915e-08,3.3795e-08,1.3519e-07,3.1667e-07,1.7958e-08,3.0996e-08,3.9002e-07,1.3357e-07,1.6753e-07,9.0167e-07,6.5025e-06,1.1788e-05,3.5381e-07,4.6174e-07,5.5034e-08,1.1269e-07,7.3419e-09,8.3791e-08,1.2338e-06,1.4758e-07,7.9452e-08,1.8155e-08,1.1943e-07,5.3176e-08,5.2768e-07,6.1163e-07,1.1144e-05,1.8905e-05,2.1484e-06,4.2141e-07,2.3792e-07,3.9463e-08,5.2096e-08,2.1307e-07,2.534e-07,4.8836e-07,9.6875e-08,3.7002e-08,4.3375e-08,2.2483e-07,3.2129e-07,2.4085e-07,8.257e-06,9.7009e-06,3.8233e-07,1.9573e-07,1.6637e-07,3.3988e-07,5.2076e-07,2.4482e-07,5.4941e-07,2.0643e-06,2.6765e-07,4.9735e-07,5.0442e-08,3.4743e-07,2.2794e-07,4.3442e-07,7.6497e-06,7.7372e-06,7.2932e-07,1.5479e-07,1.5374e-07,8.5879e-09,1.6266e-07,9.9302e-07,2.4056e-05,1.7537e-05,9.2259e-07,1.357e-07,8.5686e-09,1.6182e-07,1.5374e-07,3.2144e-07,6.2652e-06,6.6728e-06,7.9307e-07,2.4218e-08,2.8395e-08,1.8912e-08,1.5066e-08,4.7505e-07,1.9431e-06,2.3005e-06,4.6343e-08,3.4763e-08,4.8688e-08,1.0598e-07,4.359e-08,3.4879e-07,6.2039e-06,6.2849e-06,4.2814e-07,6.6526e-08,4.9416e-08,7.5791e-09,2.2351e-08,1.4515e-07,5.8227e-07,7.4487e-07,1.9878e-07,9.7172e-09,9.0807e-09,7.4008e-08,7.0492e-08,1.8791e-07,8.1393e-06,6.2113e-06,1.1039e-06,3.0156e-08,6.1742e-09,5.4248e-09,9.6445e-09,1.1357e-07,6.0389e-07,2.8747e-07,2.1538e-07,1.1872e-08,1.4989e-07,5.2802e-08,3.2242e-08,1.0207e-06,6.3906e-06,4.7412e-06,1.1987e-07,3.1296e-08,9.9921e-09,5.9014e-09,8.7405e-09,1.6491e-07,2.1494e-07,1.0062e-07,8.3154e-08,1.2188e-07,2.1698e-08,2.0326e-08,3.2829e-08,2.1858e-06,6.3137e-06,6.5708e-06,1.5915e-07,3.7588e-08,6.6181e-09,1.2767e-08,1.0365e-08,1.0374e-07,4.7165e-07,1.4141e-07,1.3656e-07,1.1802e-08,1.7399e-08,1.0138e-08,3.6681e-08,7.303e-07,6.4934e-06,6.6326e-06,2.0014e-07,6.5681e-08,2.8023e-08,5.5227e-09,1.49e-07,1.5396e-07,3.3896e-07,4.1475e-07,1.8905e-07,1.2083e-08,1.0523e-08,6.1624e-08,7.1928e-08,3.5983e-07,6.026e-06,6.3685e-06,4.5823e-07,1.0073e-07,1.901e-07,1.5307e-08,7.2495e-08,6.4169e-07,6.5266e-07,1.3972e-06,7.6709e-08,2.5583e-07,7.7751e-09,2.4879e-08,1.2411e-07,2.3164e-07,7.3598e-06,7.4355e-06,2.5783e-07,1.5038e-07,4.7562e-08,3.72e-09,1.1043e-07,5.1943e-06,9.5217e-06,9.9299e-06,1.0567e-06,2.4819e-07,4.4813e-08,7.0445e-08,1.3938e-07,3.7077e-07,8.2133e-06,8.0838e-06,2.6956e-07,1.6031e-07,2.7033e-07,4.0091e-08,7.4276e-07,1.836e-07,5.9436e-07,5.2003e-07,2.7875e-07,2.8547e-07,2.1091e-07,2.7932e-07,2.1174e-07,4.252e-07,7.646e-06,1.4523e-05,7.2942e-07,2.8417e-07,1.8407e-07,8.779e-08,3.2695e-08,1.3073e-07,1.6634e-07,2.3212e-07,3.3678e-07,2.579e-08,4.0163e-08,1.5764e-07,2.2703e-07,1.5264e-06,7.3921e-06,8.2811e-06,3.6073e-07,5.045e-07,1.8912e-07,1.297e-07,4.2717e-08,1.5864e-07,5.3205e-07,3.8466e-07,7.7501e-08,1.2375e-08,1.3528e-07,5.2408e-08,5.2763e-07,8.1429e-07,1.086e-05,8.2322e-06,8.8907e-07,1.4167e-07,1.2708e-07,4.9189e-07,1.9575e-08,5.5149e-08,2.5399e-07,5.2479e-07,6.563e-08,1.6609e-08,4.5937e-07,2.1597e-08,1.9911e-07,7.3465e-07,1.1248e-05,1.1421e-05,4.4234e-06,4.0815e-07,5.6452e-07,1.2878e-07,2.5718e-08,6.012e-08,7.5403e-07,2.2204e-07,2.4814e-07,1.9545e-08,4.6709e-07,3.8636e-07,5.2566e-07,1.2062e-06,1.7799e-05,1.5908e-05,2.8915e-06,7.4881e-07,2.8888e-07,8.6219e-08,3.31e-08,1.6624e-07,4.9295e-07,8.9943e-07,1.5192e-07,4.8147e-08,1.6644e-07,2.4682e-07,3.5222e-07,3.1307e-06,1.451e-05,1.625e-05,2.3744e-06,1.8616e-06,3.2599e-07,9.2135e-08,9.6648e-08,1.6935e-07,1.7824e-07,5.7126e-07,1.4175e-07,1.318e-07,3.4243e-07,2.2288e-07,4.7484e-07,3.6494e-06,1.1331e-05,1.7305e-05,2.7835e-06,4.3137e-06,6.9583e-07,6.4693e-08,3.3318e-07,3.235e-07,7.2997e-06,1.9002e-06,3.6539e-07,5.4863e-07,8.1942e-08,4.7993e-07,1.8424e-06,6.9624e-06,1.2668e-05,1.9181e-05,4.1595e-06,3.43e-06,1.558e-07,1.0126e-07,6.5206e-08,1.544e-06,1.7361e-06,3.9765e-06,1.4639e-06,1.3954e-07,1.1133e-07,1.2674e-07,2.6686e-06,2.8141e-06,2.5768e-05,2.7712e-05,1.6163e-05,2.2114e-06,5.7612e-07,5.4108e-08,2.3917e-07,6.2273e-07,1.8717e-06,3.533e-06,7.3045e-07,3.4045e-07,9.3965e-08,6.5857e-07,1.606e-06,2.6446e-05,2.3403e-05,1.5911e-05,1.2106e-05,3.5575e-06,2.8258e-07,7.1635e-08,1.0685e-07,5.0775e-07,5.2978e-06,1.4029e-05,1.4132e-06,1.5638e-07,9.3187e-08,4.4119e-07,2.0385e-06,1.8685e-05,1.2186e-05,1.2096e-05,2.412e-05,4.9368e-06,2.4427e-07,2.2696e-07,1.6458e-07,1.0239e-06,1.1915e-05,5.994e-06,2.8487e-05,4.3884e-06,3.8502e-07,1.0426e-07,1.1019e-06,2.0527e-05,4.9507e-06
0.015789,1.1154e-05,1.1743e-05,1.5276e-06,3.0459e-07,5.0337e-08,2.2274e-07,5.4593e-06,2.6746e-05,1.5242e-06,8.6032e-06,1.4509e-07,8.0321e-08,3.9746e-07,3.6289e-06,1.0971e-05,1.0121e-05,1.081e-05,1.3597e-05,1.0025e-06,2.4596e-07,5.7173e-08,6.8877e-07,5.5471e-07,4.8355e-06,1.6928e-06,1.0789e-06,1.9329e-07,4.6779e-08,1.2556e-07,1.2735e-06,2.6095e-05,1.0201e-05,1.1193e-05,1.1786e-05,3.3684e-06,1.2153e-07,1.4419e-07,2.1435e-06,1.3559e-06,4.9615e-06,1.8874e-06,3.2956e-06,1.895e-07,1.1122e-07,1.291e-07,9.6017e-07,1.6691e-05,8.7046e-06,1.9194e-05,2.9594e-06,8.6334e-07,3.9991e-07,7.4244e-08,1.3039e-07,3.2969e-07,4.5794e-07,6.5706e-07,2.3789e-07,2.591e-07,7.7411e-08,2.1228e-07,4.2274e-06,6.6823e-06,8.7601e-06,1.192e-05,4.7587e-06,8.9346e-07,5.7131e-07,4.1097e-08,1.5014e-07,2.2854e-07,7.6682e-07,3.1716e-07,1.7644e-07,5.8238e-08,3.1018e-08,2.1813e-07,5.0813e-07,4.8136e-06,1.193e-05,1.3508e-05,6.8365e-06,3.2181e-07,3.3024e-07,5.796e-08,4.2622e-08,4.4829e-07,4.5251e-07,1.396e-07,1.6322e-07,2.7538e-08,2.2697e-07,3.2271e-07,5.4464e-07,1.5541e-06,1.2959e-05,4.6637e-06,1.6779e-06,4.064e-07,1.2797e-06,7.3918e-08,2.0938e-08,4.0084e-08,3.1597e-07,7.9738e-08,5.5387e-08,2.7331e-08,1.4309e-07,3.7857e-07,4.5203e-07,1.8417e-06,1.5896e-05,8.3535e-06,1.1838e-06,1.8568e-07,9.5723e-08,1.8568e-07,1.6196e-08,3.4018e-08,1.1471e-07,2.7265e-07,1.8659e-08,3.2938e-08,3.9778e-07,1.1827e-07,1.4477e-07,6.8638e-07,3.0015e-06,7.5178e-06,2.0762e-07,4.5215e-07,5.8335e-08,1.1422e-07,7.4292e-09,8.3787e-08,7.4403e-07,1.3477e-07,7.8953e-08,1.8993e-08,1.2182e-07,4.9644e-08,5.4228e-07,4.8395e-07,9.3183e-06,1.1092e-05,7.5838e-07,4.7261e-07,2.1374e-07,3.9741e-08,5.7663e-08,2.1319e-07,2.2483e-07,4.4743e-07,9.2642e-08,3.8226e-08,4.3668e-08,2.4969e-07,3.2097e-07,1.0197e-07,4.9165e-06,5.8211e-06,2.7236e-07,2.1688e-07,1.877e-07,4.8354e-07,5.3687e-07,2.3839e-07,5.0249e-07,1.3711e-06,2.6159e-07,5.3648e-07,4.8903e-08,1.4152e-07,2.2179e-07,3.3573e-07,4.9256e-06,5.3575e-06,1.9691e-06,1.4496e-07,1.241e-07,8.9909e-09,1.5584e-07,1.0106e-06,2.0175e-05,1.9156e-05,8.635e-07,1.3434e-07,8.9004e-09,1.2983e-07,1.4431e-07,2.1575e-07,4.2868e-06,4.593e-06,7.492e-07,3.0345e-08,3.0209e-08,2.061e-08,1.5487e-08,4.6762e-07,1.5786e-06,1.8339e-06,4.3153e-08,3.6864e-08,5.7036e-08,3.6454e-07,2.5621e-08,2.5872e-07,4.1521e-06,4.3998e-06,4.4114e-07,6.406e-08,5.69e-08,8.4323e-09,2.4191e-08,1.3404e-07,5.1667e-07,6.6801e-07,2.1118e-07,9.9515e-09,9.6854e-09,9.353e-08,6.9216e-08,1.2518e-07,5.908e-06,4.6682e-06,1.0645e-06,2.855e-08,6.1664e-09,5.7212e-09,1.0247e-08,1.1283e-07,5.4723e-07,2.8563e-07,2.2401e-07,1.2291e-08,1.5974e-07,3.8365e-08,3.1081e-08,1.2035e-06,4.5545e-06,3.0905e-06,1.0669e-07,3.0873e-08,1.1138e-08,6.4784e-09,9.1815e-09,2.3877e-07,2.294e-07,9.5656e-08,8.228e-08,1.3771e-07,2.2452e-08,2.394e-08,3.2836e-08,1.8255e-06,4.5884e-06,4.7694e-06,1.3249e-07,3.6072e-08,6.62e-09,1.3738e-08,1.0787e-08,1.0245e-07,4.659e-07,1.3001e-07,1.3848e-07,1.2286e-08,1.8918e-08,1.0549e-08,3.5158e-08,6.9667e-07,4.7139e-06,4.766e-06,1.4293e-07,6.3181e-08,2.9665e-08,5.8041e-09,1.1049e-07,1.5801e-07,2.9791e-07,3.6734e-07,1.953e-07,1.2535e-08,1.1629e-08,7.508e-08,6.6287e-08,2.4353e-07,4.1263e-06,4.2078e-06,3.7123e-07,9.6583e-08,1.3661e-07,1.6224e-08,7.0151e-08,4.6128e-07,5.6706e-07,1.1622e-06,7.1803e-08,2.1503e-07,8.9941e-09,2.3458e-08,1.2395e-07,2.2646e-07,5.3286e-06,5.1055e-06,1.4505e-07,1.4382e-07,4.3138e-08,3.4913e-09,1.1453e-07,3.1153e-06,8.2189e-06,7.8837e-06,1.0707e-06,2.713e-07,4.7627e-08,6.4136e-08,1.3883e-07,2.6882e-07,5.4974e-06,7.4291e-06,1.3568e-07,1.5856e-07,3.6913e-07,4.1733e-08,8.3169e-07,1.7564e-07,5.5821e-07,4.2434e-07,2.7535e-07,2.901e-07,2.3321e-07,3.8948e-07,2.0755e-07,3.0267e-07,4.9997e-06,1.0423e-05,5.8473e-07,2.7461e-07,5.1785e-07,9.3683e-08,3.31e-08,1.2644e-07,1.3908e-07,1.9584e-07,3.254e-07,2.6104e-08,4.0236e-08,1.6484e-07,2.1299e-07,1.5803e-06,4.4441e-06,4.9769e-06,4.5094e-07,5.0845e-07,6.4795e-07,1.3297e-07,4.792e-08,1.8091e-07,5.248e-07,2.9469e-07,7.7065e-08,1.2934e-08,1.3884e-07,5.6982e-08,5.4153e-07,7.023e-07,7.1152e-06,6.5947e-06,6.8888e-07,5.1965e-08,1.0834e-07,5.1696e-07,2.0262e-08,5.4661e-08,2.2196e-07,4.461e-07,6.5941e-08,1.6857e-08,4.7956e-07,8.3562e-09,1.0995e-07,7.6064e-07,9.1045e-06,6.2715e-06,2.8508e-06,3.8287e-07,6.2579e-07,1.3594e-07,2.6899e-08,5.8867e-08,5.9468e-07,1.9619e-07,1.5286e-07,2.0247e-08,5.1736e-07,3.9808e-07,5.2523e-07,9.1376e-07,1.0132e-05,1.208e-05,2.8103e-06,9.5236e-07,2.932e-07,8.6531e-08,3.4388e-08,1.6162e-07,4.8573e-07,1.0776e-06,1.4688e-07,5.117e-08,1.5336e-07,2.4367e-07,6.1836e-07,2.6504e-06,1.1446e-05,1.2938e-05,1.8138e-06,2.0861e-06,3.4878e-07,9.1933e-08,9.8014e-08,1.6512e-07,1.5606e-07,5.057e-07,1.3653e-07,1.388e-07,2.8066e-07,2.2857e-07,4.6578e-07,3.1079e-06,7.1538e-06,1.311e-05,3.0594e-06,4.6795e-06,8.0834e-07,6.5769e-08,3.2012e-07,3.1763e-07,5.4003e-06,1.7063e-06,3.6117e-07,5.4554e-07,8.4797e-08,4.5588e-07,1.7118e-06,7.3259e-06,3.5499e-06,1.3126e-05,3.9714e-06,3.6317e-06,1.5307e-07,1.0463e-07,6.4547e-08,1.4354e-06,1.7558e-06,5.2203e-06,1.3579e-06,1.3653e-07,8.1201e-08,1.2215e-07,2.6687e-06,2.4685e-06,2.0596e-05,1.8688e-05,1.8397e-05,2.6648e-06,7.6319e-07,5.4601e-08,2.5799e-07,6.1841e-07,1.7023e-06,3.5493e-06,7.0278e-07,3.5316e-07,9.6127e-08,6.8124e-07,1.314e-06,2.673e-05,1.4698e-05,8.613e-06,1.2825e-05,3.5972e-06,2.7471e-07,7.2296e-08,1.0383e-07,4.7338e-07,4.658e-06,1.2101e-05,1.3348e-06,1.54e-07,9.5195e-08,4.287e-07,1.4066e-06,1.9967e-05,6.0477e-06,6.7606e-06,4.026e-05,6.6954e-06,2.4421e-07,2.1593e-07,1.607e-07,9.8543e-07,9.762e-06,4.7003e-06,1.912e-05,2.3252e-06,3.7333e-07,9.3356e-08,9.4681e-07,1.5338e-05,3.0935e-06
0.021053,5.8126e-06,1.1109e-05,1.1787e-06,2.5499e-07,4.3513e-08,1.9549e-07,4.1907e-06,1.7805e-05,1.2443e-06,7.7234e-06,1.2518e-07,7.0713e-08,3.386e-07,2.7121e-06,1.1554e-05,5.2464e-06,6.9817e-06,1.3863e-05,8.3287e-07,2.0469e-07,5.0548e-08,6.4774e-07,4.7171e-07,3.8972e-06,1.3107e-06,9.3123e-07,1.7032e-07,3.8702e-08,1.0466e-07,9.7089e-07,1.1925e-05,5.5111e-06,7.0102e-06,1.2128e-05,1.9461e-06,1.0204e-07,1.3757e-07,2.6094e-06,1.1024e-06,2.61e-06,1.3447e-06,2.5663e-06,1.5951e-07,1.0258e-07,9.9505e-08,7.5206e-07,9.035e-06,3.9071e-06,1.5185e-05,2.5748e-06,7.0982e-07,3.8816e-07,6.7464e-08,9.9349e-08,2.8453e-07,3.4759e-07,5.0046e-07,2.0018e-07,2.1982e-07,6.82e-08,1.8278e-07,3.5542e-06,6.9717e-06,4.8659e-06,8.9718e-06,2.7462e-06,7.9141e-07,5.6119e-07,3.623e-08,1.3843e-07,2.0192e-07,1.1082e-06,2.4369e-07,1.5113e-07,5.0137e-08,2.7454e-08,1.9099e-07,4.1268e-07,4.0992e-06,8.9644e-06,9.3411e-06,3.8417e-06,2.5152e-07,2.7449e-07,4.9169e-08,3.9335e-08,3.6695e-07,3.998e-07,1.0763e-07,1.3885e-07,2.474e-08,1.8015e-07,2.7042e-07,4.6e-07,1.3623e-06,9.6409e-06,2.2738e-06,1.2703e-06,3.4595e-07,6.256e-07,1.4233e-07,1.8964e-08,3.2103e-08,2.3971e-07,6.3175e-08,4.7405e-08,2.4783e-08,1.2986e-07,3.4178e-07,3.7451e-07,1.2642e-06,1.424e-05,6.6791e-06,8.4893e-07,1.4133e-07,7.0962e-08,1.5758e-07,1.4427e-08,2.996e-08,8.7148e-08,2.0797e-07,1.6928e-08,3.0726e-08,3.5219e-07,9.4057e-08,1.0978e-07,4.8145e-07,1.1763e-06,5.6875e-06,1.2541e-07,3.8815e-07,5.4102e-08,1.0122e-07,6.5524e-09,7.3362e-08,4.5723e-07,1.0806e-07,6.8699e-08,1.7381e-08,1.0874e-07,4.0923e-08,4.9717e-07,3.7366e-07,7.3451e-06,6.0596e-06,9.192e-07,5.1355e-07,2.0661e-07,3.5051e-08,5.6811e-08,1.8735e-07,1.7466e-07,3.599e-07,7.741e-08,3.454e-08,3.8487e-08,2.4487e-07,2.8697e-07,7.2206e-08,2.5442e-06,3.1995e-06,1.9346e-07,2.0811e-07,1.8843e-07,6.6821e-07,4.8905e-07,2.0335e-07,4.0478e-07,8.4396e-07,2.2399e-07,5.1408e-07,4.192e-08,1.6362e-07,1.9043e-07,2.5423e-07,2.7568e-06,3.2364e-06,1.147e-06,1.2167e-07,9.2116e-08,8.2546e-09,1.333e-07,8.9739e-07,1.5203e-05,8.8709e-06,7.0729e-07,1.1777e-07,8.0982e-09,9.6106e-08,1.2121e-07,1.4217e-07,2.6133e-06,2.699e-06,6.4303e-07,2.9823e-08,2.8238e-08,1.9711e-08,1.3914e-08,4.0317e-07,1.1521e-06,1.3206e-06,3.5074e-08,3.426e-08,5.9282e-08,2.0044e-07,2.2354e-08,1.7888e-07,2.4815e-06,2.6259e-06,4.2819e-07,5.4198e-08,5.8315e-08,8.306e-09,2.3052e-08,1.0878e-07,4.0334e-07,5.2813e-07,1.9931e-07,8.8986e-09,9.0619e-09,1.1122e-07,6.0147e-08,7.9103e-08,3.6796e-06,3.0432e-06,9.3523e-07,2.3622e-08,5.386e-09,5.289e-09,9.5597e-09,9.8275e-08,4.3844e-07,2.5208e-07,2.0559e-07,1.1115e-08,1.5002e-07,2.5873e-08,2.6213e-08,1.1335e-06,2.7534e-06,1.6388e-06,8.693e-08,2.6644e-08,1.0852e-08,6.2415e-09,8.4654e-09,2.6701e-07,2.2637e-07,8.0369e-08,7.1434e-08,1.3726e-07,2.0303e-08,2.5158e-08,2.8777e-08,1.9488e-06,2.8341e-06,2.9471e-06,9.94e-08,3.033e-08,5.8152e-09,1.2961e-08,9.8191e-09,8.8657e-08,4.2289e-07,1.0508e-07,1.2406e-07,1.1203e-08,1.805e-08,9.6383e-09,2.9538e-08,5.9519e-07,2.9157e-06,2.9285e-06,9.9146e-08,5.3392e-08,2.7525e-08,5.3431e-09,7.8138e-08,1.427e-07,2.2985e-07,2.8594e-07,1.7785e-07,1.1363e-08,1.1307e-08,8.3333e-08,5.5666e-08,2.4595e-07,2.4157e-06,2.3442e-06,2.7919e-07,8.148e-08,9.4376e-08,1.5011e-08,5.9694e-08,3.3235e-07,4.3497e-07,8.6166e-07,5.9125e-08,1.641e-07,9.138e-09,1.9841e-08,1.0983e-07,2.2826e-07,3.349e-06,3.0487e-06,7.3369e-08,1.2187e-07,3.4895e-08,2.8223e-09,1.0395e-07,1.9813e-06,6.3488e-06,5.5034e-06,9.4456e-07,2.6226e-07,4.4472e-08,5.2515e-08,1.2461e-07,1.9053e-07,3.1972e-06,3.8828e-06,8.8384e-08,1.3721e-07,1.7955e-07,3.7887e-08,8.3818e-07,1.4696e-07,4.6309e-07,3.0686e-07,2.3866e-07,2.5845e-07,2.2588e-07,1.7637e-07,1.8046e-07,2.0962e-07,2.8604e-06,7.0432e-06,4.4522e-07,2.3451e-07,2.8233e-07,8.8099e-08,2.9301e-08,1.0703e-07,1.0443e-07,1.4508e-07,2.8666e-07,2.3067e-08,3.527e-08,1.5054e-07,1.7517e-07,1.54e-06,2.3211e-06,2.6987e-06,4.5034e-07,4.5346e-07,3.4499e-07,1.1934e-07,4.766e-08,1.9297e-07,4.5771e-07,2.0445e-07,6.7235e-08,1.1824e-08,1.2463e-07,5.4175e-08,4.9561e-07,5.4968e-07,4.1917e-06,5.6841e-06,4.9192e-07,6.1531e-08,8.1598e-08,4.7258e-07,1.8373e-08,4.7398e-08,1.6962e-07,3.4913e-07,5.8055e-08,1.4949e-08,4.3556e-07,2.6336e-08,5.6717e-08,6.8013e-07,7.1773e-06,3.2701e-06,1.9654e-06,3.163e-07,6.1013e-07,1.2616e-07,2.4641e-08,5.0438e-08,4.2664e-07,1.5316e-07,1.567e-07,1.8356e-08,5.0336e-07,3.5645e-07,4.692e-07,6.5628e-07,5.4748e-06,9.1412e-06,2.4228e-06,1.0066e-06,2.6408e-07,7.5901e-08,3.1284e-08,1.378e-07,4.2843e-07,6.1823e-07,1.2439e-07,4.774e-08,1.2472e-07,2.1289e-07,7.4554e-07,1.9932e-06,8.7959e-06,1.0046e-05,1.2406e-06,2.1927e-06,3.3101e-07,8.0098e-08,8.6945e-08,1.41e-07,1.1972e-07,3.9394e-07,1.1504e-07,1.2842e-07,2.0771e-07,2.0704e-07,4.0715e-07,2.3362e-06,4.2702e-06,9.6045e-06,2.8077e-06,4.2152e-06,8.567e-07,5.854e-08,2.7032e-07,2.732e-07,3.6593e-06,1.3363e-06,3.1292e-07,4.7182e-07,7.694e-08,3.8826e-07,1.4017e-06,7.3737e-06,1.705e-06,8.6689e-06,3.3891e-06,3.4072e-06,1.3177e-07,9.4656e-08,5.6107e-08,1.1683e-06,1.6098e-06,2.5324e-06,1.1026e-06,1.1687e-07,9.3653e-08,1.0287e-07,2.3334e-06,1.9829e-06,1.5702e-05,1.1905e-05,1.8081e-05,2.9897e-06,8.2492e-07,4.8301e-08,2.4628e-07,5.4145e-07,1.3589e-06,3.1841e-06,5.9288e-07,3.2198e-07,8.6118e-08,6.2209e-07,9.5643e-07,2.3178e-05,8.4264e-06,4.2583e-06,1.2679e-05,3.2625e-06,2.3507e-07,6.3993e-08,8.8231e-08,3.8369e-07,3.5892e-06,9.1975e-06,1.1063e-06,1.33e-07,8.5308e-08,3.6465e-07,8.9418e-07,2.0089e-05,3.1209e-06,3.4044e-06,2.5691e-05,7.2057e-06,2.139e-07,1.8012e-07,1.3732e-07,8.2898e-07,7.038e-06,3.2783e-06,1.2609e-05,2.4586e-06,3.187e-07,7.2915e-08,7.1583e-07,1.0423e-05,1.6716e-06
0.026316,2.9185e-06,1.1036e-05,8.3833e-07,1.968e-07,3.4929e-08,1.583e-07,2.988e-06,1.1252e-05,9.3308e-07,6.3753e-06,9.9477e-08,5.7429e-08,2.6594e-07,1.8959e-06,1.1285e-05,2.6533e-06,3.6634e-06,9.6507e-06,6.2538e-07,1.5667e-07,4.1251e-08,5.6708e-07,3.7096e-07,2.9117e-06,9.6798e-07,7.4685e-07,1.3812e-07,2.9835e-08,8.0311e-08,6.8642e-07,6.1247e-06,2.9473e-06,4.5256e-06,6.3051e-06,1.113e-06,7.8721e-08,1.2255e-07,1.2184e-06,8.2604e-07,1.4485e-06,8.8988e-07,1.8398e-06,1.2318e-07,8.7605e-08,7.2666e-08,5.4141e-07,5.1716e-06,1.7519e-06,1.1808e-05,2.0164e-06,5.3693e-07,3.6947e-07,5.6724e-08,6.7646e-08,2.2656e-07,2.4417e-07,3.5036e-07,1.5514e-07,1.7112e-07,5.5489e-08,1.4492e-07,2.8889e-06,3.6519e-06,2.528e-06,6.7292e-06,1.5602e-06,6.5214e-07,5.2126e-07,2.9692e-08,1.1823e-07,1.6529e-07,1.4413e-06,1.7325e-07,1.1936e-07,3.9727e-08,2.2534e-08,1.5552e-07,3.0994e-07,3.1545e-06,6.7068e-06,6.6515e-06,2.2439e-06,1.7999e-07,2.1424e-07,3.85e-08,3.3529e-08,2.766e-07,3.3601e-07,7.6723e-08,1.09e-07,2.0472e-08,1.3413e-07,2.1221e-07,3.6147e-07,1.0821e-06,5.6357e-06,1.0864e-06,8.8279e-07,2.7675e-07,6.2645e-07,3.7489e-07,1.5828e-08,2.4168e-08,1.6975e-07,4.6242e-08,3.7395e-08,2.0688e-08,1.0875e-07,2.8291e-07,2.8658e-07,8.2454e-07,1.2275e-05,5.4326e-06,5.6586e-07,9.9475e-08,4.8762e-08,1.2274e-07,1.1849e-08,2.4306e-08,6.2104e-08,1.4754e-07,1.4119e-08,2.6509e-08,2.8504e-07,7.0827e-08,7.6844e-08,3.2232e-07,4.466e-07,4.4863e-06,8.6398e-08,3.0683e-07,4.6247e-08,8.2575e-08,5.2996e-09,5.922e-08,2.8007e-07,8.008e-08,5.5115e-08,1.4649e-08,8.9456e-08,3.1307e-08,4.2982e-07,2.8341e-07,5.6332e-06,3.1973e-06,9.9722e-07,2.7599e-07,3.2569e-07,2.851e-08,5.2829e-08,1.5235e-07,1.25e-07,2.6742e-07,5.9484e-08,2.8742e-08,3.1269e-08,2.2345e-07,2.4403e-07,7.3451e-08,1.2127e-06,1.6617e-06,1.3774e-07,1.6103e-07,1.7742e-07,2.2747e-07,4.1462e-07,1.6004e-07,3.0242e-07,4.976e-07,1.7698e-07,4.6374e-07,3.3435e-08,1.6947e-07,1.5205e-07,1.8827e-07,1.4232e-06,1.8102e-06,6.9733e-07,9.5424e-08,6.5346e-08,6.9997e-09,1.0696e-07,7.3207e-07,1.1102e-05,7.0039e-06,5.3237e-07,9.5983e-08,6.7976e-09,6.8124e-08,9.5073e-08,9.6872e-08,1.5048e-06,1.4431e-06,5.2198e-07,2.5555e-08,2.4433e-08,1.7424e-08,1.1502e-08,3.2039e-07,7.8952e-07,8.96e-07,2.6192e-08,2.9388e-08,5.7778e-08,1.2043e-07,2.0114e-08,1.1977e-07,1.5647e-06,1.4374e-06,3.9832e-07,4.2445e-08,5.6292e-08,7.6369e-09,2.0397e-08,8.1641e-08,2.9141e-07,3.873e-07,1.7699e-07,7.3145e-09,7.8343e-09,1.395e-07,4.8901e-08,5.0397e-08,2.1016e-06,1.8363e-06,7.8535e-07,1.7985e-08,4.3293e-09,4.5139e-09,8.2515e-09,7.9038e-08,3.2687e-07,2.0777e-07,1.7562e-07,9.2422e-09,1.3093e-07,1.6582e-08,2.0486e-08,8.9679e-07,1.5312e-06,7.5593e-07,6.6932e-08,2.119e-08,9.7317e-09,5.559e-09,7.2174e-09,2.6871e-07,2.2581e-07,6.2908e-08,5.7325e-08,1.2727e-07,1.6889e-08,2.4998e-08,2.3285e-08,1.7872e-06,1.5891e-06,1.6562e-06,6.9375e-08,2.3535e-08,4.7234e-09,1.1291e-08,8.2327e-09,7.0788e-08,3.8152e-07,7.8584e-08,1.0341e-07,9.4264e-09,1.5916e-08,8.145e-09,2.2922e-08,4.7726e-07,1.6419e-06,1.641e-06,6.8868e-08,4.1758e-08,2.3572e-08,4.5372e-09,5.381e-08,1.1959e-07,1.638e-07,2.0583e-07,1.5054e-07,9.4758e-09,1.0191e-08,9.071e-08,4.3691e-08,2.3881e-07,1.3772e-06,1.1742e-06,2.0105e-07,6.3744e-08,6.354e-08,1.2769e-08,4.7007e-08,2.3733e-07,3.0968e-07,5.9669e-07,4.5244e-08,1.1844e-07,8.5908e-09,1.5826e-08,9.119e-08,2.1597e-07,1.9409e-06,1.6813e-06,3.6787e-08,9.6116e-08,2.6404e-08,2.0675e-09,8.6933e-08,1.2788e-06,4.6816e-06,3.5847e-06,7.6309e-07,2.3676e-07,3.8409e-08,4.0574e-08,1.1088e-07,1.3698e-07,1.7176e-06,2.0013e-06,1.0683e-07,1.0962e-07,1.8089e-07,3.1566e-08,8.1233e-07,1.1327e-07,3.5737e-07,2.0695e-07,1.9125e-07,2.128e-07,2.0172e-07,1.7828e-07,1.4695e-07,1.4847e-07,1.5185e-06,4.8262e-06,3.2997e-07,1.868e-07,1.6205e-07,7.7007e-08,2.3881e-08,8.3475e-08,1.1238e-07,9.9353e-08,2.4097e-07,1.8734e-08,2.8485e-08,1.2626e-07,1.3302e-07,1.4587e-06,1.1081e-06,1.3933e-06,3.5889e-07,3.7695e-07,1.9828e-07,9.8733e-08,4.4454e-08,2.1588e-07,3.7175e-07,1.3382e-07,5.4178e-08,9.9538e-09,1.03e-07,4.7419e-08,4.2751e-07,3.9978e-07,2.332e-06,1.8789e-06,3.3442e-07,6.9541e-08,5.7078e-08,3.9564e-07,1.5371e-08,3.7855e-08,1.1917e-07,2.9594e-07,4.7165e-08,1.2193e-08,3.6245e-07,4.2236e-08,2.9378e-08,5.4235e-07,3.2854e-06,1.6473e-06,1.3727e-06,2.4241e-07,5.4951e-07,1.0848e-07,2.0818e-08,3.9815e-08,2.8968e-07,1.1115e-07,1.4931e-07,1.5337e-08,4.5283e-07,2.9141e-07,3.9654e-07,4.5269e-07,2.8552e-06,2.5626e-06,1.9357e-06,9.8e-07,2.2182e-07,6.125e-08,2.6245e-08,1.0849e-07,3.5886e-07,5.5211e-07,9.7153e-08,4.1193e-08,9.411e-08,1.729e-07,7.8108e-07,1.3904e-06,6.7878e-06,5.6958e-06,7.9483e-07,2.4045e-06,2.9441e-07,6.414e-08,7.1029e-08,1.1104e-07,8.4649e-08,2.8428e-07,8.9285e-08,1.0994e-07,1.4491e-07,1.7503e-07,3.3378e-07,1.615e-06,2.488e-06,7.202e-06,2.2877e-06,3.2687e-06,8.9434e-07,4.8043e-08,2.1126e-07,2.1675e-07,2.3535e-06,9.6103e-07,2.5025e-07,3.7357e-07,6.4463e-08,3.0954e-07,1.0632e-06,4.2989e-06,9.1917e-07,5.8957e-06,2.7224e-06,2.9866e-06,1.0465e-07,7.8928e-08,4.5115e-08,8.7641e-07,1.4305e-06,2.3564e-06,8.2503e-07,9.2161e-08,2.0918e-07,7.9662e-08,1.8752e-06,1.5125e-06,1.2031e-05,6.5849e-06,1.6721e-05,3.4539e-06,8.1412e-07,3.9443e-08,2.1961e-07,4.4046e-07,1.002e-06,2.7007e-06,4.6178e-07,2.7183e-07,7.1135e-08,5.3027e-07,6.4886e-07,1.7529e-05,4.6364e-06,2.0266e-06,1.2249e-05,2.8189e-06,1.8676e-07,5.2329e-08,6.9051e-08,2.8416e-07,2.5496e-06,6.4723e-06,8.4626e-07,1.0609e-07,7.0631e-08,2.8584e-07,5.4446e-07,1.4832e-05,1.6542e-06,1.6731e-06,1.772e-05,7.0634e-06,1.7295e-07,1.3864e-07,1.0809e-07,6.4203e-07,4.6989e-06,2.1351e-06,8.2644e-06,2.382e-06,2.5225e-07,5.2243e-08,4.991e-07,6.7195e-06,8.639e-07
0.031579,1.4374e-06,1.6488e-05,5.6165e-07,1.431e-07,2.673e-08,1.209e-07,2.0186e-06,6.828e-06,6.566e-07,4.9317e-06,7.441e-08,4.3973e-08,1.9682e-07,1.2519e-06,1.433e-05,1.3389e-06,2.3581e-06,4.6116e-06,4.3318e-07,1.1261e-07,3.1759e-08,4.7334e-07,2.7577e-07,2.0599e-06,7.4725e-07,5.6973e-07,1.0526e-07,2.1794e-08,5.7956e-08,4.5944e-07,3.3486e-06,1.5905e-06,3.2093e-06,5.2367e-06,6.2695e-07,5.6967e-08,1.0461e-07,1.117e-06,5.8283e-07,8.1298e-07,5.5866e-07,1.2406e-06,8.9126e-08,7.088e-08,5.0746e-08,3.6615e-07,2.9783e-06,7.8884e-07,7.7416e-06,1.4873e-06,3.8168e-07,3.7524e-07,4.5155e-08,4.1505e-08,1.7012e-07,1.6218e-07,2.3035e-07,1.1316e-07,1.249e-07,4.2607e-08,1.0812e-07,2.3277e-06,2.9659e-06,1.262e-06,5.1566e-06,8.6775e-07,5.1052e-07,4.7321e-07,2.3131e-08,9.5745e-08,1.2823e-07,7.4579e-07,1.1643e-07,8.8833e-08,2.9639e-08,1.7549e-08,1.2031e-07,2.198e-07,2.2218e-06,5.127e-06,4.6327e-06,1.3017e-06,1.2043e-07,1.6057e-07,2.8425e-08,2.6993e-08,1.9625e-07,2.7857e-07,5.1657e-08,8.0671e-08,1.5948e-08,9.5208e-08,1.5891e-07,2.7013e-07,7.997e-07,3.9528e-06,5.1598e-07,5.7712e-07,2.1351e-07,5.973e-07,2.1123e-07,1.2441e-08,1.7361e-08,1.1436e-07,3.1948e-08,2.7787e-08,1.6243e-08,8.5894e-08,2.1908e-07,2.0656e-07,5.1253e-07,3.1813e-06,1.4682e-06,3.5621e-07,6.6192e-08,3.1767e-08,8.974e-08,9.1773e-09,1.8563e-08,4.2283e-08,9.9319e-08,1.1066e-08,2.1635e-08,2.1557e-07,5.1634e-08,5.0727e-08,2.0754e-07,2.287e-07,3.6127e-06,6.3906e-08,2.275e-07,3.726e-08,6.3361e-08,4.0119e-09,4.504e-08,1.6945e-07,5.6032e-08,4.1667e-08,1.1618e-08,6.932e-08,2.2679e-08,3.6007e-07,2.0718e-07,2.7282e-06,1.6514e-06,1.0095e-06,2.3437e-07,1.7918e-07,2.1856e-08,4.7958e-08,1.1728e-07,8.4137e-08,1.8746e-07,4.294e-08,2.2511e-08,2.3932e-08,1.9397e-07,2.0491e-07,6.3262e-08,5.4374e-07,8.2915e-07,9.5947e-08,1.2616e-07,1.6056e-07,2.33e-07,3.346e-07,1.1881e-07,2.1419e-07,2.8422e-07,1.3191e-07,4.0628e-07,2.535e-08,1.6556e-07,1.155e-07,1.347e-07,6.9488e-07,9.6115e-07,4.24e-07,7.1262e-08,4.4938e-08,5.6047e-09,8.2187e-08,5.6098e-07,8.4146e-06,5.4608e-06,3.7539e-07,7.4176e-08,5.3813e-09,4.6881e-08,7.0993e-08,6.7319e-08,8.3582e-07,7.2256e-07,4.0833e-07,2.0102e-08,2.0015e-08,1.4554e-08,8.9404e-09,2.3966e-07,5.1665e-07,5.817e-07,1.8359e-08,2.3784e-08,5.4266e-08,7.4266e-08,1.6709e-08,7.8407e-08,7.6056e-07,7.5192e-07,3.5785e-07,3.146e-08,5.2714e-08,6.7061e-09,1.7163e-08,5.7895e-08,1.9898e-07,2.6908e-07,1.526e-07,5.648e-09,6.3988e-09,5.677e-08,3.827e-08,3.292e-08,1.1343e-06,1.064e-06,6.4603e-07,1.288e-08,3.2708e-09,3.6355e-09,6.7392e-09,6.0009e-08,2.317e-07,1.6317e-07,1.4304e-07,7.2197e-09,1.0878e-07,1.0142e-08,1.6011e-08,6.1755e-07,7.7961e-07,3.1452e-07,4.9438e-08,1.588e-08,8.2111e-09,4.6791e-09,5.8186e-09,2.5612e-07,1.2455e-07,4.6971e-08,4.3486e-08,1.124e-07,1.3203e-08,2.4259e-08,1.7792e-08,1.4421e-06,8.3396e-07,8.7269e-07,4.5592e-08,1.7233e-08,3.6253e-09,9.2846e-09,6.4976e-09,5.3313e-08,3.7129e-07,5.5563e-08,8.2046e-08,7.4835e-09,1.326e-08,6.5109e-09,1.6812e-08,3.6629e-07,8.6827e-07,8.6353e-07,4.7393e-08,3.0905e-08,1.9045e-08,3.6329e-09,3.6345e-08,9.5229e-08,1.1009e-07,1.3995e-07,1.2125e-07,7.4297e-09,8.7066e-09,1.0389e-07,3.2626e-08,2.2322e-07,6.5954e-07,5.4409e-07,1.3961e-07,4.7309e-08,4.184e-08,1.0209e-08,3.4994e-08,1.6658e-07,2.0891e-07,3.9309e-07,3.3015e-08,8.2136e-08,7.6428e-09,1.2143e-08,7.2778e-08,1.9129e-07,1.0649e-06,8.7914e-07,2.0399e-08,7.2087e-08,1.9023e-08,1.41e-09,6.8463e-08,8.2303e-07,3.4011e-06,2.2316e-06,5.7656e-07,2.0485e-07,3.1351e-08,3.0143e-08,7.2917e-08,9.9296e-08,8.7715e-07,1.0054e-06,7.0517e-08,8.2729e-08,1.7328e-07,2.4651e-08,7.9469e-07,8.2185e-08,2.6218e-07,1.3298e-07,1.449e-07,1.6571e-07,1.697e-07,1.7117e-07,1.1494e-07,1.1314e-07,7.6701e-07,2.2608e-06,2.3782e-07,1.423e-07,9.3852e-08,6.4099e-08,1.8316e-08,6.13e-08,6.9858e-08,6.4262e-08,1.9713e-07,1.4288e-08,2.166e-08,9.9243e-08,9.533e-08,1.373e-06,4.9348e-07,6.9747e-07,2.7453e-07,2.9845e-07,1.1704e-07,7.6953e-08,4.004e-08,1.0588e-07,2.8752e-07,8.3888e-08,4.1201e-08,7.8857e-09,8.0047e-08,3.9055e-08,3.5717e-07,2.7403e-07,1.2483e-06,7.995e-07,2.1796e-07,7.4883e-08,3.7876e-08,3.101e-07,1.2131e-08,2.8454e-08,7.8633e-08,5.8658e-07,3.6144e-08,9.345e-09,2.8257e-07,5.3642e-08,1.6495e-08,3.9492e-07,1.7265e-06,8.0797e-07,9.5122e-07,1.7615e-07,4.6511e-07,8.8417e-08,1.6581e-08,2.9589e-08,1.8887e-07,7.6646e-08,1.3684e-07,1.2069e-08,3.8473e-07,2.2176e-07,3.2628e-07,2.9869e-07,1.4438e-06,1.1871e-06,1.4643e-06,9.1517e-07,1.7736e-07,4.646e-08,2.0754e-08,8.0624e-08,2.956e-07,4.7897e-07,7.1505e-08,3.3623e-08,6.7271e-08,1.3317e-07,5.1171e-07,9.1661e-07,1.3862e-06,3.9997e-06,4.8445e-07,1.1881e-06,2.5212e-07,4.8222e-08,5.4611e-08,8.2416e-08,5.6323e-08,1.9423e-07,6.5216e-08,8.9011e-08,9.6869e-08,1.4212e-07,2.6174e-07,1.044e-06,1.418e-06,3.1493e-06,1.7579e-06,2.2204e-06,9.9566e-07,3.7159e-08,1.562e-07,1.621e-07,1.454e-06,6.4886e-07,1.8881e-07,2.7663e-07,5.098e-08,2.3488e-07,7.6215e-07,3.4024e-06,4.818e-07,4.2262e-06,2.1273e-06,2.5046e-06,7.8369e-08,6.198e-08,3.4309e-08,6.1908e-07,1.2993e-06,2.115e-06,5.8116e-07,6.845e-08,1.2417e-07,5.7933e-08,1.4129e-06,1.1274e-06,9.4248e-06,3.878e-06,1.5039e-05,1.6484e-06,7.6589e-07,3.039e-08,1.8762e-07,3.4059e-07,6.9688e-07,2.235e-06,3.3938e-07,2.1735e-07,5.5363e-08,4.3424e-07,4.1793e-07,1.0977e-05,2.4976e-06,9.4236e-07,1.1663e-05,2.4082e-06,1.4109e-07,4.042e-08,5.0886e-08,1.9605e-07,1.7048e-06,4.3027e-06,6.0989e-07,7.9923e-08,5.5239e-08,2.1098e-07,3.2206e-07,1.3407e-05,9.0257e-07,8.207e-07,1.3422e-05,6.1564e-06,1.3207e-07,1.0059e-07,8.0091e-08,4.681e-07,2.9672e-06,1.324e-06,5.4009e-06,2.201e-06,1.8923e-07,3.504e-08,3.2723e-07,4.1848e-06,4.3967e-07
0.036842,6.9773e-07,1.0178e-05,3.582e-07,9.9038e-08,1.982e-08,8.8008e-08,1.3039e-06,3.9937e-06,4.3781e-07,3.5964e-06,5.2926e-08,3.2077e-08,1.3868e-07,7.8231e-07,1.0132e-05,6.8326e-07,1.6062e-06,2.2968e-06,2.7948e-07,7.6726e-08,2.3308e-08,3.8171e-07,1.9588e-07,1.3938e-06,6.6873e-07,4.1871e-07,7.6095e-08,1.5189e-08,3.9716e-08,2.9372e-07,1.915e-06,8.7746e-07,1.6698e-06,4.3765e-06,3.469e-07,3.9017e-08,8.7025e-08,9.9729e-07,3.9107e-07,4.5355e-07,3.3628e-07,7.9463e-07,6.0994e-08,5.4957e-08,3.4085e-08,2.3507e-07,1.6997e-06,3.5792e-07,2.3691e-06,1.0597e-06,2.5752e-07,1.9845e-07,3.445e-08,2.2605e-08,1.2171e-07,1.0291e-07,1.437e-07,7.8479e-08,8.6331e-08,3.1196e-08,7.6683e-08,1.9086e-06,2.3931e-06,6.1268e-07,4.7393e-07,4.7154e-07,3.8347e-07,4.3314e-07,1.7309e-08,7.4484e-08,9.5379e-08,3.9333e-07,7.47e-08,6.2944e-08,2.1072e-08,1.3116e-08,8.9396e-08,1.4852e-07,1.4434e-06,4.9424e-07,3.1357e-06,7.3748e-07,7.6087e-08,1.172e-07,1.9986e-08,2.0751e-08,1.3244e-07,2.3699e-07,3.3182e-08,5.6873e-08,1.1818e-08,6.4837e-08,1.1448e-07,1.939e-07,5.6444e-07,2.8467e-06,2.4454e-07,3.5943e-07,1.6125e-07,5.529e-07,1.2189e-07,9.3051e-09,1.1965e-08,7.3912e-08,2.1039e-08,1.9654e-08,1.2117e-08,6.4667e-08,1.6011e-07,1.4148e-07,3.0439e-07,1.328e-06,5.892e-07,2.1347e-07,4.2118e-08,1.9894e-08,6.2261e-08,6.7789e-09,1.3484e-08,2.7729e-08,6.4014e-08,8.2341e-09,1.6894e-08,1.54e-07,3.6774e-08,3.1947e-08,1.2852e-07,1.5529e-07,1.1098e-06,4.665e-08,1.5923e-07,2.8608e-08,4.6192e-08,2.8679e-09,3.2607e-08,1.0069e-07,3.7391e-08,2.9994e-08,8.7607e-09,5.1129e-08,1.5695e-08,2.9783e-07,1.4398e-07,1.4905e-06,8.3821e-07,9.3613e-07,1.9648e-07,1.0208e-07,1.5957e-08,4.3921e-08,8.6455e-08,5.3764e-08,1.2512e-07,2.9404e-08,1.6767e-08,1.7435e-08,1.618e-07,1.7704e-07,4.7309e-08,2.306e-07,4.005e-07,6.4419e-08,1.0301e-07,1.4162e-07,2.2942e-07,2.5992e-07,8.4089e-08,1.4535e-07,1.5785e-07,9.375e-08,3.5478e-07,1.8462e-08,1.4098e-07,8.4417e-08,9.2761e-08,3.2441e-07,4.8943e-07,2.5357e-07,5.1173e-08,3.0126e-08,4.284e-09,6.1113e-08,4.0854e-07,4.6802e-06,4.2656e-06,2.4998e-07,5.4837e-08,4.0621e-09,3.1487e-08,5.0979e-08,4.6232e-08,4.4995e-07,3.4322e-07,3.1148e-07,1.4893e-08,1.5698e-08,1.1612e-08,6.6001e-09,1.7035e-07,3.2502e-07,3.6351e-07,1.22e-08,1.8357e-08,5.0062e-08,4.5947e-08,1.2954e-08,5.02e-08,3.3797e-07,3.867e-07,3.1301e-07,2.231e-08,4.9017e-08,5.6888e-09,1.3917e-08,3.9183e-08,1.2962e-07,1.7887e-07,1.3138e-07,4.139e-09,4.9916e-09,5.1965e-08,2.9486e-08,2.1772e-08,5.8691e-07,6.1311e-07,5.3159e-07,8.7654e-09,2.3444e-09,2.7928e-09,5.2654e-09,4.3481e-08,1.5779e-07,1.2312e-07,1.1264e-07,5.3511e-09,8.724e-08,5.8965e-09,1.0629e-08,3.8239e-07,3.771e-07,1.2559e-07,3.5227e-08,1.1338e-08,6.5865e-09,3.7622e-09,4.4853e-09,1.2819e-07,1.0223e-07,3.3903e-08,3.1534e-08,9.5763e-08,9.7977e-09,2.368e-08,1.2982e-08,1.8428e-06,4.1562e-07,4.3752e-07,2.8286e-08,1.2038e-08,2.656e-09,7.2829e-09,4.8776e-09,3.8278e-08,1.8874e-07,3.7519e-08,6.2681e-08,5.6682e-09,1.0552e-08,4.9784e-09,1.18e-08,2.7153e-07,4.3769e-07,4.326e-07,3.1768e-08,2.188e-08,1.4671e-08,2.7714e-09,2.4137e-08,7.3021e-08,7.0452e-08,9.0743e-08,9.4116e-08,5.5334e-09,7.1312e-09,4.8485e-08,2.3415e-08,2.243e-07,3.0043e-07,2.3616e-07,9.3584e-08,3.3693e-08,2.695e-08,7.7559e-09,2.4875e-08,1.1429e-07,1.3484e-07,2.4826e-07,2.3314e-08,5.5367e-08,6.5063e-09,9.0344e-09,5.6702e-08,1.6068e-07,5.596e-07,4.4103e-07,1.2974e-08,5.1975e-08,1.3127e-08,9.2631e-10,5.1294e-08,5.2242e-07,2.4885e-06,1.3413e-06,4.1144e-07,1.7273e-07,2.4432e-08,2.1697e-08,4.8487e-08,7.13e-08,4.3298e-07,4.9192e-07,6.7883e-08,5.96e-08,1.6099e-07,1.8212e-08,8.4188e-07,5.6728e-08,1.8472e-07,8.222e-08,1.0497e-07,1.2345e-07,1.3581e-07,1.5932e-07,8.7652e-08,6.6645e-08,3.7265e-07,1.184e-06,1.6585e-07,1.0524e-07,5.3907e-08,5.1524e-08,1.3359e-08,4.2819e-08,4.2627e-08,3.9659e-08,1.5892e-07,1.0338e-08,1.5668e-08,7.3719e-08,6.5153e-08,1.335e-06,2.0726e-07,3.4036e-07,1.975e-07,2.2728e-07,6.9749e-08,5.7093e-08,3.5665e-08,9.0187e-08,2.1419e-07,5.0649e-08,2.9873e-08,5.9403e-09,5.9061e-08,3.0583e-08,2.9452e-07,1.7863e-07,6.4772e-07,3.5283e-07,1.3625e-07,1.2732e-07,2.41e-08,2.3004e-07,9.1288e-09,2.0334e-08,4.9223e-08,4.5433e-07,2.6403e-08,6.7976e-09,2.087e-07,6.3245e-08,1.0363e-08,2.662e-07,8.9961e-07,3.8762e-07,6.4863e-07,1.2259e-07,3.7093e-07,6.9112e-08,1.258e-08,2.0914e-08,1.1889e-07,5.0811e-08,1.051e-07,9.0392e-09,3.1151e-07,1.5833e-07,2.6689e-07,1.8778e-07,7.0948e-07,5.7061e-07,1.0611e-06,4.794e-07,1.363e-07,3.3464e-08,1.5637e-08,5.7146e-08,2.4827e-07,4.1028e-07,5.0099e-08,2.6258e-08,4.5982e-08,9.8161e-08,2.7096e-07,5.7635e-07,5.0285e-07,2.8855e-06,2.8243e-07,1.0105e-06,2.1173e-07,3.4372e-08,3.9923e-08,5.8256e-08,3.5588e-08,1.2702e-07,4.5289e-08,6.8854e-08,6.2468e-08,1.1365e-07,1.978e-07,6.3649e-07,7.8725e-07,1.6488e-06,1.3238e-06,1.3478e-06,4.6433e-07,2.7375e-08,1.1042e-07,1.1547e-07,8.6597e-07,4.1569e-07,1.358e-07,1.9348e-07,3.8459e-08,1.7082e-07,5.2089e-07,2.6579e-06,2.4239e-07,5.2159e-07,1.6712e-06,2.0359e-06,5.5911e-08,4.6294e-08,2.4942e-08,4.1588e-07,1.3188e-06,1.8628e-06,3.8924e-07,4.8398e-08,7.5613e-08,3.9935e-08,1.0064e-06,8.5805e-07,1.3553e-06,2.3361e-06,6.9971e-06,1.4551e-06,3.8318e-07,2.2325e-08,1.5601e-07,2.5331e-07,4.6164e-07,1.8574e-06,2.3783e-07,1.6647e-07,4.1014e-08,3.4945e-07,2.5761e-07,6.0786e-06,1.3292e-06,4.2914e-07,1.0972e-05,2.1211e-06,1.026e-07,2.9815e-08,3.57e-08,1.269e-07,1.083e-06,2.7261e-06,4.1801e-07,5.7502e-08,4.125e-08,1.4813e-07,1.8603e-07,1.2138e-05,5.0706e-07,4.0389e-07,7.1869e-06,2.9498e-06,9.6387e-08,6.9469e-08,5.6415e-08,3.2486e-07,1.7891e-06,7.8843e-07,3.5157e-06,1.62e-06,1.3603e-07,2.2188e-08,2.0361e-07,2.542e-06,2.2063e-07
0.042105,3.3359e-07,5.4357e-06,2.1864e-07,6.555e-08,1.4408e-08,6.1372e-08,8.0849e-07,2.2517e-06,2.7776e-07,2.4682e-06,3.5961e-08,2.2401e-08,9.3474e-08,4.6225e-07,4.8444e-06,3.5849e-07,1.1566e-06,1.1597e-06,1.6874e-07,4.9747e-08,1.6385e-08,3.0002e-07,1.3362e-07,9.0597e-07,7.2024e-07,2.99e-07,5.2364e-08,1.0118e-08,2.5948e-08,1.7996e-07,1.1341e-06,5.0363e-07,1.1288e-06,3.6862e-06,1.8813e-07,2.5362e-08,7.1636e-08,8.7678e-07,2.5061e-07,2.4906e-07,1.9544e-07,4.8563e-07,3.963e-08,4.1094e-08,2.2113e-08,1.4395e-07,9.555e-07,1.6344e-07,8.5707e-07,7.4317e-07,1.6564e-07,1.6108e-07,2.5385e-08,1.0385e-08,8.3375e-08,6.2701e-08,8.5465e-08,5.1993e-08,5.6761e-08,2.1883e-08,5.1947e-08,1.668e-06,7.6826e-07,2.9047e-07,1.766e-07,2.5007e-07,2.7766e-07,4.2005e-07,1.2498e-08,5.6175e-08,6.8446e-08,2.0671e-07,4.595e-08,4.2657e-08,1.4381e-08,9.4644e-09,6.4168e-08,9.5907e-08,8.7212e-07,1.8197e-07,2.0581e-06,4.0426e-07,4.5612e-08,8.4469e-08,1.3439e-08,1.5321e-08,8.5425e-08,2.2323e-07,2.0429e-08,3.8367e-08,8.3722e-09,4.2442e-08,7.9614e-08,1.3416e-07,3.9123e-07,2.1138e-06,1.1547e-07,2.1442e-07,1.2039e-07,4.32e-07,7.0578e-08,6.6546e-09,7.9231e-09,4.5957e-08,1.3264e-08,1.3296e-08,8.6255e-09,4.6636e-08,1.1076e-07,9.2427e-08,1.7294e-07,5.739e-07,2.4749e-07,1.2229e-07,2.5803e-08,1.2127e-08,4.1208e-08,4.8052e-09,9.3594e-09,1.7575e-08,3.9663e-08,5.8439e-09,1.2699e-08,1.0448e-07,2.5629e-08,1.936e-08,7.6382e-08,1.0362e-07,4.2149e-07,3.2412e-08,1.0524e-07,2.105e-08,3.2137e-08,1.9404e-09,2.2574e-08,5.8474e-08,2.3901e-08,2.0657e-08,6.3084e-09,3.6071e-08,1.0416e-08,2.4796e-07,9.4532e-08,8.2702e-07,4.1778e-07,4.581e-07,1.6432e-07,5.8464e-08,1.1146e-08,4.2887e-08,6.1435e-08,3.2727e-08,7.981e-08,1.9176e-08,1.1932e-08,1.2145e-08,1.3009e-07,1.705e-07,3.198e-08,9.2227e-08,1.8776e-07,4.1445e-08,8.7123e-08,1.2292e-07,2.2008e-07,1.9548e-07,5.7037e-08,9.4987e-08,8.5269e-08,6.3859e-08,3.1978e-07,1.2978e-08,6.7989e-08,5.9731e-08,6.1692e-08,1.454e-07,2.3985e-07,1.4784e-07,3.5513e-08,1.9714e-08,3.142e-09,4.4264e-08,2.8485e-07,3.1659e-06,1.401e-06,1.5765e-07,3.8922e-08,2.9393e-09,2.0666e-08,3.5388e-08,3.0663e-08,2.3436e-07,1.5547e-07,2.3423e-07,1.0534e-08,1.1859e-08,8.8955e-09,4.6487e-09,1.1548e-07,1.9693e-07,2.1895e-07,7.7189e-09,1.358e-08,4.6276e-08,2.8186e-08,9.534e-09,3.1329e-08,1.4584e-07,1.993e-07,2.694e-07,1.5214e-08,4.6613e-08,4.689e-09,1.0974e-08,2.5422e-08,8.0859e-08,1.1425e-07,1.1777e-07,2.8923e-09,3.739e-09,4.6773e-08,2.3069e-08,1.4262e-08,2.9312e-07,3.7481e-07,4.5134e-07,5.697e-09,1.6e-09,2.0568e-09,3.9574e-09,3.023e-08,1.0375e-07,8.9451e-08,8.6589e-08,3.7796e-09,6.8245e-08,3.2259e-09,6.9195e-09,2.1857e-07,1.7436e-07,5.6835e-08,2.4232e-08,7.7519e-09,5.047e-09,2.905e-09,3.3245e-09,6.2416e-08,8.3344e-08,2.3885e-08,2.1989e-08,7.9336e-08,6.9294e-09,2.4325e-08,9.095e-09,1.0259e-06,1.98e-07,2.101e-07,1.6529e-08,8.0664e-09,1.8658e-09,5.4768e-09,3.4989e-09,2.6338e-08,1.4919e-07,2.4305e-08,4.6432e-08,4.1199e-09,8.0618e-09,3.6629e-09,7.9973e-09,1.9536e-07,2.1185e-07,2.0753e-07,2.0491e-08,1.4898e-08,1.0831e-08,2.0243e-09,1.5764e-08,5.4409e-08,4.3094e-08,5.6347e-08,7.0945e-08,3.933e-09,5.6316e-09,4.3201e-08,1.6241e-08,1.2162e-07,1.3039e-07,9.6532e-08,6.0536e-08,2.3166e-08,1.6955e-08,5.6328e-09,1.696e-08,7.6363e-08,8.3643e-08,1.5068e-07,1.607e-08,3.5537e-08,5.3307e-09,6.5326e-09,4.3652e-08,1.2936e-07,2.829e-07,2.1332e-07,8.7477e-09,3.6228e-08,8.6758e-09,6.2444e-10,3.6729e-08,3.2422e-07,1.8806e-06,7.8113e-07,2.7858e-07,1.4407e-07,1.8258e-08,1.5167e-08,3.18e-08,4.9925e-08,2.0952e-07,2.3414e-07,5.9192e-08,4.1164e-08,1.1984e-07,1.2775e-08,3.7565e-07,3.7428e-08,1.2548e-07,4.9139e-08,7.3145e-08,8.8526e-08,1.0383e-07,1.0313e-07,6.5896e-08,4.7819e-08,1.7487e-07,6.0474e-07,1.1147e-07,7.6465e-08,3.0409e-08,4.0415e-08,9.3121e-09,2.8578e-08,2.523e-08,2.3461e-08,1.2783e-07,7.1278e-09,1.0832e-08,5.1878e-08,4.2667e-08,1.0002e-06,8.306e-08,1.6192e-07,1.5562e-07,1.6703e-07,4.1642e-08,4.0512e-08,3.2448e-08,7.6208e-08,1.5471e-07,2.9492e-08,2.0746e-08,4.2747e-09,4.1511e-08,2.2874e-08,2.4449e-07,1.1133e-07,3.2636e-07,1.5831e-07,8.1586e-08,6.5354e-08,1.4798e-08,1.6243e-07,6.5857e-09,1.3876e-08,2.9374e-08,2.1654e-07,1.8478e-08,4.7124e-09,1.4692e-07,7.7531e-08,6.9805e-09,1.6728e-07,4.5402e-07,1.8215e-07,4.3415e-07,8.2023e-08,2.7676e-07,5.2153e-08,9.1362e-09,1.4123e-08,7.2374e-08,3.2649e-08,4.8997e-08,6.4733e-09,2.4096e-07,1.0631e-07,2.22e-07,1.122e-07,3.3894e-07,2.7314e-07,7.411e-07,2.5465e-07,1.0113e-07,2.2995e-08,1.1281e-08,3.8826e-08,2.2694e-07,1.5349e-07,3.3566e-08,1.974e-08,3.0175e-08,6.9494e-08,1.4583e-07,3.4706e-07,1.9562e-07,2.1519e-06,1.5768e-07,8.5395e-07,1.7765e-07,2.3322e-08,2.7879e-08,3.9404e-08,2.1423e-08,8.0007e-08,3.0033e-08,5.1113e-08,3.8947e-08,9.3112e-08,1.4427e-07,3.6756e-07,4.2438e-07,9.1409e-07,1.0193e-06,7.4874e-07,3.9861e-07,1.931e-08,7.505e-08,7.8722e-08,4.9705e-07,2.5403e-07,9.3577e-08,1.2836e-07,2.7815e-08,1.1934e-07,3.4052e-07,1.176e-06,1.1735e-07,2.2553e-07,1.3907e-06,1.6174e-06,3.8182e-08,3.3027e-08,1.7421e-08,2.6682e-07,6.1618e-07,7.0305e-07,2.489e-07,3.2752e-08,4.6321e-08,2.6183e-08,6.7936e-07,7.3715e-07,5.53e-07,9.2185e-07,3.4512e-06,1.2631e-06,1.895e-07,1.5712e-08,1.2798e-07,1.8245e-07,2.9245e-07,1.6215e-06,1.5969e-07,1.2288e-07,2.9056e-08,2.8432e-07,1.5242e-07,3.153e-06,7.0246e-07,1.9091e-07,1.0233e-05,2.096e-06,7.2263e-08,2.112e-08,2.3985e-08,7.7095e-08,6.5605e-07,1.6516e-06,2.7354e-07,3.9743e-08,2.957e-08,9.9375e-08,1.0503e-07,4.4898e-06,2.9224e-07,1.9938e-07,5.0397e-06,1.5239e-06,6.7696e-08,4.5863e-08,3.7934e-08,2.1583e-07,1.0341e-06,4.523e-07,2.2713e-06,6.9655e-07,9.4226e-08,1.3296e-08,1.2072e-07,1.5153e-06,1.0851e-07
0.047368,1.5662e-07,3.7502e-06,1.2806e-07,4.1551e-08,1.0352e-08,4.1079e-08,4.8172e-07,1.2211e-06,1.678e-07,1.5821e-06,2.337e-08,1.5e-08,6.037e-08,2.5775e-07,3.2721e-06,1.9949e-07,1.3492e-07,5.8727e-07,9.5482e-08,3.0711e-08,1.1049e-08,2.3154e-07,8.7735e-08,5.665e-07,3.9015e-07,2.0908e-07,3.4293e-08,6.4368e-09,1.6171e-08,1.0568e-07,6.9004e-07,3.1204e-07,7.9736e-07,1.1832e-06,9.9721e-08,1.5625e-08,5.9556e-08,3.3158e-07,1.535e-07,1.3363e-07,1.1065e-07,2.8344e-07,2.4452e-08,2.974e-08,1.3909e-08,8.4195e-08,5.2773e-07,7.4712e-08,3.3519e-07,5.2359e-07,1.0169e-07,1.3138e-07,1.8188e-08,3.5115e-09,5.4767e-08,3.6759e-08,4.8554e-08,3.295e-08,3.5532e-08,1.4728e-08,3.3656e-08,9.1847e-07,2.5809e-07,1.3441e-07,7.1409e-08,1.2928e-07,1.9412e-07,2.2507e-07,8.714e-09,4.1467e-08,4.7554e-08,1.0682e-07,2.7123e-08,2.7683e-08,9.4724e-09,6.6107e-09,4.4654e-08,5.9136e-08,4.9656e-07,7.1335e-08,1.304e-06,2.1279e-07,2.6021e-08,6.1279e-08,8.6512e-09,1.0892e-08,5.273e-08,1.0995e-07,1.2071e-08,2.4797e-08,5.6794e-09,2.668e-08,5.3483e-08,8.9434e-08,2.7474e-07,3.7653e-07,5.4048e-08,1.2261e-07,8.957e-08,2.0033e-07,4.056e-08,4.5573e-09,5.0362e-09,2.7486e-08,8.0108e-09,8.618e-09,5.8659e-09,3.2272e-08,7.25e-08,5.7641e-08,9.3959e-08,2.4966e-07,1.0573e-07,6.7068e-08,1.53e-08,7.2985e-09,2.6068e-08,3.2801e-09,6.2158e-09,1.0773e-08,2.3654e-08,3.961e-09,9.2185e-09,6.7467e-08,1.7429e-08,1.1401e-08,4.3431e-08,6.3601e-08,1.6942e-07,2.1208e-08,6.5474e-08,1.488e-08,2.1356e-08,1.2404e-09,1.4964e-08,3.303e-08,1.465e-08,1.3631e-08,4.343e-09,2.4379e-08,6.6393e-09,2.1411e-07,5.8485e-08,4.5183e-07,2.0373e-07,2.3225e-07,4.697e-08,3.315e-08,7.4581e-09,2.2627e-08,4.2252e-08,1.8975e-08,4.8639e-08,1.1915e-08,8.1242e-09,8.1003e-09,1.0051e-07,8.1617e-08,1.9943e-08,3.4476e-08,8.5408e-08,2.5506e-08,7.9527e-08,1.0576e-07,1.9194e-07,1.4268e-07,3.715e-08,5.9909e-08,4.4725e-08,4.1772e-08,3.2049e-07,8.8228e-09,3.4329e-08,4.1067e-08,4.0112e-08,6.257e-08,1.131e-07,8.3508e-08,2.3864e-08,1.2574e-08,2.2159e-09,3.1413e-08,1.9132e-07,2.1695e-06,5.9587e-07,9.4111e-08,2.6542e-08,2.044e-09,1.3235e-08,2.3805e-08,1.9381e-08,1.1759e-07,6.7183e-08,1.7629e-07,7.1643e-09,8.6559e-09,6.5559e-09,3.1277e-09,7.4649e-08,1.148e-07,1.2692e-07,4.6557e-09,9.6472e-09,4.4222e-08,1.7007e-08,6.7343e-09,1.8959e-08,6.1102e-08,1.0376e-07,2.2648e-07,9.9955e-09,4.8038e-08,3.7646e-09,8.4813e-09,1.583e-08,4.8326e-08,7.0187e-08,1.2172e-07,1.9301e-09,2.6954e-09,3.2377e-08,1.9729e-08,9.0898e-09,1.4164e-07,2.8303e-07,4.2445e-07,3.5418e-09,1.0395e-09,1.455e-09,2.8676e-09,2.0215e-08,6.6004e-08,6.2453e-08,6.559e-08,2.5467e-09,5.2661e-08,1.6317e-09,4.3676e-09,1.1733e-07,7.7225e-08,3.2375e-08,1.6061e-08,5.0856e-09,3.699e-09,2.1584e-09,2.3755e-09,3.1031e-08,6.802e-08,1.6589e-08,1.479e-08,6.4259e-08,4.6741e-09,2.9441e-08,6.1316e-09,6.2317e-07,9.034e-08,9.6847e-08,9.0602e-09,5.1963e-09,1.2581e-09,3.9553e-09,2.4018e-09,1.7404e-08,1.1881e-07,1.5123e-08,3.3508e-08,2.882e-09,5.9251e-09,2.6015e-09,5.2926e-09,1.3686e-07,9.8723e-08,9.5458e-08,1.2622e-08,9.7769e-09,7.6775e-09,1.4178e-09,1.011e-08,3.9729e-08,2.5205e-08,3.3532e-08,5.2222e-08,2.6717e-09,4.2995e-09,3.8025e-08,1.0921e-08,6.9107e-08,5.3887e-08,3.7327e-08,3.7771e-08,1.5425e-08,1.0391e-08,3.923e-09,1.1107e-08,4.9539e-08,4.9979e-08,8.7853e-08,1.0852e-08,2.2286e-08,4.2146e-09,4.5866e-09,3.3647e-08,1.0063e-07,1.3766e-07,9.9584e-08,5.8286e-09,2.4474e-08,5.4709e-09,4.6253e-10,2.5167e-08,1.9525e-07,1.5388e-06,4.4084e-07,1.7925e-07,1.2118e-07,1.3097e-08,1.0285e-08,2.0352e-08,3.3717e-08,1.0134e-07,1.0816e-07,4.0481e-08,2.7265e-08,5.518e-08,8.5055e-09,3.0861e-07,2.3639e-08,8.2149e-08,2.8421e-08,4.9172e-08,6.1271e-08,7.5872e-08,4.8447e-08,4.9401e-08,3.5764e-08,7.9268e-08,2.9773e-07,7.2006e-08,5.5331e-08,1.6725e-08,3.1276e-08,6.2147e-09,1.8245e-08,1.4397e-08,1.3322e-08,1.045e-07,4.6895e-09,7.1658e-09,3.4544e-08,2.6814e-08,9.5411e-07,3.2597e-08,7.4874e-08,9.1633e-08,1.183e-07,2.4788e-08,2.7532e-08,3.237e-08,3.588e-08,1.0889e-07,1.6541e-08,1.3818e-08,2.9427e-09,2.7774e-08,1.636e-08,2.108e-07,6.6532e-08,1.5941e-07,7.1089e-08,4.6684e-08,3.5178e-08,8.8106e-09,1.0947e-07,4.5652e-09,9.0521e-09,1.6739e-08,1.5304e-07,1.2413e-08,3.1156e-09,9.8906e-08,3.3781e-08,4.7831e-09,9.8275e-08,2.1966e-07,8.3712e-08,2.8544e-07,5.2753e-08,1.9041e-07,3.8146e-08,6.3617e-09,9.124e-09,4.258e-08,2.0517e-08,2.5576e-08,4.4396e-09,1.7765e-07,6.7095e-08,1.9476e-07,6.3577e-08,1.5722e-07,1.2787e-07,4.999e-07,1.4049e-07,7.2546e-08,1.5097e-08,7.8087e-09,2.5331e-08,1.173e-07,6.6274e-08,2.1529e-08,1.4333e-08,1.9026e-08,4.7277e-08,7.8398e-08,2.0029e-07,7.84e-08,3.1359e-07,8.4202e-08,4.3348e-07,1.531e-07,1.5071e-08,1.862e-08,2.5542e-08,1.2281e-08,4.8782e-08,1.9039e-08,3.6436e-08,2.3466e-08,8.6308e-08,1.0136e-07,2.0131e-07,2.2155e-07,5.1628e-07,7.293e-07,3.8971e-07,3.3933e-07,1.307e-08,4.9158e-08,5.1435e-08,2.7418e-07,1.4839e-07,6.1871e-08,8.0833e-08,1.9317e-08,8.0076e-08,2.1297e-07,5.2073e-07,5.4715e-08,1.0037e-07,7.675e-07,1.2635e-06,2.4993e-08,2.252e-08,1.171e-08,1.6361e-07,4.8713e-07,3.0569e-07,1.5207e-07,2.1263e-08,2.8209e-08,1.6319e-08,4.342e-07,3.4226e-07,2.3157e-07,4.5323e-07,1.804e-06,7.1756e-07,9.6373e-08,1.061e-08,1.0534e-07,1.2784e-07,1.7729e-07,1.6715e-06,1.0293e-07,8.7705e-08,1.9708e-08,2.4722e-07,8.6568e-08,1.7395e-06,3.7037e-07,8.256e-08,1.7595e-06,9.7316e-07,4.935e-08,1.4401e-08,1.5479e-08,4.3812e-08,3.7904e-07,9.5669e-07,1.7107e-07,2.6475e-08,2.0392e-08,6.3778e-08,5.7856e-08,1.2509e-06,1.7101e-07,9.8672e-08,3.6436e-06,8.2402e-07,4.5966e-08,2.8965e-08,2.4362e-08,1.3764e-07,5.7309e-07,2.4996e-07,1.4487e-06,3.1823e-07,6.3079e-08,7.5286e-09,6.8255e-08,8.9116e-07,5.1928e-08
0.052632,7.187e-08,8.1111e-07,7.2088e-08,2.5202e-08,7.3786e-09,2.6389e-08,2.7549e-07,6.3432e-07,9.635e-08,9.3555e-07,1.4512e-08,9.6229e-09,3.733e-08,1.3529e-07,2.3244e-06,1.262e-07,4.7994e-08,2.9883e-07,5.0586e-08,1.802e-08,7.1412e-09,1.769e-07,5.5449e-08,3.4043e-07,3.4966e-07,1.4463e-07,2.1309e-08,3.8965e-09,9.5921e-09,5.9368e-08,4.2984e-07,2.3262e-07,1.6624e-07,5.2401e-07,5.1452e-08,9.0788e-09,5.198e-08,1.4623e-07,8.9699e-08,6.9593e-08,6.2417e-08,1.5777e-07,1.4292e-08,2.0872e-08,8.5165e-09,4.6983e-08,2.8623e-07,3.3897e-08,1.3444e-07,3.8337e-07,5.9502e-08,7.8297e-08,1.279e-08,1.5187e-09,3.447e-08,2.0744e-08,2.6364e-08,1.9955e-08,2.1142e-08,9.5022e-09,2.0834e-08,6.9774e-07,9.0167e-08,6.0481e-08,3.0602e-08,6.5041e-08,1.3101e-07,1.8197e-07,5.8565e-09,3.0427e-08,3.2043e-08,5.3723e-08,1.5339e-08,1.7181e-08,6.0484e-09,4.4704e-09,3.0201e-08,3.469e-08,2.7404e-07,2.8922e-08,7.9096e-07,1.0671e-07,1.417e-08,4.6341e-08,5.3232e-09,7.4623e-09,3.1114e-08,8.4377e-08,6.8401e-09,1.5333e-08,3.6874e-09,1.6058e-08,3.4681e-08,5.7214e-08,2.0374e-07,1.2207e-07,2.4887e-08,6.7009e-08,6.7069e-08,9.8885e-08,2.297e-08,2.9857e-09,3.0651e-09,1.5771e-08,4.6271e-09,5.3478e-09,3.8054e-09,2.1413e-08,4.4788e-08,3.4268e-08,4.8705e-08,1.0742e-07,4.5203e-08,3.519e-08,8.8271e-09,4.4034e-09,1.5754e-08,2.1599e-09,3.9454e-09,6.3822e-09,1.3573e-08,2.5609e-09,6.4726e-09,4.1464e-08,1.1501e-08,6.6182e-09,2.3535e-08,3.6138e-08,6.9329e-08,1.3025e-08,3.816e-08,1.011e-08,1.3533e-08,7.4437e-10,9.4862e-09,1.8047e-08,8.5979e-09,8.6118e-09,2.8543e-09,1.5774e-08,4.0679e-09,2.0513e-07,3.4036e-08,2.4085e-07,9.6635e-08,1.1754e-07,2.038e-08,1.8418e-08,4.7743e-09,1.8176e-08,2.8209e-08,1.0449e-08,2.8233e-08,7.0383e-09,5.2867e-09,5.1662e-09,7.3809e-08,6.3024e-08,1.1573e-08,1.1923e-08,3.7597e-08,1.5015e-08,4.2467e-08,9.0563e-08,1.0296e-07,1.0107e-07,2.3229e-08,3.6467e-08,2.2703e-08,2.6235e-08,1.434e-07,5.799e-09,1.7449e-08,2.7528e-08,2.6488e-08,2.5792e-08,5.1178e-08,4.542e-08,1.5522e-08,7.7875e-09,1.5023e-09,2.203e-08,1.2466e-07,1.1006e-06,2.6325e-07,5.3035e-08,1.7362e-08,1.3667e-09,8.2421e-09,1.5523e-08,1.1579e-08,5.6517e-08,2.7604e-08,1.3681e-07,4.6997e-09,6.1134e-09,4.647e-09,2.0077e-09,4.5885e-08,6.4189e-08,7.0543e-08,2.6741e-09,6.5786e-09,4.6949e-08,1.0024e-08,4.5918e-09,1.1047e-08,2.4945e-08,5.4396e-08,1.952e-07,6.3227e-09,2.3892e-08,2.9451e-09,6.4865e-09,9.4498e-09,2.7609e-08,4.1415e-08,5.3136e-08,1.2291e-09,1.8699e-09,1.4414e-08,1.0024e-08,5.5719e-09,6.6206e-08,1.2867e-07,2.0806e-07,2.1049e-09,6.4095e-10,9.881e-10,2.0027e-09,1.3009e-08,4.0633e-08,4.1655e-08,4.9571e-08,1.6354e-09,4.0801e-08,7.4465e-10,2.6624e-09,5.9696e-08,3.2725e-08,1.9785e-08,1.0215e-08,3.1994e-09,2.59e-09,1.5431e-09,1.6367e-09,1.5407e-08,1.6709e-08,1.1536e-08,9.6084e-09,5.1087e-08,3.0007e-09,1.102e-08,3.9765e-09,4.2585e-07,3.9425e-08,4.2813e-08,4.6543e-09,3.2182e-09,8.1301e-10,2.7411e-09,1.576e-09,1.1045e-08,4.3969e-08,9.0275e-09,2.3656e-08,1.9426e-09,4.1876e-09,1.7863e-09,3.5138e-09,9.3657e-08,4.4292e-08,4.2017e-08,7.3822e-09,6.1868e-09,5.2258e-09,9.5139e-10,6.3492e-09,2.8748e-08,1.4065e-08,1.9092e-08,3.7714e-08,1.7328e-09,3.1753e-09,2.6364e-08,7.1293e-09,3.9255e-08,2.1143e-08,1.3847e-08,2.2725e-08,9.9565e-09,6.1793e-09,2.6243e-09,6.9787e-09,3.1113e-08,2.8807e-08,4.9059e-08,7.1701e-09,1.3577e-08,3.2171e-09,3.1171e-09,2.6488e-08,7.6235e-08,6.4343e-08,4.4795e-08,3.7479e-09,1.6027e-08,3.2707e-09,3.716e-10,1.6479e-08,1.1329e-07,1.5659e-06,2.4056e-07,1.0956e-07,1.0647e-07,9.0053e-09,6.7435e-09,1.2628e-08,2.1792e-08,5.0738e-08,4.8318e-08,2.8645e-08,1.7276e-08,2.6831e-08,5.3558e-09,2.5241e-07,1.428e-08,5.1591e-08,1.5891e-08,3.1935e-08,4.096e-08,5.2899e-08,2.3681e-08,3.7551e-08,2.0752e-08,3.4626e-08,1.3997e-07,4.4633e-08,4.0749e-08,8.909e-09,2.4271e-08,3.9697e-09,1.1126e-08,7.8824e-09,7.2552e-09,9.0121e-08,2.9417e-09,4.5312e-09,2.1679e-08,1.617e-08,1.0573e-06,1.3236e-08,3.348e-08,5.369e-08,8.0277e-08,1.4646e-08,1.7899e-08,1.6608e-08,1.5589e-08,7.5176e-08,8.9061e-09,8.8173e-09,1.936e-09,1.7613e-08,1.1172e-08,2.0321e-07,3.816e-08,7.5179e-08,3.1486e-08,2.5445e-08,1.9011e-08,5.107e-09,7.0482e-08,3.0416e-09,5.6369e-09,9.1045e-09,1.1302e-07,8.0002e-09,1.9606e-09,6.377e-08,3.0227e-08,3.2439e-09,5.397e-08,1.0113e-07,3.748e-08,1.8503e-07,3.2499e-08,1.1856e-07,2.7117e-08,4.243e-09,5.6314e-09,2.4183e-08,1.2803e-08,1.4241e-08,2.9128e-09,1.2392e-07,3.9702e-08,1.963e-07,3.4069e-08,7.0593e-08,5.7927e-08,3.2487e-07,7.8368e-08,5.026e-08,9.4611e-09,5.1848e-09,1.5861e-08,8.9669e-08,3.0607e-08,1.32e-08,1.007e-08,1.151e-08,3.0847e-08,4.1625e-08,1.1053e-07,3.1653e-08,1.0557e-07,4.2877e-08,1.789e-07,1.4387e-07,9.254e-09,1.1881e-08,1.5852e-08,6.6819e-09,2.9016e-08,1.1519e-08,2.4878e-08,1.3632e-08,4.2517e-08,6.8279e-08,1.0441e-07,1.117e-07,2.8876e-07,6.6968e-07,1.9397e-07,1.6256e-07,8.4901e-09,3.105e-08,3.2179e-08,1.4466e-07,8.2855e-08,3.9223e-08,4.8226e-08,1.2872e-08,5.1469e-08,1.2722e-07,2.5485e-07,2.4513e-08,4.4223e-08,5.6277e-07,9.7493e-07,1.5666e-08,1.4643e-08,7.5683e-09,9.5703e-08,3.8792e-07,1.3769e-07,8.8603e-08,1.3246e-08,1.6925e-08,9.6357e-09,2.6189e-07,2.4213e-07,9.6497e-08,2.224e-07,9.8673e-07,2.801e-07,4.91e-08,6.868e-09,8.9675e-08,8.7486e-08,1.0265e-07,7.1856e-07,6.3645e-08,6.0619e-08,1.2782e-08,1.3375e-07,4.709e-08,4.6726e-07,1.963e-07,3.4465e-08,5.1732e-07,7.5698e-07,3.2552e-08,9.4566e-09,9.6102e-09,2.3201e-08,2.0834e-07,5.2844e-07,1.0213e-07,1.7028e-08,1.3529e-08,3.9109e-08,3.0985e-08,3.9037e-07,9.8942e-08,4.9072e-08,8.5283e-07,4.6651e-07,3.0283e-08,1.7469e-08,1.4909e-08,8.4306e-08,3.0384e-07,1.3276e-07,9.0733e-07,1.4693e-07,4.0863e-08,4.0107e-09,3.6729e-08,5.2075e-07,2.3998e-08
0.057895,3.203e-08,2.1863e-07,3.9103e-08,1.4585e-08,5.2104e-09,1.6242e-08,1.5076e-07,3.1368e-07,5.2371e-08,5.0253e-07,8.5828e-09,5.8984e-09,2.2041e-08,6.6617e-08,2.9744e-07,6.1869e-08,1.8231e-08,1.5687e-07,2.5003e-08,1.001e-08,4.4095e-09,1.3541e-07,3.3684e-08,1.9605e-07,3.1139e-07,1.009e-07,1.2492e-08,2.2311e-09,5.3895e-09,3.1785e-08,2.7606e-07,1.0111e-07,4.7997e-08,2.4116e-07,2.5678e-08,4.9325e-09,5.29e-08,6.5848e-08,4.9795e-08,3.4925e-08,3.7638e-08,8.343e-08,7.8767e-09,1.4226e-08,5.0957e-09,2.4925e-08,1.5283e-07,1.5097e-08,5.3694e-08,3.1768e-07,3.3065e-08,3.4729e-08,8.9963e-09,2.1719e-09,2.0727e-08,1.1256e-08,1.3692e-08,1.1514e-08,1.1908e-08,5.858e-09,1.2282e-08,5.3534e-07,3.0631e-08,2.6298e-08,1.3542e-08,3.178e-08,8.5166e-08,1.4704e-07,3.7789e-09,2.2982e-08,2.0958e-08,2.6039e-08,8.2774e-09,1.0161e-08,3.756e-09,2.9216e-09,1.9907e-08,1.9243e-08,1.6033e-07,1.1859e-08,4.5288e-07,5.0518e-08,7.4066e-09,3.9621e-08,3.12e-09,4.9248e-09,1.7489e-08,6.5573e-08,3.7071e-09,9.0393e-09,2.286e-09,9.2045e-09,2.1678e-08,3.4875e-08,1.7383e-07,4.204e-08,1.1162e-08,3.4819e-08,5.1473e-08,4.9711e-08,1.2746e-08,1.8658e-09,1.7784e-09,8.641e-09,2.5454e-09,3.1688e-09,2.3466e-09,1.3585e-08,2.5987e-08,1.9352e-08,2.3983e-08,4.5065e-08,1.9108e-08,1.7616e-08,4.9845e-09,2.6892e-09,9.0706e-09,1.3722e-09,2.3855e-09,3.6479e-09,7.4886e-09,1.5736e-09,4.3978e-09,2.4205e-08,7.3079e-09,3.857e-09,1.209e-08,1.9178e-08,2.8289e-08,7.4875e-09,2.071e-08,6.5938e-09,8.1439e-09,4.1457e-10,5.7314e-09,9.4763e-09,4.8128e-09,5.1932e-09,1.7841e-09,9.7428e-09,2.4003e-09,9.9654e-08,1.8584e-08,1.2501e-07,4.4225e-08,5.8114e-08,9.2731e-09,9.9374e-09,2.9134e-09,1.4586e-08,1.8343e-08,5.4331e-09,1.5514e-08,3.9335e-09,3.2768e-09,3.1401e-09,5.0403e-08,3.5565e-08,6.2603e-09,3.867e-09,1.5938e-08,8.4713e-09,3.299e-08,7.6794e-08,5.7842e-08,6.9267e-08,1.3912e-08,2.139e-08,1.11e-08,1.5786e-08,1.1207e-07,3.6769e-09,8.7312e-09,1.8098e-08,2.0641e-08,1.0143e-08,2.2105e-08,2.3626e-08,9.7484e-09,4.6544e-09,9.7732e-10,1.5543e-08,7.9694e-08,6.0523e-07,1.1639e-07,2.8071e-08,1.0858e-08,8.782e-10,4.9616e-09,9.8003e-09,6.4916e-09,2.5824e-08,1.0711e-08,1.1549e-07,2.9731e-09,4.1805e-09,3.1611e-09,1.2255e-09,2.667e-08,3.4233e-08,3.7377e-08,1.4592e-09,4.2954e-09,2.1816e-08,5.7278e-09,3.0271e-09,6.1431e-09,9.9763e-09,2.8479e-08,1.7934e-07,3.8398e-09,1.9762e-08,2.2415e-09,4.9889e-09,5.39e-09,1.5007e-08,2.3386e-08,4.1417e-08,7.4493e-10,1.2462e-09,6.8152e-09,7.1366e-09,3.259e-09,2.9868e-08,8.9725e-08,1.5909e-07,1.1928e-09,3.7281e-10,6.4266e-10,1.345e-09,8.0496e-09,2.4172e-08,2.6272e-08,3.8242e-08,9.987e-10,3.2984e-08,3.0921e-10,1.563e-09,2.8861e-08,1.3219e-08,1.1525e-08,6.2009e-09,1.9248e-09,1.7264e-09,1.0593e-09,1.0858e-09,7.5522e-09,6.5008e-09,8.297e-09,6.0319e-09,3.9952e-08,1.8251e-09,9.2913e-09,2.4746e-09,2.1702e-07,1.6389e-08,1.8088e-08,2.2713e-09,1.9124e-09,5.0173e-10,1.8177e-09,9.8515e-10,6.7232e-09,1.6642e-08,5.1524e-09,1.6419e-08,1.2618e-09,2.8389e-09,1.1868e-09,2.2301e-09,6.295e-08,1.9088e-08,1.761e-08,4.0752e-09,3.7725e-09,3.4112e-09,6.0986e-10,3.8877e-09,2.1037e-08,7.4531e-09,1.036e-08,2.6867e-08,1.07e-09,2.2661e-09,1.0682e-08,4.5197e-09,2.169e-08,7.8385e-09,5.1388e-09,1.3185e-08,6.2293e-09,3.5464e-09,1.6868e-09,4.1947e-09,1.8859e-08,1.6056e-08,2.6106e-08,4.6103e-09,8.4911e-09,2.3683e-09,2.0406e-09,2.2182e-08,5.6917e-08,2.8757e-08,1.9338e-08,2.3193e-09,1.0156e-08,1.8393e-09,3.0023e-10,1.0275e-08,6.2869e-08,5.564e-07,1.264e-07,6.3457e-08,1.0698e-07,5.9114e-09,4.2512e-09,7.5524e-09,1.3393e-08,2.8214e-08,2.0761e-08,1.97e-08,1.0421e-08,1.3171e-08,3.1672e-09,1.1693e-07,8.2239e-09,3.0756e-08,8.5625e-09,2.0045e-08,2.6419e-08,3.5043e-08,1.1589e-08,2.9921e-08,7.5801e-09,1.4503e-08,6.2228e-08,2.6518e-08,3.2044e-08,4.565e-09,1.9522e-08,2.4215e-09,6.4557e-09,4.1182e-09,3.779e-09,9.0839e-08,1.7549e-09,2.7294e-09,1.2741e-08,9.3684e-09,4.1012e-07,5.8732e-09,1.437e-08,3.0387e-08,5.1577e-08,8.5423e-09,1.1094e-08,1.3291e-08,7.4743e-09,5.1677e-08,4.58e-09,5.372e-09,1.2137e-09,1.0495e-08,7.2545e-09,9.7155e-08,2.0994e-08,3.4023e-08,1.3562e-08,1.315e-08,1.0091e-08,2.8918e-09,4.3329e-08,1.9454e-09,3.3383e-09,4.7151e-09,1.9423e-08,4.9361e-09,1.1689e-09,3.9403e-08,2.6448e-08,2.1491e-09,2.7628e-08,4.3923e-08,1.6248e-08,1.1931e-07,1.9051e-08,6.5714e-08,1.8778e-08,2.7027e-09,3.3093e-09,1.3267e-08,8.2078e-09,8.2517e-09,1.8227e-09,8.0757e-08,2.1933e-08,8.7727e-08,1.719e-08,3.0527e-08,2.5163e-08,2.0151e-07,4.3327e-08,3.3509e-08,5.6445e-09,3.2955e-09,9.5103e-09,6.9374e-08,1.464e-08,7.7086e-09,6.8517e-09,6.6576e-09,1.9221e-08,2.1629e-08,5.8013e-08,1.2671e-08,3.741e-08,2.0715e-08,1.0229e-07,7.3077e-08,5.3731e-09,7.2179e-09,9.3905e-09,3.4286e-09,1.7189e-08,6.6259e-09,1.6177e-08,7.6028e-09,3.1497e-08,4.3762e-08,5.1051e-08,5.4187e-08,1.5394e-07,3.0586e-07,9.3951e-08,6.3523e-08,5.2873e-09,1.8902e-08,1.9219e-08,7.2535e-08,4.4144e-08,2.3773e-08,2.714e-08,8.2055e-09,3.1543e-08,7.2403e-08,1.2396e-07,1.0497e-08,1.8911e-08,4.189e-07,7.4434e-07,9.3736e-09,9.0346e-09,4.6886e-09,5.3172e-08,9.7501e-08,6.1879e-08,4.9014e-08,7.9087e-09,9.9234e-09,5.3533e-09,1.4829e-07,7.2745e-08,3.9221e-08,1.0673e-07,5.7273e-07,1.1672e-07,2.4627e-08,4.2479e-09,8.5224e-08,5.8767e-08,5.6529e-08,5.5414e-07,3.7674e-08,4.0596e-08,7.8983e-09,9.9523e-08,2.4431e-08,1.7619e-07,1.0634e-07,1.3764e-08,1.6704e-07,3.9974e-07,2.0541e-08,5.9729e-09,5.7406e-09,1.1568e-08,1.0837e-07,2.7688e-07,5.802e-08,1.0591e-08,8.6212e-09,2.2834e-08,1.6046e-08,1.2643e-07,5.3066e-08,2.4766e-08,2.431e-07,2.8665e-07,1.9428e-08,1.002e-08,8.6493e-09,4.9543e-08,1.5337e-07,6.7462e-08,5.5523e-07,6.6808e-08,2.5628e-08,1.9983e-09,1.8725e-08,3.0636e-07,1.062e-08
0.063158,1.3738e-08,6.4591e-08,2.0608e-08,8.0136e-09,3.6221e-09,9.5491e-09,7.8576e-08,1.4637e-07,2.6771e-08,2.4145e-07,4.8094e-09,3.4367e-09,1.2365e-08,3.0626e-08,8.5509e-08,3.9207e-08,7.022e-09,9.5344e-08,1.145e-08,5.2308e-09,2.5866e-09,1.062e-07,1.9616e-08,1.0767e-07,1.9442e-07,7.4442e-08,6.8488e-09,1.1977e-09,2.8465e-09,1.6128e-08,1.8928e-07,6.6202e-08,1.5121e-08,1.1235e-07,1.2287e-08,2.4755e-09,2.2907e-08,2.9259e-08,2.6079e-08,1.6749e-08,3.051e-08,4.1655e-08,4.0637e-09,9.4309e-09,2.9852e-09,1.2494e-08,8.1134e-08,6.5148e-09,2.0885e-08,1.5093e-07,1.7341e-08,1.6592e-08,6.6537e-09,2.1793e-09,1.1847e-08,5.8565e-09,6.8288e-09,6.2964e-09,6.3065e-09,3.4316e-09,6.8587e-09,1.6432e-07,9.6664e-09,1.0953e-08,6.0113e-09,1.5045e-08,5.3129e-08,6.2066e-08,2.3267e-09,1.9862e-08,1.3311e-08,1.203e-08,4.234e-09,5.6906e-09,2.2698e-09,1.8379e-09,1.2855e-08,1.0006e-08,7.3358e-08,4.8191e-09,2.3948e-07,2.2315e-08,3.7517e-09,1.916e-08,1.7316e-09,3.1269e-09,9.3089e-09,1.4123e-08,1.9126e-09,5.0489e-09,1.348e-09,4.9856e-09,1.3055e-08,2.0036e-08,8.2518e-08,1.4631e-08,4.8173e-09,1.7066e-08,4.2378e-08,2.4894e-08,6.8914e-09,1.1061e-09,9.7769e-10,4.4871e-09,1.3242e-09,1.7846e-09,1.3673e-09,8.1979e-09,1.4061e-08,1.032e-08,1.1139e-08,1.8178e-08,7.8926e-09,8.3703e-09,2.7713e-09,1.6571e-09,4.9509e-09,8.3964e-10,1.3663e-09,2.0095e-09,3.9776e-09,9.1346e-10,2.8916e-09,1.3368e-08,4.429e-09,2.2927e-09,5.8447e-09,9.5401e-09,1.1328e-08,4.0112e-09,1.0394e-08,4.1177e-09,4.6211e-09,2.0996e-10,3.2808e-09,4.7415e-09,2.5529e-09,2.9736e-09,1.0538e-09,5.7164e-09,1.3698e-09,7.7462e-08,9.4753e-09,6.3323e-08,1.9315e-08,2.7604e-08,4.2653e-09,5.1588e-09,1.6836e-09,4.8026e-09,1.1681e-08,2.644e-09,7.9902e-09,2.0639e-09,1.9234e-09,1.8083e-09,3.0895e-08,1.0229e-08,3.1465e-09,1.3486e-09,6.4576e-09,4.6103e-09,2.5825e-08,6.2158e-08,3.3153e-08,4.5584e-08,7.9476e-09,1.2053e-08,5.1936e-09,9.0654e-09,7.6957e-08,2.2397e-09,4.2285e-09,1.1842e-08,9.1385e-09,3.7851e-09,9.0394e-09,1.1651e-08,5.8812e-09,2.6606e-09,6.0738e-10,1.1579e-08,5.114e-08,3.7305e-07,5.015e-08,1.3853e-08,6.4559e-09,5.4097e-10,2.8632e-09,5.9734e-09,3.3879e-09,1.1107e-08,3.8819e-09,5.7563e-08,1.8082e-09,2.7699e-09,2.0549e-09,7.0733e-10,1.4531e-08,1.7275e-08,1.8715e-08,7.5295e-10,2.6725e-09,1.7955e-08,3.1452e-09,1.9258e-09,3.2234e-09,3.923e-09,1.4832e-08,2.0831e-07,2.2272e-09,1.6309e-08,1.6548e-09,3.9979e-09,2.921e-09,7.7015e-09,1.2557e-08,1.6845e-08,4.2772e-10,7.9482e-10,3.2414e-09,1.6377e-09,1.8064e-09,1.2962e-08,4.4956e-08,8.4782e-08,6.416e-10,2.0269e-10,3.986e-10,8.6449e-10,4.7807e-09,1.3856e-08,1.5423e-08,3.1819e-08,5.7917e-10,3.1322e-08,1.5848e-10,8.8047e-10,1.3224e-08,5.0561e-09,6.2461e-09,3.5664e-09,1.1015e-09,1.0888e-09,6.9545e-10,6.9112e-10,3.6341e-09,2.6493e-09,6.7842e-09,3.6607e-09,3.0646e-08,1.0439e-09,5.5649e-09,1.4705e-09,1.4317e-07,6.4438e-09,7.2609e-09,1.1044e-09,1.0859e-09,2.9396e-10,1.1473e-09,5.8324e-10,3.9164e-09,6.7653e-09,2.796e-09,1.1298e-08,7.8917e-10,1.8371e-09,7.6371e-10,1.6418e-09,4.2043e-08,7.8677e-09,6.9684e-09,2.1077e-09,2.2155e-09,2.1325e-09,3.7137e-10,2.3075e-09,1.635e-08,3.7227e-09,5.3227e-09,1.9035e-08,6.2587e-10,1.5589e-09,4.6564e-09,2.7827e-09,1.1421e-08,2.7335e-09,2.0371e-09,7.3831e-09,3.7737e-09,1.9498e-09,1.0406e-09,2.3997e-09,1.0994e-08,8.7126e-09,1.3136e-08,2.8577e-09,4.5439e-09,1.6763e-09,1.2778e-09,2.2275e-08,4.2949e-08,1.2202e-08,7.9589e-09,1.3823e-09,6.2028e-09,9.6783e-10,2.3164e-10,6.0629e-09,3.3073e-08,4.0471e-07,6.3561e-08,3.4683e-08,4.8504e-08,3.6806e-09,2.5566e-09,4.3228e-09,7.7763e-09,2.0798e-08,8.5206e-09,1.2908e-08,5.9442e-09,6.3646e-09,1.7378e-09,4.4654e-08,4.4907e-09,1.7077e-08,4.422e-09,1.2165e-08,1.6397e-08,2.1916e-08,5.5456e-09,2.7428e-08,2.9951e-09,5.7797e-09,2.587e-08,1.5101e-08,3.1465e-08,2.2329e-09,1.7809e-08,1.4055e-09,3.5407e-09,2.0392e-09,1.8738e-09,3.9222e-08,9.923e-10,1.5566e-09,6.9488e-09,5.3015e-09,3.3279e-07,2.7842e-09,5.8594e-09,1.6428e-08,3.0759e-08,4.8839e-09,6.5166e-09,9.7309e-09,3.7212e-09,3.7377e-08,2.2327e-09,3.1068e-09,7.2171e-10,5.7914e-09,4.4497e-09,7.5153e-08,1.1058e-08,1.4651e-08,5.5986e-09,6.4021e-09,5.1812e-09,1.6011e-09,2.5386e-08,1.1914e-09,1.8683e-09,2.3145e-09,7.4365e-09,2.9036e-09,6.5549e-10,2.334e-08,1.2309e-08,1.3773e-09,1.3104e-08,1.7789e-08,6.7639e-09,7.8171e-08,1.052e-08,3.2168e-08,1.2708e-08,1.635e-09,1.8408e-09,7.1253e-09,5.9088e-09,4.9042e-09,1.0817e-09,4.8227e-08,1.1241e-08,6.891e-08,8.1144e-09,1.2625e-08,1.0374e-08,1.1677e-07,2.3319e-08,2.1348e-08,3.1896e-09,1.9975e-09,5.4372e-09,1.6781e-08,7.1356e-09,4.2602e-09,4.5209e-09,3.6614e-09,1.1357e-08,1.09e-08,2.8695e-08,4.9596e-09,1.3338e-08,9.4222e-09,5.4411e-08,5.6701e-08,2.9266e-09,4.1513e-09,5.2812e-09,1.6428e-09,1.0931e-08,3.5988e-09,9.9159e-09,4.045e-09,1.846e-08,2.6371e-08,2.3349e-08,2.5164e-08,7.3504e-08,1.9073e-07,4.4947e-08,2.6298e-08,3.1513e-09,1.1075e-08,1.0899e-08,3.4275e-08,2.2366e-08,1.3706e-08,1.4303e-08,4.9755e-09,1.8302e-08,3.9168e-08,5.6926e-08,4.262e-09,7.7324e-09,1.0638e-07,5.5739e-07,5.3241e-09,5.2452e-09,2.7686e-09,2.7859e-08,3.6619e-08,2.7113e-08,2.556e-08,4.512e-09,5.6399e-09,2.7704e-09,7.8262e-08,1.9729e-08,1.5296e-08,4.985e-08,3.7724e-07,4.8848e-08,1.1981e-08,2.4956e-09,4.0743e-08,3.912e-08,2.9403e-08,1.7117e-07,2.1263e-08,2.6341e-08,4.6216e-09,7.4832e-08,1.2012e-08,6.4796e-08,6.1525e-08,5.1988e-09,5.5888e-08,1.1704e-07,1.2205e-08,3.6181e-09,3.2939e-09,5.8207e-09,5.2913e-08,1.3648e-07,3.1202e-08,6.3832e-09,5.2578e-09,1.262e-08,7.9759e-09,4.0833e-08,2.3417e-08,1.3052e-08,7.501e-08,2.2329e-07,1.2196e-08,5.4282e-09,4.7162e-09,2.7845e-08,7.3151e-08,3.2563e-08,3.3081e-07,2.9382e-08,1.557e-08,9.2911e-10,8.9747e-09,1.8726e-07,4.4548e-09
0.068421,5.5939e-09,1.9274e-08,1.0869e-08,4.1486e-09,2.454e-09,5.345e-09,3.8727e-08,6.3622e-08,1.2745e-08,1.0267e-07,2.5338e-09,1.8887e-09,6.5416e-09,1.3048e-08,2.5692e-08,1.3583e-08,2.6513e-09,4.0338e-08,4.8027e-09,2.5478e-09,1.4289e-09,8.9786e-08,1.0911e-08,5.5976e-08,6.9959e-08,6.8709e-08,3.4692e-09,5.959e-10,1.3966e-09,7.6942e-09,1.5926e-07,1.0226e-08,4.8322e-09,5.2675e-08,5.5705e-09,1.1355e-09,1.7571e-08,1.2523e-08,1.2748e-08,7.5943e-09,1.2166e-08,1.945e-08,1.9429e-09,6.1066e-09,1.7067e-09,5.8616e-09,4.4393e-08,2.6803e-09,7.7488e-09,1.0533e-07,8.5019e-09,7.9104e-09,6.1133e-09,1.7427e-09,6.3861e-09,2.9042e-09,3.3232e-09,3.2378e-09,3.1074e-09,1.8931e-09,3.5976e-09,4.8893e-08,2.779e-09,4.3182e-09,2.602e-09,6.8882e-09,3.1625e-08,2.0605e-08,1.3548e-09,9.1667e-09,8.2168e-09,5.2242e-09,2.0319e-09,2.9888e-09,1.3284e-09,1.1054e-09,8.242e-09,4.8194e-09,4.1617e-08,1.9031e-09,1.1332e-07,9.0597e-09,1.8639e-09,1.3848e-08,9.0216e-10,1.9073e-09,4.6488e-09,4.9604e-09,9.3268e-10,2.6463e-09,7.5152e-10,2.522e-09,7.6111e-09,1.0682e-08,5.9052e-08,4.9843e-09,1.9703e-09,7.8026e-09,4.3971e-08,1.2254e-08,3.6094e-09,6.1705e-10,5.0465e-10,2.1847e-09,6.4444e-10,9.4839e-10,7.4624e-10,4.6652e-09,7.0227e-09,5.1485e-09,4.8273e-09,6.9384e-09,3.1429e-09,3.7446e-09,1.5226e-09,1.0149e-09,2.5415e-09,4.9213e-10,7.3473e-10,1.0706e-09,2.0564e-09,4.9616e-10,1.8406e-09,6.941e-09,2.5285e-09,1.3947e-09,2.6308e-09,4.4412e-09,4.3778e-09,1.9875e-09,4.7856e-09,2.4538e-09,2.4456e-09,9.3114e-11,1.7631e-09,2.2355e-09,1.2701e-09,1.6037e-09,5.8245e-10,3.1619e-09,7.6175e-10,5.0457e-08,4.4753e-09,3.1604e-08,7.9297e-09,1.2381e-08,1.9302e-09,2.5476e-09,9.1203e-10,1.5485e-09,7.3762e-09,1.1881e-09,3.7997e-09,1.0053e-09,1.059e-09,9.7822e-10,1.6182e-08,3.392e-09,1.4574e-09,6.171e-10,2.4723e-09,2.4699e-09,7.9527e-09,4.2507e-08,1.9188e-08,2.8358e-08,4.3032e-09,6.4951e-09,2.3048e-09,4.9394e-09,2.2296e-08,1.3024e-09,1.9489e-09,8.0189e-09,5.9189e-09,1.3334e-09,3.4573e-09,5.3845e-09,3.3788e-09,1.4365e-09,3.5825e-10,1.102e-08,3.4928e-08,2.6137e-07,2.0555e-08,6.3068e-09,3.6196e-09,3.1849e-10,1.5654e-09,3.4989e-09,1.6283e-09,4.4354e-09,1.2923e-09,4.0911e-08,1.0505e-09,1.7831e-09,1.2679e-09,3.8297e-10,7.3307e-09,8.1519e-09,8.7464e-09,3.664e-10,1.5725e-09,1.2898e-08,1.6402e-09,1.176e-09,1.5735e-09,1.5101e-09,7.7871e-09,7.4326e-08,1.2236e-09,5.7323e-09,1.1792e-09,3.7166e-09,1.4912e-09,3.6889e-09,6.3475e-09,5.0581e-09,2.3101e-10,4.8203e-10,1.4991e-09,4.9664e-10,9.4157e-10,5.3959e-09,1.508e-08,2.2678e-08,3.2538e-10,1.0167e-10,2.34e-10,5.2755e-10,2.7198e-09,7.6187e-09,8.2428e-09,3.497e-08,3.2027e-10,1.3529e-08,1.277e-10,4.7326e-10,5.6985e-09,1.8127e-09,3.1552e-09,1.926e-09,5.9478e-10,6.4361e-10,4.3389e-10,4.1949e-10,1.713e-09,1.1004e-09,3.1362e-09,2.152e-09,2.2584e-08,5.5526e-10,1.9467e-09,8.2772e-10,6.317e-08,2.3707e-09,2.7457e-09,5.7163e-10,5.8521e-10,1.6225e-10,6.8308e-10,3.2398e-10,2.1784e-09,2.7655e-09,1.4297e-09,7.8444e-09,4.7474e-10,1.1253e-09,4.7746e-10,1.7222e-09,2.8766e-08,3.0824e-09,2.57e-09,1.0109e-09,1.2555e-09,1.2788e-09,2.129e-10,1.3179e-09,1.6036e-08,1.733e-09,2.5644e-09,1.3624e-08,3.4414e-10,1.0293e-09,2.0394e-09,1.6656e-09,5.6147e-09,8.9717e-10,8.6939e-10,4.0033e-09,2.2115e-09,1.0165e-09,6.1352e-10,1.2963e-09,6.1445e-09,4.6776e-09,6.1795e-09,1.6862e-09,2.3223e-09,1.1349e-09,7.5809e-10,9.2358e-09,3.5254e-08,4.8635e-09,3.0918e-09,7.9046e-10,3.6248e-09,4.8268e-10,1.6661e-10,3.3528e-09,1.6304e-08,1.1631e-07,3.0325e-08,1.7766e-08,3.7687e-08,2.1524e-09,1.4508e-09,2.3447e-09,4.2311e-09,8.1441e-09,3.3102e-09,8.0811e-09,3.1794e-09,2.9695e-09,8.6738e-10,1.8023e-08,2.3059e-09,8.5589e-09,2.1703e-09,7.1557e-09,9.7481e-09,1.2823e-08,2.544e-09,1.2615e-08,1.1587e-09,2.1661e-09,9.9158e-09,8.2613e-09,1.2229e-08,1.0335e-09,8.1746e-09,7.7096e-10,1.8166e-09,9.4837e-10,8.7829e-10,3.0046e-08,5.288e-10,8.3285e-10,3.4745e-09,3.2903e-09,1.8778e-07,1.3051e-09,2.2381e-09,8.4138e-09,1.6509e-08,2.7131e-09,3.5935e-09,4.2095e-09,1.8468e-09,2.009e-08,1.0211e-09,1.6899e-09,4.0447e-10,2.8892e-09,2.5522e-09,3.959e-08,5.5596e-09,5.9355e-09,2.1785e-09,2.9084e-09,2.5374e-09,8.6249e-10,1.4132e-08,6.9629e-10,9.7867e-10,1.0691e-09,3.0346e-09,1.6184e-09,3.4185e-10,1.3272e-08,4.8003e-09,8.4511e-10,5.6998e-09,6.6037e-09,2.6743e-09,5.5309e-08,5.3925e-09,1.3962e-08,8.4585e-09,9.3132e-10,9.606e-10,4.1309e-09,2.8964e-09,2.9825e-09,6.0373e-10,2.571e-08,5.2943e-09,4.0815e-08,3.5497e-09,4.9459e-09,4.0049e-09,6.0778e-08,1.2002e-08,1.2823e-08,1.6933e-09,1.1481e-09,2.9453e-09,5.6294e-09,3.5096e-09,2.2062e-09,2.9019e-09,1.8989e-09,6.2934e-09,5.272e-09,1.3187e-08,1.8692e-09,4.6354e-09,3.9898e-09,1.6446e-08,4.0735e-08,1.4769e-09,2.2405e-09,2.7966e-09,7.2449e-10,5.1982e-09,1.8272e-09,5.6391e-09,2.0338e-09,7.2538e-09,1.4669e-08,9.8658e-09,1.1109e-08,2.896e-08,4.04e-08,2.147e-08,1.0902e-08,1.7947e-09,6.2379e-09,5.822e-09,1.5112e-08,1.0719e-08,7.4576e-09,6.9821e-09,2.8436e-09,9.9472e-09,2.0184e-08,2.3885e-08,1.6212e-09,2.9762e-09,3.5331e-08,3.906e-07,2.8465e-09,2.8277e-09,1.5447e-09,1.3616e-08,1.4541e-08,1.1355e-08,1.2428e-08,2.4463e-09,3.0795e-09,1.3178e-09,3.8127e-08,6.2638e-09,5.6293e-09,2.2676e-08,1.7629e-07,1.9846e-08,5.5727e-09,1.3797e-09,3.0933e-08,2.6403e-08,1.4295e-08,4.8914e-08,1.1375e-08,1.6558e-08,2.5362e-09,1.6013e-08,5.5454e-09,2.2932e-08,4.4603e-08,1.8303e-09,1.883e-08,3.9555e-08,6.6811e-09,2.0923e-09,1.8077e-09,3.3982e-09,2.3947e-08,6.2489e-08,1.5754e-08,3.75e-09,3.0524e-09,6.5444e-09,3.7681e-09,1.278e-08,7.6226e-09,7.8816e-09,2.3269e-08,8.645e-08,7.5484e-09,2.7491e-09,2.3848e-09,1.4883e-08,3.2589e-08,1.4775e-08,1.9192e-07,1.2303e-08,9.1872e-09,4.1096e-10,3.9954e-09,1.315e-07,1.7474e-09
0.073684,2.1149e-09,5.5391e-09,6.4623e-09,2.0013e-09,1.6003e-09,2.843e-09,1.7874e-08,2.5278e-08,5.5747e-09,3.8677e-08,1.241e-09,9.6745e-10,3.2254e-09,5.0923e-09,7.6128e-09,2.7648e-09,9.5576e-10,2.3438e-08,1.8105e-09,1.1407e-09,7.3347e-10,9.5835e-08,5.7755e-09,2.7252e-08,2.6086e-08,2.6996e-08,1.5955e-09,2.7162e-10,6.2537e-10,3.414e-09,6.47e-08,2.1897e-09,1.4972e-09,2.5419e-08,2.3566e-09,4.8754e-10,6.3128e-09,5.0433e-09,5.724e-09,3.2078e-09,8.31e-09,8.3731e-09,8.4932e-10,3.9109e-09,9.4064e-10,2.5365e-09,2.453e-08,1.0296e-09,2.6768e-09,2.6679e-08,3.8407e-09,3.5987e-09,2.5329e-09,1.2e-09,3.2082e-09,1.3569e-09,1.6702e-09,1.5472e-09,1.4018e-09,9.6958e-10,1.7504e-09,1.5306e-08,8.5773e-10,1.5856e-09,1.0684e-09,3.0549e-09,1.7844e-08,7.2626e-09,7.367e-10,6.3737e-09,4.9469e-09,2.0923e-09,9.0053e-10,1.4504e-09,7.4314e-10,6.2926e-10,5.4696e-09,2.115e-09,9.7623e-09,7.1492e-10,4.6025e-08,3.3115e-09,9.1236e-10,5.2698e-09,4.3587e-10,1.1183e-09,2.1473e-09,1.9129e-09,4.2528e-10,1.2827e-09,3.933e-10,1.1705e-09,4.414e-09,5.1691e-09,1.7438e-08,1.6151e-09,7.4843e-10,3.2738e-09,1.6616e-08,5.8884e-09,1.8195e-09,3.1985e-10,2.4147e-10,9.826e-10,2.8851e-10,4.7063e-10,3.7663e-10,2.4694e-09,3.1878e-09,2.3686e-09,1.9199e-09,2.454e-09,1.1857e-09,1.5581e-09,8.253e-10,6.0723e-10,1.2122e-09,2.7304e-10,3.6605e-10,5.6592e-10,1.094e-09,2.4852e-10,1.1378e-09,3.3581e-09,1.3363e-09,8.6227e-10,1.0853e-09,1.9229e-09,1.5978e-09,8.9964e-10,1.9989e-09,1.3934e-09,1.1867e-09,3.3461e-11,8.7738e-10,9.774e-10,5.8321e-10,8.0469e-10,2.9661e-10,1.63e-09,4.1518e-10,1.4349e-08,1.9324e-09,1.6055e-08,2.9941e-09,5.1323e-09,8.3742e-10,1.1783e-09,4.5578e-10,5.1749e-10,4.776e-09,4.829e-10,1.6299e-09,4.4725e-10,5.3954e-10,4.911e-10,6.9651e-09,1.149e-09,6.134e-10,3.1217e-10,8.7905e-10,1.3948e-09,2.4599e-09,1.988e-08,1.1234e-08,1.6154e-08,2.1856e-09,3.3263e-09,9.5902e-10,2.5317e-09,7.343e-09,7.1582e-10,8.3731e-10,6.345e-09,1.5535e-09,4.4182e-10,1.2141e-09,2.2928e-09,1.822e-09,7.1964e-10,1.9839e-10,4.1575e-09,3.1944e-08,1.2119e-07,7.7937e-09,2.6136e-09,1.8907e-09,1.7808e-10,7.972e-10,1.957e-09,7.1004e-10,1.6116e-09,3.8531e-10,1.256e-08,5.7669e-10,1.1271e-09,7.3547e-10,1.9231e-10,3.3632e-09,3.5349e-09,3.745e-09,1.6745e-10,8.6447e-10,3.8338e-09,7.9852e-10,6.8314e-10,7.0112e-10,5.5801e-10,4.439e-09,4.7575e-08,6.2866e-10,1.9435e-09,8.0564e-10,1.6663e-09,7.0795e-10,1.6205e-09,2.9725e-09,1.7027e-09,1.1619e-10,2.7517e-10,6.5392e-10,2.8037e-10,4.5694e-10,2.1632e-09,6.2773e-09,6.8849e-09,1.5401e-10,4.639e-11,1.2861e-10,3.0182e-10,1.4817e-09,3.9901e-09,3.8913e-09,1.209e-08,1.7266e-10,9.7694e-09,1.0165e-10,2.404e-10,2.277e-09,5.9978e-10,1.497e-09,9.6508e-10,2.9905e-10,3.5178e-10,2.546e-10,2.4062e-10,7.8939e-10,4.5932e-10,2.1308e-09,1.2355e-09,1.4755e-08,2.704e-10,7.3117e-10,4.3578e-10,1.3082e-08,8.0297e-10,9.674e-10,3.1023e-10,2.9599e-10,8.3471e-11,3.7825e-10,1.6639e-10,1.1595e-09,1.0871e-09,6.8014e-10,5.7528e-09,2.7428e-10,6.4348e-10,2.9291e-10,5.8195e-10,2.239e-08,1.1387e-09,8.659e-10,4.4315e-10,6.9293e-10,7.4962e-10,1.1334e-10,7.1803e-10,6.0855e-09,7.3918e-10,1.1415e-09,1.0222e-08,1.7592e-10,6.4843e-10,8.6183e-10,9.7458e-10,2.5134e-09,2.8129e-10,3.6808e-10,2.1225e-09,1.2555e-09,4.9477e-10,3.4281e-10,6.5344e-10,3.289e-09,2.5648e-09,2.6724e-09,9.3161e-10,1.105e-09,7.2837e-10,4.2022e-10,6.9409e-09,1.7533e-08,1.7923e-09,1.1168e-09,4.2864e-10,2.0019e-09,2.4634e-10,1.1053e-10,1.7118e-09,7.4086e-09,3.3629e-08,1.3562e-08,8.446e-09,1.5662e-08,1.1655e-09,7.6498e-10,1.1879e-09,2.1344e-09,3.0484e-09,1.2038e-09,4.9377e-09,1.5798e-09,1.3118e-09,3.819e-10,7.2322e-09,1.0983e-09,3.6971e-09,9.9922e-10,4.1192e-09,5.5143e-09,6.9328e-09,1.095e-09,9.2261e-09,4.1636e-10,7.5036e-10,3.4373e-09,4.3886e-09,6.6642e-09,4.483e-10,5.9218e-09,3.9619e-10,8.5764e-10,4.0902e-10,3.8535e-10,1.0859e-08,2.6454e-10,4.1199e-10,1.5658e-09,1.5204e-09,6.1437e-08,5.6914e-10,7.8458e-10,4.0491e-09,7.6309e-09,1.449e-09,1.833e-09,2.9569e-09,8.8347e-10,1.2784e-08,4.3146e-10,8.5217e-10,2.1229e-10,1.2527e-09,1.3486e-09,1.0768e-08,2.6579e-09,2.227e-09,7.8238e-10,1.2157e-09,1.1656e-09,4.4541e-10,7.448e-09,3.8676e-10,4.7293e-10,4.5913e-10,1.2132e-09,8.4739e-10,1.6312e-10,7.294e-09,1.9253e-09,4.9138e-10,2.2351e-09,2.1895e-09,9.8955e-10,2.7586e-08,2.5121e-09,5.4645e-09,5.6214e-09,4.9274e-10,4.6419e-10,1.7756e-09,1.9239e-09,1.9036e-09,3.1273e-10,1.1846e-08,2.2574e-09,1.2982e-08,1.4188e-09,1.8117e-09,1.4203e-09,2.7378e-08,5.7904e-09,7.0813e-09,8.3388e-10,6.2066e-10,1.4984e-09,2.0436e-09,1.7367e-09,1.0545e-09,1.8313e-09,9.1752e-10,3.2137e-09,2.4141e-09,5.5093e-09,6.644e-10,1.5237e-09,1.5469e-09,6.1984e-09,1.0634e-08,6.7713e-10,1.1198e-09,1.3768e-09,2.8778e-10,3.0592e-09,8.5356e-10,2.9068e-09,9.5325e-10,3.2201e-09,7.3173e-09,3.7776e-09,4.6184e-09,8.8906e-09,1.0231e-08,1.0285e-08,4.3816e-09,9.7668e-10,3.3811e-09,2.8934e-09,6.1497e-09,4.8202e-09,3.783e-09,3.1062e-09,1.5093e-09,4.9843e-09,1.0119e-08,8.8741e-09,5.6806e-10,1.0569e-09,1.2421e-08,2.1984e-07,1.4146e-09,1.3861e-09,8.0319e-10,6.1054e-09,5.767e-09,4.4471e-09,5.5414e-09,1.2481e-09,1.5986e-09,5.7011e-10,1.692e-08,2.0932e-09,1.9159e-09,1.0162e-08,1.0932e-07,7.617e-09,2.439e-09,7.0704e-10,1.294e-08,1.9374e-08,6.396e-09,1.4724e-08,5.7231e-09,1.009e-08,1.286e-09,4.9264e-09,2.3726e-09,7.7044e-09,1.7185e-08,5.9001e-10,6.3022e-09,1.4369e-08,3.2844e-09,1.1473e-09,9.3964e-10,2.2701e-09,9.859e-09,2.6075e-08,7.3734e-09,2.1832e-09,1.6731e-09,3.1424e-09,1.6691e-09,3.7752e-09,1.8617e-09,3.4319e-09,6.9422e-09,2.529e-08,4.676e-09,1.2816e-09,1.0959e-09,7.49e-09,1.3329e-08,6.2035e-09,1.0948e-07,4.823e-09,5.3157e-09,1.8744e-10,1.6216e-09,5.802e-08,6.2876e-10
0.078947,7.1489e-10,1.4691e-09,2.824e-09,8.8476e-10,9.8711e-10,1.4511e-09,7.6264e-09,8.9056e-09,2.1952e-09,1.3227e-08,5.5593e-10,4.5344e-10,1.4542e-09,1.7883e-09,2.1252e-09,6.4396e-10,3.2095e-10,2.8929e-09,5.9455e-10,4.5934e-10,3.425e-10,3.0011e-08,2.9071e-09,1.2223e-08,9.2062e-09,1.1288e-08,6.4969e-10,1.1361e-10,2.4843e-10,1.3882e-09,2.5063e-08,4.881e-10,4.3116e-10,1.4354e-08,9.1094e-10,2.2729e-10,1.9196e-09,1.8557e-09,2.3018e-09,1.2334e-09,1.8682e-09,3.2501e-09,3.3352e-10,2.5927e-09,4.8785e-10,9.8956e-10,1.1293e-08,3.5832e-10,8.3281e-10,5.8063e-09,1.5629e-09,1.5042e-09,1.7563e-09,7.3019e-10,1.4751e-09,5.8328e-10,1.1136e-09,6.7528e-10,5.6427e-10,4.5045e-10,7.7522e-10,4.6278e-09,3.8801e-10,5.3028e-10,4.0331e-10,1.335e-09,9.5646e-09,2.5027e-09,3.6654e-10,1.5672e-09,2.9422e-09,7.5096e-10,3.5937e-10,6.3511e-10,3.8812e-10,3.3289e-10,4.4881e-09,8.2586e-10,2.8455e-09,2.4873e-10,1.5258e-08,1.058e-09,4.3239e-10,1.2681e-09,1.921e-10,6.353e-10,8.9702e-10,7.8311e-10,1.7815e-10,5.6158e-10,1.913e-10,4.8498e-10,2.9109e-09,2.1973e-09,3.9864e-09,4.8086e-10,2.5656e-10,1.2293e-09,9.1413e-09,2.7779e-09,8.7653e-10,1.5101e-10,1.0487e-10,3.9842e-10,1.1563e-10,2.1461e-10,1.7251e-10,1.187e-09,1.2833e-09,9.8259e-10,6.8223e-10,7.8015e-10,4.138e-10,5.9196e-10,4.3859e-10,3.5251e-10,5.2715e-10,1.4012e-10,1.6549e-10,3.4854e-10,4.8876e-10,1.1218e-10,6.9219e-10,1.4966e-09,6.3639e-10,5.4707e-10,4.0046e-10,7.6651e-10,5.3374e-10,3.6475e-10,7.4462e-10,7.6561e-10,5.1358e-10,8.9876e-12,3.9557e-10,3.8671e-10,2.4076e-10,3.6847e-10,1.3587e-10,7.6967e-10,2.2018e-10,4.9242e-09,7.4659e-10,9.5264e-09,1.0053e-09,1.9051e-09,3.3841e-10,4.9877e-10,2.0439e-10,1.68e-10,3.5696e-09,1.7173e-10,6.0754e-10,1.7743e-10,2.4849e-10,2.2463e-10,2.406e-09,3.7808e-10,2.2926e-10,1.4284e-10,2.823e-10,6.3836e-10,7.8029e-10,5.9709e-09,6.8059e-09,7.918e-09,1.0259e-09,1.6069e-09,3.6788e-10,1.2076e-09,2.4029e-09,3.6624e-10,3.257e-10,2.8492e-09,5.2312e-10,1.3778e-10,3.8026e-10,8.7638e-10,8.9918e-10,3.2595e-10,1.0137e-10,1.1485e-09,1.081e-08,7.5747e-08,2.6313e-09,9.6752e-10,9.0351e-10,9.3503e-11,3.6891e-10,1.0361e-09,2.7494e-10,5.1656e-10,9.9167e-11,2.7124e-09,2.9399e-10,7.2851e-10,3.9652e-10,8.8166e-11,1.3673e-09,1.3708e-09,1.4275e-09,7.2139e-11,4.3543e-10,1.2664e-09,3.5346e-10,3.7234e-10,2.7742e-10,1.9069e-10,1.8901e-09,1.0169e-08,2.9606e-10,6.5979e-10,5.2359e-10,1.2029e-09,3.0615e-10,6.351e-10,1.2546e-09,6.0362e-10,5.3508e-11,1.4537e-10,2.5943e-10,1.6047e-10,2.0357e-10,8.6564e-10,2.3755e-09,2.065e-09,6.6913e-11,1.9127e-11,6.4956e-11,1.5857e-10,7.7796e-10,1.9663e-09,1.5611e-09,5.2085e-09,9.6546e-11,1.6441e-09,6.9107e-11,1.1341e-10,8.235e-10,1.787e-10,6.8109e-10,4.4202e-10,1.3709e-10,1.7431e-10,1.3831e-10,1.2821e-10,3.5219e-10,1.8953e-10,4.2231e-10,7.1667e-10,6.9395e-09,1.1792e-10,2.6777e-10,2.103e-10,3.2328e-09,2.4422e-10,3.1462e-10,1.595e-10,1.3797e-10,3.9573e-11,1.9021e-10,7.7135e-11,6.0348e-10,3.9376e-10,2.9499e-10,5.262e-09,1.5201e-10,3.3508e-10,1.8284e-10,5.5165e-10,9.995e-09,3.931e-10,2.5817e-10,1.7373e-10,3.8319e-10,4.8668e-10,5.475e-11,3.6977e-10,2.5217e-09,2.8137e-10,4.5877e-10,9.0178e-09,8.2172e-11,3.8685e-10,3.3829e-10,5.7113e-10,9.8772e-10,8.6905e-11,1.4145e-10,1.135e-09,7.002e-10,2.1968e-10,1.7834e-10,3.0167e-10,1.7033e-09,1.5051e-09,1.035e-09,4.7048e-10,4.7597e-10,4.3631e-10,2.1299e-10,1.7856e-09,1.1949e-08,5.9617e-10,3.6645e-10,2.1564e-10,1.0215e-09,1.5056e-10,6.6787e-11,7.8795e-10,3.0238e-09,1.02e-08,5.5889e-09,3.681e-09,4.3775e-09,5.7297e-10,3.6662e-10,5.4921e-10,9.8334e-10,4.9261e-10,4.0442e-10,3.2106e-09,7.233e-10,5.3565e-10,1.4789e-10,2.764e-09,4.758e-10,1.3024e-09,4.2223e-10,2.4174e-09,2.941e-09,3.4066e-09,4.2983e-10,2.4043e-09,1.3332e-10,2.3373e-10,1.0476e-09,2.3595e-09,1.2715e-09,1.8026e-10,1.7215e-09,1.8759e-10,3.6247e-10,1.6055e-10,1.5588e-10,3.149e-09,1.23e-10,1.8396e-10,6.2024e-10,9.1934e-10,2.0544e-08,2.2158e-10,2.4476e-10,1.8166e-09,2.8685e-09,7.3527e-10,8.4456e-10,1.4184e-09,3.9395e-10,5.0071e-09,1.6454e-10,3.8915e-10,1.0448e-10,4.4271e-10,6.4173e-10,3.2514e-09,1.206e-09,7.5684e-10,2.5163e-10,4.5733e-10,4.9056e-10,2.1431e-10,3.7082e-09,2.0369e-10,2.0606e-10,1.7973e-10,4.4609e-10,4.1209e-10,6.9563e-11,3.9883e-09,7.4743e-10,2.6808e-10,7.6773e-10,6.2202e-10,3.3558e-10,1.7535e-08,1.03e-09,2.0046e-09,3.8944e-09,2.3702e-10,2.035e-10,7.4742e-10,5.6341e-10,1.4542e-09,1.4722e-10,4.5405e-09,8.4994e-10,4.7662e-09,5.0706e-10,6.091e-10,4.4936e-10,9.7372e-09,2.5597e-09,3.4183e-09,3.736e-10,3.12e-10,7.0759e-10,7.6096e-10,8.8039e-10,4.5381e-10,1.1794e-09,4.0584e-10,1.4682e-09,1.026e-09,2.0242e-09,2.1582e-10,4.5649e-10,5.3626e-10,3.2533e-09,3.2792e-09,2.735e-10,5.0766e-10,6.179e-10,9.9926e-11,6.3724e-10,3.5798e-10,1.3346e-09,4.073e-10,1.3896e-09,3.1325e-09,1.2707e-09,1.7881e-09,2.1379e-09,2.624e-09,4.945e-09,1.6646e-09,5.1074e-10,1.7832e-09,1.313e-09,2.2933e-09,2.0092e-09,1.7559e-09,1.2302e-09,7.2584e-10,2.2458e-09,5.5245e-09,2.8024e-09,1.7871e-10,3.3613e-10,6.3272e-09,7.7483e-08,6.408e-10,5.9632e-10,3.8119e-10,2.446e-09,2.1618e-09,1.5809e-09,2.2068e-09,5.8771e-10,7.7948e-10,2.2883e-10,6.7127e-09,6.8199e-10,5.8617e-10,4.7131e-09,1.7394e-08,2.6796e-09,9.8689e-10,3.2742e-10,3.2078e-09,9.5345e-09,2.5744e-09,4.2362e-09,2.6819e-09,5.9732e-09,5.8817e-10,1.8623e-09,9.2264e-10,2.4148e-09,4.2465e-09,1.7052e-10,2.1036e-09,5.8743e-09,1.4148e-09,5.9074e-10,4.5381e-10,1.4705e-09,3.5837e-09,9.6129e-09,3.1339e-09,1.3321e-09,8.5589e-10,1.3696e-09,6.7945e-10,1.0206e-09,3.7137e-10,1.9893e-09,1.9099e-09,3.5455e-09,3.0135e-09,5.3643e-10,4.4385e-10,3.49e-09,4.8667e-09,2.3497e-09,6.4236e-08,1.7333e-09,3.1258e-09,9.7241e-11,5.8212e-10,3.5952e-08,2.0151e-10
0.084211,2.0212e-10,3.4148e-10,1.1831e-09,3.495e-10,5.5846e-10,7.6642e-10,2.9751e-09,2.637e-09,7.5481e-10,4.3064e-09,2.2217e-10,1.8857e-10,5.7931e-10,5.4906e-10,5.2804e-10,1.4002e-10,9.7759e-11,6.6871e-10,1.6099e-10,1.6012e-10,1.4047e-10,4.9174e-08,1.4147e-09,4.9174e-09,2.8547e-09,2.4437e-09,2.2562e-10,4.6088e-11,8.3569e-11,5.0754e-10,3.6336e-09,1.0084e-10,1.0917e-10,5.3955e-09,3.1123e-10,1.2925e-10,7.3601e-10,5.9617e-10,7.9471e-10,4.1503e-10,4.9333e-10,1.0967e-09,1.1468e-10,2.2724e-09,2.2858e-10,3.349e-10,5.4378e-09,1.075e-10,2.2114e-10,1.2922e-09,5.5142e-10,5.5177e-10,4.1807e-10,3.9534e-10,6.0291e-10,2.2012e-10,3.889e-10,2.6163e-10,1.9416e-10,1.818e-10,3.0305e-10,1.2824e-09,1.8303e-10,1.5658e-10,1.3391e-10,6.3846e-10,5.4058e-09,7.9616e-10,1.6143e-10,4.422e-10,1.8158e-09,2.3026e-10,1.2355e-10,2.4116e-10,1.8196e-10,1.5865e-10,1.8434e-09,2.7687e-10,8.2537e-10,7.7079e-11,3.8754e-09,2.8217e-10,1.8955e-10,3.2366e-10,7.5384e-11,3.6625e-10,3.2598e-10,3.3447e-10,6.6496e-11,2.1342e-10,8.5818e-11,1.7099e-10,1.2021e-09,7.7878e-10,9.2025e-10,1.2484e-10,7.5919e-11,3.9588e-10,1.7858e-09,1.3691e-09,4.0355e-10,6.2781e-11,3.9959e-11,1.4176e-10,3.9459e-11,8.7686e-11,6.9529e-11,4.9543e-10,4.3886e-10,3.5437e-10,2.0665e-10,2.12e-10,1.2898e-10,1.9973e-10,2.2852e-10,2.0403e-10,2.025e-10,6.3639e-11,6.5536e-11,1.3227e-10,2.5742e-10,4.3851e-11,4.4016e-10,6.0847e-10,2.6085e-10,4.0319e-10,1.2688e-10,2.7832e-10,1.5512e-10,1.2812e-10,2.4004e-10,4.7824e-10,1.8871e-10,5.1998e-12,1.559e-10,1.33e-10,8.5333e-11,1.4918e-10,5.3689e-11,3.2455e-10,1.0965e-10,1.9793e-09,2.4867e-10,3.6066e-09,2.833e-10,6.0038e-10,1.2311e-10,1.8576e-10,7.8335e-11,5.1392e-11,1.5403e-09,5.0331e-11,1.8434e-10,6.0643e-11,9.9462e-11,9.1496e-11,6.561e-10,1.2779e-10,7.3205e-11,5.5322e-11,7.7988e-11,3.5056e-10,2.2948e-10,1.3213e-09,4.6479e-09,2.9937e-09,4.3397e-10,7.2691e-10,1.2727e-10,5.2959e-10,7.2115e-10,1.7015e-10,1.0923e-10,1.8214e-09,1.6448e-10,4.0578e-11,1.0107e-10,2.8759e-10,3.8692e-10,1.2806e-10,4.6486e-11,1.8543e-10,2.3979e-09,1.2781e-08,7.4402e-10,3.126e-10,3.8413e-10,4.5262e-11,1.4902e-10,5.1355e-10,9.1588e-11,1.3865e-10,2.1255e-11,6.0018e-10,1.3509e-10,5.9599e-10,2.0121e-10,3.6086e-11,4.7369e-10,4.5354e-10,4.6105e-10,2.9852e-11,1.9429e-10,3.9952e-10,1.3576e-10,1.8646e-10,9.3202e-11,5.6809e-11,1.0134e-09,2.3803e-09,1.2363e-10,2.0339e-10,3.235e-10,2.1262e-10,1.1654e-10,2.1222e-10,4.53e-10,2.2082e-10,2.1899e-11,6.8822e-11,8.8679e-11,8.27e-11,8.1641e-11,4.3583e-10,1.1382e-09,5.6211e-10,2.6052e-11,7.4457e-12,2.923e-11,7.3599e-11,4.0837e-10,8.865e-10,5.0495e-10,1.0307e-09,6.2241e-11,3.2972e-10,3.9493e-11,4.8192e-11,2.5818e-10,4.585e-11,3.2572e-10,1.8193e-10,5.5237e-11,7.607e-11,6.7592e-11,6.1517e-11,1.4776e-10,7.5187e-11,1.0384e-10,5.0057e-10,1.8702e-09,4.5011e-11,8.8803e-11,8.9824e-11,7.7609e-10,6.3958e-11,9.7313e-11,7.0443e-11,5.7535e-11,1.7122e-11,8.3095e-11,3.0924e-11,3.5704e-10,1.2409e-10,1.1305e-10,2.0182e-09,8.0869e-11,1.5141e-10,1.377e-10,1.4627e-10,4.1926e-09,1.2647e-10,6.45e-11,5.887e-11,2.2945e-10,2.031e-10,2.2985e-11,1.7961e-10,4.4233e-10,9.1463e-11,1.6012e-10,3.7792e-09,3.4036e-11,2.1778e-10,1.1717e-10,3.7846e-10,3.208e-10,2.6571e-11,4.5905e-11,6.9239e-10,4.1437e-10,8.5485e-11,8.359e-11,1.2362e-10,9.1705e-10,1.013e-09,3.4304e-10,2.0929e-10,1.7772e-10,2.3656e-10,9.5217e-11,4.5417e-10,2.0215e-09,1.7207e-10,1.0519e-10,9.7253e-11,4.5967e-10,1.2053e-10,3.6037e-11,3.141e-10,1.0604e-09,2.9902e-09,2.0709e-09,1.4629e-09,1.2934e-09,2.517e-10,1.5441e-10,2.2246e-10,4.049e-10,9.3332e-11,1.2354e-10,1.418e-09,3.0467e-10,1.9502e-10,7.4318e-11,9.5875e-10,1.8106e-10,3.595e-10,1.5777e-10,1.8233e-09,1.4627e-09,1.4892e-09,1.471e-10,5.4474e-10,3.8459e-11,6.2409e-11,2.6868e-10,1.5998e-09,2.8365e-10,6.6432e-11,4.1139e-10,7.9353e-11,1.3067e-10,5.5564e-11,5.6671e-11,1.0185e-09,5.2028e-11,7.1153e-11,2.0747e-10,5.3634e-10,5.7446e-09,7.3587e-11,6.4583e-11,7.6034e-10,8.1542e-10,3.5152e-10,3.3696e-10,9.7123e-10,1.5696e-10,2.5277e-09,5.4498e-11,1.5443e-10,4.9978e-11,1.1768e-10,2.6514e-10,9.52e-10,5.2602e-10,2.2559e-10,6.9032e-11,1.492e-10,1.8202e-10,9.1501e-11,1.7644e-09,1.0252e-10,7.7918e-11,6.1807e-11,1.4089e-10,1.8401e-10,2.5761e-11,2.5285e-09,2.669e-10,1.3664e-10,2.1915e-10,1.409e-10,1.0083e-10,3.0541e-09,3.5206e-10,7.4488e-10,3.322e-09,9.9781e-11,7.8406e-11,1.9062e-10,1.2824e-10,6.0013e-10,6.0706e-11,1.3785e-09,2.7043e-10,1.903e-09,1.5637e-10,1.8275e-10,1.2051e-10,3.8019e-09,1.0176e-09,1.3017e-09,1.4681e-10,1.4386e-10,3.0722e-10,2.793e-10,5.1706e-10,1.6852e-10,9.3088e-10,1.5968e-10,5.6821e-10,3.9227e-10,6.201e-10,6.0711e-11,1.1782e-10,1.6161e-10,1.3576e-09,1.0127e-09,9.1826e-11,2.0184e-10,2.4471e-10,2.9176e-11,1.738e-10,1.2937e-10,7.0093e-10,1.5282e-10,5.3241e-10,1.0808e-09,3.5582e-10,6.3925e-10,4.1438e-10,6.1158e-10,2.4261e-09,5.8503e-10,2.6126e-10,9.7096e-10,5.2793e-10,8.1073e-10,7.5933e-10,7.2313e-10,4.2204e-10,3.0215e-10,8.7227e-10,2.1961e-09,7.0436e-10,4.8443e-11,9.1167e-11,7.2187e-10,1.6343e-08,2.5652e-10,2.1068e-10,1.5877e-10,8.3634e-10,7.0804e-10,4.8726e-10,7.5002e-10,2.4511e-10,3.5273e-10,9.4684e-11,2.3151e-09,1.9962e-10,1.5412e-10,1.8838e-09,2.8086e-09,8.2819e-10,3.632e-10,1.3065e-10,8.2427e-10,6.1012e-09,9.0951e-10,1.079e-09,1.162e-09,3.4663e-09,2.3265e-10,1.0456e-09,3.1621e-10,6.9169e-10,5.3708e-10,4.3227e-11,7.4573e-10,3.2276e-09,5.2582e-10,2.8185e-10,1.9662e-10,8.3264e-10,1.0947e-09,2.9651e-09,1.1673e-09,1.1385e-09,4.0155e-10,5.2543e-10,2.4602e-10,2.4146e-10,6.2522e-11,1.5031e-10,4.5777e-10,5.2701e-10,2.3536e-09,1.9329e-10,1.5258e-10,1.4612e-09,1.5129e-09,7.6929e-10,5.0342e-08,5.5325e-10,2.2269e-09,5.3751e-11,1.7553e-10,3.0075e-09,5.4748e-11
0.089474,4.227e-11,6.5582e-11,1.7634e-10,1.1872e-10,2.6631e-10,3.0661e-10,1.117e-09,5.8696e-10,2.1492e-10,1.317e-09,7.5698e-11,6.5755e-11,1.891e-10,1.3919e-10,1.0575e-10,2.42e-11,2.6265e-11,1.3061e-10,3.2475e-11,4.4748e-11,4.7689e-11,1.1278e-08,7.6497e-10,1.6867e-09,6.932e-10,9.667e-10,6.2307e-11,1.9588e-11,2.1765e-11,1.647e-10,5.483e-10,1.7354e-11,2.1939e-11,6.4351e-10,8.7902e-11,7.2125e-11,2.8005e-10,1.5309e-10,2.181e-10,1.1176e-10,1.211e-10,3.0114e-10,3.3194e-11,7.5621e-10,8.9931e-11,9.132e-11,2.618e-10,2.5149e-11,4.5123e-11,2.4562e-10,1.5678e-10,1.6499e-10,1.1664e-10,1.9365e-10,2.0842e-10,6.5795e-11,5.7435e-11,8.6141e-11,5.2441e-11,5.8357e-11,9.9047e-11,3.3967e-10,6.7131e-11,3.9591e-11,3.6019e-11,2.249e-10,1.9887e-09,2.1855e-10,5.9155e-11,1.2576e-10,1.5336e-09,5.5133e-11,3.356e-11,7.3659e-11,7.1063e-11,6.4111e-11,9.5292e-10,7.5382e-11,2.1478e-10,1.9778e-11,6.7675e-10,5.7971e-11,7.1148e-11,7.5048e-11,2.5565e-11,2.9999e-10,9.5408e-11,1.574e-10,2.0834e-11,6.4908e-11,3.5752e-11,4.6818e-11,3.2807e-10,2.0874e-10,1.7525e-10,2.5604e-11,1.7994e-11,1.0058e-10,3.9631e-10,5.2621e-10,1.8916e-10,2.1599e-11,1.2462e-11,3.9805e-11,1.0304e-11,3.068e-11,2.33e-11,1.6313e-10,1.1673e-10,1.0459e-10,4.8358e-11,4.4652e-11,3.3979e-11,5.7621e-11,1.2569e-10,1.4233e-10,6.4703e-11,2.3472e-11,2.1192e-11,2.4689e-11,3.3213e-11,1.3697e-11,2.0371e-10,2.3327e-10,8.3756e-11,1.6105e-10,3.1919e-11,9.4149e-11,3.5686e-11,3.6662e-11,6.2809e-11,1.782e-10,5.3404e-11,4.0399e-12,5.0056e-11,3.6751e-11,2.3746e-11,5.0158e-11,1.6965e-11,1.1722e-10,4.7384e-11,6.5589e-10,6.6533e-11,4.2877e-10,5.9786e-11,1.4432e-10,4.0954e-11,5.6342e-11,2.2736e-11,1.3919e-11,5.1485e-10,1.0702e-11,3.9829e-11,1.713e-11,3.2037e-11,3.1933e-11,1.3322e-10,4.6494e-11,1.8507e-11,1.7139e-11,1.6811e-11,3.1347e-11,5.5731e-11,2.2543e-10,5.324e-09,7.4368e-10,1.5864e-10,3.1007e-10,3.8094e-11,2.1623e-10,1.805e-10,6.8382e-11,2.8687e-11,2.2026e-10,4.1564e-11,1.1236e-11,2.069e-11,7.4101e-11,1.3064e-10,4.0463e-11,1.811e-11,3.9102e-11,4.7363e-10,2.0694e-09,1.5704e-10,8.2462e-11,1.3878e-10,1.9202e-11,4.8732e-11,2.3494e-10,2.5015e-11,2.8221e-11,4.227e-12,1.1248e-10,5.271e-11,2.1099e-10,8.0552e-11,1.2856e-11,1.3152e-10,1.1652e-10,1.1431e-10,1.2117e-11,7.208e-11,1.0612e-10,4.1162e-11,8.2943e-11,2.4375e-11,1.3382e-11,3.5887e-11,4.7602e-10,4.3013e-11,5.0477e-11,2.0456e-10,4.0286e-11,3.6406e-11,5.597e-11,1.243e-10,8.0731e-11,7.5247e-12,2.7245e-11,2.3637e-11,3.9197e-11,2.8937e-11,1.3358e-10,1.3676e-10,1.2525e-10,8.5763e-12,2.9437e-12,1.1096e-11,2.7855e-11,2.672e-10,3.3064e-10,1.2076e-10,2.1573e-10,6.3361e-11,5.7398e-11,1.8064e-11,1.7318e-11,6.4295e-11,9.3166e-12,1.1802e-10,6.7985e-11,1.8204e-11,2.787e-11,2.8023e-11,2.4912e-11,5.5004e-11,2.7558e-11,3.1156e-11,1.8133e-10,2.9096e-10,1.4847e-11,2.3848e-11,3.1777e-11,1.5643e-10,1.3297e-11,2.6494e-11,2.4107e-11,2.0216e-11,6.6357e-12,2.8558e-11,9.8159e-12,1.2953e-10,3.0854e-11,3.666e-11,7.6551e-10,4.1537e-11,5.3139e-11,5.2962e-11,4.2439e-11,4.2807e-10,4.0072e-11,1.2204e-11,1.6229e-11,2.1752e-10,5.8695e-11,7.6812e-12,8.7055e-11,8.4941e-11,2.3446e-11,4.5135e-11,3.4396e-09,1.1735e-11,1.1988e-10,3.2543e-11,1.5088e-10,7.671e-11,7.3747e-12,1.1425e-11,2.7351e-10,1.7933e-10,2.7021e-11,3.3051e-11,4.2425e-11,3.6283e-10,1.0584e-09,8.8578e-11,7.6286e-11,5.2998e-11,1.0776e-10,3.5072e-11,1.089e-10,2.8545e-10,4.0194e-11,2.4932e-11,3.7103e-11,1.6299e-10,5.7887e-11,1.662e-11,1.0051e-10,2.9189e-10,8.0896e-10,6.6686e-10,6.0336e-10,3.5023e-10,9.2906e-11,5.3898e-11,7.2684e-11,1.4517e-10,1.6556e-11,3.3179e-11,3.7287e-10,1.1951e-10,5.9465e-11,6.7752e-11,2.7912e-10,5.683e-11,8.0962e-11,4.8055e-11,5.9826e-10,6.7959e-10,5.681e-10,4.043e-11,1.1904e-10,1.4846e-11,1.2958e-11,5.5149e-11,5.3211e-10,5.795e-11,2.1872e-11,9.9981e-11,2.8022e-11,3.6182e-11,1.5892e-11,1.7584e-11,4.1479e-10,1.8645e-11,2.1713e-11,5.457e-11,1.5066e-10,1.0074e-09,1.9311e-11,1.3123e-11,3.1961e-10,1.5626e-10,1.6341e-10,1.0698e-10,1.5015e-10,5.1863e-11,1.4984e-09,1.4552e-11,4.8899e-11,2.8571e-11,2.7202e-11,8.8803e-11,2.4987e-10,2.5031e-10,5.6581e-11,1.4809e-11,3.9199e-11,5.5285e-11,3.1708e-11,9.0267e-10,5.2884e-11,2.383e-11,1.7266e-11,3.4069e-11,7.6466e-11,8.1821e-12,9.1908e-10,8.1316e-11,6.7347e-11,4.635e-11,2.2246e-11,2.5104e-11,3.9884e-10,9.0044e-11,3.0675e-10,1.2103e-09,3.4268e-11,2.5106e-11,4.7578e-11,2.9451e-11,1.3149e-10,2.0509e-11,3.0525e-10,6.6974e-11,1.12e-09,3.9114e-11,4.6775e-11,2.4688e-11,3.4449e-10,4.0524e-10,3.1876e-10,4.7163e-11,6.0021e-11,1.1994e-10,1.1132e-10,1.9443e-10,4.9426e-11,3.4554e-10,5.3122e-11,1.6527e-10,1.2795e-10,1.439e-10,1.3353e-11,2.358e-11,4.3426e-11,3.9177e-10,2.8768e-10,2.2887e-11,6.6237e-11,8.0516e-11,6.8203e-12,4.3236e-11,3.731e-11,2.1263e-10,4.6626e-11,1.6228e-10,2.818e-10,7.4936e-11,2.2036e-10,6.3943e-11,1.1531e-10,1.374e-09,1.9028e-10,1.3967e-10,4.0315e-10,1.7851e-10,2.4193e-10,2.4829e-10,2.5022e-10,1.3028e-10,9.9401e-11,2.691e-10,4.5948e-10,1.2419e-10,1.0411e-11,1.9223e-11,1.0646e-10,2.3484e-09,8.6115e-11,5.2611e-11,5.3892e-11,2.2239e-10,1.7455e-10,1.1911e-10,1.9922e-10,8.2207e-11,1.4924e-10,4.1795e-11,6.6906e-10,4.628e-11,3.2014e-11,8.7995e-10,4.4198e-10,2.0863e-10,1.2423e-10,4.0409e-11,1.8181e-10,7.568e-10,2.5977e-10,2.1815e-10,4.8013e-10,1.5759e-09,7.3209e-11,3.867e-10,9.0203e-11,1.795e-10,7.0345e-11,9.1835e-12,2.4083e-10,1.225e-09,1.6644e-10,1.2348e-10,7.1338e-11,3.8014e-10,2.5703e-10,6.8333e-10,3.5335e-10,3.5569e-10,1.6892e-10,1.7042e-10,7.4294e-11,4.6118e-11,8.4322e-12,1.8152e-11,8.6611e-11,6.065e-11,9.351e-10,5.5114e-11,4.5164e-11,5.1836e-10,3.6396e-10,1.9923e-10,1.6026e-08,1.4739e-10,8.1334e-10,2.7685e-11,4.0166e-11,3.7325e-10,1.1465e-11
0.094737,4.9796e-12,9.8841e-12,3.1901e-11,3.5247e-11,7.4616e-11,3.2101e-11,3.0226e-10,7.1204e-11,4.5047e-11,2.9616e-10,1.9505e-11,1.6662e-11,4.0285e-11,2.3676e-11,1.3398e-11,2.5632e-12,7.1002e-12,1.443e-11,4.3765e-12,8.3088e-12,1.1818e-11,1.95e-10,2.5948e-10,4.1263e-10,9.5549e-11,3.0114e-10,1.1428e-11,6.9865e-12,3.7363e-12,5.7466e-11,5.4846e-11,2.1256e-12,2.6232e-12,5.6097e-11,1.7075e-11,2.6639e-11,6.6522e-11,2.4371e-11,4.2591e-11,1.9159e-11,2.6045e-11,6.0844e-11,7.3601e-12,4.4702e-11,2.4602e-11,1.6831e-11,1.6439e-11,3.4176e-12,5.3133e-12,2.9952e-11,2.971e-11,3.4692e-11,2.4064e-11,1.1664e-10,5.6729e-11,1.1568e-11,8.4356e-12,2.2625e-11,9.0179e-12,1.1411e-11,2.3966e-11,6.9995e-11,1.5764e-11,1.0703e-11,6.2612e-12,1.7259e-11,3.3637e-10,4.6167e-11,1.5189e-11,2.6884e-11,4.749e-10,8.3685e-12,5.6965e-12,1.5204e-11,1.9807e-11,1.8266e-11,7.6251e-10,1.5625e-11,6.2659e-11,3.4775e-12,6.0594e-11,7.6974e-12,1.993e-11,1.3055e-11,7.2157e-12,4.842e-11,1.8006e-11,5.4595e-11,4.7292e-12,1.2341e-11,1.6584e-11,8.189e-12,3.4283e-11,3.2946e-11,1.9185e-11,3.1483e-12,3.1591e-12,1.6211e-11,8.4604e-11,5.6308e-11,6.4592e-11,5.189e-12,2.5585e-12,7.1301e-12,1.44e-12,8.1138e-12,5.5817e-12,3.3936e-11,1.9045e-11,2.4487e-11,6.7421e-12,5.7369e-12,7.137e-12,1.5158e-11,4.73e-11,5.2633e-11,1.486e-11,5.6376e-12,4.6144e-12,3.6486e-12,4.401e-12,2.7888e-12,4.226e-11,6.946e-11,1.6071e-11,1.8368e-11,5.1909e-12,2.5702e-11,5.1999e-12,7.4222e-12,1.1052e-11,2.9366e-11,9.1587e-12,1.7713e-12,1.0927e-11,6.6932e-12,4.2059e-12,1.2004e-11,3.5783e-12,3.5321e-11,1.4397e-11,3.3018e-11,1.2083e-11,2.5324e-11,6.9089e-12,1.9797e-11,1.2317e-11,1.1305e-11,3.2033e-12,2.374e-12,5.7382e-11,9.7242e-13,4.0012e-12,3.5774e-12,6.886e-12,8.7161e-12,1.6425e-11,1.7818e-11,3.0288e-12,3.6238e-12,2.1723e-12,2.9647e-12,8.4287e-12,2.4342e-11,1.371e-09,9.4502e-11,4.8271e-11,1.355e-10,9.1288e-12,6.8892e-11,3.1631e-11,2.1023e-11,4.7149e-12,3.1017e-11,6.663e-12,3.0752e-12,2.584e-12,1.1727e-11,2.5676e-11,8.4679e-12,5.0436e-12,8.5916e-12,9.3039e-11,2.6055e-10,1.9997e-11,1.4241e-11,4.2044e-11,6.1674e-12,1.0689e-11,8.8818e-11,5.2067e-12,3.4785e-12,9.5555e-13,1.3568e-11,1.4508e-11,1.5657e-11,1.9917e-11,3.8983e-12,2.8367e-11,1.7985e-11,1.6686e-11,5.378e-12,2.0515e-11,1.8087e-11,7.6148e-12,3.0511e-11,3.9526e-12,2.0025e-12,2.5123e-12,6.4623e-11,1.052e-11,7.6246e-12,7.8966e-11,5.7574e-12,7.6023e-12,1.157e-11,1.821e-11,3.5574e-11,1.8924e-12,7.2359e-12,3.8314e-12,2.2393e-11,1.0361e-11,5.4931e-12,3.6927e-12,1.8707e-11,2.1377e-12,9.7618e-13,3.0327e-12,6.8706e-12,8.6734e-11,6.0636e-11,1.7101e-11,3.7753e-11,1.4217e-11,7.7506e-12,5.4983e-12,4.5226e-12,1.0124e-11,1.2104e-12,8.581e-12,4.1851e-11,4.0294e-12,7.5549e-12,8.0699e-12,7.0792e-12,1.6801e-11,1.0293e-11,1.1684e-11,1.2033e-11,2.4535e-11,3.9774e-12,3.5617e-12,7.8316e-12,2.0318e-11,1.7632e-12,1.9222e-12,5.1558e-12,5.2427e-12,2.1553e-12,5.7935e-12,1.8636e-12,1.3446e-11,4.7295e-12,8.589e-12,1.2871e-10,2.2239e-11,1.0465e-11,5.229e-12,9.5815e-12,3.5682e-11,1.0449e-11,1.5058e-12,3.1327e-12,3.8867e-11,9.2648e-12,1.6209e-12,3.0827e-11,1.685e-11,5.2224e-12,1.0805e-11,6.2381e-10,2.7766e-12,4.8223e-11,5.5365e-12,1.4257e-11,1.0189e-11,1.5468e-12,1.78e-12,5.7971e-11,3.4421e-11,5.801e-12,9.3111e-12,1.0611e-11,3.0733e-11,5.6244e-10,1.385e-11,1.904e-11,1.0434e-11,3.1456e-11,9.0326e-12,1.8545e-11,2.6958e-11,6.7062e-12,4.3702e-12,1.0664e-11,3.2355e-11,1.4658e-11,5.7847e-12,2.1882e-11,4.9676e-11,2.2694e-10,1.904e-10,1.6826e-10,7.5875e-11,3.6705e-11,1.3605e-11,1.5219e-11,4.8655e-11,2.2111e-12,6.2088e-12,5.918e-11,4.3127e-11,1.3221e-11,6.9656e-11,5.7862e-11,1.292e-11,1.7046e-11,9.4439e-12,2.5133e-11,3.7487e-10,2.1399e-10,7.3802e-12,2.6379e-11,1.464e-11,1.5373e-12,8.3057e-12,2.3519e-11,8.7439e-12,5.8181e-12,1.9304e-11,6.6468e-12,5.8914e-12,3.2162e-12,4.1157e-12,1.0815e-10,4.23e-12,3.8655e-12,9.7292e-12,1.0296e-11,7.2322e-11,3.4097e-12,1.6798e-12,9.949e-11,1.5291e-11,5.8511e-11,2.1537e-11,1.7946e-11,1.1753e-11,5.1266e-10,2.608e-12,9.8266e-12,1.1463e-11,6.802e-12,2.0427e-11,6.0079e-11,7.8699e-11,1.3559e-11,2.0195e-12,6.7898e-12,1.1385e-11,7.0199e-12,2.9559e-10,2.0199e-11,4.9592e-12,3.1502e-12,4.571e-12,2.4968e-11,2.1342e-12,5.073e-11,1.742e-11,2.5682e-11,4.9876e-12,1.9626e-12,4.5524e-12,3.7499e-11,1.29e-11,2.1971e-10,4.3066e-10,8.0508e-12,6.0125e-12,7.8717e-12,6.1278e-12,1.0792e-11,4.7019e-12,4.2031e-11,1.1124e-11,1.0133e-10,6.7659e-12,1.011e-11,2.8039e-12,3.1759e-11,1.1263e-10,3.2117e-11,1.0323e-11,2.4656e-11,4.7709e-11,1.8244e-11,1.2565e-11,9.1333e-12,2.8367e-11,1.3348e-11,2.5447e-11,3.3072e-11,2.053e-11,1.8495e-12,2.8849e-12,1.5881e-11,3.1139e-11,7.1321e-11,3.423e-12,1.6199e-11,1.9149e-11,1.1471e-12,7.3313e-12,7.4207e-12,2.7706e-11,9.1724e-12,3.0973e-11,6.7212e-11,1.6226e-11,5.9659e-11,7.3597e-12,1.3718e-11,2.0684e-09,8.0304e-11,5.6682e-11,5.9174e-11,4.6517e-11,4.5974e-11,6.1047e-11,6.6311e-11,3.8006e-11,2.0334e-11,5.42e-11,4.0159e-11,1.1437e-11,1.4902e-12,2.5822e-12,9.5378e-12,2.1686e-10,2.2355e-11,7.1015e-12,1.2448e-11,3.4932e-11,2.176e-11,1.872e-11,3.5784e-11,1.6851e-11,8.3443e-11,1.4172e-11,1.7972e-10,6.0477e-12,4.2788e-12,2.5827e-11,5.6366e-11,3.5554e-11,3.5494e-11,6.9116e-12,2.5883e-11,8.3469e-11,4.2174e-11,2.8208e-11,1.5671e-10,2.3487e-10,1.4708e-11,3.2021e-11,1.8428e-11,5.8569e-11,6.4816e-12,1.2587e-12,2.0051e-11,7.0744e-11,3.8597e-11,5.3767e-11,1.8429e-11,1.1394e-10,4.0133e-11,8.5796e-11,7.0556e-11,2.7201e-11,6.242e-11,6.0847e-11,1.5521e-11,5.7989e-12,6.6914e-13,1.664e-12,1.0841e-11,4.779e-12,1.494e-10,9.7436e-12,1.343e-11,1.3541e-10,5.5338e-11,3.2345e-11,6.8666e-10,2.7852e-11,6.1345e-11,1.2555e-11,5.6928e-12,3.0346e-11,1.3909e-12
0.1,8.3838e-15,1.5405e-14,4.4442e-14,1.2023e-13,3.4507e-13,4.5551e-13,7.8261e-14,1.5109e-13,5.0024e-13,1.3435e-12,2.8978e-13,1.1084e-13,6.1194e-14,2.7646e-14,5.127e-15,3.1331e-15,6.158e-16,1.3248e-14,2.465e-14,9.0144e-14,5.6268e-13,1.3905e-13,7.8871e-14,4.7674e-13,3.9327e-13,7.5605e-14,6.2826e-14,8.8581e-14,1.7807e-14,7.3442e-15,5.8533e-14,2.8848e-15,5.1513e-15,7.2813e-15,2.8683e-14,3.687e-14,5.4435e-14,1.0167e-13,1.1187e-13,3.0852e-14,1.02e-12,1.1176e-13,1.1121e-13,8.4949e-14,3.9336e-14,7.2404e-15,6.6233e-15,5.6967e-15,4.6534e-15,1.4139e-14,5.389e-14,8.8174e-13,9.1876e-14,2.5912e-13,2.9804e-14,3.1463e-14,3.5027e-14,4.7727e-14,1.2496e-13,4.2483e-14,2.7182e-13,3.2213e-14,1.4022e-14,3.0736e-15,7.3089e-15,8.7324e-15,1.3994e-13,7.4609e-14,2.2255e-13,2.8636e-13,2.7169e-14,2.4194e-14,3.7598e-14,7.1654e-14,1.148e-13,7.914e-14,5.5388e-13,1.9697e-14,1.5912e-14,8.0569e-15,1.1769e-14,3.4238e-15,2.5656e-14,5.3892e-14,6.9652e-13,2.013e-13,1.3927e-14,1.0079e-14,5.3802e-14,2.0523e-14,4.7043e-14,1.0041e-13,1.6384e-13,3.8834e-14,7.8905e-14,1.3355e-15,1.3701e-15,7.4014e-15,5.1323e-14,7.1515e-14,1.029e-13,2.5331e-14,7.9054e-15,8.7444e-14,6.8888e-14,4.6528e-14,1.1482e-13,4.1289e-14,4.5225e-14,9.7284e-14,1.1568e-14,3.1443e-15,1.5042e-14,1.0419e-14,1.204e-14,2.3299e-14,1.1517e-13,2.097e-14,3.0525e-14,1.344e-14,1.1633e-13,3.1386e-14,5.7002e-14,4.6946e-14,1.0616e-13,1.2282e-13,2.4804e-14,4.7886e-15,1.1092e-15,4.5666e-14,1.8006e-14,9.152e-14,9.9714e-14,7.237e-14,1.5816e-14,6.8205e-15,7.5301e-15,4.3872e-13,3.3431e-14,1.6037e-13,1.1087e-14,2.8159e-14,8.2896e-15,1.329e-14,3.701e-15,1.629e-14,2.3425e-14,4.5705e-14,5.2398e-13,5.4626e-14,3.5983e-14,2.0805e-14,1.478e-13,9.2241e-15,6.0175e-14,1.1329e-13,1.3117e-13,3.1357e-14,5.1953e-14,2.549e-14,7.0628e-15,3.1319e-14,4.853e-14,1.5543e-13,2.9831e-14,1.6674e-13,1.9505e-13,9.6826e-14,1.2834e-13,1.5802e-14,1.4904e-12,1.8728e-12,1.0235e-14,2.5589e-14,1.3204e-14,2.6508e-15,6.8339e-15,2.5586e-14,2.7105e-14,4.7241e-14,5.7225e-13,4.2423e-13,3.1731e-14,1.4934e-13,3.3594e-13,2.1843e-13,3.8324e-14,8.548e-14,4.2957e-14,7.7433e-14,2.028e-14,3.1616e-15,3.4837e-15,1.3389e-14,5.8295e-15,1.057e-13,2.2218e-13,7.3645e-14,4.6168e-14,8.8837e-14,4.0252e-14,2.9311e-14,1.0432e-14,1.1826e-13,1.5587e-14,1.8859e-14,8.3543e-15,5.492e-15,1.5039e-15,5.8022e-14,3.2073e-14,3.8273e-14,1.4017e-13,6.1256e-14,1.3372e-14,1.3612e-14,2.5261e-14,7.5805e-14,5.785e-14,3.004e-13,5.8472e-13,2.7307e-14,1.3628e-14,8.6422e-16,6.0217e-15,6.5694e-15,1.6714e-14,4.8597e-14,5.9393e-13,2.9459e-14,9.6002e-15,1.4619e-13,2.1219e-15,1.4719e-14,1.924e-13,5.3807e-13,2.2757e-14,1.4958e-14,1.679e-14,3.0121e-15,7.0326e-15,9.548e-15,1.1955e-14,4.4355e-14,4.1188e-14,1.0972e-14,5.7543e-14,1.7622e-14,1.8017e-14,3.5873e-14,2.1042e-14,4.078e-14,1.808e-14,1.9371e-14,5.6939e-15,4.942e-15,3.729e-15,3.2315e-15,3.8701e-14,1.3969e-14,1.5126e-14,2.4976e-14,4.1864e-14,9.1626e-15,4.513e-15,8.973e-14,9.8038e-15,1.3295e-14,5.038e-14,2.2196e-14,5.6665e-15,1.5986e-15,8.8545e-16,6.4655e-15,5.0438e-15,5.4084e-14,5.6235e-14,3.297e-14,1.6774e-14,1.2973e-13,3.719e-14,2.6286e-15,5.4938e-14,8.6315e-15,4.4883e-14,1.8578e-14,4.9175e-15,1.4076e-15,4.2762e-15,7.7676e-15,2.3026e-14,1.5346e-14,2.0004e-14,1.1515e-13,1.5231e-14,2.1768e-13,1.1783e-13,2.6905e-14,1.2818e-13,7.5268e-14,2.0763e-14,2.2332e-13,4.3177e-14,5.1784e-15,2.3152e-15,8.9395e-14,3.1117e-14,3.5013e-14,7.0686e-14,1.4894e-13,1.0468e-13,2.3949e-13,1.0591e-14,1.9122e-13,5.3933e-14,5.1023e-13,9.4182e-13,6.5386e-15,1.6631e-14,1.7826e-15,7.9789e-15,1.381e-14,7.8736e-13,5.4782e-14,3.3426e-14,1.7538e-13,2.4877e-14,6.7415e-14,1.1503e-13,7.5886e-14,2.2581e-13,3.2247e-14,4.2983e-14,2.3667e-14,1.0606e-14,2.375e-15,1.5409e-14,8.9197e-14,3.6026e-14,1.9918e-14,8.2741e-15,1.1948e-13,1.1588e-13,4.7675e-14,1.0238e-14,3.0539e-14,1.3272e-13,1.4064e-13,6.3666e-14,6.8448e-14,5.4871e-15,3.1856e-15,1.5279e-15,3.53e-14,3.2003e-14,8.9298e-14,1.174e-13,1.3418e-14,2.3904e-14,4.7125e-14,3.2893e-14,2.4733e-15,3.5843e-14,1.1401e-13,6.976e-14,1.5439e-13,2.9859e-14,5.8717e-15,6.5205e-15,1.1878e-14,3.5574e-14,5.5096e-14,8.3699e-14,3.3808e-14,1.5902e-14,8.5565e-15,1.1861e-14,5.9795e-15,6.4338e-14,2.8831e-14,1.0708e-13,1.0768e-14,9.8893e-15,3.1291e-15,2.6233e-15,1.0913e-13,1.0638e-13,6.9324e-14,4.6117e-14,6.6767e-14,2.8711e-14,1.3172e-14,5.9665e-15,5.7114e-14,6.7951e-14,2.3083e-13,7.42e-14,1.4597e-13,1.5556e-14,2.2466e-15,3.0165e-15,7.9415e-14,7.2839e-14,1.2739e-13,4.1855e-14,5.6136e-14,9.5995e-14,1.8398e-14,3.0677e-14,9.9862e-15,1.9406e-14,1.7933e-14,1.0249e-13,1.0883e-13,1.8956e-14,3.6116e-14,8.1392e-16,2.837e-14,8.6767e-14,2.5992e-13,1.4755e-13,3.1237e-13,2.2664e-14,3.4581e-14,2.8555e-14,2.1953e-14,4.4104e-14,1.0933e-13,8.9798e-14,3.0386e-14,2.4198e-14,3.49e-15,7.0455e-15,6.826e-15,1.2348e-13,3.8442e-14,6.8705e-14,2.1539e-13,1.5521e-13,5.6577e-14,5.7417e-14,1.0224e-13,1.4642e-14,3.0494e-14,1.1683e-13,9.5535e-15,2.3371e-14,1.5527e-15,2.1589e-15,1.7592e-14,2.0107e-13,3.5564e-14,7.0495e-13,7.0799e-14,6.6939e-14,3.8214e-13,6.7877e-14,1.431e-13,2.1948e-14,8.2306e-14,5.8437e-14,6.7573e-14,4.828e-15,4.6824e-15,3.9054e-15,1.853e-14,6.0737e-13,1.6161e-13,2.4526e-14,2.1919e-13,6.5757e-14,5.6974e-13,2.4502e-13,8.4914e-12,1.1082e-13,4.5854e-14,2.6575e-13,2.8288e-14,4.9501e-15,2.9333e-15,3.2532e-16,1.1111e-14,2.0392e-13,6.9703e-14,2.6798e-13,1.8316e-13,9.9565e-14,2.7701e-13,4.0188e-13,6.4181e-14,2.1709e-14,3.4594e-14,5.1423e-14,4.5479e-14,2.5167e-14,4.191e-15,3.0038e-15,1.2165e-13,1.1452e-13,5.2984e-14,1.8847e-14,3.1801e-14,4.3135e-12,2.7127e-13,4.3757e-13,9.7648e-14,2.3279e-13,9.3335e-14,2.6318e-13,4.3414e-14,2.8267e-15,6.8956e-16


==> conv_2step.tex <==
1,0.023265
2,0.0076061
3,0.005018
4,0.006332
5,0.0035765
6,0.0016317
7,7.3466e-05
8,7.3215e-06
9,6.3799e-07
10,7.9332e-08
11,5.2578e-08
12,5.148e-09
13,3.8244e-09
14,1.819e-09
15,1.4793e-09
16,7.7399e-11
17,8.5751e-10
18,3.099e-10
19,6.0547e-11


==> conv_mmax_grid_invsqrt.tex <==
5,0.21103
10,0.13499
15,0.00071895
20,0.00014395
25,2.9399e-06
30,5.7306e-07
35,7.6046e-10
40,1.6802e-09
45,3.62e-12
49,3.2436e-13


==> conv_mmax_grid_oscil.tex <==
5,466.75
10,5.386
15,0.0070504
20,1.1541e-05
25,6.4943e-08
30,3.0211e-11
34,4.5055e-13


==> conv_mmax_grid_ratfunc.tex <==
5,0.00025933
10,3.0843e-08
15,7.4909e-13
16,1.3465e-13


==> conv_mmax_grid_sqrt.tex <==
5,0.0087303
10,0.0079542
15,0.00012183
20,1.0975e-06
25,1.4707e-07
30,6.4431e-09
35,3.3712e-10
40,2.9096e-11
42,3.3273e-11


==> conv_mmax_off_grid_invsqrt.tex <==
5,0.21095
10,0.18356
15,0.0007172
20,0.00020781
25,2.9335e-06
30,1.6073e-06
35,7.5936e-10
40,3.3759e-09
45,3.7924e-12
49,1.998e-12


==> conv_mmax_off_grid_oscil.tex <==
5,163.91
10,15.272
15,0.0071098
20,1.2669e-05
25,1.8375e-07
30,8.2091e-11
34,6.6133e-12


==> conv_mmax_off_grid_ratfunc.tex <==
5,0.00026408
10,3.1184e-08
15,7.6731e-13
16,1.3955e-13


==> conv_mmax_off_grid_sqrt.tex <==
5,0.0087315
10,0.0079671
15,0.00012163
20,1.0964e-06
25,1.5116e-07
30,3.0515e-08
35,2.9763e-08
40,2.9762e-08
42,2.9767e-08


==> conv_pAAA.tex <==
1,0.99891
2,0.93245
3,0.19457
4,0.12018
5,0.13407
6,3.523
7,0.062529
8,0.061539
9,1.5474
10,0.089991
11,1.3766
12,0.59223
13,0.19878
14,0.83556
15,0.052675
16,0.19156
17,0.04099
18,0.014726
19,0.010335
20,0.0088728
21,0.19649
22,0.018609
23,0.028062
24,0.047408
25,0.0043596
26,0.0035743
27,0.0021758
28,0.0018944
29,0.0016683
30,0.0058954
31,0.0022464
32,0.00095373
33,9.5567e-05
34,0.00032739
35,7.2518e-05
36,0.00013559
37,3.4933e-07
38,1.3136e-06
39,2.5626e-08
40,2.3286e-08
41,1.4021e-07
42,4.2295e-07
43,8.2946e-10
44,2.5456e-10
45,2.3519e-09
46,1.2199e-09
47,3.1677e-09
48,5.8262e-10
49,4.9873e-10
50,5.3534e-10
51,2.2579e-10


==> degr_del_invsqrt.tex <==
0.5,19,23,23
0.25,23,27,29
0.125,29,31,33
0.0625,31,35,37
0.03125,35,41,40
0.015625,39,45,44
0.0078125,43,47,49
0.0039062,47,49,49
0.0019531,51,51,49
0.00097656,50,49,50


==> err_del_grid_invsqrt.tex <==
0.5,2.694e-12
0.25,8.6277e-13
0.125,6.3206e-13
0.0625,8.89e-13
0.03125,2.188e-12
0.015625,1.0682e-12
0.0078125,1.9334e-12
0.0039062,1.8123e-12
0.0019531,4.0652e-13
0.00097656,2.4155e-12


==> err_del_off_grid_invsqrt.tex <==
0.5,2.6959e-12
0.25,8.6338e-13
0.125,6.3205e-13
0.0625,8.8941e-13
0.03125,2.1917e-12
0.015625,1.7618e-12
0.0078125,5.2071e-12
0.0039062,8.2893e-08
0.0019531,0.0031302
0.00097656,0.82892


==> err_mLf.tex <==
2,0.219994544733518
4,0.0305912406237842
6,0.00887137584300329
8,0.0370943604374116


==> err_off_grid.tex <==
3,0.431602624783043
10,0.902809094536978
15,0.000999044624491148
18,7.01686195590256e-05
25,1.51168730921344e-05


==> err_off_grid_paaa.tex <==
1,57.6999198215123
2,382.379817008676
3,11670.6700931992
4,89.0618913647146
5,1614.82462891094
6,992.935633225328
7,210.004164581523
8,139.524214447343
9,2071.00023395329
10,1803.7463303106
11,5.38519139182062
12,148.515379656095
13,6.77300889613913
14,0.63481598298794
15,0.412123633847473
16,3.1072938830712
17,0.575213881358229
18,1.96510920228926
19,0.0194815016513693
20,1.59964713287106
21,0.00294668224537069
22,0.0543902877368788
23,0.000247398188185595
24,0.00119941753746296
25,0.0041945050376076


==> err_sqrt_AAA.tex <==
-3.992,2.1375e-05
-3.984,2.1638e-05
-3.976,2.2081e-05
-3.968,2.2415e-05
-3.96,2.273e-05
-3.952,2.3032e-05
-3.9439,2.3387e-05
-3.9359,2.3836e-05
-3.9279,2.4252e-05
-3.9199,2.4885e-05
-3.9119,2.5141e-05
-3.9039,2.5639e-05
-3.8959,2.5845e-05
-3.8879,2.6077e-05
-3.8799,2.6658e-05
-3.8719,2.7113e-05
-3.8639,2.7639e-05
-3.8559,2.796e-05
-3.8478,2.8257e-05
-3.8398,2.8899e-05
-3.8318,2.9413e-05
-3.8238,2.9614e-05
-3.8158,3.0471e-05
-3.8078,3.0734e-05
-3.7998,3.141e-05
-3.7918,3.1843e-05
-3.7838,3.2226e-05
-3.7758,3.2727e-05
-3.7678,3.3533e-05
-3.7598,3.4025e-05
-3.7518,3.4257e-05
-3.7437,3.5004e-05
-3.7357,3.5533e-05
-3.7277,3.5895e-05
-3.7197,3.6536e-05
-3.7117,3.7591e-05
-3.7037,3.7998e-05
-3.6957,3.8549e-05
-3.6877,3.9118e-05
-3.6797,3.985e-05
-3.6717,4.0566e-05
-3.6637,4.1331e-05
-3.6557,4.1925e-05
-3.6476,4.2774e-05
-3.6396,4.3625e-05
-3.6316,4.3786e-05
-3.6236,4.5003e-05
-3.6156,4.5829e-05
-3.6076,4.6532e-05
-3.5996,4.695e-05
-3.5916,4.7982e-05
-3.5836,4.8567e-05
-3.5756,4.9649e-05
-3.5676,5.0131e-05
-3.5596,5.1102e-05
-3.5516,5.2164e-05
-3.5435,5.2731e-05
-3.5355,5.3965e-05
-3.5275,5.4895e-05
-3.5195,5.5605e-05
-3.5115,5.6263e-05
-3.5035,5.7721e-05
-3.4955,5.881e-05
-3.4875,5.9825e-05
-3.4795,6.0657e-05
-3.4715,6.1763e-05
-3.4635,6.2754e-05
-3.4555,6.3512e-05
-3.4474,6.4893e-05
-3.4394,6.6023e-05
-3.4314,6.6936e-05
-3.4234,6.7977e-05
-3.4154,6.9223e-05
-3.4074,7.0346e-05
-3.3994,7.175e-05
-3.3914,7.2653e-05
-3.3834,7.4222e-05
-3.3754,7.5246e-05
-3.3674,7.6729e-05
-3.3594,7.7918e-05
-3.3514,7.959e-05
-3.3433,8.0579e-05
-3.3353,8.2488e-05
-3.3273,8.3699e-05
-3.3193,8.5398e-05
-3.3113,8.6687e-05
-3.3033,8.8425e-05
-3.2953,8.9823e-05
-3.2873,0.00010543
-3.2793,0.00010728
-3.2713,0.00010922
-3.2633,0.00011109
-3.2553,0.00011307
-3.2472,0.00011508
-3.2392,0.00011708
-3.2312,0.0001191
-3.2232,0.00012126
-3.2152,0.00012344
-3.2072,0.0001255
-3.1992,0.00012779
-3.1912,0.00013003
-3.1832,0.00013241
-3.1752,0.00013473
-3.1672,0.00013713
-3.1592,0.00013965
-3.1512,0.00014216
-3.1431,0.00014449
-3.1351,0.00014711
-3.1271,0.00014971
-3.1191,0.00015257
-3.1111,0.00015517
-3.1031,0.00015807
-3.0951,0.00016069
-3.0871,0.00016356
-3.0791,0.00016655
-3.0711,0.00016964
-3.0631,0.00017277
-3.0551,0.00017589
-3.047,0.00017907
-3.039,0.00018242
-3.031,0.0001859
-3.023,0.00018916
-3.015,0.00019246
-3.007,0.00019596
-2.999,0.00019952
-2.991,0.00020311
-2.983,0.00020688
-2.975,0.00021071
-2.967,0.00021459
-2.959,0.00021838
-2.951,0.00022242
-2.9429,0.00022668
-2.9349,0.00023089
-2.9269,0.00023528
-2.9189,0.00023962
-2.9109,0.00024409
-2.9029,0.00024875
-2.8949,0.00025258
-2.8869,0.00025756
-2.8789,0.00026272
-2.8709,0.00026741
-2.8629,0.00027234
-2.8549,0.00027759
-2.8468,0.00028272
-2.8388,0.00028825
-2.8308,0.00029326
-2.8228,0.00029913
-2.8148,0.000305
-2.8068,0.00031027
-2.7988,0.00031612
-2.7908,0.00032225
-2.7828,0.00032817
-2.7748,0.00033423
-2.7668,0.00034047
-2.7588,0.00034743
-2.7508,0.0003538
-2.7427,0.00036082
-2.7347,0.00036757
-2.7267,0.00037448
-2.7187,0.0003818
-2.7107,0.00038929
-2.7027,0.00039634
-2.6947,0.00040399
-2.6867,0.00041206
-2.6787,0.00041974
-2.6707,0.00042786
-2.6627,0.00043627
-2.6547,0.00044494
-2.6466,0.0004531
-2.6386,0.00046245
-2.6306,0.00047114
-2.6226,0.00048024
-2.6146,0.00048953
-2.6066,0.00049926
-2.5986,0.00050895
-2.5906,0.0005191
-2.5826,0.00052895
-2.5746,0.00053934
-2.5666,0.00055006
-2.5586,0.00056097
-2.5506,0.00057245
-2.5425,0.00058322
-2.5345,0.00059465
-2.5265,0.00060616
-2.5185,0.00061788
-2.5105,0.00063025
-2.5025,0.00064234
-2.4945,0.00065572
-2.4865,0.00066842
-2.4785,0.00068158
-2.4705,0.00069512
-2.4625,0.00070947
-2.4545,0.00072393
-2.4464,0.00073817
-2.4384,0.00075327
-2.4304,0.00076732
-2.4224,0.00078238
-2.4144,0.00079826
-2.4064,0.00081505
-2.3984,0.00083211
-2.3904,0.00084859
-2.3824,0.00086533
-2.3744,0.00088315
-2.3664,0.00090102
-2.3584,0.0009192
-2.3504,0.00093805
-2.3423,0.00095559
-2.3343,0.00097563
-2.3263,0.0009959
-2.3183,0.0010159
-2.3103,0.0010366
-2.3023,0.0010582
-2.2943,0.0010799
-2.2863,0.0011013
-2.2783,0.001124
-2.2703,0.0011478
-2.2623,0.0011709
-2.2543,0.0011946
-2.2462,0.0012192
-2.2382,0.001244
-2.2302,0.0012701
-2.2222,0.0012974
-2.2142,0.0013241
-2.2062,0.0013507
-2.1982,0.0013789
-2.1902,0.001408
-2.1822,0.0014374
-2.1742,0.0014669
-2.1662,0.0014974
-2.1582,0.0015294
-2.1502,0.001561
-2.1421,0.0015938
-2.1341,0.0016268
-2.1261,0.0016617
-2.1181,0.0016961
-2.1101,0.0017309
-2.1021,0.0017663
-2.0941,0.0018051
-2.0861,0.0018432
-2.0781,0.0018825
-2.0701,0.0019225
-2.0621,0.0019613
-2.0541,0.0020055
-2.046,0.0020477
-2.038,0.0020926
-2.03,0.0021332
-2.022,0.0021807
-2.014,0.0022268
-2.006,0.0022728
-1.998,0.0023214
-1.99,0.0023711
-1.982,0.0024218
-1.974,0.0024768
-1.966,0.0025284
-1.958,0.0025835
-1.9499,0.0026365
-1.9419,0.0026934
-1.9339,0.0027521
-1.9259,0.0028109
-1.9179,0.0028736
-1.9099,0.0029344
-1.9019,0.0029971
-1.8939,0.0030606
-1.8859,0.003131
-1.8779,0.0031978
-1.8699,0.0032687
-1.8619,0.0033338
-1.8539,0.0034071
-1.8458,0.0034825
-1.8378,0.0035594
-1.8298,0.0036388
-1.8218,0.0037159
-1.8138,0.0037985
-1.8058,0.0038812
-1.7978,0.0039631
-1.7898,0.0040547
-1.7818,0.00414
-1.7738,0.0042327
-1.7658,0.0043272
-1.7578,0.0044247
-1.7497,0.0045196
-1.7417,0.0046231
-1.7337,0.0047186
-1.7257,0.0048226
-1.7177,0.0049286
-1.7097,0.005037
-1.7017,0.0051532
-1.6937,0.005274
-1.6857,0.0053867
-1.6777,0.0055096
-1.6697,0.0056347
-1.6617,0.0057568
-1.6537,0.0058771
-1.6456,0.0060059
-1.6376,0.0061424
-1.6296,0.0062812
-1.6216,0.0064206
-1.6136,0.0065656
-1.6056,0.0067159
-1.5976,0.0068645
-1.5896,0.0070085
-1.5816,0.0071651
-1.5736,0.0073249
-1.5656,0.0074983
-1.5576,0.007658
-1.5495,0.0078347
-1.5415,0.0080171
-1.5335,0.0081821
-1.5255,0.0083767
-1.5175,0.0085697
-1.5095,0.0087646
-1.5015,0.0089586
-1.4935,0.0091635
-1.4855,0.0093595
-1.4775,0.0095796
-1.4695,0.0097914
-1.4615,0.010003
-1.4535,0.010231
-1.4454,0.010454
-1.4374,0.010697
-1.4294,0.010949
-1.4214,0.011186
-1.4134,0.011447
-1.4054,0.011704
-1.3974,0.011972
-1.3894,0.012246
-1.3814,0.012503
-1.3734,0.012811
-1.3654,0.013065
-1.3574,0.013397
-1.3493,0.013628
-1.3413,0.01397
-1.3333,0.014279
-1.3253,0.014647
-1.3173,0.014928
-1.3093,0.0153
-1.3013,0.015646
-1.2933,0.016009
-1.2853,0.016416
-1.2773,0.016814
-1.2693,0.017062
-1.2613,0.017532
-1.2533,0.017894
-1.2452,0.01828
-1.2372,0.018656
-1.2292,0.019183
-1.2212,0.019647
-1.2132,0.019988
-1.2052,0.020491
-1.1972,0.021043
-1.1892,0.021351
-1.1812,0.0219
-1.1732,0.022384
-1.1652,0.022839
-1.1572,0.023447
-1.1491,0.023863
-1.1411,0.024474
-1.1331,0.025015
-1.1251,0.025456
-1.1171,0.026028
-1.1091,0.026716
-1.1011,0.027337
-1.0931,0.028148
-1.0851,0.028621
-1.0771,0.028907
-1.0691,0.029709
-1.0611,0.030226
-1.0531,0.030727
-1.045,0.03179
-1.037,0.032567
-1.029,0.033197
-1.021,0.034013
-1.013,0.035111
-1.005,0.035466
-0.997,0.036762
-0.98899,0.037414
-0.98098,0.038202
-0.97297,0.038624
-0.96496,0.039703
-0.95696,0.039661
-0.94895,0.041048
-0.94094,0.041316
-0.93293,0.043517
-0.92492,0.043748
-0.91692,0.044265
-0.90891,0.046042
-0.9009,0.047439
-0.89289,0.047453
-0.88488,0.046961
-0.87688,0.051102
-0.86887,0.050697
-0.86086,0.053806
-0.85285,0.054123
-0.84484,0.055346
-0.83684,0.055941
-0.82883,0.060847
-0.82082,0.063163
-0.81281,0.064646
-0.8048,0.057926
-0.7968,0.064545
-0.78879,0.06404
-0.78078,0.1367
-0.77277,0.13903
-0.76476,0.1414
-0.75676,0.14376
-0.74875,0.14621
-0.74074,0.14866
-0.73273,0.15117
-0.72472,0.15375
-0.71672,0.15635
-0.70871,0.15897
-0.7007,0.16166
-0.69269,0.1644
-0.68468,0.16708
-0.67668,0.16988
-0.66867,0.17275
-0.66066,0.17565
-0.65265,0.17851
-0.64464,0.18149
-0.63664,0.18456
-0.62863,0.18764
-0.62062,0.19065
-0.61261,0.19387
-0.6046,0.19704
-0.5966,0.20028
-0.58859,0.2036
-0.58058,0.20703
-0.57257,0.21035
-0.56456,0.21362
-0.55656,0.21725
-0.54855,0.22073
-0.54054,0.22446
-0.53253,0.22791
-0.52452,0.23172
-0.51652,0.23563
-0.50851,0.23929
-0.5005,0.24304
-0.49249,0.24704
-0.48448,0.25108
-0.47648,0.2551
-0.46847,0.25944
-0.46046,0.26284
-0.45245,0.26754
-0.44444,0.27206
-0.43644,0.27633
-0.42843,0.28077
-0.42042,0.28425
-0.41241,0.28768
-0.4044,0.29339
-0.3964,0.29933
-0.38839,0.30049
-0.38038,0.30757
-0.37237,0.31362
-0.36436,0.31993
-0.35636,0.31848
-0.34835,0.33054
-0.34034,0.32905
-0.33233,0.34051
-0.32432,0.33751
-0.31632,0.34713
-0.30831,0.35011
-0.3003,0.35214
-0.29229,0.37944
-0.28428,0.35591
-0.27628,0.37324
-0.26827,0.39338
-0.26026,0.39611
-0.25225,0.43618
-0.24424,0.5245
-0.23624,0.33647
-0.22823,0.41594
-0.22022,0.73005
-0.21221,0.59964
-0.2042,0.68945
-0.1962,0.1488
-0.18819,0.14451
-0.18018,0.14008
-0.17217,0.13549
-0.16416,0.13077
-0.15616,0.1259
-0.14815,0.12088
-0.14014,0.1157
-0.13213,0.11039
-0.12412,0.10493
-0.11612,0.099267
-0.10811,0.093478
-0.1001,0.087622
-0.092092,0.081427
-0.084084,0.075429
-0.076076,0.068718
-0.068068,0.062289
-0.06006,0.055546
-0.052052,0.048076
-0.044044,0.040235
-0.036036,0.03483
-0.028028,0.029737
-0.02002,0.030103
-0.012012,1.1229
-0.004004,1.0727
0.004004,1.0727
0.012012,1.1229
0.02002,0.030103
0.028028,0.029737
0.036036,0.03483
0.044044,0.040235
0.052052,0.048076
0.06006,0.055546
0.068068,0.062289
0.076076,0.068718
0.084084,0.075429
0.092092,0.081427
0.1001,0.087622
0.10811,0.093478
0.11612,0.099267
0.12412,0.10493
0.13213,0.11039
0.14014,0.1157
0.14815,0.12088
0.15616,0.1259
0.16416,0.13077
0.17217,0.13549
0.18018,0.14008
0.18819,0.14451
0.1962,0.1488
0.2042,0.68945
0.21221,0.59964
0.22022,0.73005
0.22823,0.41594
0.23624,0.33647
0.24424,0.5245
0.25225,0.43618
0.26026,0.39611
0.26827,0.39338
0.27628,0.37324
0.28428,0.35591
0.29229,0.37944
0.3003,0.35214
0.30831,0.35011
0.31632,0.34713
0.32432,0.33751
0.33233,0.34051
0.34034,0.32905
0.34835,0.33054
0.35636,0.31848
0.36436,0.31993
0.37237,0.31362
0.38038,0.30757
0.38839,0.30049
0.3964,0.29933
0.4044,0.29339
0.41241,0.28768
0.42042,0.28425
0.42843,0.28077
0.43644,0.27633
0.44444,0.27206
0.45245,0.26754
0.46046,0.26284
0.46847,0.25944
0.47648,0.2551
0.48448,0.25108
0.49249,0.24704
0.5005,0.24304
0.50851,0.23929
0.51652,0.23563
0.52452,0.23172
0.53253,0.22791
0.54054,0.22446
0.54855,0.22073
0.55656,0.21725
0.56456,0.21362
0.57257,0.21035
0.58058,0.20703
0.58859,0.2036
0.5966,0.20028
0.6046,0.19704
0.61261,0.19387
0.62062,0.19065
0.62863,0.18764
0.63664,0.18456
0.64464,0.18149
0.65265,0.17851
0.66066,0.17565
0.66867,0.17275
0.67668,0.16988
0.68468,0.16708
0.69269,0.1644
0.7007,0.16166
0.70871,0.15897
0.71672,0.15635
0.72472,0.15375
0.73273,0.15117
0.74074,0.14866
0.74875,0.14621
0.75676,0.14376
0.76476,0.1414
0.77277,0.13903
0.78078,0.1367
0.78879,0.06404
0.7968,0.064545
0.8048,0.057926
0.81281,0.064646
0.82082,0.063163
0.82883,0.060847
0.83684,0.055941
0.84484,0.055346
0.85285,0.054123
0.86086,0.053806
0.86887,0.050697
0.87688,0.051102
0.88488,0.046961
0.89289,0.047453
0.9009,0.047439
0.90891,0.046042
0.91692,0.044265
0.92492,0.043748
0.93293,0.043517
0.94094,0.041316
0.94895,0.041048
0.95696,0.039661
0.96496,0.039703
0.97297,0.038624
0.98098,0.038202
0.98899,0.037414
0.997,0.036762
1.005,0.035466
1.013,0.035111
1.021,0.034013
1.029,0.033197
1.037,0.032567
1.045,0.03179
1.0531,0.030727
1.0611,0.030226
1.0691,0.029709
1.0771,0.028907
1.0851,0.028621
1.0931,0.028148
1.1011,0.027337
1.1091,0.026716
1.1171,0.026028
1.1251,0.025456
1.1331,0.025015
1.1411,0.024474
1.1491,0.023863
1.1572,0.023447
1.1652,0.022839
1.1732,0.022384
1.1812,0.0219
1.1892,0.021351
1.1972,0.021043
1.2052,0.020491
1.2132,0.019988
1.2212,0.019647
1.2292,0.019183
1.2372,0.018656
1.2452,0.01828
1.2533,0.017894
1.2613,0.017532
1.2693,0.017062
1.2773,0.016814
1.2853,0.016416
1.2933,0.016009
1.3013,0.015646
1.3093,0.0153
1.3173,0.014928
1.3253,0.014647
1.3333,0.014279
1.3413,0.01397
1.3493,0.013628
1.3574,0.013397
1.3654,0.013065
1.3734,0.012811
1.3814,0.012503
1.3894,0.012246
1.3974,0.011972
1.4054,0.011704
1.4134,0.011447
1.4214,0.011186
1.4294,0.010949
1.4374,0.010697
1.4454,0.010454
1.4535,0.010231
1.4615,0.010003
1.4695,0.0097914
1.4775,0.0095796
1.4855,0.0093595
1.4935,0.0091635
1.5015,0.0089586
1.5095,0.0087646
1.5175,0.0085697
1.5255,0.0083767
1.5335,0.0081821
1.5415,0.0080171
1.5495,0.0078347
1.5576,0.007658
1.5656,0.0074983
1.5736,0.0073249
1.5816,0.0071651
1.5896,0.0070085
1.5976,0.0068645
1.6056,0.0067159
1.6136,0.0065656
1.6216,0.0064206
1.6296,0.0062812
1.6376,0.0061424
1.6456,0.0060059
1.6537,0.0058771
1.6617,0.0057568
1.6697,0.0056347
1.6777,0.0055096
1.6857,0.0053867
1.6937,0.005274
1.7017,0.0051532
1.7097,0.005037
1.7177,0.0049286
1.7257,0.0048226
1.7337,0.0047186
1.7417,0.0046231
1.7497,0.0045196
1.7578,0.0044247
1.7658,0.0043272
1.7738,0.0042327
1.7818,0.00414
1.7898,0.0040547
1.7978,0.0039631
1.8058,0.0038812
1.8138,0.0037985
1.8218,0.0037159
1.8298,0.0036388
1.8378,0.0035594
1.8458,0.0034825
1.8539,0.0034071
1.8619,0.0033338
1.8699,0.0032687
1.8779,0.0031978
1.8859,0.003131
1.8939,0.0030606
1.9019,0.0029971
1.9099,0.0029344
1.9179,0.0028736
1.9259,0.0028109
1.9339,0.0027521
1.9419,0.0026934
1.9499,0.0026365
1.958,0.0025835
1.966,0.0025284
1.974,0.0024768
1.982,0.0024218
1.99,0.0023711
1.998,0.0023214
2.006,0.0022728
2.014,0.0022268
2.022,0.0021807
2.03,0.0021332
2.038,0.0020926
2.046,0.0020477
2.0541,0.0020055
2.0621,0.0019613
2.0701,0.0019225
2.0781,0.0018825
2.0861,0.0018432
2.0941,0.0018051
2.1021,0.0017663
2.1101,0.0017309
2.1181,0.0016961
2.1261,0.0016617
2.1341,0.0016268
2.1421,0.0015938
2.1502,0.001561
2.1582,0.0015294
2.1662,0.0014974
2.1742,0.0014669
2.1822,0.0014374
2.1902,0.001408
2.1982,0.0013789
2.2062,0.0013507
2.2142,0.0013241
2.2222,0.0012974
2.2302,0.0012701
2.2382,0.001244
2.2462,0.0012192
2.2543,0.0011946
2.2623,0.0011709
2.2703,0.0011478
2.2783,0.001124
2.2863,0.0011013
2.2943,0.0010799
2.3023,0.0010582
2.3103,0.0010366
2.3183,0.0010159
2.3263,0.0009959
2.3343,0.00097563
2.3423,0.00095559
2.3504,0.00093805
2.3584,0.0009192
2.3664,0.00090102
2.3744,0.00088315
2.3824,0.00086533
2.3904,0.00084859
2.3984,0.00083211
2.4064,0.00081505
2.4144,0.00079826
2.4224,0.00078238
2.4304,0.00076732
2.4384,0.00075327
2.4464,0.00073817
2.4545,0.00072393
2.4625,0.00070947
2.4705,0.00069512
2.4785,0.00068158
2.4865,0.00066842
2.4945,0.00065572
2.5025,0.00064234
2.5105,0.00063025
2.5185,0.00061788
2.5265,0.00060616
2.5345,0.00059465
2.5425,0.00058322
2.5506,0.00057245
2.5586,0.00056097
2.5666,0.00055006
2.5746,0.00053934
2.5826,0.00052895
2.5906,0.0005191
2.5986,0.00050895
2.6066,0.00049926
2.6146,0.00048953
2.6226,0.00048024
2.6306,0.00047114
2.6386,0.00046245
2.6466,0.0004531
2.6547,0.00044494
2.6627,0.00043627
2.6707,0.00042786
2.6787,0.00041974
2.6867,0.00041206
2.6947,0.00040399
2.7027,0.00039634
2.7107,0.00038929
2.7187,0.0003818
2.7267,0.00037448
2.7347,0.00036757
2.7427,0.00036082
2.7508,0.0003538
2.7588,0.00034743
2.7668,0.00034047
2.7748,0.00033423
2.7828,0.00032817
2.7908,0.00032225
2.7988,0.00031612
2.8068,0.00031027
2.8148,0.000305
2.8228,0.00029913
2.8308,0.00029326
2.8388,0.00028825
2.8468,0.00028272
2.8549,0.00027759
2.8629,0.00027234
2.8709,0.00026741
2.8789,0.00026272
2.8869,0.00025756
2.8949,0.00025258
2.9029,0.00024875
2.9109,0.00024409
2.9189,0.00023962
2.9269,0.00023528
2.9349,0.00023089
2.9429,0.00022668
2.951,0.00022242
2.959,0.00021838
2.967,0.00021459
2.975,0.00021071
2.983,0.00020688
2.991,0.00020311
2.999,0.00019952
3.007,0.00019596
3.015,0.00019246
3.023,0.00018916
3.031,0.0001859
3.039,0.00018242
3.047,0.00017907
3.0551,0.00017589
3.0631,0.00017277
3.0711,0.00016964
3.0791,0.00016655
3.0871,0.00016356
3.0951,0.00016069
3.1031,0.00015807
3.1111,0.00015517
3.1191,0.00015257
3.1271,0.00014971
3.1351,0.00014711
3.1431,0.00014449
3.1512,0.00014216
3.1592,0.00013965
3.1672,0.00013713
3.1752,0.00013473
3.1832,0.00013241
3.1912,0.00013003
3.1992,0.00012779
3.2072,0.0001255
3.2152,0.00012344
3.2232,0.00012126
3.2312,0.0001191
3.2392,0.00011708
3.2472,0.00011508
3.2553,0.00011307
3.2633,0.00011109
3.2713,0.00010922
3.2793,0.00010728
3.2873,0.00010543
3.2953,8.9823e-05
3.3033,8.8425e-05
3.3113,8.6687e-05
3.3193,8.5398e-05
3.3273,8.3699e-05
3.3353,8.2488e-05
3.3433,8.0579e-05
3.3514,7.959e-05
3.3594,7.7918e-05
3.3674,7.6729e-05
3.3754,7.5246e-05
3.3834,7.4222e-05
3.3914,7.2653e-05
3.3994,7.175e-05
3.4074,7.0346e-05
3.4154,6.9223e-05
3.4234,6.7977e-05
3.4314,6.6936e-05
3.4394,6.6023e-05
3.4474,6.4893e-05
3.4555,6.3512e-05
3.4635,6.2754e-05
3.4715,6.1763e-05
3.4795,6.0657e-05
3.4875,5.9825e-05
3.4955,5.881e-05
3.5035,5.7721e-05
3.5115,5.6263e-05
3.5195,5.5605e-05
3.5275,5.4895e-05
3.5355,5.3965e-05
3.5435,5.2731e-05
3.5516,5.2164e-05
3.5596,5.1102e-05
3.5676,5.0131e-05
3.5756,4.9649e-05
3.5836,4.8567e-05
3.5916,4.7982e-05
3.5996,4.695e-05
3.6076,4.6532e-05
3.6156,4.5829e-05
3.6236,4.5003e-05
3.6316,4.3786e-05
3.6396,4.3625e-05
3.6476,4.2774e-05
3.6557,4.1925e-05
3.6637,4.1331e-05
3.6717,4.0566e-05
3.6797,3.985e-05
3.6877,3.9118e-05
3.6957,3.8549e-05
3.7037,3.7998e-05
3.7117,3.7591e-05
3.7197,3.6536e-05
3.7277,3.5895e-05
3.7357,3.5533e-05
3.7437,3.5004e-05
3.7518,3.4257e-05
3.7598,3.4025e-05
3.7678,3.3533e-05
3.7758,3.2727e-05
3.7838,3.2226e-05
3.7918,3.1843e-05
3.7998,3.141e-05
3.8078,3.0734e-05
3.8158,3.0471e-05
3.8238,2.9614e-05
3.8318,2.9413e-05
3.8398,2.8899e-05
3.8478,2.8257e-05
3.8559,2.796e-05
3.8639,2.7639e-05
3.8719,2.7113e-05
3.8799,2.6658e-05
3.8879,2.6077e-05
3.8959,2.5845e-05
3.9039,2.5639e-05
3.9119,2.5141e-05
3.9199,2.4885e-05
3.9279,2.4252e-05
3.9359,2.3836e-05
3.9439,2.3387e-05
3.952,2.3032e-05
3.96,2.273e-05
3.968,2.2415e-05
3.976,2.2081e-05
3.984,2.1638e-05
3.992,2.1375e-05


==> err_sqrt_QRAAA.tex <==
-3.992,0.13179
-3.984,0.13299
-3.976,0.13413
-3.968,0.13521
-3.96,0.13623
-3.952,0.1372
-3.9439,0.13811
-3.9359,0.13896
-3.9279,0.13976
-3.9199,0.1405
-3.9119,0.14119
-3.9039,0.14183
-3.8959,0.14242
-3.8879,0.14295
-3.8799,0.14344
-3.8719,0.14388
-3.8639,0.14427
-3.8559,0.14462
-3.8478,0.14492
-3.8398,0.14518
-3.8318,0.1454
-3.8238,0.14558
-3.8158,0.14573
-3.8078,0.14584
-3.7998,0.14591
-3.7918,0.14595
-3.7838,0.14596
-3.7758,0.14593
-3.7678,0.14588
-3.7598,0.14581
-3.7518,0.1457
-3.7437,0.14558
-3.7357,0.14543
-3.7277,0.14526
-3.7197,0.14507
-3.7117,0.14486
-3.7037,0.14463
-3.6957,0.14439
-3.6877,0.14414
-3.6797,0.14387
-3.6717,0.14359
-3.6637,0.1433
-3.6557,0.14301
-3.6476,0.1427
-3.6396,0.14239
-3.6316,0.14207
-3.6236,0.14175
-3.6156,0.14143
-3.6076,0.1411
-3.5996,0.14078
-3.5916,0.14045
-3.5836,0.14012
-3.5756,0.1398
-3.5676,0.13948
-3.5596,0.13916
-3.5516,0.13884
-3.5435,0.13853
-3.5355,0.13823
-3.5275,0.13793
-3.5195,0.13763
-3.5115,0.13735
-3.5035,0.13707
-3.4955,0.1368
-3.4875,0.13654
-3.4795,0.13628
-3.4715,0.13604
-3.4635,0.13581
-3.4555,0.13558
-3.4474,0.13537
-3.4394,0.13516
-3.4314,0.13497
-3.4234,0.13478
-3.4154,0.13461
-3.4074,0.13445
-3.3994,0.1343
-3.3914,0.13416
-3.3834,0.13403
-3.3754,0.13391
-3.3674,0.1338
-3.3594,0.1337
-3.3514,0.13361
-3.3433,0.13353
-3.3353,0.13346
-3.3273,0.1334
-3.3193,0.13334
-3.3113,0.1333
-3.3033,0.13327
-3.2953,0.13324
-3.2873,0.13322
-3.2793,0.13321
-3.2713,0.1332
-3.2633,0.13321
-3.2553,0.13321
-3.2472,0.13323
-3.2392,0.13324
-3.2312,0.13327
-3.2232,0.13329
-3.2152,0.13332
-3.2072,0.13335
-3.1992,0.13338
-3.1912,0.13342
-3.1832,0.13346
-3.1752,0.13349
-3.1672,0.13353
-3.1592,0.13356
-3.1512,0.13359
-3.1431,0.13362
-3.1351,0.13365
-3.1271,0.13368
-3.1191,0.13369
-3.1111,0.13371
-3.1031,0.13372
-3.0951,0.13372
-3.0871,0.13371
-3.0791,0.1337
-3.0711,0.13368
-3.0631,0.13364
-3.0551,0.1336
-3.047,0.13355
-3.039,0.13349
-3.031,0.13341
-3.023,0.13332
-3.015,0.13322
-3.007,0.13311
-2.999,0.13298
-2.991,0.13283
-2.983,0.13267
-2.975,0.13249
-2.967,0.1323
-2.959,0.13208
-2.951,0.13185
-2.9429,0.1316
-2.9349,0.13133
-2.9269,0.13105
-2.9189,0.13074
-2.9109,0.13041
-2.9029,0.13006
-2.8949,0.12969
-2.8869,0.1293
-2.8789,0.12888
-2.8709,0.12844
-2.8629,0.12798
-2.8549,0.1275
-2.8468,0.12699
-2.8388,0.12646
-2.8308,0.12591
-2.8228,0.12533
-2.8148,0.12473
-2.8068,0.1241
-2.7988,0.12346
-2.7908,0.12278
-2.7828,0.12209
-2.7748,0.12137
-2.7668,0.12062
-2.7588,0.11986
-2.7508,0.11906
-2.7427,0.11825
-2.7347,0.11742
-2.7267,0.11656
-2.7187,0.11568
-2.7107,0.11478
-2.7027,0.11385
-2.6947,0.11291
-2.6867,0.11195
-2.6787,0.11096
-2.6707,0.10996
-2.6627,0.10894
-2.6547,0.10791
-2.6466,0.10685
-2.6386,0.10578
-2.6306,0.1047
-2.6226,0.1036
-2.6146,0.10249
-2.6066,0.10137
-2.5986,0.10023
-2.5906,0.099089
-2.5826,0.097936
-2.5746,0.096775
-2.5666,0.095607
-2.5586,0.094434
-2.5506,0.093256
-2.5425,0.092076
-2.5345,0.090894
-2.5265,0.089712
-2.5185,0.08853
-2.5105,0.087351
-2.5025,0.086176
-2.4945,0.085005
-2.4865,0.083841
-2.4785,0.082686
-2.4705,0.081539
-2.4625,0.080404
-2.4545,0.07928
-2.4464,0.078171
-2.4384,0.077077
-2.4304,0.075999
-2.4224,0.07494
-2.4144,0.073901
-2.4064,0.072882
-2.3984,0.071886
-2.3904,0.070914
-2.3824,0.069967
-2.3744,0.069047
-2.3664,0.068155
-2.3584,0.067292
-2.3504,0.06646
-2.3423,0.06566
-2.3343,0.064893
-2.3263,0.06416
-2.3183,0.063463
-2.3103,0.062802
-2.3023,0.062178
-2.2943,0.061592
-2.2863,0.061046
-2.2783,0.06054
-2.2703,0.060074
-2.2623,0.05965
-2.2543,0.059268
-2.2462,0.058929
-2.2382,0.058632
-2.2302,0.058379
-2.2222,0.058169
-2.2142,0.058003
-2.2062,0.057881
-2.1982,0.057803
-2.1902,0.057768
-2.1822,0.057777
-2.1742,0.057829
-2.1662,0.057924
-2.1582,0.058061
-2.1502,0.05824
-2.1421,0.05846
-2.1341,0.058719
-2.1261,0.059018
-2.1181,0.059355
-2.1101,0.059729
-2.1021,0.060138
-2.0941,0.060582
-2.0861,0.061058
-2.0781,0.061566
-2.0701,0.062103
-2.0621,0.062667
-2.0541,0.063257
-2.046,0.063871
-2.038,0.064507
-2.03,0.065162
-2.022,0.065834
-2.014,0.066521
-2.006,0.067221
-1.998,0.06793
-1.99,0.068646
-1.982,0.069367
-1.974,0.070089
-1.966,0.070811
-1.958,0.071528
-1.9499,0.072239
-1.9419,0.07294
-1.9339,0.073629
-1.9259,0.074301
-1.9179,0.074955
-1.9099,0.075587
-1.9019,0.076194
-1.8939,0.076774
-1.8859,0.077322
-1.8779,0.077837
-1.8699,0.078315
-1.8619,0.078752
-1.8539,0.079148
-1.8458,0.079497
-1.8378,0.079798
-1.8298,0.080049
-1.8218,0.080245
-1.8138,0.080385
-1.8058,0.080467
-1.7978,0.080487
-1.7898,0.080445
-1.7818,0.080337
-1.7738,0.080161
-1.7658,0.079917
-1.7578,0.079602
-1.7497,0.079215
-1.7417,0.078754
-1.7337,0.078218
-1.7257,0.077607
-1.7177,0.076919
-1.7097,0.076154
-1.7017,0.075312
-1.6937,0.074392
-1.6857,0.073395
-1.6777,0.07232
-1.6697,0.071169
-1.6617,0.069942
-1.6537,0.068639
-1.6456,0.067262
-1.6376,0.065813
-1.6296,0.064293
-1.6216,0.062704
-1.6136,0.061048
-1.6056,0.059328
-1.5976,0.057546
-1.5896,0.055705
-1.5816,0.053808
-1.5736,0.051858
-1.5656,0.049859
-1.5576,0.047815
-1.5495,0.045729
-1.5415,0.043606
-1.5335,0.041451
-1.5255,0.039266
-1.5175,0.037058
-1.5095,0.034831
-1.5015,0.032591
-1.4935,0.030342
-1.4855,0.028089
-1.4775,0.025839
-1.4695,0.023596
-1.4615,0.021367
-1.4535,0.019157
-1.4454,0.016971
-1.4374,0.014817
-1.4294,0.012698
-1.4214,0.010622
-1.4134,0.0085939
-1.4054,0.0066197
-1.3974,0.004705
-1.3894,0.0028556
-1.3814,0.0010771
-1.3734,0.00062507
-1.3654,0.0022456
-1.3574,0.0037792
-1.3493,0.0052208
-1.3413,0.0065657
-1.3333,0.0078092
-1.3253,0.0089468
-1.3173,0.0099745
-1.3093,0.010888
-1.3013,0.011684
-1.2933,0.01236
-1.2853,0.012911
-1.2773,0.013336
-1.2693,0.013632
-1.2613,0.013797
-1.2533,0.013829
-1.2452,0.013728
-1.2372,0.013492
-1.2292,0.013122
-1.2212,0.012617
-1.2132,0.011977
-1.2052,0.011204
-1.1972,0.010299
-1.1892,0.0092634
-1.1812,0.0080999
-1.1732,0.006811
-1.1652,0.0053999
-1.1572,0.0038701
-1.1491,0.0022258
-1.1411,0.00047123
-1.1331,0.0013885
-1.1251,0.0033483
-1.1171,0.0054022
-1.1091,0.0075442
-1.1011,0.0097678
-1.0931,0.012066
-1.0851,0.014432
-1.0771,0.016857
-1.0691,0.019335
-1.0611,0.021857
-1.0531,0.024414
-1.045,0.026998
-1.037,0.029601
-1.029,0.032212
-1.021,0.034823
-1.013,0.037424
-1.005,0.040007
-0.997,0.042562
-0.98899,0.045079
-0.98098,0.047549
-0.97297,0.049962
-0.96496,0.05231
-0.95696,0.054583
-0.94895,0.056772
-0.94094,0.058868
-0.93293,0.060863
-0.92492,0.062749
-0.91692,0.064517
-0.90891,0.06616
-0.9009,0.06767
-0.89289,0.069042
-0.88488,0.070268
-0.87688,0.071342
-0.86887,0.07226
-0.86086,0.073016
-0.85285,0.073606
-0.84484,0.074027
-0.83684,0.074275
-0.82883,0.074348
-0.82082,0.074244
-0.81281,0.073962
-0.8048,0.073502
-0.7968,0.072864
-0.78879,0.072049
-0.78078,0.071059
-0.77277,0.069897
-0.76476,0.068565
-0.75676,0.067067
-0.74875,0.065409
-0.74074,0.063595
-0.73273,0.061632
-0.72472,0.059527
-0.71672,0.057286
-0.70871,0.054919
-0.7007,0.052433
-0.69269,0.049838
-0.68468,0.047144
-0.67668,0.044361
-0.66867,0.041501
-0.66066,0.038574
-0.65265,0.035593
-0.64464,0.032569
-0.63664,0.029516
-0.62863,0.026445
-0.62062,0.023369
-0.61261,0.020303
-0.6046,0.017259
-0.5966,0.01425
-0.58859,0.011289
-0.58058,0.0083913
-0.57257,0.0055682
-0.56456,0.0028332
-0.55656,0.00019894
-0.54855,0.0023222
-0.54054,0.0047181
-0.53253,0.0069773
-0.52452,0.0090886
-0.51652,0.011041
-0.50851,0.012826
-0.5005,0.014432
-0.49249,0.015852
-0.48448,0.017078
-0.47648,0.018103
-0.46847,0.018921
-0.46046,0.019526
-0.45245,0.019913
-0.44444,0.020081
-0.43644,0.020026
-0.42843,0.019748
-0.42042,0.019246
-0.41241,0.01852
-0.4044,0.017574
-0.3964,0.01641
-0.38839,0.015034
-0.38038,0.013449
-0.37237,0.011663
-0.36436,0.0096845
-0.35636,0.0075214
-0.34835,0.0051843
-0.34034,0.0026842
-0.33233,3.342e-05
-0.32432,0.0027546
-0.31632,0.0056656
-0.30831,0.0086841
-0.3003,0.011794
-0.29229,0.014978
-0.28428,0.018218
-0.27628,0.021495
-0.26827,0.024789
-0.26026,0.028082
-0.25225,0.03135
-0.24424,0.034574
-0.23624,0.037732
-0.22823,0.0408
-0.22022,0.043758
-0.21221,0.046581
-0.2042,0.049247
-0.1962,0.051733
-0.18819,0.054017
-0.18018,0.056074
-0.17217,0.057884
-0.16416,0.059422
-0.15616,0.060668
-0.14815,0.061599
-0.14014,0.062194
-0.13213,0.062433
-0.12412,0.062297
-0.11612,0.061765
-0.10811,0.06082
-0.1001,0.059445
-0.092092,0.057622
-0.084084,0.055336
-0.076076,0.052574
-0.068068,0.049322
-0.06006,0.045568
-0.052052,0.041302
-0.044044,0.036513
-0.036036,0.031193
-0.028028,0.025337
-0.02002,0.018937
-0.012012,0.011992
-0.004004,0.0044964
0.004004,0.0044587
0.012012,0.011879
0.02002,0.01875
0.028028,0.025076
0.036036,0.03086
0.044044,0.036109
0.052052,0.04083
0.06006,0.045031
0.068068,0.048723
0.076076,0.051916
0.084084,0.054622
0.092092,0.056856
0.1001,0.058631
0.10811,0.059964
0.11612,0.06087
0.12412,0.061368
0.13213,0.061476
0.14014,0.061214
0.14815,0.060601
0.15616,0.059657
0.16416,0.058405
0.17217,0.056865
0.18018,0.05506
0.18819,0.053012
0.1962,0.050743
0.2042,0.048278
0.21221,0.045637
0.22022,0.042845
0.22823,0.039923
0.23624,0.036895
0.24424,0.033782
0.25225,0.030608
0.26026,0.027392
0.26827,0.024157
0.27628,0.020922
0.28428,0.017709
0.29229,0.014535
0.3003,0.01142
0.30831,0.0083804
0.31632,0.005434
0.32432,0.0025965
0.33233,0.00011726
0.34034,0.0026932
0.34835,0.0051185
0.35636,0.0073811
0.36436,0.0094702
0.37237,0.011376
0.38038,0.01309
0.38839,0.014605
0.3964,0.015915
0.4044,0.017014
0.41241,0.017897
0.42042,0.018564
0.42843,0.01901
0.43644,0.019237
0.44444,0.019243
0.45245,0.019032
0.46046,0.018604
0.46847,0.017964
0.47648,0.017116
0.48448,0.016066
0.49249,0.014819
0.5005,0.013383
0.50851,0.011765
0.51652,0.0099753
0.52452,0.0080218
0.53253,0.0059149
0.54054,0.003665
0.54855,0.0012833
0.55656,0.0012188
0.56456,0.0038293
0.57257,0.0065361
0.58058,0.0093265
0.58859,0.012188
0.5966,0.015107
0.6046,0.018071
0.61261,0.021067
0.62062,0.024082
0.62863,0.027103
0.63664,0.030117
0.64464,0.033111
0.65265,0.036073
0.66066,0.03899
0.66867,0.041851
0.67668,0.044645
0.68468,0.04736
0.69269,0.049985
0.7007,0.052511
0.70871,0.054928
0.71672,0.057227
0.72472,0.059399
0.73273,0.061438
0.74074,0.063334
0.74875,0.065083
0.75676,0.066678
0.76476,0.068114
0.77277,0.069386
0.78078,0.070491
0.78879,0.071427
0.7968,0.072189
0.8048,0.072778
0.81281,0.073191
0.82082,0.073429
0.82883,0.073493
0.83684,0.073382
0.84484,0.0731
0.85285,0.072649
0.86086,0.072031
0.86887,0.071251
0.87688,0.070313
0.88488,0.069221
0.89289,0.067981
0.9009,0.066599
0.90891,0.06508
0.91692,0.063433
0.92492,0.061663
0.93293,0.059779
0.94094,0.057788
0.94895,0.055698
0.95696,0.053518
0.96496,0.051256
0.97297,0.048922
0.98098,0.046523
0.98899,0.04407
0.997,0.041571
1.005,0.039036
1.013,0.036474
1.021,0.033894
1.029,0.031305
1.037,0.028717
1.045,0.026137
1.0531,0.023576
1.0611,0.021042
1.0691,0.018543
1.0771,0.016087
1.0851,0.013683
1.0931,0.011338
1.1011,0.0090591
1.1091,0.0068539
1.1171,0.004729
1.1251,0.0026907
1.1331,0.00074497
1.1411,0.0011025
1.1491,0.0028465
1.1572,0.0044822
1.1652,0.0060053
1.1732,0.0074118
1.1812,0.0086982
1.1892,0.0098613
1.1972,0.010898
1.2052,0.011807
1.2132,0.012587
1.2212,0.013234
1.2292,0.01375
1.2372,0.014133
1.2452,0.014383
1.2533,0.014501
1.2613,0.014486
1.2693,0.014341
1.2773,0.014067
1.2853,0.013666
1.2933,0.01314
1.3013,0.012491
1.3093,0.011723
1.3173,0.010838
1.3253,0.0098398
1.3333,0.0087328
1.3413,0.0075206
1.3493,0.0062075
1.3574,0.004798
1.3654,0.0032968
1.3734,0.0017087
1.3814,3.8864e-05
1.3894,0.0017076
1.3974,0.0035254
1.4054,0.0054091
1.4134,0.0073532
1.4214,0.0093521
1.4294,0.0114
1.4374,0.013492
1.4454,0.015621
1.4535,0.017782
1.4615,0.01997
1.4695,0.022179
1.4775,0.024403
1.4855,0.026636
1.4935,0.028874
1.5015,0.031111
1.5095,0.033341
1.5175,0.03556
1.5255,0.037763
1.5335,0.039944
1.5415,0.0421
1.5495,0.044225
1.5576,0.046316
1.5656,0.048368
1.5736,0.050377
1.5816,0.05234
1.5896,0.054252
1.5976,0.056112
1.6056,0.057914
1.6136,0.059658
1.6216,0.06134
1.6296,0.062957
1.6376,0.064507
1.6456,0.065989
1.6537,0.067401
1.6617,0.068741
1.6697,0.070008
1.6777,0.071201
1.6857,0.072319
1.6937,0.073361
1.7017,0.074328
1.7097,0.075218
1.7177,0.076032
1.7257,0.076771
1.7337,0.077434
1.7417,0.078022
1.7497,0.078536
1.7578,0.078978
1.7658,0.079348
1.7738,0.079647
1.7818,0.079878
1.7898,0.080042
1.7978,0.08014
1.8058,0.080175
1.8138,0.080149
1.8218,0.080063
1.8298,0.079921
1.8378,0.079724
1.8458,0.079476
1.8539,0.079178
1.8619,0.078834
1.8699,0.078446
1.8779,0.078016
1.8859,0.077549
1.8939,0.077046
1.9019,0.076511
1.9099,0.075946
1.9179,0.075355
1.9259,0.07474
1.9339,0.074105
1.9419,0.073452
1.9499,0.072784
1.958,0.072105
1.966,0.071417
1.974,0.070723
1.982,0.070025
1.99,0.069328
1.998,0.068633
2.006,0.067943
2.014,0.067261
2.022,0.066589
2.03,0.06593
2.038,0.065286
2.046,0.06466
2.0541,0.064053
2.0621,0.063468
2.0701,0.062907
2.0781,0.062372
2.0861,0.061865
2.0941,0.061387
2.1021,0.06094
2.1101,0.060526
2.1181,0.060146
2.1261,0.059801
2.1341,0.059493
2.1421,0.059223
2.1502,0.058992
2.1582,0.058801
2.1662,0.058651
2.1742,0.058542
2.1822,0.058475
2.1902,0.05845
2.1982,0.058468
2.2062,0.05853
2.2142,0.058635
2.2222,0.058783
2.2302,0.058975
2.2382,0.05921
2.2462,0.059489
2.2543,0.05981
2.2623,0.060174
2.2703,0.06058
2.2783,0.061028
2.2863,0.061517
2.2943,0.062046
2.3023,0.062615
2.3103,0.063223
2.3183,0.063869
2.3263,0.064551
2.3343,0.06527
2.3423,0.066023
2.3504,0.06681
2.3584,0.06763
2.3664,0.068481
2.3744,0.069363
2.3824,0.070273
2.3904,0.071211
2.3984,0.072175
2.4064,0.073164
2.4144,0.074176
2.4224,0.07521
2.4304,0.076265
2.4384,0.077339
2.4464,0.07843
2.4545,0.079538
2.4625,0.08066
2.4705,0.081795
2.4785,0.082941
2.4865,0.084098
2.4945,0.085264
2.5025,0.086436
2.5105,0.087615
2.5185,0.088797
2.5265,0.089983
2.5345,0.09117
2.5425,0.092356
2.5506,0.093542
2.5586,0.094725
2.5666,0.095903
2.5746,0.097077
2.5826,0.098244
2.5906,0.099403
2.5986,0.10055
2.6066,0.10169
2.6146,0.10282
2.6226,0.10394
2.6306,0.10504
2.6386,0.10613
2.6466,0.1072
2.6547,0.10826
2.6627,0.1093
2.6707,0.11032
2.6787,0.11133
2.6867,0.11231
2.6947,0.11328
2.7027,0.11422
2.7107,0.11514
2.7187,0.11604
2.7267,0.11692
2.7347,0.11778
2.7427,0.11861
2.7508,0.11942
2.7588,0.1202
2.7668,0.12096
2.7748,0.1217
2.7828,0.12241
2.7908,0.1231
2.7988,0.12376
2.8068,0.12439
2.8148,0.12501
2.8228,0.12559
2.8308,0.12616
2.8388,0.12669
2.8468,0.12721
2.8549,0.12769
2.8629,0.12816
2.8709,0.1286
2.8789,0.12902
2.8869,0.12941
2.8949,0.12978
2.9029,0.13013
2.9109,0.13046
2.9189,0.13076
2.9269,0.13104
2.9349,0.13131
2.9429,0.13155
2.951,0.13177
2.959,0.13198
2.967,0.13216
2.975,0.13233
2.983,0.13248
2.991,0.13261
2.999,0.13273
3.007,0.13284
3.015,0.13293
3.023,0.133
3.031,0.13306
3.039,0.13311
3.047,0.13315
3.0551,0.13318
3.0631,0.1332
3.0711,0.13321
3.0791,0.13321
3.0871,0.1332
3.0951,0.13318
3.1031,0.13316
3.1111,0.13314
3.1191,0.13311
3.1271,0.13307
3.1351,0.13303
3.1431,0.13299
3.1512,0.13295
3.1592,0.13291
3.1672,0.13286
3.1752,0.13282
3.1832,0.13278
3.1912,0.13274
3.1992,0.1327
3.2072,0.13267
3.2152,0.13264
3.2232,0.13261
3.2312,0.13259
3.2392,0.13257
3.2472,0.13256
3.2553,0.13256
3.2633,0.13256
3.2713,0.13257
3.2793,0.13259
3.2873,0.13262
3.2953,0.13265
3.3033,0.1327
3.3113,0.13275
3.3193,0.13282
3.3273,0.13289
3.3353,0.13298
3.3433,0.13307
3.3514,0.13318
3.3594,0.13329
3.3674,0.13342
3.3754,0.13356
3.3834,0.13371
3.3914,0.13387
3.3994,0.13404
3.4074,0.13422
3.4154,0.13441
3.4234,0.13462
3.4314,0.13483
3.4394,0.13506
3.4474,0.13529
3.4555,0.13554
3.4635,0.13579
3.4715,0.13606
3.4795,0.13633
3.4875,0.13661
3.4955,0.1369
3.5035,0.13719
3.5115,0.1375
3.5195,0.13781
3.5275,0.13812
3.5355,0.13844
3.5435,0.13877
3.5516,0.1391
3.5596,0.13943
3.5676,0.13976
3.5756,0.14009
3.5836,0.14043
3.5916,0.14076
3.5996,0.1411
3.6076,0.14143
3.6156,0.14175
3.6236,0.14208
3.6316,0.14239
3.6396,0.1427
3.6476,0.14301
3.6557,0.1433
3.6637,0.14359
3.6717,0.14386
3.6797,0.14412
3.6877,0.14437
3.6957,0.1446
3.7037,0.14482
3.7117,0.14502
3.7197,0.1452
3.7277,0.14537
3.7357,0.14551
3.7437,0.14563
3.7518,0.14573
3.7598,0.1458
3.7678,0.14585
3.7758,0.14587
3.7838,0.14586
3.7918,0.14582
3.7998,0.14576
3.8078,0.14566
3.8158,0.14553
3.8238,0.14536
3.8318,0.14516
3.8398,0.14493
3.8478,0.14466
3.8559,0.14435
3.8639,0.144
3.8719,0.14361
3.8799,0.14319
3.8879,0.14272
3.8959,0.14221
3.9039,0.14167
3.9119,0.14107
3.9199,0.14044
3.9279,0.13977
3.9359,0.13905
3.9439,0.13829
3.952,0.13749
3.96,0.13665
3.968,0.13576
3.976,0.13483
3.984,0.13387
3.992,0.13286


==> err_sqrt_pAAA.tex <==
-3.992,3.0715e-06
-3.984,3.1493e-06
-3.976,3.2292e-06
-3.968,3.3113e-06
-3.96,3.3958e-06
-3.952,3.4827e-06
-3.9439,3.5719e-06
-3.9359,3.6639e-06
-3.9279,3.7578e-06
-3.9199,3.8547e-06
-3.9119,3.9538e-06
-3.9039,4.0559e-06
-3.8959,4.1605e-06
-3.8879,4.2673e-06
-3.8799,4.378e-06
-3.8719,4.491e-06
-3.8639,4.6071e-06
-3.8559,4.7255e-06
-3.8478,4.8471e-06
-3.8398,4.9716e-06
-3.8318,5.0998e-06
-3.8238,5.23e-06
-3.8158,5.3647e-06
-3.8078,5.503e-06
-3.7998,5.6435e-06
-3.7918,5.788e-06
-3.7838,5.9351e-06
-3.7758,6.0866e-06
-3.7678,6.2412e-06
-3.7598,6.3999e-06
-3.7518,6.5622e-06
-3.7437,6.7286e-06
-3.7357,6.8985e-06
-3.7277,7.0721e-06
-3.7197,7.2503e-06
-3.7117,7.4324e-06
-3.7037,7.6186e-06
-3.6957,7.8091e-06
-3.6877,8.0038e-06
-3.6797,8.2027e-06
-3.6717,8.4064e-06
-3.6637,8.6149e-06
-3.6557,8.828e-06
-3.6476,9.0454e-06
-3.6396,9.2677e-06
-3.6316,9.4953e-06
-3.6236,9.7276e-06
-3.6156,9.9652e-06
-3.6076,1.0208e-05
-3.5996,1.0456e-05
-3.5916,1.0709e-05
-3.5836,1.0968e-05
-3.5756,1.1232e-05
-3.5676,1.1502e-05
-3.5596,1.1778e-05
-3.5516,1.206e-05
-3.5435,1.2348e-05
-3.5355,1.2642e-05
-3.5275,1.2942e-05
-3.5195,1.3248e-05
-3.5115,1.3562e-05
-3.5035,1.3881e-05
-3.4955,1.4207e-05
-3.4875,1.454e-05
-3.4795,1.4879e-05
-3.4715,1.5227e-05
-3.4635,1.5581e-05
-3.4555,1.5942e-05
-3.4474,1.631e-05
-3.4394,1.6687e-05
-3.4314,1.7071e-05
-3.4234,1.7463e-05
-3.4154,1.7862e-05
-3.4074,1.8271e-05
-3.3994,1.8687e-05
-3.3914,1.9112e-05
-3.3834,1.9544e-05
-3.3754,1.9986e-05
-3.3674,2.0437e-05
-3.3594,2.0897e-05
-3.3514,2.1365e-05
-3.3433,2.1844e-05
-3.3353,2.2332e-05
-3.3273,2.2829e-05
-3.3193,2.3336e-05
-3.3113,2.3853e-05
-3.3033,2.4381e-05
-3.2953,2.4919e-05
-3.2873,2.5467e-05
-3.2793,2.6026e-05
-3.2713,2.6596e-05
-3.2633,2.7177e-05
-3.2553,2.7769e-05
-3.2472,2.8372e-05
-3.2392,2.8989e-05
-3.2312,2.9616e-05
-3.2232,3.0255e-05
-3.2152,3.0907e-05
-3.2072,3.1571e-05
-3.1992,3.2248e-05
-3.1912,3.2938e-05
-3.1832,3.3641e-05
-3.1752,3.4357e-05
-3.1672,3.5088e-05
-3.1592,3.5832e-05
-3.1512,3.659e-05
-3.1431,3.7362e-05
-3.1351,3.8149e-05
-3.1271,3.8951e-05
-3.1191,3.9768e-05
-3.1111,4.06e-05
-3.1031,4.1448e-05
-3.0951,4.2312e-05
-3.0871,4.3192e-05
-3.0791,4.4087e-05
-3.0711,4.5001e-05
-3.0631,4.5931e-05
-3.0551,4.6878e-05
-3.047,4.7843e-05
-3.039,4.8826e-05
-3.031,4.9827e-05
-3.023,5.0846e-05
-3.015,5.1885e-05
-3.007,5.2942e-05
-2.999,5.4019e-05
-2.991,5.5116e-05
-2.983,5.6233e-05
-2.975,5.7371e-05
-2.967,5.8529e-05
-2.959,5.9709e-05
-2.951,6.091e-05
-2.9429,6.2133e-05
-2.9349,6.3379e-05
-2.9269,6.4647e-05
-2.9189,6.5939e-05
-2.9109,6.7254e-05
-2.9029,6.8594e-05
-2.8949,6.9957e-05
-2.8869,7.1345e-05
-2.8789,7.2759e-05
-2.8709,7.4198e-05
-2.8629,7.5663e-05
-2.8549,7.7156e-05
-2.8468,7.8675e-05
-2.8388,8.0222e-05
-2.8308,8.1797e-05
-2.8228,8.34e-05
-2.8148,8.5034e-05
-2.8068,8.6696e-05
-2.7988,8.8388e-05
-2.7908,9.0111e-05
-2.7828,9.1866e-05
-2.7748,9.3652e-05
-2.7668,9.5472e-05
-2.7588,9.7323e-05
-2.7508,9.9209e-05
-2.7427,0.00010113
-2.7347,0.00010308
-2.7267,0.00010508
-2.7187,0.0001071
-2.7107,0.00010917
-2.7027,0.00011127
-2.6947,0.00011341
-2.6867,0.00011559
-2.6787,0.00011781
-2.6707,0.00012006
-2.6627,0.00012237
-2.6547,0.00012471
-2.6466,0.0001271
-2.6386,0.00012953
-2.6306,0.000132
-2.6226,0.00013452
-2.6146,0.00013709
-2.6066,0.00013971
-2.5986,0.00014237
-2.5906,0.00014509
-2.5826,0.00014785
-2.5746,0.00015066
-2.5666,0.00015353
-2.5586,0.00015645
-2.5506,0.00015943
-2.5425,0.00016247
-2.5345,0.00016556
-2.5265,0.0001687
-2.5185,0.00017191
-2.5105,0.00017518
-2.5025,0.00017851
-2.4945,0.00018191
-2.4865,0.00018537
-2.4785,0.00018889
-2.4705,0.00019249
-2.4625,0.00019615
-2.4545,0.00019989
-2.4464,0.00020369
-2.4384,0.00020757
-2.4304,0.00021153
-2.4224,0.00021556
-2.4144,0.00021968
-2.4064,0.00022387
-2.3984,0.00022815
-2.3904,0.00023251
-2.3824,0.00023696
-2.3744,0.0002415
-2.3664,0.00024612
-2.3584,0.00025085
-2.3504,0.00025566
-2.3423,0.00026058
-2.3343,0.00026559
-2.3263,0.00027071
-2.3183,0.00027593
-2.3103,0.00028125
-2.3023,0.00028669
-2.2943,0.00029224
-2.2863,0.0002979
-2.2783,0.00030369
-2.2703,0.00030959
-2.2623,0.00031562
-2.2543,0.00032177
-2.2462,0.00032805
-2.2382,0.00033447
-2.2302,0.00034102
-2.2222,0.00034771
-2.2142,0.00035455
-2.2062,0.00036153
-2.1982,0.00036867
-2.1902,0.00037595
-2.1822,0.0003834
-2.1742,0.00039101
-2.1662,0.00039878
-2.1582,0.00040673
-2.1502,0.00041485
-2.1421,0.00042315
-2.1341,0.00043163
-2.1261,0.0004403
-2.1181,0.00044917
-2.1101,0.00045823
-2.1021,0.00046751
-2.0941,0.00047698
-2.0861,0.00048667
-2.0781,0.00049659
-2.0701,0.00050672
-2.0621,0.00051709
-2.0541,0.00052771
-2.046,0.00053856
-2.038,0.00054966
-2.03,0.00056101
-2.022,0.00057263
-2.014,0.00058453
-2.006,0.0005967
-1.998,0.00060915
-1.99,0.0006219
-1.982,0.00063494
-1.974,0.0006483
-1.966,0.00066196
-1.958,0.00067596
-1.9499,0.00069028
-1.9419,0.00070494
-1.9339,0.00071996
-1.9259,0.00073533
-1.9179,0.00075106
-1.9099,0.00076719
-1.9019,0.00078369
-1.8939,0.0008006
-1.8859,0.00081791
-1.8779,0.00083564
-1.8699,0.00085379
-1.8619,0.00087237
-1.8539,0.00089143
-1.8458,0.00091095
-1.8378,0.00093094
-1.8298,0.00095139
-1.8218,0.00097237
-1.8138,0.00099385
-1.8058,0.0010159
-1.7978,0.0010384
-1.7898,0.0010615
-1.7818,0.0010852
-1.7738,0.0011094
-1.7658,0.0011342
-1.7578,0.0011597
-1.7497,0.0011857
-1.7417,0.0012124
-1.7337,0.0012398
-1.7257,0.0012678
-1.7177,0.0012966
-1.7097,0.001326
-1.7017,0.0013561
-1.6937,0.001387
-1.6857,0.0014187
-1.6777,0.0014511
-1.6697,0.0014843
-1.6617,0.0015183
-1.6537,0.0015532
-1.6456,0.0015889
-1.6376,0.0016254
-1.6296,0.0016629
-1.6216,0.0017013
-1.6136,0.0017406
-1.6056,0.0017808
-1.5976,0.0018221
-1.5896,0.0018643
-1.5816,0.0019076
-1.5736,0.0019519
-1.5656,0.0019972
-1.5576,0.0020437
-1.5495,0.0020912
-1.5415,0.0021399
-1.5335,0.0021898
-1.5255,0.0022408
-1.5175,0.0022931
-1.5095,0.0023466
-1.5015,0.0024013
-1.4935,0.0024574
-1.4855,0.0025147
-1.4775,0.0025734
-1.4695,0.0026335
-1.4615,0.0026949
-1.4535,0.0027578
-1.4454,0.0028221
-1.4374,0.0028879
-1.4294,0.0029552
-1.4214,0.003024
-1.4134,0.0030944
-1.4054,0.0031664
-1.3974,0.00324
-1.3894,0.0033152
-1.3814,0.0033921
-1.3734,0.0034707
-1.3654,0.0035511
-1.3574,0.0036331
-1.3493,0.003717
-1.3413,0.0038027
-1.3333,0.0038902
-1.3253,0.0039796
-1.3173,0.0040709
-1.3093,0.0041641
-1.3013,0.0042593
-1.2933,0.0043564
-1.2853,0.0044556
-1.2773,0.0045567
-1.2693,0.00466
-1.2613,0.0047653
-1.2533,0.0048727
-1.2452,0.0049822
-1.2372,0.0050939
-1.2292,0.0052078
-1.2212,0.0053238
-1.2132,0.0054421
-1.2052,0.0055626
-1.1972,0.0056853
-1.1892,0.0058104
-1.1812,0.0059377
-1.1732,0.0060673
-1.1652,0.0061992
-1.1572,0.0063334
-1.1491,0.00647
-1.1411,0.0066089
-1.1331,0.0067502
-1.1251,0.0068938
-1.1171,0.0070398
-1.1091,0.0071882
-1.1011,0.0073389
-1.0931,0.0074919
-1.0851,0.0076473
-1.0771,0.0078051
-1.0691,0.0079652
-1.0611,0.0081276
-1.0531,0.0082922
-1.045,0.0084592
-1.037,0.0086285
-1.029,0.0087999
-1.021,0.0089736
-1.013,0.0091494
-1.005,0.0093274
-0.997,0.0095075
-0.98899,0.0096897
-0.98098,0.0098738
-0.97297,0.01006
-0.96496,0.010248
-0.95696,0.010438
-0.94895,0.010629
-0.94094,0.010823
-0.93293,0.011018
-0.92492,0.011214
-0.91692,0.011412
-0.90891,0.011611
-0.9009,0.011812
-0.89289,0.012014
-0.88488,0.012217
-0.87688,0.012421
-0.86887,0.012626
-0.86086,0.012831
-0.85285,0.013037
-0.84484,0.013244
-0.83684,0.013451
-0.82883,0.013658
-0.82082,0.013865
-0.81281,0.014072
-0.8048,0.014279
-0.7968,0.014485
-0.78879,0.014691
-0.78078,0.014896
-0.77277,0.0151
-0.76476,0.015303
-0.75676,0.015505
-0.74875,0.015705
-0.74074,0.015903
-0.73273,0.0161
-0.72472,0.016294
-0.71672,0.016486
-0.70871,0.016675
-0.7007,0.016862
-0.69269,0.017045
-0.68468,0.017225
-0.67668,0.017402
-0.66867,0.017575
-0.66066,0.017745
-0.65265,0.01791
-0.64464,0.018071
-0.63664,0.018227
-0.62863,0.018378
-0.62062,0.018525
-0.61261,0.018666
-0.6046,0.018802
-0.5966,0.018932
-0.58859,0.019057
-0.58058,0.019175
-0.57257,0.019288
-0.56456,0.019394
-0.55656,0.019494
-0.54855,0.019587
-0.54054,0.019674
-0.53253,0.019754
-0.52452,0.019828
-0.51652,0.019893
-0.50851,0.019953
-0.5005,0.020006
-0.49249,0.020052
-0.48448,0.020092
-0.47648,0.020124
-0.46847,0.02015
-0.46046,0.020169
-0.45245,0.020182
-0.44444,0.020188
-0.43644,0.020189
-0.42843,0.020183
-0.42042,0.020173
-0.41241,0.020155
-0.4044,0.020134
-0.3964,0.020107
-0.38839,0.020076
-0.38038,0.020039
-0.37237,0.02
-0.36436,0.019954
-0.35636,0.019906
-0.34835,0.019853
-0.34034,0.019795
-0.33233,0.019739
-0.32432,0.019679
-0.31632,0.019606
-0.30831,0.019532
-0.3003,0.019454
-0.29229,0.019363
-0.28428,0.019271
-0.27628,0.019169
-0.26827,0.019048
-0.26026,0.018929
-0.25225,0.018789
-0.24424,0.018633
-0.23624,0.018442
-0.22823,0.018239
-0.22022,0.018004
-0.21221,0.017723
-0.2042,0.017409
-0.1962,0.017042
-0.18819,0.016624
-0.18018,0.01616
-0.17217,0.015619
-0.16416,0.015007
-0.15616,0.014313
-0.14815,0.013516
-0.14014,0.012663
-0.13213,0.011677
-0.12412,0.010643
-0.11612,0.0095103
-0.10811,0.0082756
-0.1001,0.0070172
-0.092092,0.0057218
-0.084084,0.0044733
-0.076076,0.0033279
-0.068068,0.0023735
-0.06006,0.0017604
-0.052052,0.0016077
-0.044044,0.0018987
-0.036036,0.0029662
-0.028028,0.0043037
-0.02002,0.0054747
-0.012012,0.0049926
-0.004004,0.0014874
0.004004,0.0014428
0.012012,0.0050491
0.02002,0.0053089
0.028028,0.0040928
0.036036,0.0025957
0.044044,0.0015235
0.052052,0.0010217
0.06006,0.0011359
0.068068,0.0016956
0.076076,0.0026494
0.084084,0.0037797
0.092092,0.0050062
0.1001,0.006304
0.10811,0.0075535
0.11612,0.0087944
0.12412,0.0099655
0.13213,0.011019
0.14014,0.012012
0.14815,0.012919
0.15616,0.01373
0.16416,0.014466
0.17217,0.015124
0.18018,0.015702
0.18819,0.01623
0.1962,0.016696
0.2042,0.017111
0.21221,0.017486
0.22022,0.017822
0.22823,0.018125
0.23624,0.018396
0.24424,0.018644
0.25225,0.018874
0.26026,0.019085
0.26827,0.019283
0.27628,0.01947
0.28428,0.019643
0.29229,0.019811
0.3003,0.019969
0.30831,0.020122
0.31632,0.020269
0.32432,0.020411
0.33233,0.020548
0.34034,0.020678
0.34835,0.020804
0.35636,0.020925
0.36436,0.021042
0.37237,0.021153
0.38038,0.021258
0.38839,0.021358
0.3964,0.021451
0.4044,0.021538
0.41241,0.021618
0.42042,0.02169
0.42843,0.021755
0.43644,0.021813
0.44444,0.021862
0.45245,0.021904
0.46046,0.021937
0.46847,0.021961
0.47648,0.021977
0.48448,0.021984
0.49249,0.021982
0.5005,0.021971
0.50851,0.021951
0.51652,0.021922
0.52452,0.021884
0.53253,0.021838
0.54054,0.021782
0.54855,0.021718
0.55656,0.021644
0.56456,0.021563
0.57257,0.021473
0.58058,0.021375
0.58859,0.02127
0.5966,0.021156
0.6046,0.021035
0.61261,0.020907
0.62062,0.020771
0.62863,0.020629
0.63664,0.02048
0.64464,0.020325
0.65265,0.020164
0.66066,0.019997
0.66867,0.019825
0.67668,0.019647
0.68468,0.019464
0.69269,0.019277
0.7007,0.019085
0.70871,0.01889
0.71672,0.01869
0.72472,0.018487
0.73273,0.01828
0.74074,0.018071
0.74875,0.017858
0.75676,0.017643
0.76476,0.017426
0.77277,0.017206
0.78078,0.016985
0.78879,0.016762
0.7968,0.016537
0.8048,0.016312
0.81281,0.016085
0.82082,0.015858
0.82883,0.01563
0.83684,0.015401
0.84484,0.015173
0.85285,0.014944
0.86086,0.014715
0.86887,0.014487
0.87688,0.014259
0.88488,0.014032
0.89289,0.013806
0.9009,0.01358
0.90891,0.013356
0.91692,0.013132
0.92492,0.01291
0.93293,0.012689
0.94094,0.01247
0.94895,0.012252
0.95696,0.012036
0.96496,0.011822
0.97297,0.01161
0.98098,0.011399
0.98899,0.01119
0.997,0.010984
1.005,0.01078
1.013,0.010577
1.021,0.010377
1.029,0.01018
1.037,0.0099843
1.045,0.0097913
1.0531,0.0096007
1.0611,0.0094125
1.0691,0.0092268
1.0771,0.0090436
1.0851,0.0088629
1.0931,0.0086848
1.1011,0.0085092
1.1091,0.0083361
1.1171,0.0081657
1.1251,0.0079978
1.1331,0.0078325
1.1411,0.0076698
1.1491,0.0075097
1.1572,0.0073522
1.1652,0.0071972
1.1732,0.0070449
1.1812,0.0068951
1.1892,0.0067478
1.1972,0.0066031
1.2052,0.006461
1.2132,0.0063213
1.2212,0.0061842
1.2292,0.0060495
1.2372,0.0059173
1.2452,0.0057875
1.2533,0.0056602
1.2613,0.0055353
1.2693,0.0054127
1.2773,0.0052925
1.2853,0.0051746
1.2933,0.0050591
1.3013,0.0049458
1.3093,0.0048347
1.3173,0.0047259
1.3253,0.0046192
1.3333,0.0045147
1.3413,0.0044124
1.3493,0.0043122
1.3574,0.004214
1.3654,0.0041179
1.3734,0.0040238
1.3814,0.0039317
1.3894,0.0038415
1.3974,0.0037533
1.4054,0.0036669
1.4134,0.0035824
1.4214,0.0034998
1.4294,0.0034189
1.4374,0.0033398
1.4454,0.0032625
1.4535,0.0031868
1.4615,0.0031129
1.4695,0.0030406
1.4775,0.0029699
1.4855,0.0029008
1.4935,0.0028333
1.5015,0.0027673
1.5095,0.0027027
1.5175,0.0026397
1.5255,0.0025781
1.5335,0.0025179
1.5415,0.0024592
1.5495,0.0024017
1.5576,0.0023456
1.5656,0.0022908
1.5736,0.0022373
1.5816,0.0021851
1.5896,0.002134
1.5976,0.0020842
1.6056,0.0020355
1.6136,0.001988
1.6216,0.0019416
1.6296,0.0018964
1.6376,0.0018522
1.6456,0.001809
1.6537,0.0017669
1.6617,0.0017258
1.6697,0.0016856
1.6777,0.0016465
1.6857,0.0016082
1.6937,0.0015709
1.7017,0.0015345
1.7097,0.001499
1.7177,0.0014643
1.7257,0.0014305
1.7337,0.0013975
1.7417,0.0013653
1.7497,0.0013338
1.7578,0.0013031
1.7658,0.0012732
1.7738,0.001244
1.7818,0.0012155
1.7898,0.0011877
1.7978,0.0011606
1.8058,0.0011342
1.8138,0.0011083
1.8218,0.0010832
1.8298,0.0010586
1.8378,0.0010346
1.8458,0.0010112
1.8539,0.0009884
1.8619,0.00096613
1.8699,0.00094441
1.8779,0.00092321
1.8859,0.00090253
1.8939,0.00088235
1.9019,0.00086266
1.9099,0.00084345
1.9179,0.00082471
1.9259,0.00080642
1.9339,0.00078857
1.9419,0.00077115
1.9499,0.00075415
1.958,0.00073757
1.966,0.00072138
1.974,0.00070558
1.982,0.00069016
1.99,0.00067512
1.998,0.00066043
2.006,0.0006461
2.014,0.0006321
2.022,0.00061845
2.03,0.00060511
2.038,0.0005921
2.046,0.00057939
2.0541,0.00056698
2.0621,0.00055487
2.0701,0.00054304
2.0781,0.00053149
2.0861,0.00052022
2.0941,0.0005092
2.1021,0.00049845
2.1101,0.00048794
2.1181,0.00047768
2.1261,0.00046766
2.1341,0.00045787
2.1421,0.00044831
2.1502,0.00043897
2.1582,0.00042984
2.1662,0.00042092
2.1742,0.00041221
2.1822,0.00040369
2.1902,0.00039537
2.1982,0.00038723
2.2062,0.00037929
2.2142,0.00037152
2.2222,0.00036392
2.2302,0.00035649
2.2382,0.00034924
2.2462,0.00034214
2.2543,0.0003352
2.2623,0.00032841
2.2703,0.00032178
2.2783,0.00031529
2.2863,0.00030894
2.2943,0.00030273
2.3023,0.00029666
2.3103,0.00029072
2.3183,0.00028491
2.3263,0.00027922
2.3343,0.00027366
2.3423,0.00026821
2.3504,0.00026288
2.3584,0.00025767
2.3664,0.00025256
2.3744,0.00024757
2.3824,0.00024268
2.3904,0.00023789
2.3984,0.0002332
2.4064,0.00022861
2.4144,0.00022412
2.4224,0.00021972
2.4304,0.00021541
2.4384,0.00021119
2.4464,0.00020706
2.4545,0.00020301
2.4625,0.00019905
2.4705,0.00019516
2.4785,0.00019136
2.4865,0.00018763
2.4945,0.00018397
2.5025,0.00018039
2.5105,0.00017689
2.5185,0.00017345
2.5265,0.00017008
2.5345,0.00016678
2.5425,0.00016354
2.5506,0.00016037
2.5586,0.00015726
2.5666,0.00015421
2.5746,0.00015122
2.5826,0.00014829
2.5906,0.00014542
2.5986,0.0001426
2.6066,0.00013984
2.6146,0.00013713
2.6226,0.00013448
2.6306,0.00013187
2.6386,0.00012932
2.6466,0.00012681
2.6547,0.00012435
2.6627,0.00012194
2.6707,0.00011958
2.6787,0.00011726
2.6867,0.00011499
2.6947,0.00011275
2.7027,0.00011056
2.7107,0.00010841
2.7187,0.00010631
2.7267,0.00010424
2.7347,0.00010221
2.7427,0.00010022
2.7508,9.8267e-05
2.7588,9.635e-05
2.7668,9.4471e-05
2.7748,9.2625e-05
2.7828,9.0815e-05
2.7908,8.9037e-05
2.7988,8.7293e-05
2.8068,8.5582e-05
2.8148,8.3904e-05
2.8228,8.2256e-05
2.8308,8.0638e-05
2.8388,7.905e-05
2.8468,7.7493e-05
2.8549,7.5964e-05
2.8629,7.4463e-05
2.8709,7.2991e-05
2.8789,7.1545e-05
2.8869,7.0128e-05
2.8949,6.8734e-05
2.9029,6.7369e-05
2.9109,6.6029e-05
2.9189,6.4712e-05
2.9269,6.3421e-05
2.9349,6.2154e-05
2.9429,6.0911e-05
2.951,5.969e-05
2.959,5.849e-05
2.967,5.7316e-05
2.975,5.6162e-05
2.983,5.5029e-05
2.991,5.3918e-05
2.999,5.2827e-05
3.007,5.1757e-05
3.015,5.0706e-05
3.023,4.9676e-05
3.031,4.8665e-05
3.039,4.7672e-05
3.047,4.6698e-05
3.0551,4.5743e-05
3.0631,4.4806e-05
3.0711,4.3886e-05
3.0791,4.2983e-05
3.0871,4.2098e-05
3.0951,4.1229e-05
3.1031,4.0377e-05
3.1111,3.9541e-05
3.1191,3.8721e-05
3.1271,3.7915e-05
3.1351,3.7126e-05
3.1431,3.6352e-05
3.1512,3.5593e-05
3.1592,3.4848e-05
3.1672,3.4117e-05
3.1752,3.34e-05
3.1832,3.2697e-05
3.1912,3.2008e-05
3.1992,3.1332e-05
3.2072,3.0669e-05
3.2152,3.0019e-05
3.2232,2.9382e-05
3.2312,2.8757e-05
3.2392,2.8144e-05
3.2472,2.7543e-05
3.2553,2.6955e-05
3.2633,2.6377e-05
3.2713,2.5811e-05
3.2793,2.5256e-05
3.2873,2.4713e-05
3.2953,2.418e-05
3.3033,2.3657e-05
3.3113,2.3145e-05
3.3193,2.2644e-05
3.3273,2.2152e-05
3.3353,2.167e-05
3.3433,2.1198e-05
3.3514,2.0736e-05
3.3594,2.0283e-05
3.3674,1.9839e-05
3.3754,1.9404e-05
3.3834,1.8978e-05
3.3914,1.8561e-05
3.3994,1.8153e-05
3.4074,1.7753e-05
3.4154,1.7361e-05
3.4234,1.6977e-05
3.4314,1.6601e-05
3.4394,1.6234e-05
3.4474,1.5874e-05
3.4555,1.5521e-05
3.4635,1.5176e-05
3.4715,1.4838e-05
3.4795,1.4508e-05
3.4875,1.4184e-05
3.4955,1.3868e-05
3.5035,1.3558e-05
3.5115,1.3255e-05
3.5195,1.2958e-05
3.5275,1.2668e-05
3.5355,1.2384e-05
3.5435,1.2107e-05
3.5516,1.1835e-05
3.5596,1.157e-05
3.5676,1.131e-05
3.5756,1.1056e-05
3.5836,1.0808e-05
3.5916,1.0566e-05
3.5996,1.0328e-05
3.6076,1.0097e-05
3.6156,9.8701e-06
3.6236,9.6487e-06
3.6316,9.4325e-06
3.6396,9.2211e-06
3.6476,9.0146e-06
3.6557,8.8129e-06
3.6637,8.6158e-06
3.6717,8.4234e-06
3.6797,8.2355e-06
3.6877,8.052e-06
3.6957,7.873e-06
3.7037,7.6981e-06
3.7117,7.5275e-06
3.7197,7.361e-06
3.7277,7.1984e-06
3.7357,7.0397e-06
3.7437,6.8851e-06
3.7518,6.7341e-06
3.7598,6.5869e-06
3.7678,6.4434e-06
3.7758,6.3034e-06
3.7838,6.1669e-06
3.7918,6.0339e-06
3.7998,5.9042e-06
3.8078,5.7779e-06
3.8158,5.6547e-06
3.8238,5.5348e-06
3.8318,5.418e-06
3.8398,5.3042e-06
3.8478,5.1934e-06
3.8559,5.0855e-06
3.8639,4.9805e-06
3.8719,4.8784e-06
3.8799,4.7789e-06
3.8879,4.6822e-06
3.8959,4.5881e-06
3.9039,4.4967e-06
3.9119,4.4077e-06
3.9199,4.3212e-06
3.9279,4.2372e-06
3.9359,4.1556e-06
3.9439,4.0763e-06
3.952,3.9992e-06
3.96,3.9245e-06
3.968,3.8519e-06
3.976,3.7814e-06
3.984,3.7131e-06
3.992,3.6469e-06


==> poles_starfish.tex <==
-0.95296,0.72517
2.0469,0.66229
-0.54639,0.99604
-0.17692,1.1492
0.17993,1.2288
0.53244,1.2493
1.6216,0.9407
0.88553,1.2137
1.2447,1.1167
2.0479,-0.66059
-0.95131,-0.72468
-0.54468,-0.99606
1.6225,-0.93973
-0.17538,-1.1493
1.2457,-1.1161
0.18131,-1.2289
0.88668,-1.2135
0.5337,-1.2492


==> qraaaErr.tex <==
0,4.3172e-15,3.3148e-15,1.2084e-15,3.9781e-15,7.8184e-16
0.0052632,3.0189e-05,3.0189e-05,3.0189e-05,3.0189e-05,2.9422e-05
0.010526,2.6166e-05,2.6166e-05,2.6166e-05,2.6166e-05,2.6695e-05
0.015789,1.8013e-05,1.8013e-05,1.8012e-05,1.8013e-05,1.8004e-05
0.021053,1.1444e-05,1.1445e-05,1.1444e-05,1.1444e-05,1.1194e-05
0.026316,7.0138e-06,7.0138e-06,7.0137e-06,7.0138e-06,6.7446e-06
0.031579,4.2019e-06,4.202e-06,4.2019e-06,4.2019e-06,3.9886e-06
0.036842,2.4681e-06,2.4681e-06,2.4681e-06,2.4681e-06,2.3194e-06
0.042105,1.4198e-06,1.4199e-06,1.4198e-06,1.4199e-06,1.3237e-06
0.047368,7.9754e-07,7.9757e-07,7.9754e-07,7.9756e-07,7.388e-07
0.052632,4.355e-07,4.3553e-07,4.355e-07,4.3552e-07,4.0129e-07
0.057895,2.2983e-07,2.2985e-07,2.2983e-07,2.2984e-07,2.1083e-07
0.063158,1.1632e-07,1.1632e-07,1.1632e-07,1.1632e-07,1.0629e-07
0.068421,5.5857e-08,5.5862e-08,5.5858e-08,5.5861e-08,5.0875e-08
0.073684,2.5068e-08,2.5071e-08,2.5069e-08,2.507e-08,2.2766e-08
0.078947,1.0271e-08,1.0272e-08,1.0271e-08,1.0272e-08,9.3036e-09
0.084211,3.6914e-09,3.6922e-09,3.6918e-09,3.692e-09,3.3361e-09
0.089474,1.0744e-09,1.0747e-09,1.0746e-09,1.0745e-09,9.6888e-10
0.094737,2.0298e-10,2.0307e-10,2.0309e-10,2.0298e-10,1.8273e-10
0.1,3.356e-13,3.1956e-13,3.315e-13,3.1508e-13,2.9428e-13


==> quad_err_besselfunc.tex <==
0.1,7.7671e-13
0.10298,7.7682e-13
0.10596,7.7649e-13
0.10894,7.7671e-13
0.11192,7.7671e-13
0.1149,7.7671e-13
0.11788,7.7671e-13
0.12086,7.7671e-13
0.12384,7.7682e-13
0.12683,7.766e-13
0.12981,7.7693e-13
0.13279,7.7671e-13
0.13577,7.7649e-13
0.13875,7.7671e-13
0.14173,7.7682e-13
0.14471,7.766e-13
0.14769,7.766e-13
0.15067,7.7671e-13
0.15365,7.766e-13
0.15663,7.7693e-13
0.15961,7.7671e-13
0.16259,7.7671e-13
0.16557,7.7649e-13
0.16855,7.7671e-13
0.17153,7.7671e-13
0.17451,7.766e-13
0.1775,7.7671e-13
0.18048,7.7649e-13
0.18346,7.7682e-13
0.18644,7.7693e-13
0.18942,7.766e-13
0.1924,7.7671e-13
0.19538,7.7682e-13
0.19836,7.7693e-13
0.20134,7.766e-13
0.20432,7.7682e-13
0.2073,7.7705e-13
0.21028,7.7682e-13
0.21326,7.766e-13
0.21624,7.7671e-13
0.21922,7.7671e-13
0.2222,7.7671e-13
0.22519,7.7682e-13
0.22817,7.7682e-13
0.23115,7.7693e-13
0.23413,7.7671e-13
0.23711,7.7649e-13
0.24009,7.7693e-13
0.24307,7.7682e-13
0.24605,7.7671e-13
0.24903,7.7693e-13
0.25201,7.7682e-13
0.25499,7.7649e-13
0.25797,7.766e-13
0.26095,7.7649e-13
0.26393,7.7705e-13
0.26691,7.7627e-13
0.26989,7.7671e-13
0.27287,7.7682e-13
0.27586,7.7682e-13
0.27884,7.7693e-13
0.28182,7.7671e-13
0.2848,7.7671e-13
0.28778,7.7705e-13
0.29076,7.766e-13
0.29374,7.7682e-13
0.29672,7.766e-13
0.2997,7.7671e-13
0.30268,7.7682e-13
0.30566,7.766e-13
0.30864,7.7671e-13
0.31162,7.766e-13
0.3146,7.7693e-13
0.31758,7.7693e-13
0.32056,7.7693e-13
0.32354,7.7671e-13
0.32653,7.7705e-13
0.32951,7.7671e-13
0.33249,7.7671e-13
0.33547,7.7671e-13
0.33845,7.7682e-13
0.34143,7.7671e-13
0.34441,7.7682e-13
0.34739,7.7693e-13
0.35037,7.7671e-13
0.35335,7.7671e-13
0.35633,7.7682e-13
0.35931,7.7671e-13
0.36229,7.7693e-13
0.36527,7.7705e-13
0.36825,7.7693e-13
0.37123,7.766e-13
0.37421,7.7682e-13
0.3772,7.7682e-13
0.38018,7.7716e-13
0.38316,7.7693e-13
0.38614,7.7671e-13
0.38912,7.7693e-13
0.3921,7.7671e-13
0.39508,7.7682e-13
0.39806,7.7682e-13
0.40104,7.7649e-13
0.40402,7.7671e-13
0.407,7.766e-13
0.40998,7.7671e-13
0.41296,7.7693e-13
0.41594,7.7682e-13
0.41892,7.7682e-13
0.4219,7.7682e-13
0.42488,7.7693e-13
0.42787,7.7682e-13
0.43085,7.7671e-13
0.43383,7.7671e-13
0.43681,7.7682e-13
0.43979,7.7671e-13
0.44277,7.7693e-13
0.44575,7.7682e-13
0.44873,7.7682e-13
0.45171,7.766e-13
0.45469,7.7682e-13
0.45767,7.7671e-13
0.46065,7.7682e-13
0.46363,7.7705e-13
0.46661,7.7682e-13
0.46959,7.7705e-13
0.47257,7.7682e-13
0.47556,7.7705e-13
0.47854,7.7682e-13
0.48152,7.7705e-13
0.4845,7.7705e-13
0.48748,7.7682e-13
0.49046,7.7671e-13
0.49344,7.7682e-13
0.49642,7.7671e-13
0.4994,7.7682e-13
0.50238,7.7693e-13
0.50536,7.7705e-13
0.50834,7.7682e-13
0.51132,7.7682e-13
0.5143,7.7671e-13
0.51728,7.7671e-13
0.52026,7.7682e-13
0.52324,7.7693e-13
0.52623,7.7705e-13
0.52921,7.7671e-13
0.53219,7.7671e-13
0.53517,7.766e-13
0.53815,7.7671e-13
0.54113,7.7671e-13
0.54411,7.7705e-13
0.54709,7.7693e-13
0.55007,7.7693e-13
0.55305,7.7705e-13
0.55603,7.7693e-13
0.55901,7.7671e-13
0.56199,7.7705e-13
0.56497,7.7682e-13
0.56795,7.7705e-13
0.57093,7.7682e-13
0.57391,7.7693e-13
0.5769,7.7705e-13
0.57988,7.7705e-13
0.58286,7.7693e-13
0.58584,7.7693e-13
0.58882,7.7682e-13
0.5918,7.7682e-13
0.59478,7.766e-13
0.59776,7.7716e-13
0.60074,7.7693e-13
0.60372,7.7671e-13
0.6067,7.7693e-13
0.60968,7.7705e-13
0.61266,7.7693e-13
0.61564,7.7671e-13
0.61862,7.7693e-13
0.6216,7.7671e-13
0.62458,7.7693e-13
0.62757,7.7682e-13
0.63055,7.7671e-13
0.63353,7.7693e-13
0.63651,7.7682e-13
0.63949,7.7727e-13
0.64247,7.7693e-13
0.64545,7.7671e-13
0.64843,7.7693e-13
0.65141,7.7716e-13
0.65439,7.7716e-13
0.65737,7.766e-13
0.66035,7.7716e-13
0.66333,7.7705e-13
0.66631,7.7693e-13
0.66929,7.7693e-13
0.67227,7.7693e-13
0.67526,7.7727e-13
0.67824,7.7705e-13
0.68122,7.7705e-13
0.6842,7.7693e-13
0.68718,7.7693e-13
0.69016,7.7705e-13
0.69314,7.7693e-13
0.69612,7.7682e-13
0.6991,7.7705e-13
0.70208,7.7693e-13
0.70506,7.7693e-13
0.70804,7.7705e-13
0.71102,7.7693e-13
0.714,7.7693e-13
0.71698,7.7716e-13
0.71996,7.7705e-13
0.72294,7.7716e-13
0.72593,7.7682e-13
0.72891,7.7671e-13
0.73189,7.7693e-13
0.73487,7.7705e-13
0.73785,7.766e-13
0.74083,7.7682e-13
0.74381,7.7693e-13
0.74679,7.7682e-13
0.74977,7.7671e-13
0.75275,7.7682e-13
0.75573,7.7682e-13
0.75871,7.7705e-13
0.76169,7.7705e-13
0.76467,7.7716e-13
0.76765,7.7716e-13
0.77063,7.7705e-13
0.77361,7.7738e-13
0.7766,7.7716e-13
0.77958,7.7716e-13
0.78256,7.7705e-13
0.78554,7.7693e-13
0.78852,7.7705e-13
0.7915,7.7705e-13
0.79448,7.7693e-13
0.79746,7.7716e-13
0.80044,7.7705e-13
0.80342,7.7693e-13
0.8064,7.7705e-13
0.80938,7.7716e-13
0.81236,7.7705e-13
0.81534,7.7716e-13
0.81832,7.7693e-13
0.8213,7.7693e-13
0.82428,7.7705e-13
0.82727,7.7716e-13
0.83025,7.7705e-13
0.83323,7.7716e-13
0.83621,7.7705e-13
0.83919,7.7705e-13
0.84217,7.7705e-13
0.84515,7.7682e-13
0.84813,7.7716e-13
0.85111,7.7705e-13
0.85409,7.7705e-13
0.85707,7.7705e-13
0.86005,7.7705e-13
0.86303,7.7716e-13
0.86601,7.7716e-13
0.86899,7.7716e-13
0.87197,7.7727e-13
0.87495,7.7705e-13
0.87794,7.7705e-13
0.88092,7.7727e-13
0.8839,7.7705e-13
0.88688,7.7738e-13
0.88986,7.7716e-13
0.89284,7.7705e-13
0.89582,7.7705e-13
0.8988,7.7705e-13
0.90178,7.7693e-13
0.90476,7.7705e-13
0.90774,7.7716e-13
0.91072,7.7716e-13
0.9137,7.7727e-13
0.91668,7.7705e-13
0.91966,7.7705e-13
0.92264,7.7682e-13
0.92563,7.7716e-13
0.92861,7.7727e-13
0.93159,7.7716e-13
0.93457,7.7705e-13
0.93755,7.7727e-13
0.94053,7.7716e-13
0.94351,7.7727e-13
0.94649,7.7716e-13
0.94947,7.7716e-13
0.95245,7.7716e-13
0.95543,7.7716e-13
0.95841,7.7716e-13
0.96139,7.7716e-13
0.96437,7.7716e-13
0.96735,7.7716e-13
0.97033,7.7693e-13
0.97331,7.7693e-13
0.9763,7.7705e-13
0.97928,7.7727e-13
0.98226,7.7716e-13
0.98524,7.7705e-13
0.98822,7.7705e-13
0.9912,7.7749e-13
0.99418,7.7716e-13
0.99716,7.7705e-13
1.0001,7.7705e-13
1.0031,7.7693e-13
1.0061,7.7716e-13
1.0091,7.7693e-13
1.0121,7.7705e-13
1.015,7.7682e-13
1.018,7.7716e-13
1.021,7.7727e-13
1.024,7.7705e-13
1.027,7.7738e-13
1.0299,7.7727e-13
1.0329,7.7727e-13
1.0359,7.7727e-13
1.0389,7.7716e-13
1.0419,7.7738e-13
1.0448,7.7716e-13
1.0478,7.7705e-13
1.0508,7.7716e-13
1.0538,7.7738e-13
1.0568,7.7727e-13
1.0598,7.7727e-13
1.0627,7.7705e-13
1.0657,7.7727e-13
1.0687,7.7727e-13
1.0717,7.7749e-13
1.0747,7.7716e-13
1.0776,7.7738e-13
1.0806,7.7716e-13
1.0836,7.7727e-13
1.0866,7.7705e-13
1.0896,7.7705e-13
1.0925,7.7738e-13
1.0955,7.7738e-13
1.0985,7.7749e-13
1.1015,7.7727e-13
1.1045,7.7727e-13
1.1074,7.7727e-13
1.1104,7.7693e-13
1.1134,7.7716e-13
1.1164,7.7738e-13
1.1194,7.7716e-13
1.1223,7.7727e-13
1.1253,7.7738e-13
1.1283,7.7705e-13
1.1313,7.7738e-13
1.1343,7.7716e-13
1.1372,7.7738e-13
1.1402,7.7727e-13
1.1432,7.7716e-13
1.1462,7.776e-13
1.1492,7.7716e-13
1.1522,7.7716e-13
1.1551,7.7693e-13
1.1581,7.776e-13
1.1611,7.7727e-13
1.1641,7.7716e-13
1.1671,7.7716e-13
1.17,7.7727e-13
1.173,7.7749e-13
1.176,7.7749e-13
1.179,7.776e-13
1.182,7.7727e-13
1.1849,7.7727e-13
1.1879,7.7727e-13
1.1909,7.7727e-13
1.1939,7.7727e-13
1.1969,7.7738e-13
1.1998,7.7738e-13
1.2028,7.7749e-13
1.2058,7.7738e-13
1.2088,7.776e-13
1.2118,7.7738e-13
1.2147,7.7727e-13
1.2177,7.7727e-13
1.2207,7.7749e-13
1.2237,7.7716e-13
1.2267,7.7705e-13
1.2296,7.7771e-13
1.2326,7.7738e-13
1.2356,7.7749e-13
1.2386,7.776e-13
1.2416,7.7727e-13
1.2445,7.7716e-13
1.2475,7.7727e-13
1.2505,7.7738e-13
1.2535,7.7727e-13
1.2565,7.7738e-13
1.2595,7.7749e-13
1.2624,7.7738e-13
1.2654,7.7771e-13
1.2684,7.7738e-13
1.2714,7.7727e-13
1.2744,7.7771e-13
1.2773,7.776e-13
1.2803,7.7716e-13
1.2833,7.776e-13
1.2863,7.7727e-13
1.2893,7.7749e-13
1.2922,7.7793e-13
1.2952,7.7727e-13
1.2982,7.7782e-13
1.3012,7.7738e-13
1.3042,7.7716e-13
1.3071,7.7749e-13
1.3101,7.7771e-13
1.3131,7.7771e-13
1.3161,7.776e-13
1.3191,7.7771e-13
1.322,7.7749e-13
1.325,7.7749e-13
1.328,7.7749e-13
1.331,7.7738e-13
1.334,7.776e-13
1.3369,7.7727e-13
1.3399,7.7771e-13
1.3429,7.7727e-13
1.3459,7.7738e-13
1.3489,7.7749e-13
1.3519,7.7771e-13
1.3548,7.7749e-13
1.3578,7.776e-13
1.3608,7.7771e-13
1.3638,7.7738e-13
1.3668,7.7727e-13
1.3697,7.7749e-13
1.3727,7.7749e-13
1.3757,7.7738e-13
1.3787,7.7749e-13
1.3817,7.7738e-13
1.3846,7.776e-13
1.3876,7.776e-13
1.3906,7.7749e-13
1.3936,7.7749e-13
1.3966,7.7727e-13
1.3995,7.7738e-13
1.4025,7.7771e-13
1.4055,7.7738e-13
1.4085,7.7782e-13
1.4115,7.7727e-13
1.4144,7.7749e-13
1.4174,7.7738e-13
1.4204,7.776e-13
1.4234,7.776e-13
1.4264,7.7738e-13
1.4293,7.7782e-13
1.4323,7.7771e-13
1.4353,7.776e-13
1.4383,7.7771e-13
1.4413,7.7749e-13
1.4442,7.7782e-13
1.4472,7.7727e-13
1.4502,7.7749e-13
1.4532,7.7749e-13
1.4562,7.7738e-13
1.4592,7.7738e-13
1.4621,7.7738e-13
1.4651,7.7727e-13
1.4681,7.7771e-13
1.4711,7.7716e-13
1.4741,7.7738e-13
1.477,7.7738e-13
1.48,7.776e-13
1.483,7.7738e-13
1.486,7.7749e-13
1.489,7.7749e-13
1.4919,7.7771e-13
1.4949,7.7782e-13
1.4979,7.7749e-13
1.5009,7.7749e-13
1.5039,7.7793e-13
1.5068,7.7749e-13
1.5098,7.7782e-13
1.5128,7.7727e-13
1.5158,7.7771e-13
1.5188,7.7749e-13
1.5217,7.7749e-13
1.5247,7.776e-13
1.5277,7.7749e-13
1.5307,7.7782e-13
1.5337,7.776e-13
1.5366,7.7771e-13
1.5396,7.776e-13
1.5426,7.7738e-13
1.5456,7.776e-13
1.5486,7.7727e-13
1.5516,7.776e-13
1.5545,7.7782e-13
1.5575,7.7771e-13
1.5605,7.7771e-13
1.5635,7.7749e-13
1.5665,7.7793e-13
1.5694,7.7749e-13
1.5724,7.7749e-13
1.5754,7.7749e-13
1.5784,7.7727e-13
1.5814,7.776e-13
1.5843,7.7749e-13
1.5873,7.7771e-13
1.5903,7.776e-13
1.5933,7.7738e-13
1.5963,7.7793e-13
1.5992,7.7738e-13
1.6022,7.7749e-13
1.6052,7.7749e-13
1.6082,7.7727e-13
1.6112,7.7716e-13
1.6141,7.7771e-13
1.6171,7.7727e-13
1.6201,7.7749e-13
1.6231,7.7771e-13
1.6261,7.7782e-13
1.629,7.7749e-13
1.632,7.7738e-13
1.635,7.776e-13
1.638,7.776e-13
1.641,7.7749e-13
1.6439,7.7793e-13
1.6469,7.776e-13
1.6499,7.7771e-13
1.6529,7.7771e-13
1.6559,7.7793e-13
1.6589,7.7771e-13
1.6618,7.7771e-13
1.6648,7.7771e-13
1.6678,7.7782e-13
1.6708,7.7738e-13
1.6738,7.7716e-13
1.6767,7.7749e-13
1.6797,7.7749e-13
1.6827,7.7771e-13
1.6857,7.776e-13
1.6887,7.776e-13
1.6916,7.7782e-13
1.6946,7.7771e-13
1.6976,7.7749e-13
1.7006,7.776e-13
1.7036,7.7771e-13
1.7065,7.7782e-13
1.7095,7.7749e-13
1.7125,7.7727e-13
1.7155,7.7738e-13
1.7185,7.7749e-13
1.7214,7.7749e-13
1.7244,7.776e-13
1.7274,7.776e-13
1.7304,7.7749e-13
1.7334,7.7749e-13
1.7363,7.776e-13
1.7393,7.7782e-13
1.7423,7.7782e-13
1.7453,7.7749e-13
1.7483,7.776e-13
1.7513,7.7771e-13
1.7542,7.7771e-13
1.7572,7.776e-13
1.7602,7.7782e-13
1.7632,7.7738e-13
1.7662,7.7782e-13
1.7691,7.776e-13
1.7721,7.776e-13
1.7751,7.7771e-13
1.7781,7.7771e-13
1.7811,7.7827e-13
1.784,7.7738e-13
1.787,7.7716e-13
1.79,7.7771e-13
1.793,7.776e-13
1.796,7.7782e-13
1.7989,7.7782e-13
1.8019,7.776e-13
1.8049,7.7782e-13
1.8079,7.7771e-13
1.8109,7.776e-13
1.8138,7.7738e-13
1.8168,7.7727e-13
1.8198,7.7749e-13
1.8228,7.7738e-13
1.8258,7.7738e-13
1.8287,7.7749e-13
1.8317,7.7727e-13
1.8347,7.7771e-13
1.8377,7.7782e-13
1.8407,7.7738e-13
1.8436,7.7738e-13
1.8466,7.7705e-13
1.8496,7.7749e-13
1.8526,7.7793e-13
1.8556,7.776e-13
1.8586,7.7771e-13
1.8615,7.7727e-13
1.8645,7.7771e-13
1.8675,7.7738e-13
1.8705,7.7782e-13
1.8735,7.776e-13
1.8764,7.776e-13
1.8794,7.776e-13
1.8824,7.7716e-13
1.8854,7.7782e-13
1.8884,7.7749e-13
1.8913,7.7738e-13
1.8943,7.776e-13
1.8973,7.776e-13
1.9003,7.7771e-13
1.9033,7.7738e-13
1.9062,7.7782e-13
1.9092,7.7771e-13
1.9122,7.7749e-13
1.9152,7.7771e-13
1.9182,7.7727e-13
1.9211,7.7738e-13
1.9241,7.776e-13
1.9271,7.7771e-13
1.9301,7.7738e-13
1.9331,7.7771e-13
1.936,7.776e-13
1.939,7.7738e-13
1.942,7.7738e-13
1.945,7.7782e-13
1.948,7.7749e-13
1.951,7.7716e-13
1.9539,7.7716e-13
1.9569,7.7738e-13
1.9599,7.7782e-13
1.9629,7.7771e-13
1.9659,7.7727e-13
1.9688,7.7738e-13
1.9718,7.7771e-13
1.9748,7.7738e-13
1.9778,7.7749e-13
1.9808,7.7771e-13
1.9837,7.7727e-13
1.9867,7.7727e-13
1.9897,7.7771e-13
1.9927,7.7749e-13
1.9957,7.7693e-13
1.9986,7.7738e-13
2.0016,7.7771e-13
2.0046,7.7716e-13
2.0076,7.7771e-13
2.0106,7.7716e-13
2.0135,7.7771e-13
2.0165,7.7771e-13
2.0195,7.7693e-13
2.0225,7.7749e-13
2.0255,7.7749e-13
2.0284,7.776e-13
2.0314,7.776e-13
2.0344,7.7782e-13
2.0374,7.7771e-13
2.0404,7.7749e-13
2.0433,7.776e-13
2.0463,7.7716e-13
2.0493,7.7749e-13
2.0523,7.7771e-13
2.0553,7.7749e-13
2.0583,7.7727e-13
2.0612,7.7738e-13
2.0642,7.7771e-13
2.0672,7.7749e-13
2.0702,7.776e-13
2.0732,7.776e-13
2.0761,7.776e-13
2.0791,7.776e-13
2.0821,7.7727e-13
2.0851,7.7749e-13
2.0881,7.7738e-13
2.091,7.7716e-13
2.094,7.7738e-13
2.097,7.7749e-13
2.1,7.7749e-13
2.103,7.7705e-13
2.1059,7.7705e-13
2.1089,7.7738e-13
2.1119,7.7727e-13
2.1149,7.7738e-13
2.1179,7.7749e-13
2.1208,7.776e-13
2.1238,7.7682e-13
2.1268,7.7716e-13
2.1298,7.776e-13
2.1328,7.7705e-13
2.1357,7.7727e-13
2.1387,7.776e-13
2.1417,7.7705e-13
2.1447,7.7749e-13
2.1477,7.776e-13
2.1507,7.7682e-13
2.1536,7.7693e-13
2.1566,7.7705e-13
2.1596,7.7749e-13
2.1626,7.7738e-13
2.1656,7.7738e-13
2.1685,7.7738e-13
2.1715,7.7705e-13
2.1745,7.7738e-13
2.1775,7.7738e-13
2.1805,7.7705e-13
2.1834,7.7705e-13
2.1864,7.7727e-13
2.1894,7.7693e-13
2.1924,7.7738e-13
2.1954,7.7727e-13
2.1983,7.7716e-13
2.2013,7.7705e-13
2.2043,7.7705e-13
2.2073,7.7682e-13
2.2103,7.7716e-13
2.2132,7.7705e-13
2.2162,7.7749e-13
2.2192,7.766e-13
2.2222,7.7682e-13
2.2252,7.7705e-13
2.2281,7.7693e-13
2.2311,7.7738e-13
2.2341,7.7727e-13
2.2371,7.7693e-13
2.2401,7.7727e-13
2.243,7.7682e-13
2.246,7.7716e-13
2.249,7.7705e-13
2.252,7.7705e-13
2.255,7.7716e-13
2.258,7.7705e-13
2.2609,7.7716e-13
2.2639,7.766e-13
2.2669,7.7727e-13
2.2699,7.766e-13
2.2729,7.7671e-13
2.2758,7.7693e-13
2.2788,7.7682e-13
2.2818,7.7693e-13
2.2848,7.7716e-13
2.2878,7.7705e-13
2.2907,7.7682e-13
2.2937,7.7649e-13
2.2967,7.7682e-13
2.2997,7.7682e-13
2.3027,7.7671e-13
2.3056,7.7671e-13
2.3086,7.7693e-13
2.3116,7.7716e-13
2.3146,7.7671e-13
2.3176,7.7671e-13
2.3205,7.7716e-13
2.3235,7.7682e-13
2.3265,7.7693e-13
2.3295,7.7693e-13
2.3325,7.7693e-13
2.3354,7.7682e-13
2.3384,7.7682e-13
2.3414,7.766e-13
2.3444,7.7682e-13
2.3474,7.766e-13
2.3504,7.766e-13
2.3533,7.7671e-13
2.3563,7.7693e-13
2.3593,7.7693e-13
2.3623,7.7671e-13
2.3653,7.7693e-13
2.3682,7.7682e-13
2.3712,7.7649e-13
2.3742,7.7671e-13
2.3772,7.766e-13
2.3802,7.7682e-13
2.3831,7.7649e-13
2.3861,7.766e-13
2.3891,7.766e-13
2.3921,7.7627e-13
2.3951,7.7627e-13
2.398,7.766e-13
2.401,7.7649e-13
2.404,7.7649e-13
2.407,7.7638e-13
2.41,7.7627e-13
2.4129,7.7649e-13
2.4159,7.7605e-13
2.4189,7.7638e-13
2.4219,7.7638e-13
2.4249,7.7649e-13
2.4278,7.7638e-13
2.4308,7.7627e-13
2.4338,7.7627e-13
2.4368,7.7627e-13
2.4398,7.7627e-13
2.4427,7.766e-13
2.4457,7.7616e-13
2.4487,7.7627e-13
2.4517,7.7627e-13
2.4547,7.7605e-13
2.4577,7.7616e-13
2.4606,7.7616e-13
2.4636,7.7638e-13
2.4666,7.7616e-13
2.4696,7.7627e-13
2.4726,7.7593e-13
2.4755,7.7582e-13
2.4785,7.7605e-13
2.4815,7.7605e-13
2.4845,7.7627e-13
2.4875,7.7616e-13
2.4904,7.7616e-13
2.4934,7.7605e-13
2.4964,7.7627e-13
2.4994,7.7616e-13
2.5024,7.7627e-13
2.5053,7.7627e-13
2.5083,7.7593e-13
2.5113,7.7616e-13
2.5143,7.7582e-13
2.5173,7.7616e-13
2.5202,7.7605e-13
2.5232,7.7582e-13
2.5262,7.7571e-13
2.5292,7.756e-13
2.5322,7.7549e-13
2.5351,7.7605e-13
2.5381,7.756e-13
2.5411,7.7571e-13
2.5441,7.7571e-13
2.5471,7.7582e-13
2.5501,7.7582e-13
2.553,7.7571e-13
2.556,7.7527e-13
2.559,7.7593e-13
2.562,7.7538e-13
2.565,7.7593e-13
2.5679,7.7527e-13
2.5709,7.7527e-13
2.5739,7.756e-13
2.5769,7.7549e-13
2.5799,7.7571e-13
2.5828,7.756e-13
2.5858,7.7538e-13
2.5888,7.756e-13
2.5918,7.7538e-13
2.5948,7.7527e-13
2.5977,7.756e-13
2.6007,7.7494e-13
2.6037,7.756e-13
2.6067,7.7538e-13
2.6097,7.7538e-13
2.6126,7.756e-13
2.6156,7.7516e-13
2.6186,7.7538e-13
2.6216,7.7527e-13
2.6246,7.7538e-13
2.6275,7.7505e-13
2.6305,7.7505e-13
2.6335,7.7527e-13
2.6365,7.7482e-13
2.6395,7.7494e-13
2.6424,7.7494e-13
2.6454,7.7494e-13
2.6484,7.7494e-13
2.6514,7.7482e-13
2.6544,7.7494e-13
2.6574,7.7505e-13
2.6603,7.7482e-13
2.6633,7.7482e-13
2.6663,7.7494e-13
2.6693,7.7516e-13
2.6723,7.7494e-13
2.6752,7.7505e-13
2.6782,7.7482e-13
2.6812,7.7494e-13
2.6842,7.7482e-13
2.6872,7.7482e-13
2.6901,7.7449e-13
2.6931,7.746e-13
2.6961,7.746e-13
2.6991,7.7427e-13
2.7021,7.7449e-13
2.705,7.7416e-13
2.708,7.7471e-13
2.711,7.7416e-13
2.714,7.7449e-13
2.717,7.7482e-13
2.7199,7.7438e-13
2.7229,7.7416e-13
2.7259,7.7449e-13
2.7289,7.7427e-13
2.7319,7.7449e-13
2.7348,7.7427e-13
2.7378,7.7427e-13
2.7408,7.7438e-13
2.7438,7.7427e-13
2.7468,7.7427e-13
2.7497,7.746e-13
2.7527,7.7405e-13
2.7557,7.7405e-13
2.7587,7.7394e-13
2.7617,7.7416e-13
2.7647,7.7383e-13
2.7676,7.7371e-13
2.7706,7.7438e-13
2.7736,7.7405e-13
2.7766,7.7394e-13
2.7796,7.736e-13
2.7825,7.7349e-13
2.7855,7.7371e-13
2.7885,7.7371e-13
2.7915,7.7394e-13
2.7945,7.7416e-13
2.7974,7.736e-13
2.8004,7.7349e-13
2.8034,7.736e-13
2.8064,7.7349e-13
2.8094,7.7371e-13
2.8123,7.7371e-13
2.8153,7.7327e-13
2.8183,7.7327e-13
2.8213,7.736e-13
2.8243,7.7327e-13
2.8272,7.7305e-13
2.8302,7.7338e-13
2.8332,7.7316e-13
2.8362,7.7316e-13
2.8392,7.7294e-13
2.8421,7.7316e-13
2.8451,7.7305e-13
2.8481,7.7327e-13
2.8511,7.7321e-13
2.8541,7.7321e-13
2.8571,7.7272e-13
2.86,7.7283e-13
2.863,7.7283e-13
2.866,7.731e-13
2.869,7.7283e-13
2.872,7.7305e-13
2.8749,7.7277e-13
2.8779,7.7288e-13
2.8809,7.7288e-13
2.8839,7.7255e-13
2.8869,7.7283e-13
2.8898,7.7305e-13
2.8928,7.7305e-13
2.8958,7.7238e-13
2.8988,7.7255e-13
2.9018,7.7255e-13
2.9047,7.726e-13
2.9077,7.7188e-13
2.9107,7.7244e-13
2.9137,7.7249e-13
2.9167,7.7249e-13
2.9196,7.7244e-13
2.9226,7.7238e-13
2.9256,7.7249e-13
2.9286,7.7238e-13
2.9316,7.721e-13
2.9345,7.7222e-13
2.9375,7.7216e-13
2.9405,7.7194e-13
2.9435,7.7222e-13
2.9465,7.7172e-13
2.9494,7.7205e-13
2.9524,7.7177e-13
2.9554,7.7149e-13
2.9584,7.7172e-13
2.9614,7.7194e-13
2.9644,7.7144e-13
2.9673,7.7166e-13
2.9703,7.7183e-13
2.9733,7.7166e-13
2.9763,7.7144e-13
2.9793,7.7161e-13
2.9822,7.7138e-13
2.9852,7.7155e-13
2.9882,7.7177e-13
2.9912,7.7133e-13
2.9942,7.7161e-13
2.9971,7.7138e-13
3.0001,7.7172e-13
3.0031,7.7122e-13
3.0061,7.7133e-13
3.0091,7.7144e-13
3.012,7.7127e-13
3.015,7.7127e-13
3.018,7.7105e-13
3.021,7.7099e-13
3.024,7.7138e-13
3.0269,7.7077e-13
3.0299,7.7099e-13
3.0329,7.7077e-13
3.0359,7.7099e-13
3.0389,7.7061e-13
3.0418,7.7066e-13
3.0448,7.7061e-13
3.0478,7.7011e-13
3.0508,7.7038e-13
3.0538,7.7033e-13
3.0568,7.7083e-13
3.0597,7.7038e-13
3.0627,7.7038e-13
3.0657,7.7055e-13
3.0687,7.7033e-13
3.0717,7.7005e-13
3.0746,7.7044e-13
3.0776,7.7e-13
3.0806,7.7027e-13
3.0836,7.7016e-13
3.0866,7.6966e-13
3.0895,7.6988e-13
3.0925,7.6961e-13
3.0955,7.6933e-13
3.0985,7.6938e-13
3.1015,7.6961e-13
3.1044,7.6983e-13
3.1074,7.7e-13
3.1104,7.6977e-13
3.1134,7.6972e-13
3.1164,7.695e-13
3.1193,7.6983e-13
3.1223,7.6883e-13
3.1253,7.6961e-13
3.1283,7.695e-13
3.1313,7.6894e-13
3.1342,7.6916e-13
3.1372,7.6944e-13
3.1402,7.6877e-13
3.1432,7.6888e-13
3.1462,7.69e-13
3.1491,7.6894e-13
3.1521,7.6855e-13
3.1551,7.6844e-13
3.1581,7.6877e-13
3.1611,7.6883e-13
3.1641,7.6883e-13
3.167,7.685e-13
3.17,7.6839e-13
3.173,7.685e-13
3.176,7.6833e-13
3.179,7.6833e-13
3.1819,7.6822e-13
3.1849,7.6822e-13
3.1879,7.6811e-13
3.1909,7.6777e-13
3.1939,7.6805e-13
3.1968,7.6833e-13
3.1998,7.6761e-13
3.2028,7.6772e-13
3.2058,7.6766e-13
3.2088,7.6772e-13
3.2117,7.6789e-13
3.2147,7.68e-13
3.2177,7.6733e-13
3.2207,7.6772e-13
3.2237,7.675e-13
3.2266,7.6766e-13
3.2296,7.6711e-13
3.2326,7.675e-13
3.2356,7.6716e-13
3.2386,7.6705e-13
3.2415,7.6705e-13
3.2445,7.6694e-13
3.2475,7.6689e-13
3.2505,7.6722e-13
3.2535,7.6728e-13
3.2565,7.6711e-13
3.2594,7.6661e-13
3.2624,7.665e-13
3.2654,7.6633e-13
3.2684,7.665e-13
3.2714,7.6678e-13
3.2743,7.6678e-13
3.2773,7.6616e-13
3.2803,7.6678e-13
3.2833,7.6655e-13
3.2863,7.6594e-13
3.2892,7.6644e-13
3.2922,7.6567e-13
3.2952,7.6605e-13
3.2982,7.6572e-13
3.3012,7.6561e-13
3.3041,7.6589e-13
3.3071,7.6567e-13
3.3101,7.6578e-13
3.3131,7.6539e-13
3.3161,7.655e-13
3.319,7.6594e-13
3.322,7.6511e-13
3.325,7.6583e-13
3.328,7.6517e-13
3.331,7.6494e-13
3.3339,7.6483e-13
3.3369,7.6511e-13
3.3399,7.6483e-13
3.3429,7.645e-13
3.3459,7.6505e-13
3.3488,7.6461e-13
3.3518,7.6433e-13
3.3548,7.6494e-13
3.3578,7.6456e-13
3.3608,7.6433e-13
3.3638,7.6456e-13
3.3667,7.645e-13
3.3697,7.6422e-13
3.3727,7.64e-13
3.3757,7.6417e-13
3.3787,7.6389e-13
3.3816,7.6361e-13
3.3846,7.6372e-13
3.3876,7.635e-13
3.3906,7.6394e-13
3.3936,7.6433e-13
3.3965,7.6344e-13
3.3995,7.6322e-13
3.4025,7.6367e-13
3.4055,7.6344e-13
3.4085,7.63e-13
3.4114,7.6317e-13
3.4144,7.63e-13
3.4174,7.6317e-13
3.4204,7.6306e-13
3.4234,7.6283e-13
3.4263,7.6261e-13
3.4293,7.6283e-13
3.4323,7.6245e-13
3.4353,7.6289e-13
3.4383,7.6239e-13
3.4412,7.6217e-13
3.4442,7.6245e-13
3.4472,7.6206e-13
3.4502,7.625e-13
3.4532,7.6161e-13
3.4562,7.6195e-13
3.4591,7.6167e-13
3.4621,7.6161e-13
3.4651,7.6211e-13
3.4681,7.6161e-13
3.4711,7.6145e-13
3.474,7.615e-13
3.477,7.6139e-13
3.48,7.6156e-13
3.483,7.615e-13
3.486,7.6128e-13
3.4889,7.6161e-13
3.4919,7.6122e-13
3.4949,7.6089e-13
3.4979,7.6067e-13
3.5009,7.61e-13
3.5038,7.6117e-13
3.5068,7.6067e-13
3.5098,7.6061e-13
3.5128,7.6034e-13
3.5158,7.5995e-13
3.5187,7.6011e-13
3.5217,7.5956e-13
3.5247,7.6006e-13
3.5277,7.5995e-13
3.5307,7.6e-13
3.5336,7.595e-13
3.5366,7.5939e-13
3.5396,7.5945e-13
3.5426,7.5945e-13
3.5456,7.6017e-13
3.5485,7.5923e-13
3.5515,7.5878e-13
3.5545,7.5873e-13
3.5575,7.5867e-13
3.5605,7.58e-13
3.5635,7.5884e-13
3.5664,7.5806e-13
3.5694,7.5895e-13
3.5724,7.5828e-13
3.5754,7.5817e-13
3.5784,7.5828e-13
3.5813,7.5817e-13
3.5843,7.58e-13
3.5873,7.5806e-13
3.5903,7.5845e-13
3.5933,7.5812e-13
3.5962,7.5734e-13
3.5992,7.5762e-13
3.6022,7.5734e-13
3.6052,7.5745e-13
3.6082,7.5695e-13
3.6111,7.5701e-13
3.6141,7.5723e-13
3.6171,7.5678e-13
3.6201,7.5706e-13
3.6231,7.5706e-13
3.626,7.5673e-13
3.629,7.5623e-13
3.632,7.5656e-13
3.635,7.5662e-13
3.638,7.559e-13
3.6409,7.5645e-13
3.6439,7.5567e-13
3.6469,7.5634e-13
3.6499,7.5612e-13
3.6529,7.5567e-13
3.6559,7.554e-13
3.6588,7.5517e-13
3.6618,7.5562e-13
3.6648,7.5534e-13
3.6678,7.5562e-13
3.6708,7.5534e-13
3.6737,7.549e-13
3.6767,7.5451e-13
3.6797,7.5523e-13
3.6827,7.5523e-13
3.6857,7.5462e-13
3.6886,7.5528e-13
3.6916,7.5451e-13
3.6946,7.5395e-13
3.6976,7.5462e-13
3.7006,7.5384e-13
3.7035,7.5367e-13
3.7065,7.5362e-13
3.7095,7.5329e-13
3.7125,7.5373e-13
3.7155,7.5329e-13
3.7184,7.5351e-13
3.7214,7.5284e-13
3.7244,7.5323e-13
3.7274,7.5356e-13
3.7304,7.5284e-13
3.7333,7.5262e-13
3.7363,7.5301e-13
3.7393,7.529e-13
3.7423,7.529e-13
3.7453,7.5179e-13
3.7482,7.5256e-13
3.7512,7.5184e-13
3.7542,7.5134e-13
3.7572,7.5157e-13
3.7602,7.5195e-13
3.7632,7.5118e-13
3.7661,7.5107e-13
3.7691,7.514e-13
3.7721,7.5101e-13
3.7751,7.509e-13
3.7781,7.5107e-13
3.781,7.5068e-13
3.784,7.5051e-13
3.787,7.5018e-13
3.79,7.5007e-13
3.793,7.499e-13
3.7959,7.4962e-13
3.7989,7.494e-13
3.8019,7.4996e-13
3.8049,7.4979e-13
3.8079,7.4951e-13
3.8108,7.4923e-13
3.8138,7.4957e-13
3.8168,7.4929e-13
3.8198,7.4896e-13
3.8228,7.4846e-13
3.8257,7.489e-13
3.8287,7.4829e-13
3.8317,7.4868e-13
3.8347,7.4801e-13
3.8377,7.4823e-13
3.8406,7.4796e-13
3.8436,7.4779e-13
3.8466,7.4801e-13
3.8496,7.4796e-13
3.8526,7.4751e-13
3.8556,7.4768e-13
3.8585,7.469e-13
3.8615,7.469e-13
3.8645,7.469e-13
3.8675,7.4668e-13
3.8705,7.4668e-13
3.8734,7.4685e-13
3.8764,7.4685e-13
3.8794,7.4657e-13
3.8824,7.459e-13
3.8854,7.4662e-13
3.8883,7.459e-13
3.8913,7.4574e-13
3.8943,7.4579e-13
3.8973,7.4618e-13
3.9003,7.459e-13
3.9032,7.4513e-13
3.9062,7.4518e-13
3.9092,7.4502e-13
3.9122,7.4507e-13
3.9152,7.4463e-13
3.9181,7.4452e-13
3.9211,7.4452e-13
3.9241,7.4402e-13
3.9271,7.4457e-13
3.9301,7.444e-13
3.933,7.4402e-13
3.936,7.4302e-13
3.939,7.4324e-13
3.942,7.4302e-13
3.945,7.4313e-13
3.9479,7.4252e-13
3.9509,7.4285e-13
3.9539,7.4279e-13
3.9569,7.4218e-13
3.9599,7.4202e-13
3.9629,7.423e-13
3.9658,7.4152e-13
3.9688,7.418e-13
3.9718,7.4157e-13
3.9748,7.4124e-13
3.9778,7.4102e-13
3.9807,7.4113e-13
3.9837,7.4124e-13
3.9867,7.4041e-13
3.9897,7.4063e-13
3.9927,7.3991e-13
3.9956,7.4074e-13
3.9986,7.3985e-13
4.0016,7.4002e-13
4.0046,7.4002e-13
4.0076,7.3963e-13
4.0105,7.3958e-13
4.0135,7.3985e-13
4.0165,7.3958e-13
4.0195,7.3935e-13
4.0225,7.3869e-13
4.0254,7.3902e-13
4.0284,7.3852e-13
4.0314,7.3797e-13
4.0344,7.3863e-13
4.0374,7.3813e-13
4.0403,7.373e-13
4.0433,7.3785e-13
4.0463,7.3819e-13
4.0493,7.3733e-13
4.0523,7.3686e-13
4.0553,7.3741e-13
4.0582,7.3699e-13
4.0612,7.3719e-13
4.0642,7.3683e-13
4.0672,7.3624e-13
4.0702,7.3599e-13
4.0731,7.3597e-13
4.0761,7.3661e-13
4.0791,7.3586e-13
4.0821,7.3538e-13
4.0851,7.3497e-13
4.088,7.3511e-13
4.091,7.3491e-13
4.094,7.3469e-13
4.097,7.348e-13
4.1,7.3438e-13
4.1029,7.3455e-13
4.1059,7.3347e-13
4.1089,7.3383e-13
4.1119,7.3314e-13
4.1149,7.3283e-13
4.1178,7.3361e-13
4.1208,7.3355e-13
4.1238,7.3336e-13
4.1268,7.335e-13
4.1298,7.3302e-13
4.1327,7.325e-13
4.1357,7.3133e-13
4.1387,7.3277e-13
4.1417,7.328e-13
4.1447,7.3155e-13
4.1476,7.3078e-13
4.1506,7.313e-13
4.1536,7.3108e-13
4.1566,7.3117e-13
4.1596,7.303e-13
4.1626,7.2989e-13
4.1655,7.2992e-13
4.1685,7.2878e-13
4.1715,7.3111e-13
4.1745,7.3036e-13
4.1775,7.3028e-13
4.1804,7.2828e-13
4.1834,7.2911e-13
4.1864,7.2836e-13
4.1894,7.29e-13
4.1924,7.285e-13
4.1953,7.2789e-13
4.1983,7.2767e-13
4.2013,7.28e-13
4.2043,7.2739e-13
4.2073,7.2753e-13
4.2102,7.2686e-13
4.2132,7.2628e-13
4.2162,7.2634e-13
4.2192,7.2659e-13
4.2222,7.26e-13
4.2251,7.2589e-13
4.2281,7.2578e-13
4.2311,7.2528e-13
4.2341,7.2584e-13
4.2371,7.262e-13
4.24,7.2511e-13
4.243,7.252e-13
4.246,7.2564e-13
4.249,7.2425e-13
4.252,7.2439e-13
4.255,7.2425e-13
4.2579,7.2378e-13
4.2609,7.2273e-13
4.2639,7.235e-13
4.2669,7.2198e-13
4.2699,7.2287e-13
4.2728,7.2262e-13
4.2758,7.2289e-13
4.2788,7.214e-13
4.2818,7.2234e-13
4.2848,7.2128e-13
4.2877,7.2031e-13
4.2907,7.2106e-13
4.2937,7.202e-13
4.2967,7.1995e-13
4.2997,7.2115e-13
4.3026,7.2009e-13
4.3056,7.2042e-13
4.3086,7.1906e-13
4.3116,7.2004e-13
4.3146,7.1934e-13
4.3175,7.1923e-13
4.3205,7.189e-13
4.3235,7.1823e-13
4.3265,7.1818e-13
4.3295,7.1909e-13
4.3324,7.1687e-13
4.3354,7.1834e-13
4.3384,7.1743e-13
4.3414,7.1695e-13
4.3444,7.1806e-13
4.3473,7.1709e-13
4.3503,7.1684e-13
4.3533,7.1715e-13
4.3563,7.1568e-13
4.3593,7.1598e-13
4.3623,7.1582e-13
4.3652,7.1532e-13
4.3682,7.1465e-13
4.3712,7.1601e-13
4.3742,7.1446e-13
4.3772,7.144e-13
4.3801,7.1493e-13
4.3831,7.141e-13
4.3861,7.1401e-13
4.3891,7.1285e-13
4.3921,7.1307e-13
4.395,7.124e-13
4.398,7.1335e-13
4.401,7.1348e-13
4.404,7.1268e-13
4.407,7.126e-13
4.4099,7.1135e-13
4.4129,7.1215e-13
4.4159,7.1138e-13
4.4189,7.1085e-13
4.4219,7.1088e-13
4.4248,7.1071e-13
4.4278,7.1079e-13
4.4308,7.1035e-13
4.4338,7.0879e-13
4.4368,7.1035e-13
4.4397,7.1015e-13
4.4427,7.0943e-13
4.4457,7.0857e-13
4.4487,7.0824e-13
4.4517,7.0849e-13
4.4547,7.0799e-13
4.4576,7.0841e-13
4.4606,7.0771e-13
4.4636,7.0643e-13
4.4666,7.0707e-13
4.4696,7.0619e-13
4.4725,7.0591e-13
4.4755,7.0619e-13
4.4785,7.058e-13
4.4815,7.0571e-13
4.4845,7.0588e-13
4.4874,7.0521e-13
4.4904,7.0449e-13
4.4934,7.0413e-13
4.4964,7.0363e-13
4.4994,7.0355e-13
4.5023,7.0371e-13
4.5053,7.0394e-13
4.5083,7.033e-13
4.5113,7.0199e-13
4.5143,7.0294e-13
4.5172,7.0149e-13
4.5202,7.0149e-13
4.5232,7.0149e-13
4.5262,7.0119e-13
4.5292,7.0152e-13
4.5321,7.0119e-13
4.5351,7.0058e-13
4.5381,7.008e-13
4.5411,6.9988e-13
4.5441,6.998e-13
4.547,6.9914e-13
4.55,6.9891e-13
4.553,6.9797e-13
4.556,6.9769e-13
4.559,6.9866e-13
4.562,6.9769e-13
4.5649,6.9769e-13
4.5679,6.9655e-13
4.5709,6.9716e-13
4.5739,6.9605e-13
4.5769,6.9614e-13
4.5798,6.95e-13
4.5828,6.9561e-13
4.5858,6.9525e-13
4.5888,6.9583e-13
4.5918,6.9494e-13
4.5947,6.9403e-13
4.5977,6.9456e-13
4.6007,6.9372e-13
4.6037,6.9297e-13
4.6067,6.9394e-13
4.6096,6.9325e-13
4.6126,6.9142e-13
4.6156,6.9172e-13
4.6186,6.9189e-13
4.6216,6.9153e-13
4.6245,6.9003e-13
4.6275,6.91e-13
4.6305,6.9081e-13
4.6335,6.9081e-13
4.6365,6.8981e-13
4.6394,6.8964e-13
4.6424,6.8931e-13
4.6454,6.8925e-13
4.6484,6.8928e-13
4.6514,6.892e-13
4.6544,6.8712e-13
4.6573,6.8823e-13
4.6603,6.8773e-13
4.6633,6.8778e-13
4.6663,6.8678e-13
4.6693,6.8726e-13
4.6722,6.8581e-13
4.6752,6.8645e-13
4.6782,6.8601e-13
4.6812,6.8617e-13
4.6842,6.8578e-13
4.6871,6.8473e-13
4.6901,6.8417e-13
4.6931,6.8401e-13
4.6961,6.8262e-13
4.6991,6.8343e-13
4.702,6.8351e-13
4.705,6.8254e-13
4.708,6.8184e-13
4.711,6.8157e-13
4.714,6.8118e-13
4.7169,6.8048e-13
4.7199,6.8145e-13
4.7229,6.7996e-13
4.7259,6.7943e-13
4.7289,6.8059e-13
4.7318,6.7862e-13
4.7348,6.7829e-13
4.7378,6.7846e-13
4.7408,6.7862e-13
4.7438,6.781e-13
4.7467,6.7824e-13
4.7497,6.781e-13
4.7527,6.7654e-13
4.7557,6.7668e-13
4.7587,6.7663e-13
4.7617,6.7493e-13
4.7646,6.759e-13
4.7676,6.7457e-13
4.7706,6.7632e-13
4.7736,6.7438e-13
4.7766,6.7366e-13
4.7795,6.7485e-13
4.7825,6.728e-13
4.7855,6.7349e-13
4.7885,6.7252e-13
4.7915,6.7105e-13
4.7944,6.7227e-13
4.7974,6.7216e-13
4.8004,6.708e-13
4.8034,6.7049e-13
4.8064,6.7049e-13
4.8093,6.6991e-13
4.8123,6.701e-13
4.8153,6.7016e-13
4.8183,6.6977e-13
4.8213,6.6724e-13
4.8242,6.6733e-13
4.8272,6.6844e-13
4.8302,6.688e-13
4.8332,6.6558e-13
4.8362,6.6611e-13
4.8391,6.6633e-13
4.8421,6.648e-13
4.8451,6.6519e-13
4.8481,6.6477e-13
4.8511,6.6472e-13
4.8541,6.6544e-13
4.857,6.6208e-13
4.86,6.6314e-13
4.863,6.6405e-13
4.866,6.6064e-13
4.869,6.6125e-13
4.8719,6.6167e-13
4.8749,6.6228e-13
4.8779,6.6036e-13
4.8809,6.5961e-13
4.8839,6.6019e-13
4.8868,6.59e-13
4.8898,6.5917e-13
4.8928,6.575e-13
4.8958,6.5803e-13
4.8988,6.5875e-13
4.9017,6.6044e-13
4.9047,6.575e-13
4.9077,6.5895e-13
4.9107,6.5722e-13
4.9137,6.5473e-13
4.9166,6.5609e-13
4.9196,6.5303e-13
4.9226,6.5417e-13
4.9256,6.5545e-13
4.9286,6.5262e-13
4.9315,6.5314e-13
4.9345,6.5273e-13
4.9375,6.5295e-13
4.9405,6.5156e-13
4.9435,6.5106e-13
4.9464,6.5023e-13
4.9494,6.5131e-13
4.9524,6.4929e-13
4.9554,6.4801e-13
4.9584,6.4873e-13
4.9614,6.4984e-13
4.9643,6.5073e-13
4.9673,6.4893e-13
4.9703,6.4909e-13
4.9733,6.479e-13
4.9763,6.4793e-13
4.9792,6.487e-13
4.9822,6.4559e-13
4.9852,6.4804e-13
4.9882,6.4432e-13
4.9912,6.4446e-13
4.9941,6.436e-13
4.9971,6.4285e-13
5.0001,6.4246e-13
5.0031,6.4213e-13
5.0061,6.4251e-13
5.009,6.4165e-13
5.012,6.4063e-13
5.015,6.4085e-13
5.018,6.3896e-13
5.021,6.4121e-13
5.0239,6.406e-13
5.0269,6.4093e-13
5.0299,6.3877e-13
5.0329,6.3913e-13
5.0359,6.3882e-13
5.0388,6.3599e-13
5.0418,6.3746e-13
5.0448,6.3516e-13
5.0478,6.3607e-13
5.0508,6.3582e-13
5.0538,6.3666e-13
5.0567,6.3421e-13
5.0597,6.3363e-13
5.0627,6.3383e-13
5.0657,6.3419e-13
5.0687,6.3177e-13
5.0716,6.3316e-13
5.0746,6.2989e-13
5.0776,6.3255e-13
5.0806,6.3258e-13
5.0836,6.3138e-13
5.0865,6.3005e-13
5.0895,6.2994e-13
5.0925,6.2947e-13
5.0955,6.2905e-13
5.0985,6.2869e-13
5.1014,6.2797e-13
5.1044,6.2661e-13
5.1074,6.2711e-13
5.1104,6.2658e-13
5.1134,6.2428e-13
5.1163,6.2347e-13
5.1193,6.2358e-13
5.1223,6.232e-13
5.1253,6.2533e-13
5.1283,6.1984e-13
5.1312,6.2372e-13
5.1342,6.2195e-13
5.1372,6.2031e-13
5.1402,6.1928e-13
5.1432,6.197e-13
5.1461,6.2012e-13
5.1491,6.2025e-13
5.1521,6.1845e-13
5.1551,6.2103e-13
5.1581,6.1676e-13
5.1611,6.1634e-13
5.164,6.1642e-13
5.167,6.1634e-13
5.17,6.152e-13
5.173,6.1537e-13
5.176,6.1476e-13
5.1789,6.1556e-13
5.1819,6.1298e-13
5.1849,6.1409e-13
5.1879,6.1195e-13
5.1909,6.1273e-13
5.1938,6.1251e-13
5.1968,6.0915e-13
5.1998,6.0879e-13
5.2028,6.0973e-13
5.2058,6.0973e-13
5.2087,6.0843e-13
5.2117,6.0707e-13
5.2147,6.0638e-13
5.2177,6.0849e-13
5.2207,6.064e-13
5.2236,6.0574e-13
5.2266,6.0724e-13
5.2296,6.0427e-13
5.2326,6.0513e-13
5.2356,6.0496e-13
5.2385,6.0488e-13
5.2415,6.0213e-13
5.2445,6.0199e-13
5.2475,6.0119e-13
5.2505,6.0149e-13
5.2535,5.9952e-13
5.2564,6.006e-13
5.2594,6.0113e-13
5.2624,5.9824e-13
5.2654,5.9791e-13
5.2684,5.9702e-13
5.2713,5.9686e-13
5.2743,5.9752e-13
5.2773,5.9452e-13
5.2803,5.9561e-13
5.2833,5.9461e-13
5.2862,5.9394e-13
5.2892,5.9214e-13
5.2922,5.9472e-13
5.2952,5.9439e-13
5.2982,5.9239e-13
5.3011,5.9214e-13
5.3041,5.9086e-13
5.3071,5.9008e-13
5.3101,5.9058e-13
5.3131,5.8897e-13
5.316,5.887e-13
5.319,5.8809e-13
5.322,5.8822e-13
5.325,5.8667e-13
5.328,5.8575e-13
5.3309,5.8545e-13
5.3339,5.8498e-13
5.3369,5.8267e-13
5.3399,5.8284e-13
5.3429,5.8312e-13
5.3458,5.8131e-13
5.3488,5.8215e-13
5.3518,5.8287e-13
5.3548,5.8001e-13
5.3578,5.7931e-13
5.3608,5.8031e-13
5.3637,5.7915e-13
5.3667,5.7912e-13
5.3697,5.7698e-13
5.3727,5.7851e-13
5.3757,5.7784e-13
5.3786,5.7485e-13
5.3816,5.774e-13
5.3846,5.7485e-13
5.3876,5.7351e-13
5.3906,5.7213e-13
5.3935,5.6929e-13
5.3965,5.7296e-13
5.3995,5.7288e-13
5.4025,5.7078e-13
5.4055,5.705e-13
5.4084,5.6814e-13
5.4114,5.6946e-13
5.4144,5.6904e-13
5.4174,5.6823e-13
5.4204,5.6534e-13
5.4233,5.6674e-13
5.4263,5.6585e-13
5.4293,5.6594e-13
5.4323,5.6544e-13
5.4353,5.6517e-13
5.4382,5.6487e-13
5.4412,5.6331e-13
5.4442,5.6197e-13
5.4472,5.6209e-13
5.4502,5.5947e-13
5.4532,5.6079e-13
5.4561,5.5669e-13
5.4591,5.6005e-13
5.4621,5.5995e-13
5.4651,5.5821e-13
5.4681,5.5797e-13
5.471,5.536e-13
5.474,5.5385e-13
5.477,5.5313e-13
5.48,5.5127e-13
5.483,5.5132e-13
5.4859,5.5012e-13
5.4889,5.5286e-13
5.4919,5.5025e-13
5.4949,5.512e-13
5.4979,5.4919e-13
5.5008,5.4858e-13
5.5038,5.4537e-13
5.5068,5.4663e-13
5.5098,5.4523e-13
5.5128,5.4348e-13
5.5157,5.4463e-13
5.5187,5.4222e-13
5.5217,5.429e-13
5.5247,5.4408e-13
5.5277,5.4053e-13
5.5306,5.4207e-13
5.5336,5.3911e-13
5.5366,5.3985e-13
5.5396,5.3971e-13
5.5426,5.3628e-13
5.5455,5.3534e-13
5.5485,5.3711e-13
5.5515,5.347e-13
5.5545,5.3664e-13
5.5575,5.3409e-13
5.5605,5.3188e-13
5.5634,5.3303e-13
5.5664,5.3361e-13
5.5694,5.3314e-13
5.5724,5.3119e-13
5.5754,5.3063e-13
5.5783,5.3098e-13
5.5813,5.2992e-13
5.5843,5.2623e-13
5.5873,5.2758e-13
5.5903,5.2779e-13
5.5932,5.2545e-13
5.5962,5.24e-13
5.5992,5.2515e-13
5.6022,5.2298e-13
5.6052,5.2391e-13
5.6081,5.2265e-13
5.6111,5.2119e-13
5.6141,5.2017e-13
5.6171,5.2067e-13
5.6201,5.1896e-13
5.623,5.2107e-13
5.626,5.1717e-13
5.629,5.1757e-13
5.632,5.1623e-13
5.635,5.1574e-13
5.6379,5.1305e-13
5.6409,5.1337e-13
5.6439,5.1432e-13
5.6469,5.0986e-13
5.6499,5.099e-13
5.6529,5.1177e-13
5.6558,5.0727e-13
5.6588,5.1147e-13
5.6618,5.079e-13
5.6648,5.059e-13
5.6678,5.0426e-13
5.6707,5.0317e-13
5.6737,5.0419e-13
5.6767,5.0349e-13
5.6797,5.0676e-13
5.6827,5.0218e-13
5.6856,5.0379e-13
5.6886,5.0047e-13
5.6916,5.0181e-13
5.6946,4.9884e-13
5.6976,4.962e-13
5.7005,4.9824e-13
5.7035,4.9485e-13
5.7065,4.9463e-13
5.7095,4.9535e-13
5.7125,4.9478e-13
5.7154,4.9291e-13
5.7184,4.9463e-13
5.7214,4.9243e-13
5.7244,4.907e-13
5.7274,4.9044e-13
5.7303,4.8801e-13
5.7333,4.886e-13
5.7363,4.8783e-13
5.7393,4.8787e-13
5.7423,4.8736e-13
5.7452,4.8549e-13
5.7482,4.8291e-13
5.7512,4.8095e-13
5.7542,4.818e-13
5.7572,4.7881e-13
5.7602,4.798e-13
5.7631,4.8075e-13
5.7661,4.8168e-13
5.7691,4.783e-13
5.7721,4.7845e-13
5.7751,4.7792e-13
5.778,4.7516e-13
5.781,4.776e-13
5.784,4.7257e-13
5.787,4.7276e-13
5.79,4.7098e-13
5.7929,4.7237e-13
5.7959,4.7067e-13
5.7989,4.6922e-13
5.8019,4.6782e-13
5.8049,4.6883e-13
5.8078,4.6789e-13
5.8108,4.6549e-13
5.8138,4.6625e-13
5.8168,4.6284e-13
5.8198,4.6345e-13
5.8227,4.6209e-13
5.8257,4.6008e-13
5.8287,4.5967e-13
5.8317,4.6201e-13
5.8347,4.584e-13
5.8376,4.5504e-13
5.8406,4.5892e-13
5.8436,4.5822e-13
5.8466,4.562e-13
5.8496,4.5476e-13
5.8526,4.5405e-13
5.8555,4.5648e-13
5.8585,4.5405e-13
5.8615,4.4999e-13
5.8645,4.5249e-13
5.8675,4.4668e-13
5.8704,4.4867e-13
5.8734,4.4774e-13
5.8764,4.4866e-13
5.8794,4.4474e-13
5.8824,4.4038e-13
5.8853,4.4216e-13
5.8883,4.4258e-13
5.8913,4.389e-13
5.8943,4.3984e-13
5.8973,4.3945e-13
5.9002,4.4156e-13
5.9032,4.3608e-13
5.9062,4.3308e-13
5.9092,4.3411e-13
5.9122,4.3429e-13
5.9151,4.3131e-13
5.9181,4.3097e-13
5.9211,4.2959e-13
5.9241,4.2774e-13
5.9271,4.2591e-13
5.93,4.2673e-13
5.933,4.2907e-13
5.936,4.2739e-13
5.939,4.2651e-13
5.942,4.2437e-13
5.9449,4.2123e-13
5.9479,4.2097e-13
5.9509,4.1948e-13
5.9539,4.1922e-13
5.9569,4.1971e-13
5.9599,4.2145e-13
5.9628,4.1571e-13
5.9658,4.1674e-13
5.9688,4.1457e-13
5.9718,4.1557e-13
5.9748,4.1038e-13
5.9777,4.0803e-13
5.9807,4.1202e-13
5.9837,4.0931e-13
5.9867,4.0934e-13
5.9897,4.0618e-13
5.9926,4.0679e-13
5.9956,4.0595e-13
5.9986,4.0805e-13
6.0016,4e-13
6.0046,4.0364e-13
6.0075,3.9997e-13
6.0105,4.0136e-13
6.0135,4.0046e-13
6.0165,3.9715e-13
6.0195,3.9668e-13
6.0224,3.9566e-13
6.0254,3.9356e-13
6.0284,3.9763e-13
6.0314,3.8902e-13
6.0344,3.9123e-13
6.0373,3.8949e-13
6.0403,3.9348e-13
6.0433,3.9259e-13
6.0463,3.889e-13
6.0493,3.8598e-13
6.0523,3.8224e-13
6.0552,3.8393e-13
6.0582,3.8025e-13
6.0612,3.8147e-13
6.0642,3.8211e-13
6.0672,3.7888e-13
6.0701,3.7978e-13
6.0731,3.7741e-13
6.0761,3.7467e-13
6.0791,3.7606e-13
6.0821,3.7456e-13
6.085,3.7259e-13
6.088,3.7181e-13
6.091,3.7259e-13
6.094,3.7194e-13
6.097,3.6821e-13
6.0999,3.6665e-13
6.1029,3.6567e-13
6.1059,3.6456e-13
6.1089,3.6576e-13
6.1119,3.6464e-13
6.1148,3.5993e-13
6.1178,3.6106e-13
6.1208,3.6036e-13
6.1238,3.6288e-13
6.1268,3.5506e-13
6.1297,3.5727e-13
6.1327,3.5508e-13
6.1357,3.5175e-13
6.1387,3.4985e-13
6.1417,3.5281e-13
6.1446,3.4946e-13
6.1476,3.4873e-13
6.1506,3.493e-13
6.1536,3.4803e-13
6.1566,3.4861e-13
6.1596,3.4664e-13
6.1625,3.4316e-13
6.1655,3.4463e-13
6.1685,3.3985e-13
6.1715,3.4008e-13
6.1745,3.3752e-13
6.1774,3.3688e-13
6.1804,3.368e-13
6.1834,3.3691e-13
6.1864,3.3443e-13
6.1894,3.3339e-13
6.1923,3.3379e-13
6.1953,3.3307e-13
6.1983,3.2714e-13
6.2013,3.3322e-13
6.2043,3.262e-13
6.2072,3.2603e-13
6.2102,3.2199e-13
6.2132,3.2262e-13
6.2162,3.2088e-13
6.2192,3.2567e-13
6.2221,3.2438e-13
6.2251,3.1523e-13
6.2281,3.1736e-13
6.2311,3.175e-13
6.2341,3.129e-13
6.237,3.1412e-13
6.24,3.102e-13
6.243,3.1407e-13
6.246,3.1172e-13
6.249,3.0757e-13
6.252,3.1157e-13
6.2549,3.0803e-13
6.2579,3.043e-13
6.2609,3.0198e-13
6.2639,3.0695e-13
6.2669,3.0155e-13
6.2698,2.9876e-13
6.2728,2.9658e-13
6.2758,2.9513e-13
6.2788,2.95e-13
6.2818,2.9733e-13
6.2847,2.9532e-13
6.2877,2.9286e-13
6.2907,2.877e-13
6.2937,2.9129e-13
6.2967,2.8708e-13
6.2996,2.872e-13
6.3026,2.8379e-13
6.3056,2.839e-13
6.3086,2.8308e-13
6.3116,2.8322e-13
6.3145,2.8082e-13
6.3175,2.789e-13
6.3205,2.7735e-13
6.3235,2.7604e-13
6.3265,2.7425e-13
6.3294,2.7618e-13
6.3324,2.7697e-13
6.3354,2.7611e-13
6.3384,2.6848e-13
6.3414,2.7021e-13
6.3443,2.6772e-13
6.3473,2.6364e-13
6.3503,2.6518e-13
6.3533,2.6187e-13
6.3563,2.5788e-13
6.3593,2.585e-13
6.3622,2.5412e-13
6.3652,2.512e-13
6.3682,2.5541e-13
6.3712,2.5463e-13
6.3742,2.5366e-13
6.3771,2.4857e-13
6.3801,2.5274e-13
6.3831,2.477e-13
6.3861,2.4664e-13
6.3891,2.4369e-13
6.392,2.4405e-13
6.395,2.4769e-13
6.398,2.4818e-13
6.401,2.4303e-13
6.404,2.4193e-13
6.4069,2.3624e-13
6.4099,2.3767e-13
6.4129,2.3524e-13
6.4159,2.3236e-13
6.4189,2.2932e-13
6.4218,2.2704e-13
6.4248,2.2454e-13
6.4278,2.2649e-13
6.4308,2.2678e-13
6.4338,2.2682e-13
6.4367,2.2186e-13
6.4397,2.2042e-13
6.4427,2.1956e-13
6.4457,2.1948e-13
6.4487,2.1476e-13
6.4517,2.1461e-13
6.4546,2.1355e-13
6.4576,2.1548e-13
6.4606,2.1362e-13
6.4636,2.0536e-13
6.4666,2.0785e-13
6.4695,2.099e-13
6.4725,2.0586e-13
6.4755,2.0431e-13
6.4785,2.0299e-13
6.4815,2.0021e-13
6.4844,1.9681e-13
6.4874,1.9436e-13
6.4904,2.0418e-13
6.4934,1.9824e-13
6.4964,1.9988e-13
6.4993,1.9533e-13
6.5023,1.9154e-13
6.5053,1.8903e-13
6.5083,1.8494e-13
6.5113,1.8652e-13
6.5142,1.8474e-13
6.5172,1.8321e-13
6.5202,1.8063e-13
6.5232,1.846e-13
6.5262,1.8074e-13
6.5291,1.8197e-13
6.5321,1.7941e-13
6.5351,1.7067e-13
6.5381,1.6848e-13
6.5411,1.7125e-13
6.544,1.7628e-13
6.547,1.6689e-13
6.55,1.7278e-13
6.553,1.6467e-13
6.556,1.6084e-13
6.559,1.6562e-13
6.5619,1.584e-13
6.5649,1.6126e-13
6.5679,1.579e-13
6.5709,1.5135e-13
6.5739,1.5565e-13
6.5768,1.4971e-13
6.5798,1.4805e-13
6.5828,1.4835e-13
6.5858,1.4494e-13
6.5888,1.4402e-13
6.5917,1.45e-13
6.5947,1.3892e-13
6.5977,1.4536e-13
6.6007,1.4266e-13
6.6037,1.34e-13
6.6066,1.3645e-13
6.6096,1.3545e-13
6.6126,1.3478e-13
6.6156,1.3795e-13
6.6186,1.342e-13
6.6215,1.2645e-13
6.6245,1.3056e-13
6.6275,1.1793e-13
6.6305,1.2487e-13
6.6335,1.2843e-13
6.6364,1.1929e-13
6.6394,1.1896e-13
6.6424,1.2199e-13
6.6454,1.1571e-13
6.6484,1.1233e-13
6.6514,1.0975e-13
6.6543,1.1632e-13
6.6573,1.0777e-13
6.6603,1.0583e-13
6.6633,1.0958e-13
6.6663,9.4535e-14
6.6692,9.9615e-14
6.6722,1.0211e-13
6.6752,9.9809e-14
6.6782,9.5812e-14
6.6812,9.6811e-14
6.6841,9.1899e-14
6.6871,8.99e-14
6.6901,9.1649e-14
6.6931,8.7791e-14
6.6961,8.718e-14
6.699,8.1574e-14
6.702,8.4571e-14
6.705,8.3267e-14
6.708,7.8743e-14
6.711,7.8548e-14
6.7139,7.8798e-14
6.7169,7.3302e-14
6.7199,7.2109e-14
6.7229,7.1915e-14
6.7259,6.331e-14
6.7288,6.5614e-14
6.7318,6.1978e-14
6.7348,5.8814e-14
6.7378,6.5531e-14
6.7408,5.0321e-14
6.7437,5.7399e-14
6.7467,5.3596e-14
6.7497,5.1958e-14
6.7527,5.2319e-14
6.7557,5.2042e-14
6.7587,4.9405e-14
6.7616,4.3826e-14
6.7646,4.6574e-14
6.7676,4.2105e-14
6.7706,3.5916e-14
6.7736,4.0551e-14
6.7765,3.7997e-14
6.7795,3.2863e-14
6.7825,3.3251e-14
6.7855,3.1308e-14
6.7885,2.7034e-14
6.7914,2.5729e-14
6.7944,2.3592e-14
6.7974,2.82e-14
6.8004,1.7653e-14
6.8034,2.201e-14
6.8063,2.5424e-14
6.8093,2.6007e-14
6.8123,1.6959e-14
6.8153,7.7438e-15
6.8183,1.5377e-14
6.8212,6.356e-15
6.8242,1.1796e-14
6.8272,7.9103e-15
6.8302,7.2164e-15
6.8332,0
6.8361,2.8866e-15
6.8391,6.1062e-15
6.8421,1.4988e-15
6.8451,5.3291e-15
6.8481,6.8556e-15
6.8511,1.1074e-14
6.854,1.6487e-14
6.857,8.5765e-15
6.86,1.6959e-14
6.863,2.4009e-14
6.866,2.3676e-14
6.8689,1.5987e-14
6.8719,2.4869e-14
6.8749,2.6701e-14
6.8779,2.6645e-14
6.8809,3.092e-14
6.8838,4.1245e-14
6.8868,3.5666e-14
6.8898,3.0614e-14
6.8928,4.2077e-14
6.8958,4.0551e-14
6.8987,3.389e-14
6.9017,4.7712e-14
6.9047,4.3215e-14
6.9077,4.2438e-14
6.9107,4.1606e-14
6.9136,5.0376e-14
6.9166,5.1237e-14
6.9196,5.9008e-14
6.9226,5.0987e-14
6.9256,5.3402e-14
6.9285,6.1201e-14
6.9315,6.5309e-14
6.9345,6.7529e-14
6.9375,6.7668e-14
6.9405,6.5142e-14
6.9434,7.4662e-14
6.9464,7.3441e-14
6.9494,7.3247e-14
6.9524,7.8271e-14
6.9554,8.1324e-14
6.9584,8.2656e-14
6.9613,8.3655e-14
6.9643,8.4238e-14
6.9673,8.5459e-14
6.9703,8.8957e-14
6.9733,8.9567e-14
6.9762,1.0142e-13
6.9792,9.4452e-14
6.9822,9.4424e-14
6.9852,9.9865e-14
6.9882,1.0819e-13
6.9911,1.0952e-13
6.9941,1.0658e-13
6.9971,1.0991e-13
7.0001,1.1427e-13
7.0031,1.1735e-13
7.006,1.131e-13
7.009,1.2498e-13
7.012,1.2751e-13
7.015,1.2279e-13
7.018,1.2601e-13
7.0209,1.347e-13
7.0239,1.3123e-13
7.0269,1.292e-13
7.0299,1.2579e-13
7.0329,1.3897e-13
7.0358,1.4225e-13
7.0388,1.4586e-13
7.0418,1.486e-13
7.0448,1.4977e-13
7.0478,1.493e-13
7.0508,1.4458e-13
7.0537,1.6065e-13
7.0567,1.526e-13
7.0597,1.5543e-13
7.0627,1.5718e-13
7.0657,1.5984e-13
7.0686,1.6609e-13
7.0716,1.6573e-13
7.0746,1.6309e-13
7.0776,1.687e-13
7.0806,1.7025e-13
7.0835,1.7042e-13
7.0865,1.7938e-13
7.0895,1.7761e-13
7.0925,1.8344e-13
7.0955,1.8527e-13
7.0984,1.9454e-13
7.1014,1.9038e-13
7.1044,1.8829e-13
7.1074,1.9301e-13
7.1104,1.9437e-13
7.1133,1.9515e-13
7.1163,1.994e-13
7.1193,2.0467e-13
7.1223,2.0225e-13
7.1253,2.0581e-13
7.1282,2.1327e-13
7.1312,2.1039e-13
7.1342,2.1788e-13
7.1372,2.1635e-13
7.1402,2.1505e-13
7.1431,2.2327e-13
7.1461,2.1899e-13
7.1491,2.2263e-13
7.1521,2.3218e-13
7.1551,2.2751e-13
7.1581,2.4142e-13
7.161,2.3678e-13
7.164,2.4303e-13
7.167,2.4661e-13
7.17,2.445e-13
7.173,2.4727e-13
7.1759,2.3909e-13
7.1789,2.4486e-13
7.1819,2.4949e-13
7.1849,2.4949e-13
7.1879,2.6429e-13
7.1908,2.6223e-13
7.1938,2.6121e-13
7.1968,2.6865e-13
7.1998,2.6754e-13
7.2028,2.7187e-13
7.2057,2.6562e-13
7.2087,2.6573e-13
7.2117,2.7126e-13
7.2147,2.8313e-13
7.2177,2.8161e-13
7.2206,2.8536e-13
7.2236,2.7334e-13
7.2266,2.9954e-13
7.2296,2.9038e-13
7.2326,2.9879e-13
7.2355,2.9865e-13
7.2385,3.0578e-13
7.2415,3.0906e-13
7.2445,3.1494e-13
7.2475,3.1802e-13
7.2505,3.1269e-13
7.2534,3.0881e-13
7.2564,3.2713e-13
7.2594,3.2355e-13
7.2624,3.3165e-13
7.2654,3.2971e-13
7.2683,3.2435e-13
7.2713,3.2635e-13
7.2743,3.3631e-13
7.2773,3.3556e-13
7.2803,3.357e-13
7.2832,3.4184e-13
7.2862,3.4481e-13
7.2892,3.4422e-13
7.2922,3.53e-13
7.2952,3.5405e-13
7.2981,3.5111e-13
7.3011,3.5258e-13
7.3041,3.6168e-13
7.3071,3.6357e-13
7.3101,3.5555e-13
7.313,3.6249e-13
7.316,3.6993e-13
7.319,3.7739e-13
7.322,3.8469e-13
7.325,3.737e-13
7.3279,3.7512e-13
7.3309,3.8522e-13
7.3339,3.9757e-13
7.3369,3.782e-13
7.3399,3.8383e-13
7.3428,3.8447e-13
7.3458,3.9921e-13
7.3488,4.0126e-13
7.3518,3.9926e-13
7.3548,4.0742e-13
7.3578,4.0881e-13
7.3607,4.0642e-13
7.3637,4.1431e-13
7.3667,4.2161e-13
7.3697,4.1261e-13
7.3727,4.1742e-13
7.3756,4.2322e-13
7.3786,4.286e-13
7.3816,4.2871e-13
7.3846,4.3091e-13
7.3876,4.3371e-13
7.3905,4.3551e-13
7.3935,4.3418e-13
7.3965,4.4983e-13
7.3995,4.4667e-13
7.4025,4.3712e-13
7.4054,4.5242e-13
7.4084,4.5941e-13
7.4114,4.5192e-13
7.4144,4.5747e-13
7.4174,4.5827e-13
7.4203,4.7196e-13
7.4233,4.5702e-13
7.4263,4.7085e-13
7.4293,4.7953e-13
7.4323,4.6574e-13
7.4352,4.6915e-13
7.4382,4.7631e-13
7.4412,4.9225e-13
7.4442,4.8475e-13
7.4472,4.9205e-13
7.4502,4.9172e-13
7.4531,4.8858e-13
7.4561,4.9852e-13
7.4591,5.0002e-13
7.4621,5.1409e-13
7.4651,5.119e-13
7.468,5.1811e-13
7.471,5.1367e-13
7.474,5.3391e-13
7.477,5.3724e-13
7.48,5.3132e-13
7.4829,5.1936e-13
7.4859,5.3815e-13
7.4889,5.2888e-13
7.4919,5.3713e-13
7.4949,5.3629e-13
7.4978,5.3457e-13
7.5008,5.3527e-13
7.5038,5.4778e-13
7.5068,5.3937e-13
7.5098,5.6041e-13
7.5127,5.5289e-13
7.5157,5.6691e-13
7.5187,5.623e-13
7.5217,5.6752e-13
7.5247,5.5342e-13
7.5276,5.6707e-13
7.5306,5.5858e-13
7.5336,5.7077e-13
7.5366,5.7301e-13
7.5396,5.9394e-13
7.5425,5.93e-13
7.5455,5.9297e-13
7.5485,5.8639e-13
7.5515,5.9194e-13
7.5545,5.9677e-13
7.5575,5.9494e-13
7.5604,6.0466e-13
7.5634,6.1365e-13
7.5664,6.1914e-13
7.5694,6.1737e-13
7.5724,6.2109e-13
7.5753,6.1701e-13
7.5783,6.3699e-13
7.5813,6.4246e-13
7.5843,6.3116e-13
7.5873,6.4215e-13
7.5902,6.3774e-13
7.5932,6.4182e-13
7.5962,6.3963e-13
7.5992,6.494e-13
7.6022,6.4504e-13
7.6051,6.4704e-13
7.6081,6.5228e-13
7.6111,6.4579e-13
7.6141,6.7707e-13
7.6171,6.6394e-13
7.62,6.6336e-13
7.623,6.6785e-13
7.626,6.7008e-13
7.629,6.7027e-13
7.632,6.8381e-13
7.6349,6.8665e-13
7.6379,6.9128e-13
7.6409,6.955e-13
7.6439,6.9444e-13
7.6469,7.0327e-13
7.6498,7.1526e-13
7.6528,7.0594e-13
7.6558,7.0674e-13
7.6588,7.1357e-13
7.6618,7.2281e-13
7.6648,7.2792e-13
7.6677,7.3222e-13
7.6707,7.2961e-13
7.6737,7.3844e-13
7.6767,7.4057e-13
7.6797,7.537e-13
7.6826,7.6736e-13
7.6856,7.5162e-13
7.6886,7.5384e-13
7.6916,7.5329e-13
7.6946,7.627e-13
7.6975,7.7313e-13
7.7005,7.5909e-13
7.7035,7.6023e-13
7.7065,7.5887e-13
7.7095,7.925e-13
7.7124,7.8101e-13
7.7154,7.9087e-13
7.7184,7.7793e-13
7.7214,7.7471e-13
7.7244,7.9498e-13
7.7273,8.0833e-13
7.7303,7.9134e-13
7.7333,8.0855e-13
7.7363,8.028e-13
7.7393,8.1013e-13
7.7422,8.1432e-13
7.7452,8.0483e-13
7.7482,8.2415e-13
7.7512,8.2784e-13
7.7542,8.3097e-13
7.7572,8.423e-13
7.7601,8.3483e-13
7.7631,8.358e-13
7.7661,8.4849e-13
7.7691,8.3367e-13
7.7721,8.5756e-13
7.775,8.5948e-13
7.778,8.6833e-13
7.781,8.6514e-13
7.784,8.6969e-13
7.787,8.758e-13
7.7899,8.7261e-13
7.7929,8.7311e-13
7.7959,8.8402e-13
7.7989,8.7097e-13
7.8019,8.8465e-13
7.8048,8.7158e-13
7.8078,8.8715e-13
7.8108,9.0311e-13
7.8138,9.0028e-13
7.8168,9.0186e-13
7.8197,9.2315e-13
7.8227,9.2334e-13
7.8257,9.0142e-13
7.8287,9.2201e-13
7.8317,9.2754e-13
7.8346,9.3187e-13
7.8376,9.3969e-13
7.8406,9.4461e-13
7.8436,9.3778e-13
7.8466,9.5188e-13
7.8495,9.6259e-13
7.8525,9.5768e-13
7.8555,9.5313e-13
7.8585,9.7536e-13
7.8615,9.5468e-13
7.8645,9.6972e-13
7.8674,9.7988e-13
7.8704,9.6229e-13
7.8734,9.9465e-13
7.8764,9.9723e-13
7.8794,9.8671e-13
7.8823,9.967e-13
7.8853,1.0059e-12
7.8883,1.0071e-12
7.8913,1.0118e-12
7.8943,1.0186e-12
7.8972,1.0122e-12
7.9002,1.0236e-12
7.9032,1.023e-12
7.9062,1.032e-12
7.9092,1.0239e-12
7.9121,1.0259e-12
7.9151,1.0167e-12
7.9181,1.0345e-12
7.9211,1.0471e-12
7.9241,1.0373e-12
7.927,1.0557e-12
7.93,1.0534e-12
7.933,1.0589e-12
7.936,1.0503e-12
7.939,1.078e-12
7.9419,1.052e-12
7.9449,1.0532e-12
7.9479,1.0634e-12
7.9509,1.0729e-12
7.9539,1.0991e-12
7.9569,1.0866e-12
7.9598,1.0897e-12
7.9628,1.101e-12
7.9658,1.1066e-12
7.9688,1.0989e-12
7.9718,1.1154e-12
7.9747,1.0925e-12
7.9777,1.1197e-12
7.9807,1.1152e-12
7.9837,1.1288e-12
7.9867,1.1404e-12
7.9896,1.1365e-12
7.9926,1.15e-12
7.9956,1.1461e-12
7.9986,1.1641e-12
8.0016,1.1459e-12
8.0045,1.1605e-12
8.0075,1.1634e-12
8.0105,1.1562e-12
8.0135,1.1406e-12
8.0165,1.1739e-12
8.0194,1.1641e-12
8.0224,1.1862e-12
8.0254,1.1876e-12
8.0284,1.1897e-12
8.0314,1.2132e-12
8.0343,1.185e-12
8.0373,1.1967e-12
8.0403,1.2098e-12
8.0433,1.1965e-12
8.0463,1.2113e-12
8.0492,1.2413e-12
8.0522,1.2267e-12
8.0552,1.2352e-12
8.0582,1.261e-12
8.0612,1.2138e-12
8.0642,1.2298e-12
8.0671,1.244e-12
8.0701,1.2536e-12
8.0731,1.2369e-12
8.0761,1.2494e-12
8.0791,1.2526e-12
8.082,1.2616e-12
8.085,1.2651e-12
8.088,1.2633e-12
8.091,1.2574e-12
8.094,1.2793e-12
8.0969,1.2912e-12
8.0999,1.2887e-12
8.1029,1.309e-12
8.1059,1.3247e-12
8.1089,1.3107e-12
8.1118,1.3017e-12
8.1148,1.3207e-12
8.1178,1.3267e-12
8.1208,1.3397e-12
8.1238,1.3498e-12
8.1267,1.3392e-12
8.1297,1.3488e-12
8.1327,1.3523e-12
8.1357,1.3577e-12
8.1387,1.3738e-12
8.1416,1.3715e-12
8.1446,1.3908e-12
8.1476,1.3755e-12
8.1506,1.3695e-12
8.1536,1.3912e-12
8.1566,1.3936e-12
8.1595,1.394e-12
8.1625,1.3638e-12
8.1655,1.3818e-12
8.1685,1.4127e-12
8.1715,1.4256e-12
8.1744,1.4257e-12
8.1774,1.4341e-12
8.1804,1.437e-12
8.1834,1.4275e-12
8.1864,1.4307e-12
8.1893,1.4481e-12
8.1923,1.4428e-12
8.1953,1.4446e-12
8.1983,1.4544e-12
8.2013,1.4465e-12
8.2042,1.4964e-12
8.2072,1.4609e-12
8.2102,1.4642e-12
8.2132,1.4816e-12
8.2162,1.4761e-12
8.2191,1.4869e-12
8.2221,1.4747e-12
8.2251,1.5051e-12
8.2281,1.4823e-12
8.2311,1.5141e-12
8.234,1.5081e-12
8.237,1.51e-12
8.24,1.5097e-12
8.243,1.5084e-12
8.246,1.4932e-12
8.2489,1.5548e-12
8.2519,1.5441e-12
8.2549,1.5392e-12
8.2579,1.5855e-12
8.2609,1.5499e-12
8.2639,1.5737e-12
8.2668,1.5579e-12
8.2698,1.5664e-12
8.2728,1.5733e-12
8.2758,1.6186e-12
8.2788,1.5806e-12
8.2817,1.6138e-12
8.2847,1.5874e-12
8.2877,1.6191e-12
8.2907,1.6302e-12
8.2937,1.6159e-12
8.2966,1.602e-12
8.2996,1.6232e-12
8.3026,1.6155e-12
8.3056,1.6289e-12
8.3086,1.6463e-12
8.3115,1.6884e-12
8.3145,1.6052e-12
8.3175,1.678e-12
8.3205,1.64e-12
8.3235,1.6734e-12
8.3264,1.6925e-12
8.3294,1.658e-12
8.3324,1.6638e-12
8.3354,1.6895e-12
8.3384,1.7169e-12
8.3413,1.6713e-12
8.3443,1.6937e-12
8.3473,1.6918e-12
8.3503,1.7109e-12
8.3533,1.7535e-12
8.3563,1.7298e-12
8.3592,1.7389e-12
8.3622,1.7322e-12
8.3652,1.7527e-12
8.3682,1.7321e-12
8.3712,1.7358e-12
8.3741,1.7419e-12
8.3771,1.7454e-12
8.3801,1.7483e-12
8.3831,1.7727e-12
8.3861,1.7868e-12
8.389,1.7656e-12
8.392,1.7872e-12
8.395,1.7951e-12
8.398,1.7892e-12
8.401,1.7906e-12
8.4039,1.8077e-12
8.4069,1.8114e-12
8.4099,1.8484e-12
8.4129,1.8151e-12
8.4159,1.8348e-12
8.4188,1.8409e-12
8.4218,1.7939e-12
8.4248,1.8682e-12
8.4278,1.8724e-12
8.4308,1.8787e-12
8.4337,1.8659e-12
8.4367,1.8949e-12
8.4397,1.8799e-12
8.4427,1.8929e-12
8.4457,1.9333e-12
8.4486,1.8573e-12
8.4516,1.8876e-12
8.4546,1.8856e-12
8.4576,1.9287e-12
8.4606,1.9187e-12
8.4636,1.9318e-12
8.4665,1.8962e-12
8.4695,1.9346e-12
8.4725,1.9527e-12
8.4755,1.8972e-12
8.4785,1.9394e-12
8.4814,1.9559e-12
8.4844,1.9206e-12
8.4874,1.9517e-12
8.4904,1.9579e-12
8.4934,1.9649e-12
8.4963,1.9682e-12
8.4993,1.9801e-12
8.5023,1.9779e-12
8.5053,1.9698e-12
8.5083,2.0008e-12
8.5112,2.0321e-12
8.5142,1.9968e-12
8.5172,2.0103e-12
8.5202,1.9859e-12
8.5232,2.0653e-12
8.5261,2.0599e-12
8.5291,2.0434e-12
8.5321,2.0433e-12
8.5351,2.0574e-12
8.5381,2.0857e-12
8.541,2.061e-12
8.544,2.1161e-12
8.547,2.0897e-12
8.55,2.1147e-12
8.553,2.0869e-12
8.556,2.0891e-12
8.5589,2.111e-12
8.5619,2.1047e-12
8.5649,2.1501e-12
8.5679,2.1129e-12
8.5709,2.1466e-12
8.5738,2.1612e-12
8.5768,2.1176e-12
8.5798,2.162e-12
8.5828,2.154e-12
8.5858,2.1403e-12
8.5887,2.1647e-12
8.5917,2.1678e-12
8.5947,2.15e-12
8.5977,2.1812e-12
8.6007,2.2014e-12
8.6036,2.1912e-12
8.6066,2.2035e-12
8.6096,2.235e-12
8.6126,2.1916e-12
8.6156,2.2357e-12
8.6185,2.2452e-12
8.6215,2.2666e-12
8.6245,2.2407e-12
8.6275,2.2607e-12
8.6305,2.237e-12
8.6334,2.2542e-12
8.6364,2.2976e-12
8.6394,2.2895e-12
8.6424,2.3099e-12
8.6454,2.3236e-12
8.6483,2.2762e-12
8.6513,2.3147e-12
8.6543,2.2893e-12
8.6573,2.3278e-12
8.6603,2.3471e-12
8.6633,2.3021e-12
8.6662,2.3258e-12
8.6692,2.2916e-12
8.6722,2.36e-12
8.6752,2.3526e-12
8.6782,2.3539e-12
8.6811,2.3691e-12
8.6841,2.3677e-12
8.6871,2.3742e-12
8.6901,2.4077e-12
8.6931,2.3855e-12
8.696,2.3838e-12
8.699,2.3925e-12
8.702,2.4282e-12
8.705,2.442e-12
8.708,2.453e-12
8.7109,2.4018e-12
8.7139,2.4271e-12
8.7169,2.4716e-12
8.7199,2.4416e-12
8.7229,2.456e-12
8.7258,2.4795e-12
8.7288,2.4498e-12
8.7318,2.4797e-12
8.7348,2.4762e-12
8.7378,2.4855e-12
8.7407,2.5196e-12
8.7437,2.4919e-12
8.7467,2.5033e-12
8.7497,2.5168e-12
8.7527,2.52e-12
8.7557,2.5375e-12
8.7586,2.56e-12
8.7616,2.5669e-12
8.7646,2.5679e-12
8.7676,2.5467e-12
8.7706,2.5537e-12
8.7735,2.5615e-12
8.7765,2.6121e-12
8.7795,2.6011e-12
8.7825,2.5933e-12
8.7855,2.595e-12
8.7884,2.598e-12
8.7914,2.5847e-12
8.7944,2.5991e-12
8.7974,2.6426e-12
8.8004,2.624e-12
8.8033,2.6413e-12
8.8063,2.6323e-12
8.8093,2.6519e-12
8.8123,2.6717e-12
8.8153,2.6359e-12
8.8182,2.7112e-12
8.8212,2.728e-12
8.8242,2.6857e-12
8.8272,2.7042e-12
8.8302,2.6944e-12
8.8331,2.7241e-12
8.8361,2.7543e-12
8.8391,2.7383e-12
8.8421,2.7073e-12
8.8451,2.7668e-12
8.848,2.7164e-12
8.851,2.7718e-12
8.854,2.8158e-12
8.857,2.7768e-12
8.86,2.8372e-12
8.863,2.8033e-12
8.8659,2.8497e-12
8.8689,2.8084e-12
8.8719,2.8297e-12
8.8749,2.807e-12
8.8779,2.8004e-12
8.8808,2.8684e-12
8.8838,2.8537e-12
8.8868,2.8798e-12
8.8898,2.8666e-12
8.8928,2.828e-12
8.8957,2.9185e-12
8.8987,2.8755e-12
8.9017,2.8695e-12
8.9047,2.9276e-12
8.9077,2.9343e-12
8.9106,2.9294e-12
8.9136,2.8648e-12
8.9166,2.9206e-12
8.9196,2.9367e-12
8.9226,2.9296e-12
8.9255,2.9377e-12
8.9285,2.9763e-12
8.9315,2.9504e-12
8.9345,2.9845e-12
8.9375,2.9547e-12
8.9404,3.0029e-12
8.9434,3.031e-12
8.9464,3.0176e-12
8.9494,3.0583e-12
8.9524,3.0233e-12
8.9554,3.0949e-12
8.9583,3.0206e-12
8.9613,3.0666e-12
8.9643,3.1038e-12
8.9673,3.1202e-12
8.9703,3.0435e-12
8.9732,3.0776e-12
8.9762,3.0664e-12
8.9792,3.1074e-12
8.9822,3.099e-12
8.9852,3.0992e-12
8.9881,3.1918e-12
8.9911,3.1629e-12
8.9941,3.0919e-12
8.9971,3.1208e-12
9.0001,3.1312e-12
9.003,3.1822e-12
9.006,3.1331e-12
9.009,3.1534e-12
9.012,3.1602e-12
9.015,3.2062e-12
9.0179,3.2778e-12
9.0209,3.2537e-12
9.0239,3.2795e-12
9.0269,3.2069e-12
9.0299,3.2505e-12
9.0328,3.2757e-12
9.0358,3.2084e-12
9.0388,3.2658e-12
9.0418,3.2991e-12
9.0448,3.2952e-12
9.0477,3.3115e-12
9.0507,3.2932e-12
9.0537,3.3184e-12
9.0567,3.2981e-12
9.0597,3.3329e-12
9.0627,3.3292e-12
9.0656,3.3334e-12
9.0686,3.3211e-12
9.0716,3.417e-12
9.0746,3.3537e-12
9.0776,3.4251e-12
9.0805,3.3377e-12
9.0835,3.3569e-12
9.0865,3.3221e-12
9.0895,3.4075e-12
9.0925,3.4248e-12
9.0954,3.4667e-12
9.0984,3.4615e-12
9.1014,3.4603e-12
9.1044,3.4383e-12
9.1074,3.4695e-12
9.1103,3.4963e-12
9.1133,3.4602e-12
9.1163,3.4926e-12
9.1193,3.5112e-12
9.1223,3.4921e-12
9.1252,3.5227e-12
9.1282,3.5269e-12
9.1312,3.4976e-12
9.1342,3.5801e-12
9.1372,3.5497e-12
9.1401,3.594e-12
9.1431,3.5935e-12
9.1461,3.5208e-12
9.1491,3.5326e-12
9.1521,3.5917e-12
9.1551,3.6187e-12
9.158,3.5821e-12
9.161,3.5925e-12
9.164,3.6849e-12
9.167,3.6682e-12
9.17,3.6882e-12
9.1729,3.5868e-12
9.1759,3.6112e-12
9.1789,3.6548e-12
9.1819,3.717e-12
9.1849,3.6717e-12
9.1878,3.7262e-12
9.1908,3.7208e-12
9.1938,3.7298e-12
9.1968,3.6928e-12
9.1998,3.7432e-12
9.2027,3.7504e-12
9.2057,3.8182e-12
9.2087,3.7668e-12
9.2117,3.813e-12
9.2147,3.8201e-12
9.2176,3.7677e-12
9.2206,3.8508e-12
9.2236,3.7941e-12
9.2266,3.8665e-12
9.2296,3.79e-12
9.2325,3.8756e-12
9.2355,3.8705e-12
9.2385,3.7415e-12
9.2415,3.9219e-12
9.2445,3.9187e-12
9.2474,3.8292e-12
9.2504,3.9508e-12
9.2534,3.8988e-12
9.2564,3.8844e-12
9.2594,3.9444e-12
9.2624,3.9429e-12
9.2653,3.9162e-12
9.2683,3.98e-12
9.2713,4.0044e-12
9.2743,3.9833e-12
9.2773,4.0324e-12
9.2802,4.0366e-12
9.2832,4.0211e-12
9.2862,3.9971e-12
9.2892,4.0792e-12
9.2922,4.0296e-12
9.2951,4.112e-12
9.2981,4.1002e-12
9.3011,4.0973e-12
9.3041,4.0553e-12
9.3071,4.1131e-12
9.31,4.0511e-12
9.313,4.1435e-12
9.316,4.1166e-12
9.319,4.1455e-12
9.322,4.1262e-12
9.3249,4.2032e-12
9.3279,4.2023e-12
9.3309,4.1863e-12
9.3339,4.2387e-12
9.3369,4.2059e-12
9.3398,4.1567e-12
9.3428,4.2628e-12
9.3458,4.2799e-12
9.3488,4.283e-12
9.3518,4.2132e-12
9.3548,4.2561e-12
9.3577,4.2003e-12
9.3607,4.2882e-12
9.3637,4.2948e-12
9.3667,4.2929e-12
9.3697,4.3523e-12
9.3726,4.3218e-12
9.3756,4.3227e-12
9.3786,4.3465e-12
9.3816,4.3293e-12
9.3846,4.4473e-12
9.3875,4.4443e-12
9.3905,4.3877e-12
9.3935,4.3228e-12
9.3965,4.3864e-12
9.3995,4.4392e-12
9.4024,4.4713e-12
9.4054,4.4665e-12
9.4084,4.4227e-12
9.4114,4.5037e-12
9.4144,4.4505e-12
9.4173,4.5187e-12
9.4203,4.4905e-12
9.4233,4.4836e-12
9.4263,4.5048e-12
9.4293,4.4776e-12
9.4322,4.5493e-12
9.4352,4.5264e-12
9.4382,4.5295e-12
9.4412,4.5452e-12
9.4442,4.6144e-12
9.4471,4.6738e-12
9.4501,4.6491e-12
9.4531,4.5397e-12
9.4561,4.6628e-12
9.4591,4.6639e-12
9.4621,4.6351e-12
9.465,4.5958e-12
9.468,4.5996e-12
9.471,4.6574e-12
9.474,4.7338e-12
9.477,4.7296e-12
9.4799,4.7167e-12
9.4829,4.7604e-12
9.4859,4.6856e-12
9.4889,4.7342e-12
9.4919,4.7763e-12
9.4948,4.7864e-12
9.4978,4.7606e-12
9.5008,4.7998e-12
9.5038,4.7972e-12
9.5068,4.8273e-12
9.5097,4.7636e-12
9.5127,4.8697e-12
9.5157,4.893e-12
9.5187,4.9152e-12
9.5217,4.891e-12
9.5246,4.8361e-12
9.5276,4.8879e-12
9.5306,4.8841e-12
9.5336,4.9627e-12
9.5366,4.9657e-12
9.5395,4.9477e-12
9.5425,4.99e-12
9.5455,4.9693e-12
9.5485,5.0241e-12
9.5515,4.9781e-12
9.5545,4.9639e-12
9.5574,5.0099e-12
9.5604,5.0127e-12
9.5634,5.0546e-12
9.5664,5.0869e-12
9.5694,5.0627e-12
9.5723,5.1407e-12
9.5753,5.1018e-12
9.5783,5.1402e-12
9.5813,5.1232e-12
9.5843,5.1844e-12
9.5872,5.193e-12
9.5902,5.2095e-12
9.5932,5.227e-12
9.5962,5.1354e-12
9.5992,5.1753e-12
9.6021,5.1111e-12
9.6051,5.2064e-12
9.6081,5.2067e-12
9.6111,5.2639e-12
9.6141,5.306e-12
9.617,5.3385e-12
9.62,5.3103e-12
9.623,5.2843e-12
9.626,5.3535e-12
9.629,5.4204e-12
9.6319,5.4056e-12
9.6349,5.3395e-12
9.6379,5.384e-12
9.6409,5.3586e-12
9.6439,5.3988e-12
9.6468,5.4274e-12
9.6498,5.3538e-12
9.6528,5.3886e-12
9.6558,5.5343e-12
9.6588,5.4704e-12
9.6618,5.5093e-12
9.6647,5.5266e-12
9.6677,5.5292e-12
9.6707,5.4834e-12
9.6737,5.4302e-12
9.6767,5.5232e-12
9.6796,5.5782e-12
9.6826,5.5574e-12
9.6856,5.6203e-12
9.6886,5.5932e-12
9.6916,5.5831e-12
9.6945,5.5953e-12
9.6975,5.577e-12
9.7005,5.7162e-12
9.7035,5.6619e-12
9.7065,5.6402e-12
9.7094,5.7346e-12
9.7124,5.6463e-12
9.7154,5.7057e-12
9.7184,5.6989e-12
9.7214,5.669e-12
9.7243,5.6849e-12
9.7273,5.6659e-12
9.7303,5.7266e-12
9.7333,5.7868e-12
9.7363,5.814e-12
9.7392,5.8655e-12
9.7422,5.8458e-12
9.7452,5.7614e-12
9.7482,5.8506e-12
9.7512,5.7639e-12
9.7542,5.8751e-12
9.7571,5.8695e-12
9.7601,5.9221e-12
9.7631,5.9257e-12
9.7661,5.9015e-12
9.7691,5.9178e-12
9.772,6.0305e-12
9.775,6.0077e-12
9.778,5.9937e-12
9.781,6.0372e-12
9.784,6.0291e-12
9.7869,6.06e-12
9.7899,6.049e-12
9.7929,6.0224e-12
9.7959,5.9675e-12
9.7989,6.0712e-12
9.8018,6.076e-12
9.8048,6.2155e-12
9.8078,6.1709e-12
9.8108,6.2481e-12
9.8138,6.1705e-12
9.8167,6.2148e-12
9.8197,6.2362e-12
9.8227,6.1771e-12
9.8257,6.1684e-12
9.8287,6.1858e-12
9.8316,6.368e-12
9.8346,6.1533e-12
9.8376,6.1988e-12
9.8406,6.2412e-12
9.8436,6.3537e-12
9.8465,6.395e-12
9.8495,6.3029e-12
9.8525,6.439e-12
9.8555,6.4866e-12
9.8585,6.3071e-12
9.8615,6.3057e-12
9.8644,6.3764e-12
9.8674,6.3391e-12
9.8704,6.4958e-12
9.8734,6.4763e-12
9.8764,6.4033e-12
9.8793,6.5716e-12
9.8823,6.5629e-12
9.8853,6.4466e-12
9.8883,6.4409e-12
9.8913,6.511e-12
9.8942,6.496e-12
9.8972,6.5358e-12
9.9002,6.5652e-12
9.9032,6.5037e-12
9.9062,6.6425e-12
9.9091,6.5789e-12
9.9121,6.6216e-12
9.9151,6.6347e-12
9.9181,6.6911e-12
9.9211,6.6574e-12
9.924,6.8694e-12
9.927,6.7884e-12
9.93,6.694e-12
9.933,6.7392e-12
9.936,6.6491e-12
9.9389,6.7367e-12
9.9419,6.8971e-12
9.9449,6.7929e-12
9.9479,6.7718e-12
9.9509,6.7898e-12
9.9539,6.8847e-12
9.9568,6.9277e-12
9.9598,6.8955e-12
9.9628,7.0236e-12
9.9658,6.9132e-12
9.9688,7.0148e-12
9.9717,6.918e-12
9.9747,6.9189e-12
9.9777,7.0734e-12
9.9807,7.0261e-12
9.9837,7.1105e-12
9.9866,7.0488e-12
9.9896,7.1415e-12
9.9926,7.1075e-12
9.9956,7.104e-12
9.9986,7.1354e-12
10.002,7.1705e-12
10.005,7.0749e-12
10.008,7.181e-12
10.01,7.2196e-12
10.013,7.1552e-12
10.016,7.1247e-12
10.019,7.1418e-12
10.022,7.1962e-12
10.025,7.3208e-12
10.028,7.2164e-12
10.031,7.2733e-12
10.034,7.3064e-12
10.037,7.2738e-12
10.04,7.3739e-12
10.043,7.4252e-12
10.046,7.4183e-12
10.049,7.4902e-12
10.052,7.3943e-12
10.055,7.3148e-12
10.058,7.3575e-12
10.061,7.5327e-12
10.064,7.5512e-12
10.067,7.4492e-12
10.07,7.4367e-12
10.073,7.4953e-12
10.076,7.4535e-12
10.079,7.6223e-12
10.082,7.5648e-12
10.085,7.6443e-12
10.088,7.5156e-12
10.091,7.6279e-12
10.094,7.6247e-12
10.097,7.7535e-12
10.1,7.7254e-12
10.103,7.7021e-12
10.106,7.7725e-12
10.109,7.7196e-12
10.112,7.7329e-12
10.115,7.7324e-12
10.118,7.6496e-12
10.121,7.7885e-12
10.124,7.8488e-12
10.127,7.8198e-12
10.13,7.7848e-12
10.133,7.9139e-12
10.136,7.9262e-12
10.139,7.8324e-12
10.142,7.9957e-12
10.145,7.9637e-12
10.148,7.8919e-12
10.151,8.0108e-12
10.154,7.9676e-12
10.157,7.8963e-12
10.16,8.0708e-12
10.162,8.0073e-12
10.165,8.0413e-12
10.168,8.0792e-12
10.171,8.094e-12
10.174,8.1277e-12
10.177,8.0772e-12
10.18,8.2329e-12
10.183,8.2133e-12
10.186,8.2654e-12
10.189,8.2383e-12
10.192,8.268e-12
10.195,8.2805e-12
10.198,8.4053e-12
10.201,8.4041e-12
10.204,8.3351e-12
10.207,8.3923e-12
10.21,8.3655e-12
10.213,8.3667e-12
10.216,8.4241e-12
10.219,8.5075e-12
10.222,8.5251e-12
10.225,8.5183e-12
10.228,8.5761e-12
10.231,8.5738e-12
10.234,8.4921e-12
10.237,8.6304e-12
10.24,8.5446e-12
10.243,8.5497e-12
10.246,8.6626e-12
10.249,8.6293e-12
10.252,8.691e-12
10.255,8.678e-12
10.258,8.675e-12
10.261,8.7763e-12
10.264,8.7273e-12
10.267,8.7246e-12
10.27,8.8132e-12
10.273,8.9084e-12
10.276,8.6577e-12
10.279,8.8174e-12
10.282,8.7858e-12
10.285,8.8757e-12
10.288,8.8399e-12
10.291,8.9393e-12
10.294,8.9453e-12
10.297,8.984e-12
10.3,8.8748e-12
10.303,9.0664e-12
10.306,8.9841e-12
10.309,9.0019e-12
10.312,9.0557e-12
10.315,9.1274e-12
10.317,9.0353e-12
10.32,9.1259e-12
10.323,9.1548e-12
10.326,9.2166e-12
10.329,9.1125e-12
10.332,9.2218e-12
10.335,9.1678e-12
10.338,9.3377e-12
10.341,9.2895e-12
10.344,9.2083e-12
10.347,9.1797e-12
10.35,9.3952e-12
10.353,9.4415e-12
10.356,9.2588e-12
10.359,9.5183e-12
10.362,9.4206e-12
10.365,9.4342e-12
10.368,9.5028e-12
10.371,9.4426e-12
10.374,9.4137e-12
10.377,9.6027e-12
10.38,9.6605e-12
10.383,9.5967e-12
10.386,9.4874e-12
10.389,9.7228e-12
10.392,9.7243e-12
10.395,9.571e-12
10.398,9.8228e-12
10.401,9.5833e-12
10.404,9.8263e-12
10.407,9.9836e-12
10.41,9.6699e-12
10.413,9.8452e-12
10.416,1.0011e-11
10.419,9.8564e-12
10.422,9.9214e-12
10.425,1.0066e-11
10.428,9.8003e-12
10.431,9.9484e-12
10.434,9.9791e-12
10.437,9.9692e-12
10.44,1.0076e-11
10.443,9.9891e-12
10.446,1.0136e-11
10.449,1.0143e-11
10.452,1.0097e-11
10.455,1.011e-11
10.458,1.0131e-11
10.461,1.0161e-11
10.464,1.0214e-11
10.467,1.0142e-11
10.469,1.0152e-11
10.472,1.0213e-11
10.475,1.026e-11
10.478,1.0262e-11
10.481,1.0247e-11
10.484,1.0269e-11
10.487,1.0376e-11
10.49,1.0588e-11
10.493,1.0345e-11
10.496,1.0553e-11
10.499,1.0543e-11
10.502,1.0581e-11
10.505,1.0381e-11
10.508,1.0627e-11
10.511,1.0366e-11
10.514,1.0722e-11
10.517,1.0769e-11
10.52,1.0596e-11
10.523,1.0796e-11
10.526,1.0917e-11
10.529,1.0765e-11
10.532,1.068e-11
10.535,1.0896e-11
10.538,1.0907e-11
10.541,1.072e-11
10.544,1.0775e-11
10.547,1.0883e-11
10.55,1.0793e-11
10.553,1.0813e-11
10.556,1.0872e-11
10.559,1.1e-11
10.562,1.1145e-11
10.565,1.1051e-11
10.568,1.1024e-11
10.571,1.0999e-11
10.574,1.0949e-11
10.577,1.1031e-11
10.58,1.1146e-11
10.583,1.1124e-11
10.586,1.0895e-11
10.589,1.12e-11
10.592,1.1315e-11
10.595,1.1248e-11
10.598,1.118e-11
10.601,1.1446e-11
10.604,1.1363e-11
10.607,1.128e-11
10.61,1.147e-11
10.613,1.1382e-11
10.616,1.1377e-11
10.619,1.1625e-11
10.622,1.1621e-11
10.624,1.1635e-11
10.627,1.1377e-11
10.63,1.1583e-11
10.633,1.1671e-11
10.636,1.185e-11
10.639,1.1673e-11
10.642,1.1764e-11
10.645,1.1465e-11
10.648,1.1946e-11
10.651,1.1916e-11
10.654,1.1803e-11
10.657,1.1891e-11
10.66,1.1999e-11
10.663,1.1933e-11
10.666,1.1964e-11
10.669,1.2031e-11
10.672,1.1732e-11
10.675,1.1944e-11
10.678,1.2028e-11
10.681,1.1999e-11
10.684,1.2056e-11
10.687,1.2177e-11
10.69,1.1877e-11
10.693,1.2225e-11
10.696,1.1945e-11
10.699,1.2227e-11
10.702,1.2222e-11
10.705,1.2373e-11
10.708,1.2469e-11
10.711,1.2195e-11
10.714,1.226e-11
10.717,1.2204e-11
10.72,1.2464e-11
10.723,1.2361e-11
10.726,1.243e-11
10.729,1.2387e-11
10.732,1.2536e-11
10.735,1.2556e-11
10.738,1.2704e-11
10.741,1.2618e-11
10.744,1.2487e-11
10.747,1.2745e-11
10.75,1.2913e-11
10.753,1.2657e-11
10.756,1.2652e-11
10.759,1.2895e-11
10.762,1.2841e-11
10.765,1.2617e-11
10.768,1.2897e-11
10.771,1.3044e-11
10.774,1.2953e-11
10.776,1.3193e-11
10.779,1.3049e-11
10.782,1.3177e-11
10.785,1.2912e-11
10.788,1.3159e-11
10.791,1.3298e-11
10.794,1.3351e-11
10.797,1.31e-11
10.8,1.3173e-11
10.803,1.3198e-11
10.806,1.324e-11
10.809,1.3286e-11
10.812,1.3495e-11
10.815,1.3535e-11
10.818,1.3486e-11
10.821,1.335e-11
10.824,1.3303e-11
10.827,1.3567e-11
10.83,1.3513e-11
10.833,1.3574e-11
10.836,1.3613e-11
10.839,1.3768e-11
10.842,1.3922e-11
10.845,1.3649e-11
10.848,1.3742e-11
10.851,1.3465e-11
10.854,1.3765e-11
10.857,1.3962e-11
10.86,1.3916e-11
10.863,1.3918e-11
10.866,1.3933e-11
10.869,1.3785e-11
10.872,1.4091e-11
10.875,1.4117e-11
10.878,1.4039e-11
10.881,1.3954e-11
10.884,1.4066e-11
10.887,1.4259e-11
10.89,1.4184e-11
10.893,1.4197e-11
10.896,1.4058e-11
10.899,1.4327e-11
10.902,1.4247e-11
10.905,1.4515e-11
10.908,1.4125e-11
10.911,1.4066e-11
10.914,1.4264e-11
10.917,1.449e-11
10.92,1.4481e-11
10.923,1.4256e-11
10.926,1.465e-11
10.929,1.4745e-11
10.931,1.4858e-11
10.934,1.447e-11
10.937,1.4612e-11
10.94,1.4638e-11
10.943,1.4856e-11
10.946,1.4829e-11
10.949,1.4855e-11
10.952,1.4868e-11
10.955,1.4941e-11
10.958,1.4958e-11
10.961,1.5273e-11
10.964,1.4945e-11
10.967,1.5122e-11
10.97,1.5156e-11
10.973,1.5061e-11
10.976,1.5087e-11
10.979,1.5135e-11
10.982,1.5218e-11
10.985,1.5149e-11
10.988,1.5354e-11
10.991,1.5073e-11
10.994,1.5469e-11
10.997,1.5291e-11
11,1.5404e-11
11.003,1.5576e-11
11.006,1.5573e-11
11.009,1.5518e-11
11.012,1.5611e-11
11.015,1.5842e-11
11.018,1.5771e-11
11.021,1.6003e-11
11.024,1.581e-11
11.027,1.5905e-11
11.03,1.5665e-11
11.033,1.584e-11
11.036,1.5981e-11
11.039,1.5835e-11
11.042,1.5995e-11
11.045,1.6019e-11
11.048,1.5958e-11
11.051,1.6142e-11
11.054,1.5872e-11
11.057,1.614e-11
11.06,1.6347e-11
11.063,1.6048e-11
11.066,1.6463e-11
11.069,1.6074e-11
11.072,1.6321e-11
11.075,1.6251e-11
11.078,1.6191e-11
11.081,1.6216e-11
11.083,1.6343e-11
11.086,1.6241e-11
11.089,1.6376e-11
11.092,1.6717e-11
11.095,1.6556e-11
11.098,1.6449e-11
11.101,1.6657e-11
11.104,1.6854e-11
11.107,1.6228e-11
11.11,1.6559e-11
11.113,1.7015e-11
11.116,1.6678e-11
11.119,1.6699e-11
11.122,1.7081e-11
11.125,1.6673e-11
11.128,1.725e-11
11.131,1.7134e-11
11.134,1.7261e-11
11.137,1.6863e-11
11.14,1.7404e-11
11.143,1.7094e-11
11.146,1.737e-11
11.149,1.7188e-11
11.152,1.7405e-11
11.155,1.7497e-11
11.158,1.7785e-11
11.161,1.767e-11
11.164,1.7795e-11
11.167,1.753e-11
11.17,1.7813e-11
11.173,1.7715e-11
11.176,1.7619e-11
11.179,1.772e-11
11.182,1.7724e-11
11.185,1.7626e-11
11.188,1.7545e-11
11.191,1.8058e-11
11.194,1.7855e-11
11.197,1.7883e-11
11.2,1.7974e-11
11.203,1.826e-11
11.206,1.8228e-11
11.209,1.823e-11
11.212,1.8154e-11
11.215,1.8349e-11
11.218,1.8489e-11
11.221,1.8495e-11
11.224,1.8321e-11
11.227,1.8413e-11
11.23,1.86e-11
11.233,1.8761e-11
11.236,1.8853e-11
11.238,1.8491e-11
11.241,1.879e-11
11.244,1.8952e-11
11.247,1.8985e-11
11.25,1.8624e-11
11.253,1.8816e-11
11.256,1.8911e-11
11.259,1.8967e-11
11.262,1.8869e-11
11.265,1.9017e-11
11.268,1.9079e-11
11.271,1.9009e-11
11.274,1.965e-11
11.277,1.9814e-11
11.28,1.8837e-11
11.283,1.9367e-11
11.286,1.8725e-11
11.289,1.9504e-11
11.292,1.9762e-11
11.295,1.9103e-11
11.298,1.9468e-11
11.301,1.965e-11
11.304,1.9402e-11
11.307,1.9801e-11
11.31,1.9466e-11
11.313,2.0151e-11
11.316,2.0219e-11
11.319,1.9843e-11
11.322,2.039e-11
11.325,1.9946e-11
11.328,2.0198e-11
11.331,2.0166e-11
11.334,1.9934e-11
11.337,2.1108e-11
11.34,2.0259e-11
11.343,2.0131e-11
11.346,2.0349e-11
11.349,2.0228e-11
11.352,2.0594e-11
11.355,2.0701e-11
11.358,2.0283e-11
11.361,2.0464e-11
11.364,2.0409e-11
11.367,2.1125e-11
11.37,2.1129e-11
11.373,2.0818e-11
11.376,2.0972e-11
11.379,2.0839e-11
11.382,2.0922e-11
11.385,2.1185e-11
11.388,2.1119e-11
11.39,2.1109e-11
11.393,2.1386e-11
11.396,2.0759e-11
11.399,2.1093e-11
11.402,2.1505e-11
11.405,2.1413e-11
11.408,2.116e-11
11.411,2.1349e-11
11.414,2.14e-11
11.417,2.1281e-11
11.42,2.1636e-11
11.423,2.1425e-11
11.426,2.1579e-11
11.429,2.1769e-11
11.432,2.1752e-11
11.435,2.2332e-11
11.438,2.1359e-11
11.441,2.1863e-11
11.444,2.2259e-11
11.447,2.2313e-11
11.45,2.2245e-11
11.453,2.2012e-11
11.456,2.2219e-11
11.459,2.2216e-11
11.462,2.227e-11
11.465,2.2339e-11
11.468,2.239e-11
11.471,2.2402e-11
11.474,2.2585e-11
11.477,2.2548e-11
11.48,2.2696e-11
11.483,2.2373e-11
11.486,2.3037e-11
11.489,2.2964e-11
11.492,2.2985e-11
11.495,2.3108e-11
11.498,2.3089e-11
11.501,2.306e-11
11.504,2.2799e-11
11.507,2.3309e-11
11.51,2.306e-11
11.513,2.3319e-11
11.516,2.3304e-11
11.519,2.3805e-11
11.522,2.3462e-11
11.525,2.3385e-11
11.528,2.4023e-11
11.531,2.359e-11
11.534,2.373e-11
11.537,2.355e-11
11.54,2.344e-11
11.543,2.3554e-11
11.545,2.3971e-11
11.548,2.3809e-11
11.551,2.4153e-11
11.554,2.3855e-11
11.557,2.4102e-11
11.56,2.4166e-11
11.563,2.4193e-11
11.566,2.3932e-11
11.569,2.4135e-11
11.572,2.4001e-11
11.575,2.4578e-11
11.578,2.4251e-11
11.581,2.4485e-11
11.584,2.4475e-11
11.587,2.4708e-11
11.59,2.4489e-11
11.593,2.4655e-11
11.596,2.4628e-11
11.599,2.4546e-11
11.602,2.4263e-11
11.605,2.5367e-11
11.608,2.4935e-11
11.611,2.5368e-11
11.614,2.5394e-11
11.617,2.5417e-11
11.62,2.5367e-11
11.623,2.5322e-11
11.626,2.5253e-11
11.629,2.5092e-11
11.632,2.5187e-11
11.635,2.562e-11
11.638,2.5775e-11
11.641,2.5722e-11
11.644,2.5688e-11
11.647,2.5689e-11
11.65,2.5759e-11
11.653,2.6175e-11
11.656,2.603e-11
11.659,2.5956e-11
11.662,2.5934e-11
11.665,2.5767e-11
11.668,2.6851e-11
11.671,2.6286e-11
11.674,2.643e-11
11.677,2.6018e-11
11.68,2.6294e-11
11.683,2.6818e-11
11.686,2.68e-11
11.689,2.7042e-11
11.692,2.6472e-11
11.695,2.6861e-11
11.697,2.6757e-11
11.7,2.7114e-11
11.703,2.7012e-11
11.706,2.7559e-11
11.709,2.7253e-11
11.712,2.7643e-11
11.715,2.8012e-11
11.718,2.7532e-11
11.721,2.7771e-11
11.724,2.7813e-11
11.727,2.7727e-11
11.73,2.7455e-11
11.733,2.7562e-11
11.736,2.7993e-11
11.739,2.7678e-11
11.742,2.8186e-11
11.745,2.8332e-11
11.748,2.8557e-11
11.751,2.8057e-11
11.754,2.8192e-11
11.757,2.8608e-11
11.76,2.835e-11
11.763,2.81e-11
11.766,2.8468e-11
11.769,2.8941e-11
11.772,2.9072e-11
11.775,2.9258e-11
11.778,2.9066e-11
11.781,2.9129e-11
11.784,2.9101e-11
11.787,2.8898e-11
11.79,2.8903e-11
11.793,2.8976e-11
11.796,2.9277e-11
11.799,2.9453e-11
11.802,2.9456e-11
11.805,2.9393e-11
11.808,2.987e-11
11.811,3.0133e-11
11.814,2.9452e-11
11.817,2.9755e-11
11.82,2.9791e-11
11.823,2.9713e-11
11.826,2.9931e-11
11.829,3.0161e-11
11.832,2.9848e-11
11.835,3.058e-11
11.838,3.0091e-11
11.841,3.0323e-11
11.844,3.0448e-11
11.847,3.077e-11
11.85,3.1164e-11
11.852,3.0588e-11
11.855,3.0449e-11
11.858,3.1492e-11
11.861,3.1113e-11
11.864,3.0755e-11
11.867,3.0902e-11
11.87,3.1479e-11
11.873,3.1779e-11
11.876,3.1441e-11
11.879,3.238e-11
11.882,3.162e-11
11.885,3.1512e-11
11.888,3.1861e-11
11.891,3.2281e-11
11.894,3.1905e-11
11.897,3.1515e-11
11.9,3.2354e-11
11.903,3.2097e-11
11.906,3.2168e-11
11.909,3.2479e-11
11.912,3.2426e-11
11.915,3.2006e-11
11.918,3.3226e-11
11.921,3.3042e-11
11.924,3.3076e-11
11.927,3.3339e-11
11.93,3.2109e-11
11.933,3.204e-11
11.936,3.3029e-11
11.939,3.31e-11
11.942,3.304e-11
11.945,3.4213e-11
11.948,3.4049e-11
11.951,3.3427e-11
11.954,3.3602e-11
11.957,3.3611e-11
11.96,3.4057e-11
11.963,3.4301e-11
11.966,3.435e-11
11.969,3.3593e-11
11.972,3.3657e-11
11.975,3.3388e-11
11.978,3.3933e-11
11.981,3.4308e-11
11.984,3.4491e-11
11.987,3.4534e-11
11.99,3.4629e-11
11.993,3.5297e-11
11.996,3.5502e-11
11.999,3.4524e-11
12.002,3.4816e-11
12.005,3.4982e-11
12.007,3.5391e-11
12.01,3.5535e-11
12.013,3.5928e-11
12.016,3.4535e-11
12.019,3.485e-11
12.022,3.55e-11
12.025,3.5766e-11
12.028,3.5437e-11
12.031,3.5017e-11
12.034,3.5987e-11
12.037,3.6224e-11
12.04,3.5607e-11
12.043,3.6164e-11
12.046,3.6524e-11
12.049,3.5604e-11
12.052,3.5741e-11
12.055,3.6129e-11
12.058,3.5854e-11
12.061,3.6438e-11
12.064,3.6044e-11
12.067,3.6696e-11
12.07,3.6957e-11
12.073,3.7864e-11
12.076,3.7663e-11
12.079,3.7737e-11
12.082,3.7238e-11
12.085,3.7743e-11
12.088,3.7039e-11
12.091,3.7694e-11
12.094,3.7744e-11
12.097,3.7299e-11
12.1,3.7141e-11
12.103,3.8106e-11
12.106,3.7709e-11
12.109,3.7655e-11
12.112,3.8247e-11
12.115,3.8481e-11
12.118,3.788e-11
12.121,3.8867e-11
12.124,3.8907e-11
12.127,3.9416e-11
12.13,3.8312e-11
12.133,3.8979e-11
12.136,3.9511e-11
12.139,3.8938e-11
12.142,3.9239e-11
12.145,3.9731e-11
12.148,3.9688e-11
12.151,3.9549e-11
12.154,3.9258e-11
12.157,4.0826e-11
12.159,4.0447e-11
12.162,4.0301e-11
12.165,3.9738e-11
12.168,4.0663e-11
12.171,4.0127e-11
12.174,4.0165e-11
12.177,4.0924e-11
12.18,3.9959e-11
12.183,4.0965e-11
12.186,4.0859e-11
12.189,4.0549e-11
12.192,4.0618e-11
12.195,4.0096e-11
12.198,4.1257e-11
12.201,4.0689e-11
12.204,4.0673e-11
12.207,4.1366e-11
12.21,4.1781e-11
12.213,4.1176e-11
12.216,4.2278e-11
12.219,4.2083e-11
12.222,4.2441e-11
12.225,4.2479e-11
12.228,4.2346e-11
12.231,4.1938e-11
12.234,4.1676e-11
12.237,4.1938e-11
12.24,4.177e-11
12.243,4.2856e-11
12.246,4.3025e-11
12.249,4.3342e-11
12.252,4.2923e-11
12.255,4.3657e-11
12.258,4.3947e-11
12.261,4.3243e-11
12.264,4.396e-11
12.267,4.4549e-11
12.27,4.4913e-11
12.273,4.3961e-11
12.276,4.4271e-11
12.279,4.4689e-11
12.282,4.4247e-11
12.285,4.425e-11
12.288,4.4105e-11
12.291,4.5839e-11
12.294,4.4972e-11
12.297,4.5286e-11
12.3,4.4482e-11
12.303,4.487e-11
12.306,4.5025e-11
12.309,4.6165e-11
12.312,4.517e-11
12.314,4.5114e-11
12.317,4.4693e-11
12.32,4.4583e-11
12.323,4.5938e-11
12.326,4.6593e-11
12.329,4.6144e-11
12.332,4.681e-11
12.335,4.7108e-11
12.338,4.6935e-11
12.341,4.6729e-11
12.344,4.6557e-11
12.347,4.6674e-11
12.35,4.7402e-11
12.353,4.6937e-11
12.356,4.6692e-11
12.359,4.7492e-11
12.362,4.8123e-11
12.365,4.7846e-11
12.368,4.7101e-11
12.371,4.8069e-11
12.374,4.844e-11
12.377,4.7587e-11
12.38,4.8857e-11
12.383,4.7751e-11
12.386,4.8188e-11
12.389,4.9484e-11
12.392,4.8325e-11
12.395,4.901e-11
12.398,4.8757e-11
12.401,4.8351e-11
12.404,4.9461e-11
12.407,5.0055e-11
12.41,4.911e-11
12.413,4.9709e-11
12.416,4.8555e-11
12.419,5.0569e-11
12.422,5.0653e-11
12.425,5.0448e-11
12.428,5.045e-11
12.431,4.9898e-11
12.434,5.1289e-11
12.437,5.0342e-11
12.44,5.12e-11
12.443,4.9895e-11
12.446,5.2015e-11
12.449,5.1862e-11
12.452,5.1088e-11
12.455,5.2177e-11
12.458,5.2872e-11
12.461,5.0974e-11
12.464,5.1896e-11
12.466,5.1973e-11
12.469,5.2798e-11
12.472,5.3296e-11
12.475,5.2066e-11
12.478,5.2133e-11
12.481,5.2395e-11
12.484,5.2848e-11
12.487,5.295e-11
12.49,5.3083e-11
12.493,5.416e-11
12.496,5.3756e-11
12.499,5.4619e-11
12.502,5.3723e-11
12.505,5.3948e-11
12.508,5.483e-11
12.511,5.4738e-11
12.514,5.4698e-11
12.517,5.4382e-11
12.52,5.5529e-11
12.523,5.506e-11
12.526,5.4864e-11
12.529,5.5811e-11
12.532,5.4408e-11
12.535,5.5597e-11
12.538,5.5956e-11
12.541,5.5726e-11
12.544,5.6763e-11
12.547,5.5533e-11
12.55,5.5992e-11
12.553,5.7146e-11
12.556,5.5898e-11
12.559,5.5363e-11
12.562,5.6795e-11
12.565,5.5615e-11
12.568,5.7421e-11
12.571,5.7103e-11
12.574,5.7023e-11
12.577,5.8017e-11
12.58,5.8393e-11
12.583,5.8745e-11
12.586,5.8763e-11
12.589,5.8979e-11
12.592,5.9461e-11
12.595,5.8905e-11
12.598,5.8628e-11
12.601,5.8855e-11
12.604,5.8843e-11
12.607,6.0232e-11
12.61,5.8547e-11
12.613,5.9072e-11
12.616,5.9547e-11
12.619,5.8589e-11
12.621,6.0247e-11
12.624,6.0161e-11
12.627,6.1709e-11
12.63,6.0092e-11
12.633,5.9561e-11
12.636,6.06e-11
12.639,6.0624e-11
12.642,6.0349e-11
12.645,6.1229e-11
12.648,6.053e-11
12.651,6.0749e-11
12.654,6.0915e-11
12.657,6.2962e-11
12.66,6.1605e-11
12.663,6.2864e-11
12.666,6.2118e-11
12.669,6.2164e-11
12.672,6.3438e-11
12.675,6.505e-11
12.678,6.232e-11
12.681,6.542e-11
12.684,6.1681e-11
12.687,6.3396e-11
12.69,6.408e-11
12.693,6.3917e-11
12.696,6.3508e-11
12.699,6.2617e-11
12.702,6.4338e-11
12.705,6.5354e-11
12.708,6.544e-11
12.711,6.4256e-11
12.714,6.3992e-11
12.717,6.4938e-11
12.72,6.4124e-11
12.723,6.4815e-11
12.726,6.7249e-11
12.729,6.5779e-11
12.732,6.613e-11
12.735,6.6025e-11
12.738,6.5388e-11
12.741,6.4407e-11
12.744,6.5926e-11
12.747,6.6026e-11
12.75,6.6676e-11
12.753,6.6969e-11
12.756,6.5276e-11
12.759,6.8341e-11
12.762,6.7466e-11
12.765,6.6898e-11
12.768,6.7585e-11
12.771,6.8158e-11
12.773,6.84e-11
12.776,7.0044e-11
12.779,6.7687e-11
12.782,6.9905e-11
12.785,6.998e-11
12.788,6.9468e-11
12.791,6.9984e-11
12.794,6.9353e-11
12.797,7.0925e-11
12.8,6.9832e-11
12.803,6.9957e-11
12.806,6.8953e-11
12.809,7.0931e-11
12.812,7.1752e-11
12.815,7.1674e-11
12.818,7.19e-11
12.821,7.2275e-11
12.824,7.3521e-11
12.827,7.283e-11
12.83,7.174e-11
12.833,7.2209e-11
12.836,7.1921e-11
12.839,7.335e-11
12.842,7.2266e-11
12.845,7.1816e-11
12.848,7.2801e-11
12.851,7.3054e-11
12.854,7.1831e-11
12.857,7.587e-11
12.86,7.5549e-11
12.863,7.4413e-11
12.866,7.4235e-11
12.869,7.5901e-11
12.872,7.5495e-11
12.875,7.5179e-11
12.878,7.5479e-11
12.881,7.566e-11
12.884,7.4983e-11
12.887,7.6071e-11
12.89,7.8144e-11
12.893,7.6707e-11
12.896,7.5758e-11
12.899,7.6346e-11
12.902,7.7131e-11
12.905,7.7048e-11
12.908,7.8519e-11
12.911,7.6366e-11
12.914,7.6994e-11
12.917,7.7398e-11
12.92,7.7675e-11
12.923,7.7885e-11
12.926,8.0668e-11
12.928,7.9643e-11
12.931,7.8629e-11
12.934,8.0413e-11
12.937,8.0019e-11
12.94,8.0102e-11
12.943,8.176e-11
12.946,8.1596e-11
12.949,8.0683e-11
12.952,8.1871e-11
12.955,8.063e-11
12.958,8.0072e-11
12.961,8.1344e-11
12.964,7.9674e-11
12.967,8.0844e-11
12.97,8.2521e-11
12.973,8.3031e-11
12.976,8.418e-11
12.979,8.424e-11
12.982,8.3868e-11
12.985,8.549e-11
12.988,8.4331e-11
12.991,8.3761e-11
12.994,8.4908e-11
12.997,8.3634e-11
13,8.4515e-11
13.003,8.4219e-11
13.006,8.4588e-11
13.009,8.3166e-11
13.012,8.5269e-11
13.015,8.619e-11
13.018,8.6479e-11
13.021,8.6711e-11
13.024,8.641e-11
13.027,8.5109e-11
13.03,8.6702e-11
13.033,8.7629e-11
13.036,8.5161e-11
13.039,8.6858e-11
13.042,8.9568e-11
13.045,8.8375e-11
13.048,8.7984e-11
13.051,8.9293e-11
13.054,8.7805e-11
13.057,8.8269e-11
13.06,8.9094e-11
13.063,8.9539e-11
13.066,9.0089e-11
13.069,8.9953e-11
13.072,9.1512e-11
13.075,8.9723e-11
13.078,8.9989e-11
13.08,9.0836e-11
13.083,8.9402e-11
13.086,9.2124e-11
13.089,9.0538e-11
13.092,9.1369e-11
13.095,9.3346e-11
13.098,9.141e-11
13.101,9.1064e-11
13.104,9.1771e-11
13.107,9.4043e-11
13.11,9.4308e-11
13.113,9.4246e-11
13.116,9.4546e-11
13.119,9.4677e-11
13.122,9.3014e-11
13.125,9.3482e-11
13.128,9.5563e-11
13.131,9.4867e-11
13.134,9.5411e-11
13.137,9.8338e-11
13.14,9.472e-11
13.143,9.6849e-11
13.146,9.4788e-11
13.149,9.6637e-11
13.152,9.6337e-11
13.155,9.7088e-11
13.158,9.6983e-11
13.161,9.9503e-11
13.164,9.7721e-11
13.167,9.9965e-11
13.17,9.9583e-11
13.173,9.9624e-11
13.176,1.0156e-10
13.179,1.0008e-10
13.182,1.0138e-10
13.185,1.0016e-10
13.188,9.976e-11
13.191,1.0149e-10
13.194,9.9077e-11
13.197,1.0196e-10
13.2,1.0182e-10
13.203,1.0211e-10
13.206,1.0333e-10
13.209,1.023e-10
13.212,1.0317e-10
13.215,1.0362e-10
13.218,1.0297e-10
13.221,1.0302e-10
13.224,1.0228e-10
13.227,1.0307e-10
13.23,1.0395e-10
13.233,1.0365e-10
13.235,1.0318e-10
13.238,1.0523e-10
13.241,1.0544e-10
13.244,1.0618e-10
13.247,1.0685e-10
13.25,1.0654e-10
13.253,1.0582e-10
13.256,1.0886e-10
13.259,1.0602e-10
13.262,1.0731e-10
13.265,1.0924e-10
13.268,1.0853e-10
13.271,1.103e-10
13.274,1.0925e-10
13.277,1.1043e-10
13.28,1.0926e-10
13.283,1.0923e-10
13.286,1.12e-10
13.289,1.1244e-10
13.292,1.1097e-10
13.295,1.1014e-10
13.298,1.137e-10
13.301,1.1202e-10
13.304,1.1153e-10
13.307,1.1432e-10
13.31,1.1332e-10
13.313,1.1423e-10
13.316,1.1284e-10
13.319,1.1396e-10
13.322,1.1433e-10
13.325,1.136e-10
13.328,1.1448e-10
13.331,1.1519e-10
13.334,1.1261e-10
13.337,1.1529e-10
13.34,1.1679e-10
13.343,1.1744e-10
13.346,1.1681e-10
13.349,1.1442e-10
13.352,1.2024e-10
13.355,1.1993e-10
13.358,1.1888e-10
13.361,1.2081e-10
13.364,1.1892e-10
13.367,1.1633e-10
13.37,1.179e-10
13.373,1.2016e-10
13.376,1.2204e-10
13.379,1.206e-10
13.382,1.1783e-10
13.385,1.2297e-10
13.387,1.1845e-10
13.39,1.2102e-10
13.393,1.2203e-10
13.396,1.1778e-10
13.399,1.2434e-10
13.402,1.2093e-10
13.405,1.2474e-10
13.408,1.2262e-10
13.411,1.176e-10
13.414,1.2406e-10
13.417,1.2079e-10
13.42,1.2473e-10
13.423,1.263e-10
13.426,1.294e-10
13.429,1.2612e-10
13.432,1.2244e-10
13.435,1.2553e-10
13.438,1.2921e-10
13.441,1.2881e-10
13.444,1.2615e-10
13.447,1.3042e-10
13.45,1.2926e-10
13.453,1.2991e-10
13.456,1.2975e-10
13.459,1.3317e-10
13.462,1.3112e-10
13.465,1.275e-10
13.468,1.3062e-10
13.471,1.3465e-10
13.474,1.3145e-10
13.477,1.3383e-10
13.48,1.3394e-10
13.483,1.3445e-10
13.486,1.3687e-10
13.489,1.3221e-10
13.492,1.3895e-10
13.495,1.3734e-10
13.498,1.3413e-10
13.501,1.3641e-10
13.504,1.3674e-10
13.507,1.3761e-10
13.51,1.3506e-10
13.513,1.3926e-10
13.516,1.3842e-10
13.519,1.3997e-10
13.522,1.3961e-10
13.525,1.3739e-10
13.528,1.3871e-10
13.531,1.3749e-10
13.534,1.3664e-10
13.537,1.4164e-10
13.54,1.4061e-10
13.542,1.3935e-10
13.545,1.3918e-10
13.548,1.4563e-10
13.551,1.4004e-10
13.554,1.3976e-10
13.557,1.4271e-10
13.56,1.4245e-10
13.563,1.4292e-10
13.566,1.4331e-10
13.569,1.4576e-10
13.572,1.4761e-10
13.575,1.4766e-10
13.578,1.4669e-10
13.581,1.4286e-10
13.584,1.4628e-10
13.587,1.457e-10
13.59,1.4593e-10
13.593,1.4732e-10
13.596,1.5114e-10
13.599,1.4869e-10
13.602,1.5079e-10
13.605,1.5113e-10
13.608,1.4923e-10
13.611,1.5046e-10
13.614,1.5148e-10
13.617,1.5003e-10
13.62,1.4958e-10
13.623,1.5447e-10
13.626,1.5091e-10
13.629,1.5363e-10
13.632,1.5211e-10
13.635,1.5485e-10
13.638,1.5369e-10
13.641,1.5393e-10
13.644,1.5737e-10
13.647,1.5798e-10
13.65,1.5353e-10
13.653,1.5787e-10
13.656,1.5445e-10
13.659,1.5571e-10
13.662,1.556e-10
13.665,1.5814e-10
13.668,1.5457e-10
13.671,1.5813e-10
13.674,1.5667e-10
13.677,1.635e-10
13.68,1.6189e-10
13.683,1.5917e-10
13.686,1.6396e-10
13.689,1.614e-10
13.692,1.6242e-10
13.694,1.609e-10
13.697,1.6326e-10
13.7,1.6445e-10
13.703,1.6501e-10
13.706,1.6582e-10
13.709,1.6466e-10
13.712,1.6376e-10
13.715,1.6526e-10
13.718,1.6734e-10
13.721,1.6731e-10
13.724,1.6459e-10
13.727,1.6691e-10
13.73,1.6608e-10
13.733,1.6631e-10
13.736,1.7144e-10
13.739,1.7036e-10
13.742,1.7072e-10
13.745,1.7075e-10
13.748,1.7098e-10
13.751,1.6898e-10
13.754,1.7426e-10
13.757,1.7395e-10
13.76,1.7211e-10
13.763,1.7486e-10
13.766,1.7355e-10
13.769,1.7459e-10
13.772,1.7758e-10
13.775,1.7224e-10
13.778,1.7636e-10
13.781,1.7482e-10
13.784,1.7745e-10
13.787,1.8253e-10
13.79,1.7876e-10
13.793,1.8106e-10
13.796,1.8151e-10
13.799,1.8168e-10
13.802,1.7975e-10
13.805,1.8064e-10
13.808,1.8323e-10
13.811,1.8165e-10
13.814,1.8395e-10
13.817,1.8542e-10
13.82,1.8612e-10
13.823,1.8442e-10
13.826,1.8694e-10
13.829,1.8497e-10
13.832,1.8939e-10
13.835,1.8658e-10
13.838,1.8777e-10
13.841,1.8481e-10
13.844,1.8863e-10
13.847,1.9096e-10
13.849,1.8808e-10
13.852,1.9069e-10
13.855,1.8844e-10
13.858,1.9248e-10
13.861,1.9076e-10
13.864,1.9055e-10
13.867,1.9323e-10
13.87,1.9177e-10
13.873,1.925e-10
13.876,1.9674e-10
13.879,1.9469e-10
13.882,1.9488e-10
13.885,1.9629e-10
13.888,1.994e-10
13.891,1.9615e-10
13.894,1.9358e-10
13.897,1.9809e-10
13.9,1.947e-10
13.903,1.9628e-10
13.906,1.9973e-10
13.909,2.0077e-10
13.912,1.9711e-10
13.915,2.04e-10
13.918,2.0477e-10
13.921,2.0717e-10
13.924,2.0247e-10
13.927,2.0356e-10
13.93,2.0885e-10
13.933,2.0473e-10
13.936,2.031e-10
13.939,2.0746e-10
13.942,2.062e-10
13.945,2.0868e-10
13.948,2.1116e-10
13.951,2.0887e-10
13.954,2.1048e-10
13.957,2.1521e-10
13.96,2.1037e-10
13.963,2.1341e-10
13.966,2.1606e-10
13.969,2.1471e-10
13.972,2.1625e-10
13.975,2.1172e-10
13.978,2.1776e-10
13.981,2.1077e-10
13.984,2.2139e-10
13.987,2.1995e-10
13.99,2.2217e-10
13.993,2.2401e-10
13.996,2.189e-10
13.999,2.1735e-10
14.002,2.1896e-10
14.004,2.2108e-10
14.007,2.2486e-10
14.01,2.1943e-10
14.013,2.2892e-10
14.016,2.2565e-10
14.019,2.2394e-10
14.022,2.2164e-10
14.025,2.2489e-10
14.028,2.2616e-10
14.031,2.2827e-10
14.034,2.3024e-10
14.037,2.3245e-10
14.04,2.3318e-10
14.043,2.3143e-10
14.046,2.3001e-10
14.049,2.3242e-10
14.052,2.3598e-10
14.055,2.3041e-10
14.058,2.3079e-10
14.061,2.304e-10
14.064,2.3104e-10
14.067,2.3811e-10
14.07,2.3422e-10
14.073,2.3467e-10
14.076,2.365e-10
14.079,2.365e-10
14.082,2.3647e-10
14.085,2.3825e-10
14.088,2.4238e-10
14.091,2.3737e-10
14.094,2.3526e-10
14.097,2.375e-10
14.1,2.4584e-10
14.103,2.47e-10
14.106,2.4329e-10
14.109,2.4091e-10
14.112,2.4712e-10
14.115,2.4363e-10
14.118,2.3667e-10
14.121,2.4452e-10
14.124,2.4665e-10
14.127,2.5386e-10
14.13,2.5226e-10
14.133,2.4521e-10
14.136,2.5147e-10
14.139,2.5492e-10
14.142,2.5637e-10
14.145,2.531e-10
14.148,2.4917e-10
14.151,2.5202e-10
14.154,2.6346e-10
14.156,2.5524e-10
14.159,2.6094e-10
14.162,2.6212e-10
14.165,2.5817e-10
14.168,2.5416e-10
14.171,2.6072e-10
14.174,2.6317e-10
14.177,2.5877e-10
14.18,2.6775e-10
14.183,2.5853e-10
14.186,2.6654e-10
14.189,2.6952e-10
14.192,2.6739e-10
14.195,2.6821e-10
14.198,2.6484e-10
14.201,2.7452e-10
14.204,2.6829e-10
14.207,2.7054e-10
14.21,2.657e-10
14.213,2.689e-10
14.216,2.7377e-10
14.219,2.7462e-10
14.222,2.76e-10
14.225,2.733e-10
14.228,2.7758e-10
14.231,2.6896e-10
14.234,2.8389e-10
14.237,2.8693e-10
14.24,2.8411e-10
14.243,2.7062e-10
14.246,2.8385e-10
14.249,2.7937e-10
14.252,2.7876e-10
14.255,2.809e-10
14.258,2.8245e-10
14.261,2.9145e-10
14.264,2.8727e-10
14.267,2.9171e-10
14.27,2.946e-10
14.273,2.8792e-10
14.276,2.9375e-10
14.279,2.868e-10
14.282,2.8826e-10
14.285,2.8938e-10
14.288,2.9449e-10
14.291,2.9699e-10
14.294,3.0218e-10
14.297,2.977e-10
14.3,2.9875e-10
14.303,3.0236e-10
14.306,2.9462e-10
14.309,2.9548e-10
14.311,3.0177e-10
14.314,3.0258e-10
14.317,2.9901e-10
14.32,3.0358e-10
14.323,2.9706e-10
14.326,3.0591e-10
14.329,3.0076e-10
14.332,3.0498e-10
14.335,3.0603e-10
14.338,3.0375e-10
14.341,3.0461e-10
14.344,3.1114e-10
14.347,3.1452e-10
14.35,3.0919e-10
14.353,3.1431e-10
14.356,3.1199e-10
14.359,3.1417e-10
14.362,3.1282e-10
14.365,3.2011e-10
14.368,3.1482e-10
14.371,3.1784e-10
14.374,3.1456e-10
14.377,3.1973e-10
14.38,3.2257e-10
14.383,3.1662e-10
14.386,3.1764e-10
14.389,3.1925e-10
14.392,3.1819e-10
14.395,3.2994e-10
14.398,3.2539e-10
14.401,3.2491e-10
14.404,3.2925e-10
14.407,3.2955e-10
14.41,3.3187e-10
14.413,3.2895e-10
14.416,3.2862e-10
14.419,3.3771e-10
14.422,3.2955e-10
14.425,3.3775e-10
14.428,3.3576e-10
14.431,3.4198e-10
14.434,3.3411e-10
14.437,3.3502e-10
14.44,3.4065e-10
14.443,3.3524e-10
14.446,3.4871e-10
14.449,3.4443e-10
14.452,3.4494e-10
14.455,3.4862e-10
14.458,3.4758e-10
14.461,3.4484e-10
14.463,3.479e-10
14.466,3.5228e-10
14.469,3.5375e-10
14.472,3.5242e-10
14.475,3.5617e-10
14.478,3.5425e-10
14.481,3.6143e-10
14.484,3.6085e-10
14.487,3.5724e-10
14.49,3.5933e-10
14.493,3.5794e-10
14.496,3.5545e-10
14.499,3.5441e-10
14.502,3.6342e-10
14.505,3.6066e-10
14.508,3.7334e-10
14.511,3.6816e-10
14.514,3.7389e-10
14.517,3.6638e-10
14.52,3.6734e-10
14.523,3.6946e-10
14.526,3.7261e-10
14.529,3.7224e-10
14.532,3.759e-10
14.535,3.69e-10
14.538,3.7368e-10
14.541,3.8035e-10
14.544,3.8478e-10
14.547,3.8577e-10
14.55,3.8039e-10
14.553,3.8678e-10
14.556,3.7708e-10
14.559,3.9132e-10
14.562,3.9588e-10
14.565,3.914e-10
14.568,3.9376e-10
14.571,3.8901e-10
14.574,3.9662e-10
14.577,3.9152e-10
14.58,3.97e-10
14.583,3.9612e-10
14.586,3.9746e-10
14.589,3.9551e-10
14.592,3.9652e-10
14.595,3.9831e-10
14.598,3.9711e-10
14.601,4.0842e-10
14.604,4.041e-10
14.607,3.9963e-10
14.61,4.0594e-10
14.613,4.0802e-10
14.616,4.1304e-10
14.618,4.1517e-10
14.621,4.1122e-10
14.624,4.0987e-10
14.627,4.1983e-10
14.63,4.1522e-10
14.633,4.1188e-10
14.636,4.1641e-10
14.639,4.1902e-10
14.642,4.1935e-10
14.645,4.2164e-10
14.648,4.2963e-10
14.651,4.1986e-10
14.654,4.1993e-10
14.657,4.2109e-10
14.66,4.3069e-10
14.663,4.2553e-10
14.666,4.2653e-10
14.669,4.2742e-10
14.672,4.3059e-10
14.675,4.2886e-10
14.678,4.3254e-10
14.681,4.2651e-10
14.684,4.2945e-10
14.687,4.3328e-10
14.69,4.386e-10
14.693,4.4647e-10
14.696,4.4404e-10
14.699,4.4459e-10
14.702,4.4605e-10
14.705,4.4803e-10
14.708,4.4284e-10
14.711,4.4661e-10
14.714,4.5133e-10
14.717,4.4326e-10
14.72,4.4869e-10
14.723,4.5276e-10
14.726,4.5225e-10
14.729,4.4918e-10
14.732,4.4894e-10
14.735,4.7036e-10
14.738,4.585e-10
14.741,4.622e-10
14.744,4.5239e-10
14.747,4.5582e-10
14.75,4.6235e-10
14.753,4.7088e-10
14.756,4.5898e-10
14.759,4.8206e-10
14.762,4.7123e-10
14.765,4.6751e-10
14.768,4.7615e-10
14.77,4.7316e-10
14.773,4.8347e-10
14.776,4.6931e-10
14.779,4.7679e-10
14.782,4.8376e-10
14.785,4.7816e-10
14.788,4.8008e-10
14.791,4.8193e-10
14.794,4.9387e-10
14.797,4.8998e-10
14.8,4.8711e-10
14.803,4.9942e-10
14.806,4.8984e-10
14.809,4.8898e-10
14.812,4.9781e-10
14.815,4.994e-10
14.818,4.9881e-10
14.821,4.992e-10
14.824,4.996e-10
14.827,5.0658e-10
14.83,5.0657e-10
14.833,5.0702e-10
14.836,5.1555e-10
14.839,5.1488e-10
14.842,4.984e-10
14.845,5.1505e-10
14.848,5.1574e-10
14.851,5.0976e-10
14.854,5.2151e-10
14.857,5.1396e-10
14.86,5.2731e-10
14.863,5.3063e-10
14.866,5.3249e-10
14.869,5.311e-10
14.872,5.2218e-10
14.875,5.346e-10
14.878,5.2888e-10
14.881,5.2492e-10
14.884,5.3468e-10
14.887,5.3108e-10
14.89,5.3118e-10
14.893,5.4591e-10
14.896,5.2846e-10
14.899,5.3701e-10
14.902,5.43e-10
14.905,5.4543e-10
14.908,5.2944e-10
14.911,5.4565e-10
14.914,5.4451e-10
14.917,5.4821e-10
14.92,5.4814e-10
14.923,5.6489e-10
14.925,5.4728e-10
14.928,5.3835e-10
14.931,5.4722e-10
14.934,5.6873e-10
14.937,5.687e-10
14.94,5.6952e-10
14.943,5.7818e-10
14.946,5.7385e-10
14.949,5.6711e-10
14.952,5.745e-10
14.955,5.7696e-10
14.958,5.6626e-10
14.961,5.798e-10
14.964,5.8399e-10
14.967,5.693e-10
14.97,5.8573e-10
14.973,5.7941e-10
14.976,5.7766e-10
14.979,5.9501e-10
14.982,5.7724e-10
14.985,5.7814e-10
14.988,5.8354e-10
14.991,5.891e-10
14.994,6.0088e-10
14.997,5.8345e-10
15,6.0824e-10


==> quad_err_cosfunc.tex <==
0,7.7671e-13
0.005005,3.4851e-12
0.01001,5.4351e-12
0.015015,6.0847e-12
0.02002,6.7957e-12
0.025025,7.1494e-12
0.03003,7.2246e-12
0.035035,7.0855e-12
0.04004,6.7873e-12
0.045045,6.3731e-12
0.05005,5.8788e-12
0.055055,5.3345e-12
0.06006,4.7625e-12
0.065065,4.1818e-12
0.07007,3.6071e-12
0.075075,3.0479e-12
0.08008,2.5142e-12
0.085085,2.0107e-12
0.09009,1.5418e-12
0.095095,1.1098e-12
0.1001,7.1655e-13
0.10511,3.6119e-13
0.11011,4.4251e-14
0.11512,2.3572e-13
0.12012,4.8065e-13
0.12513,6.9191e-13
0.13013,4.7676e-13
0.13514,6.5897e-13
0.14014,8.1199e-13
0.14515,9.3809e-13
0.15015,1.0396e-12
0.15516,1.1191e-12
0.16016,1.1781e-12
0.16517,1.2194e-12
0.17017,1.244e-12
0.17518,1.2551e-12
0.18018,1.2533e-12
0.18519,1.241e-12
0.19019,1.2188e-12
0.1952,1.1891e-12
0.2002,1.1523e-12
0.20521,1.1102e-12
0.21021,1.0632e-12
0.21522,1.0128e-12
0.22022,9.5913e-13
0.22523,9.0396e-13
0.23023,8.4688e-13
0.23524,7.8928e-13
0.24024,7.3075e-13
0.24525,4.5113e-13
0.25025,4.1625e-13
0.25526,3.7957e-13
0.26026,3.4222e-13
0.26527,3.0394e-13
0.27027,2.659e-13
0.27528,2.2784e-13
0.28028,1.8974e-13
0.28529,1.5228e-13
0.29029,1.1599e-13
0.2953,8.0086e-14
0.3003,4.4834e-14
0.30531,1.1052e-14
0.31031,2.2193e-14
0.31532,5.3806e-14
0.32032,8.4315e-14
0.32533,1.1371e-13
0.33033,1.4169e-13
0.33534,1.684e-13
0.34034,1.9435e-13
0.34535,3.4843e-13
0.35035,3.5621e-13
0.35536,3.6491e-13
0.36036,3.7298e-13
0.36537,3.8226e-13
0.37037,3.9148e-13
0.37538,4.0078e-13
0.38038,4.1046e-13
0.38539,4.2008e-13
0.39039,4.2965e-13
0.3954,4.3901e-13
0.4004,4.4802e-13
0.40541,4.5756e-13
0.41041,4.6659e-13
0.41542,4.7542e-13
0.42042,4.8432e-13
0.42543,4.9272e-13
0.43043,5.0089e-13
0.43544,5.6714e-13
0.44044,5.6481e-13
0.44545,5.6369e-13
0.45045,5.6378e-13
0.45546,5.6449e-13
0.46046,5.6629e-13
0.46547,5.6841e-13
0.47047,5.7165e-13
0.47548,5.7492e-13
0.48048,5.7869e-13
0.48549,6.1182e-13
0.49049,6.0386e-13
0.4955,5.9902e-13
0.5005,5.9188e-13
0.50551,5.9662e-13
0.51051,5.9849e-13
0.51552,6.0184e-13
0.52052,6.067e-13
0.52553,6.1242e-13
0.53053,6.2981e-13
0.53554,6.3504e-13
0.54054,6.4082e-13
0.54555,6.4631e-13
0.55055,6.5236e-13
0.55556,6.5762e-13
0.56056,6.6326e-13
0.56557,6.6895e-13
0.57057,6.7453e-13
0.57558,6.7963e-13
0.58058,6.8494e-13
0.58559,6.9083e-13
0.59059,6.9589e-13
0.5956,7.0135e-13
0.6006,7.0685e-13
0.60561,7.1204e-13
0.61061,7.1727e-13
0.61562,7.2272e-13
0.62062,7.284e-13
0.62563,7.3357e-13
0.63063,7.3897e-13
0.63564,7.4404e-13
0.64064,7.4971e-13
0.64565,7.5485e-13
0.65065,7.606e-13
0.65566,7.6601e-13
0.66066,7.7127e-13
0.66567,7.7695e-13
0.67067,7.8229e-13
0.67568,7.8766e-13
0.68068,8.3852e-13
0.68569,8.4382e-13
0.69069,8.4875e-13
0.6957,8.5351e-13
0.7007,8.5829e-13
0.70571,8.633e-13
0.71071,8.6813e-13
0.71572,8.7299e-13
0.72072,8.7766e-13
0.72573,8.8235e-13
0.73073,8.8706e-13
0.73574,8.9179e-13
0.74074,8.9674e-13
0.74575,9.0129e-13
0.75075,9.0649e-13
0.75576,9.1128e-13
0.76076,9.1608e-13
0.76577,9.2111e-13
0.77077,9.2593e-13
0.77578,9.312e-13
0.78078,9.367e-13
0.78579,9.4156e-13
0.79079,9.4687e-13
0.7958,9.5196e-13
0.8008,9.5729e-13
0.80581,9.6307e-13
0.81081,9.6841e-13
0.81582,9.7409e-13
0.82082,9.7968e-13
0.82583,9.8492e-13
0.83083,9.9097e-13
0.83584,9.9668e-13
0.84084,1.0027e-12
0.84585,1.0089e-12
0.85085,1.0146e-12
0.85586,1.0201e-12
0.86086,1.0267e-12
0.86587,1.0326e-12
0.87087,1.039e-12
0.87588,1.0452e-12
0.88088,1.0514e-12
0.88589,1.0578e-12
0.89089,1.1473e-12
0.8959,1.1474e-12
0.9009,1.1478e-12
0.90591,1.1485e-12
0.91091,1.1493e-12
0.91592,1.1505e-12
0.92092,1.1524e-12
0.92593,1.1544e-12
0.93093,1.1565e-12
0.93594,1.1588e-12
0.94094,1.1617e-12
0.94595,1.1645e-12
0.95095,1.1675e-12
0.95596,1.1711e-12
0.96096,1.1746e-12
0.96597,1.1785e-12
0.97097,1.1827e-12
0.97598,1.187e-12
0.98098,1.1914e-12
0.98599,1.1959e-12
0.99099,1.2007e-12
0.996,1.206e-12
1.001,1.2111e-12
1.006,1.216e-12
1.011,1.2215e-12
1.016,1.2274e-12
1.021,1.2329e-12
1.026,1.2385e-12
1.031,1.2444e-12
1.036,1.2504e-12
1.041,1.2561e-12
1.046,1.2623e-12
1.0511,1.2688e-12
1.0561,1.2748e-12
1.0611,1.2813e-12
1.0661,1.2874e-12
1.0711,1.2938e-12
1.0761,1.3001e-12
1.0811,1.3068e-12
1.0861,1.313e-12
1.0911,1.3195e-12
1.0961,1.3259e-12
1.1011,1.3325e-12
1.1061,1.3391e-12
1.1111,1.3456e-12
1.1161,1.3522e-12
1.1211,1.359e-12
1.1261,1.3652e-12
1.1311,1.372e-12
1.1361,1.3782e-12
1.1411,1.3852e-12
1.1461,1.3915e-12
1.1512,1.3979e-12
1.1562,1.4042e-12
1.1612,1.4105e-12
1.1662,1.4173e-12
1.1712,1.4233e-12
1.1762,1.4296e-12
1.1812,1.4362e-12
1.1862,1.4428e-12
1.1912,1.4492e-12
1.1962,1.455e-12
1.2012,1.4615e-12
1.2062,1.4677e-12
1.2112,1.4738e-12
1.2162,1.48e-12
1.2212,1.4858e-12
1.2262,1.4927e-12
1.2312,1.4984e-12
1.2362,1.5044e-12
1.2412,1.5107e-12
1.2462,1.5168e-12
1.2513,1.5228e-12
1.2563,1.5286e-12
1.2613,1.5345e-12
1.2663,1.5405e-12
1.2713,1.5464e-12
1.2763,1.5525e-12
1.2813,1.5581e-12
1.2863,1.5639e-12
1.2913,1.5699e-12
1.2963,1.5757e-12
1.3013,1.5813e-12
1.3063,1.5871e-12
1.3113,1.593e-12
1.3163,1.5989e-12
1.3213,1.6046e-12
1.3263,1.6101e-12
1.3313,1.6158e-12
1.3363,1.6216e-12
1.3413,1.6272e-12
1.3463,1.6331e-12
1.3514,1.6385e-12
1.3564,1.6446e-12
1.3614,1.6504e-12
1.3664,1.6558e-12
1.3714,1.6616e-12
1.3764,1.6671e-12
1.3814,1.6732e-12
1.3864,1.679e-12
1.3914,1.6845e-12
1.3964,1.6901e-12
1.4014,1.696e-12
1.4064,1.7018e-12
1.4114,1.7075e-12
1.4164,1.7134e-12
1.4214,1.7189e-12
1.4264,1.7247e-12
1.4314,1.7305e-12
1.4364,1.7363e-12
1.4414,1.7423e-12
1.4464,1.7481e-12
1.4515,1.7541e-12
1.4565,1.7596e-12
1.4615,1.7655e-12
1.4665,1.7716e-12
1.4715,1.7775e-12
1.4765,1.7831e-12
1.4815,1.7893e-12
1.4865,1.7952e-12
1.4915,1.801e-12
1.4965,1.807e-12
1.5015,1.8128e-12
1.5065,1.8189e-12
1.5115,1.8249e-12
1.5165,1.831e-12
1.5215,1.837e-12
1.5265,1.8428e-12
1.5315,1.8491e-12
1.5365,1.8551e-12
1.5415,1.861e-12
1.5465,1.8672e-12
1.5516,1.8729e-12
1.5566,1.8792e-12
1.5616,1.8853e-12
1.5666,1.891e-12
1.5716,1.8973e-12
1.5766,1.9031e-12
1.5816,1.9093e-12
1.5866,1.9154e-12
1.5916,1.9213e-12
1.5966,1.9274e-12
1.6016,1.9332e-12
1.6066,1.9392e-12
1.6116,1.9452e-12
1.6166,1.9507e-12
1.6216,1.9568e-12
1.6266,1.9629e-12
1.6316,1.9687e-12
1.6366,1.9746e-12
1.6416,1.9801e-12
1.6466,1.9861e-12
1.6517,1.9915e-12
1.6567,1.9972e-12
1.6617,2.0029e-12
1.6667,2.0084e-12
1.6717,2.014e-12
1.6767,2.0192e-12
1.6817,2.0248e-12
1.6867,2.0301e-12
1.6917,2.0354e-12
1.6967,2.0406e-12
1.7017,2.0458e-12
1.7067,2.0507e-12
1.7117,2.0556e-12
1.7167,2.0606e-12
1.7217,2.0651e-12
1.7267,2.0699e-12
1.7317,2.0747e-12
1.7367,2.0789e-12
1.7417,2.0831e-12
1.7467,2.0873e-12
1.7518,2.0911e-12
1.7568,2.0956e-12
1.7618,2.0996e-12
1.7668,2.1033e-12
1.7718,2.1066e-12
1.7768,2.1099e-12
1.7818,2.1131e-12
1.7868,2.1164e-12
1.7918,2.1191e-12
1.7968,2.1219e-12
1.8018,2.1243e-12
1.8068,2.1271e-12
1.8118,2.1292e-12
1.8168,2.1311e-12
1.8218,2.1329e-12
1.8268,2.1344e-12
1.8318,2.1355e-12
1.8368,2.1368e-12
1.8418,2.1375e-12
1.8468,2.1384e-12
1.8519,2.1386e-12
1.8569,2.1387e-12
1.8619,2.1385e-12
1.8669,2.1382e-12
1.8719,2.137e-12
1.8769,2.1364e-12
1.8819,2.1353e-12
1.8869,2.1334e-12
1.8919,2.1319e-12
1.8969,2.1292e-12
1.9019,2.1266e-12
1.9069,2.1238e-12
1.9119,2.1205e-12
1.9169,2.1166e-12
1.9219,2.1126e-12
1.9269,2.1082e-12
1.9319,2.1035e-12
1.9369,2.0985e-12
1.9419,2.0927e-12
1.9469,2.0864e-12
1.952,2.08e-12
1.957,2.0733e-12
1.962,2.0658e-12
1.967,2.0577e-12
1.972,2.0494e-12
1.977,2.0406e-12
1.982,2.0314e-12
1.987,2.0214e-12
1.992,2.0111e-12
1.997,2e-12
2.002,1.9886e-12
2.007,1.9767e-12
2.012,1.9637e-12
2.017,1.9508e-12
2.022,1.9365e-12
2.027,1.9222e-12
2.032,1.907e-12
2.037,1.8916e-12
2.042,1.8749e-12
2.047,1.858e-12
2.0521,1.84e-12
2.0571,1.8215e-12
2.0621,1.8022e-12
2.0671,1.7823e-12
2.0721,1.7614e-12
2.0771,1.7399e-12
2.0821,1.7175e-12
2.0871,1.6948e-12
2.0921,1.6706e-12
2.0971,1.6457e-12
2.1021,1.6199e-12
2.1071,1.5935e-12
2.1121,1.5664e-12
2.1171,1.5379e-12
2.1221,1.5088e-12
2.1271,1.4783e-12
2.1321,1.4473e-12
2.1371,1.4152e-12
2.1421,1.3821e-12
2.1471,1.3475e-12
2.1522,1.3126e-12
2.1572,1.2764e-12
2.1622,1.2393e-12
2.1672,1.2006e-12
2.1722,1.1608e-12
2.1772,1.1199e-12
2.1822,1.0782e-12
2.1872,1.0349e-12
2.1922,9.9084e-13
2.1972,9.4511e-13
2.2022,8.9843e-13
2.2072,8.5006e-13
2.2122,8.0056e-13
2.2172,7.4993e-13
2.2222,6.9743e-13
2.2272,6.4362e-13
2.2322,5.8921e-13
2.2372,5.3294e-13
2.2422,4.75e-13
2.2472,4.1573e-13
2.2523,3.5478e-13
2.2573,2.9233e-13
2.2623,2.2855e-13
2.2673,1.6308e-13
2.2723,9.5927e-14
2.2773,2.7085e-14
2.2823,4.3451e-14
2.2873,1.155e-13
2.2923,1.8961e-13
2.2973,2.6524e-13
2.3023,3.4257e-13
2.3073,4.2197e-13
2.3123,5.0344e-13
2.3173,5.8609e-13
2.3223,6.7117e-13
2.3273,7.5833e-13
2.3323,8.4739e-13
2.3373,9.382e-13
2.3423,1.0309e-12
2.3473,1.1263e-12
2.3524,1.2232e-12
2.3574,1.3226e-12
2.3624,1.4243e-12
2.3674,1.5279e-12
2.3724,1.6339e-12
2.3774,1.7421e-12
2.3824,1.8527e-12
2.3874,1.9656e-12
2.3924,2.0809e-12
2.3974,2.1987e-12
2.4024,2.3192e-12
2.4074,2.4419e-12
2.4124,2.5673e-12
2.4174,2.6952e-12
2.4224,2.826e-12
2.4274,2.9591e-12
2.4324,3.0948e-12
2.4374,3.2334e-12
2.4424,3.3751e-12
2.4474,3.5193e-12
2.4525,3.6665e-12
2.4575,3.8166e-12
2.4625,3.9695e-12
2.4675,4.1254e-12
2.4725,4.2849e-12
2.4775,4.4469e-12
2.4825,4.6123e-12
2.4875,4.7806e-12
2.4925,4.9524e-12
2.4975,5.127e-12
2.5025,5.3054e-12
2.5075,5.4868e-12
2.5125,5.672e-12
2.5175,5.8606e-12
2.5225,6.0523e-12
2.5275,6.2479e-12
2.5325,6.4464e-12
2.5375,6.6491e-12
2.5425,6.8556e-12
2.5475,7.0657e-12
2.5526,7.2796e-12
2.5576,7.4972e-12
2.5626,7.7187e-12
2.5676,7.9438e-12
2.5726,8.1733e-12
2.5776,8.4068e-12
2.5826,8.6441e-12
2.5876,8.8857e-12
2.5926,9.1315e-12
2.5976,9.3813e-12
2.6026,9.6356e-12
2.6076,9.894e-12
2.6126,1.0157e-11
2.6176,1.0424e-11
2.6226,1.0696e-11
2.6276,1.0972e-11
2.6326,1.1253e-11
2.6376,1.1538e-11
2.6426,1.1828e-11
2.6476,1.2123e-11
2.6527,1.2423e-11
2.6577,1.2727e-11
2.6627,1.3036e-11
2.6677,1.335e-11
2.6727,1.367e-11
2.6777,1.3994e-11
2.6827,1.4323e-11
2.6877,1.4657e-11
2.6927,1.4997e-11
2.6977,1.5341e-11
2.7027,1.5691e-11
2.7077,1.6047e-11
2.7127,1.6407e-11
2.7177,1.6773e-11
2.7227,1.7145e-11
2.7277,1.7522e-11
2.7327,1.7905e-11
2.7377,1.8293e-11
2.7427,1.8687e-11
2.7477,1.9087e-11
2.7528,1.9492e-11
2.7578,1.9903e-11
2.7628,2.0321e-11
2.7678,2.0743e-11
2.7728,2.1172e-11
2.7778,2.1607e-11
2.7828,2.2048e-11
2.7878,2.2495e-11
2.7928,2.2948e-11
2.7978,2.3408e-11
2.8028,2.3873e-11
2.8078,2.4345e-11
2.8128,2.4823e-11
2.8178,2.5307e-11
2.8228,2.5798e-11
2.8278,2.6295e-11
2.8328,2.6799e-11
2.8378,2.7309e-11
2.8428,2.7825e-11
2.8478,2.8348e-11
2.8529,2.8878e-11
2.8579,2.9415e-11
2.8629,2.9958e-11
2.8679,3.0508e-11
2.8729,3.1063e-11
2.8779,3.1627e-11
2.8829,3.2197e-11
2.8879,3.2773e-11
2.8929,3.3356e-11
2.8979,3.3947e-11
2.9029,3.4544e-11
2.9079,3.5148e-11
2.9129,3.5758e-11
2.9179,3.6376e-11
2.9229,3.7001e-11
2.9279,3.7633e-11
2.9329,3.8272e-11
2.9379,3.8917e-11
2.9429,3.957e-11
2.9479,4.023e-11
2.953,4.0896e-11
2.958,4.157e-11
2.963,4.225e-11
2.968,4.2938e-11
2.973,4.3633e-11
2.978,4.4335e-11
2.983,4.5043e-11
2.988,4.5759e-11
2.993,4.6481e-11
2.998,4.7211e-11
3.003,4.7948e-11
3.008,4.8691e-11
3.013,4.9442e-11
3.018,5.02e-11
3.023,5.0965e-11
3.028,5.1736e-11
3.033,5.2514e-11
3.038,5.33e-11
3.043,5.4091e-11
3.048,5.489e-11
3.0531,5.5696e-11
3.0581,5.6509e-11
3.0631,5.7327e-11
3.0681,5.8153e-11
3.0731,5.8986e-11
3.0781,5.9825e-11
3.0831,6.0671e-11
3.0881,6.1523e-11
3.0931,6.2382e-11
3.0981,6.3247e-11
3.1031,6.4119e-11
3.1081,6.4997e-11
3.1131,6.5881e-11
3.1181,6.6771e-11
3.1231,6.7668e-11
3.1281,6.8571e-11
3.1331,6.9479e-11
3.1381,7.0394e-11
3.1431,7.1314e-11
3.1481,7.2241e-11
3.1532,7.3173e-11
3.1582,7.4111e-11
3.1632,7.5055e-11
3.1682,7.6004e-11
3.1732,7.6959e-11
3.1782,7.7919e-11
3.1832,7.8885e-11
3.1882,7.9856e-11
3.1932,8.0832e-11
3.1982,8.1813e-11
3.2032,8.2798e-11
3.2082,8.3789e-11
3.2132,8.4785e-11
3.2182,8.5786e-11
3.2232,8.6791e-11
3.2282,8.78e-11
3.2332,8.8814e-11
3.2382,8.9832e-11
3.2432,9.0855e-11
3.2482,9.1881e-11
3.2533,9.2912e-11
3.2583,9.3947e-11
3.2633,9.4985e-11
3.2683,9.6027e-11
3.2733,9.7072e-11
3.2783,9.8122e-11
3.2833,9.9174e-11
3.2883,1.0023e-10
3.2933,1.0129e-10
3.2983,1.0235e-10
3.3033,1.0341e-10
3.3083,1.0448e-10
3.3133,1.0555e-10
3.3183,1.0662e-10
3.3233,1.077e-10
3.3283,1.0878e-10
3.3333,1.0986e-10
3.3383,1.1094e-10
3.3433,1.1202e-10
3.3483,1.131e-10
3.3534,1.1419e-10
3.3584,1.1528e-10
3.3634,1.1637e-10
3.3684,1.1746e-10
3.3734,1.1855e-10
3.3784,1.1964e-10
3.3834,1.2074e-10
3.3884,1.2183e-10
3.3934,1.2293e-10
3.3984,1.2402e-10
3.4034,1.2512e-10
3.4084,1.2621e-10
3.4134,1.2731e-10
3.4184,1.284e-10
3.4234,1.295e-10
3.4284,1.306e-10
3.4334,1.3169e-10
3.4384,1.3278e-10
3.4434,1.3388e-10
3.4484,1.3497e-10
3.4535,1.3606e-10
3.4585,1.3715e-10
3.4635,1.3824e-10
3.4685,1.3933e-10
3.4735,1.4041e-10
3.4785,1.415e-10
3.4835,1.4258e-10
3.4885,1.4366e-10
3.4935,1.4474e-10
3.4985,1.4581e-10
3.5035,1.4689e-10
3.5085,1.4796e-10
3.5135,1.4903e-10
3.5185,1.5009e-10
3.5235,1.5116e-10
3.5285,1.5222e-10
3.5335,1.5327e-10
3.5385,1.5433e-10
3.5435,1.5538e-10
3.5485,1.5642e-10
3.5536,1.5747e-10
3.5586,1.5851e-10
3.5636,1.5954e-10
3.5686,1.6057e-10
3.5736,1.616e-10
3.5786,1.6262e-10
3.5836,1.6364e-10
3.5886,1.6465e-10
3.5936,1.6566e-10
3.5986,1.6667e-10
3.6036,1.6766e-10
3.6086,1.6866e-10
3.6136,1.6965e-10
3.6186,1.7063e-10
3.6236,1.7161e-10
3.6286,1.7258e-10
3.6336,1.7355e-10
3.6386,1.7451e-10
3.6436,1.7547e-10
3.6486,1.7641e-10
3.6537,1.7736e-10
3.6587,1.7829e-10
3.6637,1.7922e-10
3.6687,1.8015e-10
3.6737,1.8107e-10
3.6787,1.8198e-10
3.6837,1.8288e-10
3.6887,1.8378e-10
3.6937,1.8467e-10
3.6987,1.8555e-10
3.7037,1.8642e-10
3.7087,1.8729e-10
3.7137,1.8815e-10
3.7187,1.89e-10
3.7237,1.8985e-10
3.7287,1.9069e-10
3.7337,1.9152e-10
3.7387,1.9234e-10
3.7437,1.9315e-10
3.7487,1.9395e-10
3.7538,1.9475e-10
3.7588,1.9553e-10
3.7638,1.9631e-10
3.7688,1.9708e-10
3.7738,1.9784e-10
3.7788,1.9859e-10
3.7838,1.9934e-10
3.7888,2.0007e-10
3.7938,2.0079e-10
3.7988,2.0151e-10
3.8038,2.0221e-10
3.8088,2.0291e-10
3.8138,2.0359e-10
3.8188,2.0426e-10
3.8238,2.0493e-10
3.8288,2.0558e-10
3.8338,2.0623e-10
3.8388,2.0686e-10
3.8438,2.0748e-10
3.8488,2.081e-10
3.8539,2.087e-10
3.8589,2.0929e-10
3.8639,2.0987e-10
3.8689,2.1043e-10
3.8739,2.1099e-10
3.8789,2.1153e-10
3.8839,2.1207e-10
3.8889,2.1259e-10
3.8939,2.131e-10
3.8989,2.136e-10
3.9039,2.1408e-10
3.9089,2.1455e-10
3.9139,2.1502e-10
3.9189,2.1546e-10
3.9239,2.159e-10
3.9289,2.1632e-10
3.9339,2.1673e-10
3.9389,2.1713e-10
3.9439,2.1751e-10
3.9489,2.1788e-10
3.954,2.1823e-10
3.959,2.1858e-10
3.964,2.189e-10
3.969,2.1922e-10
3.974,2.1952e-10
3.979,2.198e-10
3.984,2.2007e-10
3.989,2.2033e-10
3.994,2.2057e-10
3.999,2.208e-10
4.004,2.2101e-10
4.009,2.212e-10
4.014,2.2138e-10
4.019,2.2154e-10
4.024,2.2169e-10
4.029,2.2182e-10
4.034,2.2194e-10
4.039,2.2204e-10
4.044,2.2212e-10
4.049,2.2219e-10
4.0541,2.2223e-10
4.0591,2.2226e-10
4.0641,2.2228e-10
4.0691,2.2227e-10
4.0741,2.2225e-10
4.0791,2.2221e-10
4.0841,2.2215e-10
4.0891,2.2208e-10
4.0941,2.2198e-10
4.0991,2.2187e-10
4.1041,2.2173e-10
4.1091,2.2158e-10
4.1141,2.214e-10
4.1191,2.2121e-10
4.1241,2.21e-10
4.1291,2.2077e-10
4.1341,2.2051e-10
4.1391,2.2024e-10
4.1441,2.1994e-10
4.1491,2.1962e-10
4.1542,2.1928e-10
4.1592,2.1892e-10
4.1642,2.1854e-10
4.1692,2.1813e-10
4.1742,2.1771e-10
4.1792,2.1726e-10
4.1842,2.1678e-10
4.1892,2.1628e-10
4.1942,2.1576e-10
4.1992,2.1522e-10
4.2042,2.1465e-10
4.2092,2.1405e-10
4.2142,2.1343e-10
4.2192,2.1279e-10
4.2242,2.1212e-10
4.2292,2.1142e-10
4.2342,2.107e-10
4.2392,2.0995e-10
4.2442,2.0917e-10
4.2492,2.0837e-10
4.2543,2.0754e-10
4.2593,2.0668e-10
4.2643,2.058e-10
4.2693,2.0488e-10
4.2743,2.0394e-10
4.2793,2.0297e-10
4.2843,2.0196e-10
4.2893,2.0093e-10
4.2943,1.9987e-10
4.2993,1.9877e-10
4.3043,1.9765e-10
4.3093,1.9649e-10
4.3143,1.9531e-10
4.3193,1.9409e-10
4.3243,1.9283e-10
4.3293,1.9155e-10
4.3343,1.9023e-10
4.3393,1.8888e-10
4.3443,1.8749e-10
4.3493,1.8607e-10
4.3544,1.8462e-10
4.3594,1.8312e-10
4.3644,1.816e-10
4.3694,1.8003e-10
4.3744,1.7843e-10
4.3794,1.768e-10
4.3844,1.7512e-10
4.3894,1.7341e-10
4.3944,1.7166e-10
4.3994,1.6987e-10
4.4044,1.6804e-10
4.4094,1.6617e-10
4.4144,1.6426e-10
4.4194,1.6231e-10
4.4244,1.6032e-10
4.4294,1.5828e-10
4.4344,1.5621e-10
4.4394,1.5409e-10
4.4444,1.5193e-10
4.4494,1.4972e-10
4.4545,1.4747e-10
4.4595,1.4518e-10
4.4645,1.4284e-10
4.4695,1.4045e-10
4.4745,1.3802e-10
4.4795,1.3555e-10
4.4845,1.3302e-10
4.4895,1.3045e-10
4.4945,1.2783e-10
4.4995,1.2516e-10
4.5045,1.2244e-10
4.5095,1.1967e-10
4.5145,1.1685e-10
4.5195,1.1398e-10
4.5245,1.1105e-10
4.5295,1.0808e-10
4.5345,1.0505e-10
4.5395,1.0197e-10
4.5445,9.8836e-11
4.5495,9.5647e-11
4.5546,9.2403e-11
4.5596,8.9104e-11
4.5646,8.5748e-11
4.5696,8.2336e-11
4.5746,7.8866e-11
4.5796,7.5339e-11
4.5846,7.1753e-11
4.5896,6.8108e-11
4.5946,6.4403e-11
4.5996,6.0638e-11
4.6046,5.6813e-11
4.6096,5.2926e-11
4.6146,4.8977e-11
4.6196,4.4965e-11
4.6246,4.089e-11
4.6296,3.6751e-11
4.6346,3.2547e-11
4.6396,2.8279e-11
4.6446,2.3945e-11
4.6496,1.9544e-11
4.6547,1.5077e-11
4.6597,1.0542e-11
4.6647,5.9392e-12
4.6697,1.2674e-12
4.6747,3.4736e-12
4.6797,8.2847e-12
4.6847,1.3166e-11
4.6897,1.8119e-11
4.6947,2.3143e-11
4.6997,2.8241e-11
4.7047,3.3411e-11
4.7097,3.8654e-11
4.7147,4.3972e-11
4.7197,4.9364e-11
4.7247,5.4833e-11
4.7297,6.0377e-11
4.7347,6.5997e-11
4.7397,7.1696e-11
4.7447,7.7471e-11
4.7497,8.3326e-11
4.7548,8.9259e-11
4.7598,9.5272e-11
4.7648,1.0137e-10
4.7698,1.0754e-10
4.7748,1.1379e-10
4.7798,1.2013e-10
4.7848,1.2655e-10
4.7898,1.3305e-10
4.7948,1.3964e-10
4.7998,1.4631e-10
4.8048,1.5307e-10
4.8098,1.5991e-10
4.8148,1.6683e-10
4.8198,1.7385e-10
4.8248,1.8095e-10
4.8298,1.8813e-10
4.8348,1.9541e-10
4.8398,2.0277e-10
4.8448,2.1023e-10
4.8498,2.1777e-10
4.8549,2.254e-10
4.8599,2.3312e-10
4.8649,2.4093e-10
4.8699,2.4884e-10
4.8749,2.5683e-10
4.8799,2.6492e-10
4.8849,2.731e-10
4.8899,2.8138e-10
4.8949,2.8975e-10
4.8999,2.9821e-10
4.9049,3.0676e-10
4.9099,3.1541e-10
4.9149,3.2416e-10
4.9199,3.33e-10
4.9249,3.4194e-10
4.9299,3.5097e-10
4.9349,3.601e-10
4.9399,3.6933e-10
4.9449,3.7865e-10
4.9499,3.8807e-10
4.955,3.9759e-10
4.96,4.0721e-10
4.965,4.1692e-10
4.97,4.2673e-10
4.975,4.3665e-10
4.98,4.4666e-10
4.985,4.5677e-10
4.99,4.6697e-10
4.995,4.7728e-10
5,4.8769e-10


==> quad_errors.tex <==
1e-05,2.7009e-07,2.8103e-07,5.631e-05
1e-06,4.2564e-08,4.8899e-08,1.9427e-05
1e-07,7.3652e-10,7.4875e-10,2.1602e-07
1e-08,2.2354e-11,2.712e-11,7.8163e-10
1e-09,6.4715e-12,7.2766e-12,2.5722e-09
1e-10,5.2641e-13,1.5509e-12,4.5584e-10


==> quad_errors_use_exact_int.tex <==
1e-05,3.1508e-08,1.603e-07,1.5689e-06
1e-06,4.0063e-09,2.9327e-08,1.683e-06
1e-07,2.8377e-10,2.1252e-09,1.1064e-07
1e-08,7.4698e-12,8.1423e-11,1.4668e-09
1e-09,6.29e-13,7.207e-12,7.4744e-10
1e-10,6.134e-14,1.5775e-12,4.0987e-11


==> quad_poles.tex <==
-3.4137,0
2.6198,0
-0.55262,1.1228
-0.55262,-1.1228
0.34902,1.0018
0.34902,-1.0018
-0.41045,0
0.60279,0.82612
0.60279,-0.82612
0.84098,0.62425
0.84098,-0.62425
0.96312,0.51641
0.96312,-0.51641
1.0798,0.40705
1.0798,-0.40705
1.1744,0.30347
1.1744,-0.30347
1.2441,0.19643
1.2441,-0.19643
1.3377,0
1.2944,0.084266
1.2944,-0.084266
-0.15567,0
-0.072563,0
-0.035998,0
-0.018275,0
-0.0093442,0
-0.0047777,0
-0.0024358,0
-0.001238,0
-0.00062805,0
-0.00031854,0
-0.00016168,0
-8.2111e-05,0
-4.1637e-05,0
-2.0982e-05,0
-1.042e-05,0
-5.0255e-06,0
-2.2935e-06,0
-9.486e-07,0
-3.2953e-07,0
-8.1382e-08,0
-8.0753e-09,0


==> quad_sing_err_besselfunc.tex <==
0.1,2.8721e-13,2.1316e-13
0.10298,2.8721e-13,2.0739e-13
0.10596,2.8733e-13,2.025e-13
0.10894,2.8733e-13,1.9762e-13
0.11192,2.8721e-13,1.9273e-13
0.1149,2.8721e-13,1.8785e-13
0.11788,2.8733e-13,1.8296e-13
0.12086,2.8744e-13,1.7897e-13
0.12384,2.8733e-13,1.7364e-13
0.12683,2.871e-13,1.7009e-13
0.12981,2.8755e-13,1.6565e-13
0.13279,2.8733e-13,1.6209e-13
0.13577,2.871e-13,1.5721e-13
0.13875,2.8733e-13,1.5277e-13
0.14173,2.8733e-13,1.4988e-13
0.14471,2.8744e-13,1.4633e-13
0.14769,2.8744e-13,1.4189e-13
0.15067,2.8733e-13,1.3833e-13
0.15365,2.8744e-13,1.3523e-13
0.15663,2.8744e-13,1.3212e-13
0.15961,2.8733e-13,1.2812e-13
0.16259,2.8744e-13,1.2501e-13
0.16557,2.871e-13,1.2079e-13
0.16855,2.8766e-13,1.1835e-13
0.17153,2.8755e-13,1.1524e-13
0.17451,2.8744e-13,1.1191e-13
0.1775,2.8744e-13,1.0902e-13
0.18048,2.8744e-13,1.0569e-13
0.18346,2.8744e-13,1.0281e-13
0.18644,2.8766e-13,1.0014e-13
0.18942,2.8744e-13,9.7033e-14
0.1924,2.8755e-13,9.4147e-14
0.19538,2.8755e-13,9.1482e-14
0.19836,2.8777e-13,8.8596e-14
0.20134,2.8766e-13,8.5487e-14
0.20432,2.8777e-13,8.3267e-14
0.2073,2.8766e-13,8.0158e-14
0.21028,2.8788e-13,7.7938e-14
0.21326,2.8766e-13,7.5717e-14
0.21624,2.8777e-13,7.2831e-14
0.21922,2.8777e-13,6.9944e-14
0.2222,2.8766e-13,6.7946e-14
0.22519,2.8788e-13,6.6169e-14
0.22817,2.8788e-13,6.3505e-14
0.23115,2.8788e-13,6.0618e-14
0.23413,2.8788e-13,5.8842e-14
0.23711,2.8788e-13,5.5733e-14
0.24009,2.881e-13,5.3957e-14
0.24307,2.8788e-13,5.1958e-14
0.24605,2.8788e-13,4.9294e-14
0.24903,2.8788e-13,4.7518e-14
0.25201,2.8799e-13,4.4853e-14
0.25499,2.8788e-13,4.3077e-14
0.25797,2.8799e-13,4.0634e-14
0.26095,2.881e-13,3.8414e-14
0.26393,2.8821e-13,3.6637e-14
0.26691,2.8777e-13,3.5305e-14
0.26989,2.8788e-13,3.2863e-14
0.27287,2.881e-13,3.1086e-14
0.27586,2.8844e-13,2.8644e-14
0.27884,2.8821e-13,2.7089e-14
0.28182,2.8832e-13,2.5091e-14
0.2848,2.8832e-13,2.3537e-14
0.28778,2.8844e-13,2.1094e-14
0.29076,2.881e-13,1.9762e-14
0.29374,2.8832e-13,1.7764e-14
0.29672,2.8821e-13,1.5765e-14
0.2997,2.8821e-13,1.4211e-14
0.30268,2.8832e-13,1.2434e-14
0.30566,2.8821e-13,1.0436e-14
0.30864,2.8844e-13,8.6597e-15
0.31162,2.881e-13,7.3275e-15
0.3146,2.8855e-13,5.5511e-15
0.31758,2.8855e-13,3.7748e-15
0.32056,2.8855e-13,1.9984e-15
0.32354,2.8844e-13,2.2204e-16
0.32653,2.8877e-13,8.8818e-16
0.32951,2.8855e-13,2.6645e-15
0.33249,2.8832e-13,4.6629e-15
0.33547,2.8855e-13,6.2172e-15
0.33845,2.8877e-13,7.3275e-15
0.34143,2.8844e-13,9.5479e-15
0.34441,2.8855e-13,1.0658e-14
0.34739,2.8888e-13,1.199e-14
0.35037,2.8855e-13,1.3989e-14
0.35335,2.8855e-13,1.5543e-14
0.35633,2.8866e-13,1.6875e-14
0.35931,2.8866e-13,1.8208e-14
0.36229,2.8888e-13,1.9984e-14
0.36527,2.8899e-13,2.176e-14
0.36825,2.8899e-13,2.2871e-14
0.37123,2.8888e-13,2.4203e-14
0.37421,2.8899e-13,2.5757e-14
0.3772,2.8899e-13,2.7311e-14
0.38018,2.891e-13,2.8866e-14
0.38316,2.891e-13,3.042e-14
0.38614,2.8899e-13,3.1974e-14
0.38912,2.8921e-13,3.3307e-14
0.3921,2.8899e-13,3.4417e-14
0.39508,2.891e-13,3.5083e-14
0.39806,2.8921e-13,3.6859e-14
0.40104,2.8888e-13,3.8192e-14
0.40402,2.891e-13,3.908e-14
0.407,2.8921e-13,4.0856e-14
0.40998,2.8932e-13,4.1966e-14
0.41296,2.8955e-13,4.3743e-14
0.41594,2.8944e-13,4.4631e-14
0.41892,2.8944e-13,4.6185e-14
0.4219,2.8921e-13,4.7073e-14
0.42488,2.8955e-13,4.8628e-14
0.42787,2.8932e-13,4.9738e-14
0.43085,2.8932e-13,5.1514e-14
0.43383,2.8932e-13,5.218e-14
0.43681,2.8944e-13,5.3291e-14
0.43979,2.8944e-13,5.4623e-14
0.44277,2.8977e-13,5.6177e-14
0.44575,2.8977e-13,5.751e-14
0.44873,2.8977e-13,5.8398e-14
0.45171,2.8955e-13,6.0174e-14
0.45469,2.8966e-13,6.084e-14
0.45767,2.8977e-13,6.1728e-14
0.46065,2.8988e-13,6.3061e-14
0.46363,2.8988e-13,6.4171e-14
0.46661,2.8999e-13,6.5281e-14
0.46959,2.8999e-13,6.6613e-14
0.47257,2.8999e-13,6.7946e-14
0.47556,2.901e-13,6.8834e-14
0.47854,2.8988e-13,7.0166e-14
0.48152,2.9021e-13,7.0832e-14
0.4845,2.901e-13,7.1942e-14
0.48748,2.901e-13,7.3053e-14
0.49046,2.8999e-13,7.3941e-14
0.49344,2.901e-13,7.5273e-14
0.49642,2.9032e-13,7.6383e-14
0.4994,2.9032e-13,7.7272e-14
0.50238,2.9055e-13,7.8382e-14
0.50536,2.9055e-13,7.9492e-14
0.50834,2.9021e-13,8.0824e-14
0.51132,2.9055e-13,8.1934e-14
0.5143,2.9055e-13,8.2601e-14
0.51728,2.9032e-13,8.3711e-14
0.52026,2.9077e-13,8.4377e-14
0.52324,2.9077e-13,8.5709e-14
0.52623,2.9077e-13,8.7264e-14
0.52921,2.9077e-13,8.7708e-14
0.53219,2.9066e-13,8.793e-14
0.53517,2.9043e-13,8.9928e-14
0.53815,2.9077e-13,9.0816e-14
0.54113,2.9055e-13,9.1926e-14
0.54411,2.9088e-13,9.2815e-14
0.54709,2.9099e-13,9.4147e-14
0.55007,2.911e-13,9.4369e-14
0.55305,2.9132e-13,9.5479e-14
0.55603,2.9099e-13,9.6811e-14
0.55901,2.911e-13,9.7256e-14
0.56199,2.9121e-13,9.8366e-14
0.56497,2.9099e-13,9.9254e-14
0.56795,2.9132e-13,1.0036e-13
0.57093,2.9132e-13,1.0103e-13
0.57391,2.9132e-13,1.0214e-13
0.5769,2.9143e-13,1.0281e-13
0.57988,2.9121e-13,1.0392e-13
0.58286,2.9143e-13,1.0503e-13
0.58584,2.9154e-13,1.0569e-13
0.58882,2.9154e-13,1.068e-13
0.5918,2.9166e-13,1.0747e-13
0.59478,2.9154e-13,1.0858e-13
0.59776,2.9199e-13,1.0902e-13
0.60074,2.9166e-13,1.0991e-13
0.60372,2.9177e-13,1.1136e-13
0.6067,2.9177e-13,1.1213e-13
0.60968,2.9199e-13,1.1291e-13
0.61266,2.9177e-13,1.1335e-13
0.61564,2.9188e-13,1.1469e-13
0.61862,2.9199e-13,1.1557e-13
0.6216,2.9177e-13,1.1602e-13
0.62458,2.9199e-13,1.1691e-13
0.62757,2.9199e-13,1.1768e-13
0.63055,2.9199e-13,1.1879e-13
0.63353,2.9221e-13,1.1935e-13
0.63651,2.9188e-13,1.2024e-13
0.63949,2.9254e-13,1.2146e-13
0.64247,2.9232e-13,1.2168e-13
0.64545,2.921e-13,1.2257e-13
0.64843,2.9243e-13,1.2368e-13
0.65141,2.9277e-13,1.2434e-13
0.65439,2.9254e-13,1.2568e-13
0.65737,2.9243e-13,1.2623e-13
0.66035,2.9277e-13,1.2657e-13
0.66333,2.9277e-13,1.2768e-13
0.66631,2.9265e-13,1.2845e-13
0.66929,2.9277e-13,1.2945e-13
0.67227,2.9288e-13,1.3012e-13
0.67526,2.9299e-13,1.309e-13
0.67824,2.9299e-13,1.3167e-13
0.68122,2.931e-13,1.3245e-13
0.6842,2.9299e-13,1.3312e-13
0.68718,2.9288e-13,1.3367e-13
0.69016,2.931e-13,1.3467e-13
0.69314,2.9321e-13,1.3545e-13
0.69612,2.931e-13,1.36e-13
0.6991,2.9332e-13,1.3689e-13
0.70208,2.9321e-13,1.3778e-13
0.70506,2.9332e-13,1.3867e-13
0.70804,2.9332e-13,1.39e-13
0.71102,2.9343e-13,1.4011e-13
0.714,2.9343e-13,1.4067e-13
0.71698,2.9377e-13,1.4178e-13
0.71996,2.9377e-13,1.4166e-13
0.72294,2.9354e-13,1.4289e-13
0.72593,2.9343e-13,1.4388e-13
0.72891,2.9365e-13,1.4444e-13
0.73189,2.9399e-13,1.4488e-13
0.73487,2.9399e-13,1.4577e-13
0.73785,2.9354e-13,1.4666e-13
0.74083,2.9388e-13,1.4699e-13
0.74381,2.9399e-13,1.481e-13
0.74679,2.9399e-13,1.4866e-13
0.74977,2.9377e-13,1.4932e-13
0.75275,2.941e-13,1.501e-13
0.75573,2.941e-13,1.5077e-13
0.75871,2.9421e-13,1.5143e-13
0.76169,2.9432e-13,1.5243e-13
0.76467,2.9443e-13,1.5277e-13
0.76765,2.9454e-13,1.5354e-13
0.77063,2.9476e-13,1.5399e-13
0.77361,2.9465e-13,1.5454e-13
0.7766,2.9465e-13,1.5565e-13
0.77958,2.9465e-13,1.5632e-13
0.78256,2.9454e-13,1.5699e-13
0.78554,2.9476e-13,1.5776e-13
0.78852,2.9465e-13,1.5821e-13
0.7915,2.9488e-13,1.5921e-13
0.79448,2.9476e-13,1.5976e-13
0.79746,2.951e-13,1.5998e-13
0.80044,2.9488e-13,1.612e-13
0.80342,2.951e-13,1.6154e-13
0.8064,2.9521e-13,1.6198e-13
0.80938,2.951e-13,1.6309e-13
0.81236,2.9521e-13,1.6354e-13
0.81534,2.9554e-13,1.6398e-13
0.81832,2.9532e-13,1.6454e-13
0.8213,2.951e-13,1.6553e-13
0.82428,2.9521e-13,1.6587e-13
0.82727,2.9565e-13,1.6664e-13
0.83025,2.9543e-13,1.6709e-13
0.83323,2.9554e-13,1.6764e-13
0.83621,2.9565e-13,1.6875e-13
0.83919,2.9576e-13,1.6931e-13
0.84217,2.9587e-13,1.6975e-13
0.84515,2.9565e-13,1.7053e-13
0.84813,2.9599e-13,1.7109e-13
0.85111,2.9587e-13,1.7186e-13
0.85409,2.9599e-13,1.7242e-13
0.85707,2.961e-13,1.7286e-13
0.86005,2.961e-13,1.7364e-13
0.86303,2.9621e-13,1.7386e-13
0.86601,2.9621e-13,1.7519e-13
0.86899,2.9632e-13,1.7586e-13
0.87197,2.9643e-13,1.7608e-13
0.87495,2.9643e-13,1.7686e-13
0.87794,2.9632e-13,1.7764e-13
0.88092,2.9676e-13,1.7752e-13
0.8839,2.9654e-13,1.7819e-13
0.88688,2.9676e-13,1.7919e-13
0.88986,2.9665e-13,1.7986e-13
0.89284,2.9676e-13,1.8019e-13
0.89582,2.9687e-13,1.8097e-13
0.8988,2.9687e-13,1.8152e-13
0.90178,2.9676e-13,1.823e-13
0.90476,2.9687e-13,1.8208e-13
0.90774,2.971e-13,1.8319e-13
0.91072,2.9732e-13,1.8341e-13
0.9137,2.9743e-13,1.8374e-13
0.91668,2.9732e-13,1.8496e-13
0.91966,2.9721e-13,1.8541e-13
0.92264,2.9721e-13,1.8618e-13
0.92563,2.9732e-13,1.8696e-13
0.92861,2.9765e-13,1.8718e-13
0.93159,2.9754e-13,1.8785e-13
0.93457,2.9754e-13,1.8863e-13
0.93755,2.9765e-13,1.8918e-13
0.94053,2.9776e-13,1.8929e-13
0.94351,2.9787e-13,1.8996e-13
0.94649,2.9776e-13,1.9074e-13
0.94947,2.9798e-13,1.9129e-13
0.95245,2.9809e-13,1.9174e-13
0.95543,2.9809e-13,1.9229e-13
0.95841,2.9821e-13,1.9262e-13
0.96139,2.9798e-13,1.9318e-13
0.96437,2.9832e-13,1.9384e-13
0.96735,2.9832e-13,1.9496e-13
0.97033,2.9821e-13,1.9507e-13
0.97331,2.9821e-13,1.9573e-13
0.9763,2.9821e-13,1.964e-13
0.97928,2.9843e-13,1.9673e-13
0.98226,2.9854e-13,1.9729e-13
0.98524,2.9854e-13,1.9806e-13
0.98822,2.9865e-13,1.984e-13
0.9912,2.9898e-13,1.9884e-13
0.99418,2.9876e-13,1.9906e-13
0.99716,2.9887e-13,1.9995e-13
1.0001,2.9898e-13,2.004e-13
1.0031,2.9876e-13,2.0117e-13
1.0061,2.9909e-13,2.0162e-13
1.0091,2.9898e-13,2.0239e-13
1.0121,2.9909e-13,2.0262e-13
1.015,2.9909e-13,2.0339e-13
1.018,2.9921e-13,2.0406e-13
1.021,2.9954e-13,2.0428e-13
1.024,2.9932e-13,2.0473e-13
1.027,2.9954e-13,2.0539e-13
1.0299,2.9976e-13,2.0572e-13
1.0329,2.9987e-13,2.065e-13
1.0359,2.9965e-13,2.075e-13
1.0389,2.9976e-13,2.075e-13
1.0419,2.9998e-13,2.0806e-13
1.0448,2.9998e-13,2.0861e-13
1.0478,2.9987e-13,2.0928e-13
1.0508,2.9998e-13,2.0972e-13
1.0538,3.0009e-13,2.1017e-13
1.0568,3.002e-13,2.1039e-13
1.0598,3.002e-13,2.1116e-13
1.0627,3.002e-13,2.1161e-13
1.0657,3.0054e-13,2.1227e-13
1.0687,3.0054e-13,2.1272e-13
1.0717,3.0076e-13,2.1316e-13
1.0747,3.0032e-13,2.1361e-13
1.0776,3.0076e-13,2.1383e-13
1.0806,3.0065e-13,2.1472e-13
1.0836,3.0087e-13,2.1527e-13
1.0866,3.0076e-13,2.1572e-13
1.0896,3.0076e-13,2.1605e-13
1.0925,3.012e-13,2.1649e-13
1.0955,3.0109e-13,2.1705e-13
1.0985,3.012e-13,2.176e-13
1.1015,3.012e-13,2.1794e-13
1.1045,3.0109e-13,2.1894e-13
1.1074,3.012e-13,2.1894e-13
1.1104,3.012e-13,2.196e-13
1.1134,3.0143e-13,2.2005e-13
1.1164,3.0154e-13,2.2038e-13
1.1194,3.0154e-13,2.2082e-13
1.1223,3.0154e-13,2.2127e-13
1.1253,3.0187e-13,2.2216e-13
1.1283,3.0165e-13,2.226e-13
1.1313,3.0176e-13,2.2293e-13
1.1343,3.0198e-13,2.2338e-13
1.1372,3.0198e-13,2.2382e-13
1.1402,3.0187e-13,2.2427e-13
1.1432,3.0198e-13,2.2482e-13
1.1462,3.022e-13,2.2526e-13
1.1492,3.022e-13,2.2571e-13
1.1522,3.022e-13,2.2649e-13
1.1551,3.0209e-13,2.2693e-13
1.1581,3.0254e-13,2.2737e-13
1.1611,3.0242e-13,2.2782e-13
1.1641,3.0265e-13,2.2826e-13
1.1671,3.0254e-13,2.2882e-13
1.17,3.0276e-13,2.2904e-13
1.173,3.0298e-13,2.2937e-13
1.176,3.0276e-13,2.3004e-13
1.179,3.0298e-13,2.307e-13
1.182,3.0287e-13,2.3137e-13
1.1849,3.0287e-13,2.3159e-13
1.1879,3.0309e-13,2.3204e-13
1.1909,3.0309e-13,2.3226e-13
1.1939,3.0309e-13,2.3281e-13
1.1969,3.0331e-13,2.3326e-13
1.1998,3.0331e-13,2.3404e-13
1.2028,3.0353e-13,2.3415e-13
1.2058,3.0342e-13,2.3437e-13
1.2088,3.0376e-13,2.3481e-13
1.2118,3.0365e-13,2.3531e-13
1.2147,3.0365e-13,2.3631e-13
1.2177,3.0387e-13,2.3648e-13
1.2207,3.0387e-13,2.3714e-13
1.2237,3.0387e-13,2.3714e-13
1.2267,3.0353e-13,2.3792e-13
1.2296,3.0431e-13,2.3831e-13
1.2326,3.042e-13,2.3909e-13
1.2356,3.0431e-13,2.3936e-13
1.2386,3.0431e-13,2.4009e-13
1.2416,3.042e-13,2.4014e-13
1.2445,3.0431e-13,2.4059e-13
1.2475,3.0442e-13,2.4108e-13
1.2505,3.0442e-13,2.4142e-13
1.2535,3.0442e-13,2.4203e-13
1.2565,3.0465e-13,2.4247e-13
1.2595,3.0487e-13,2.4281e-13
1.2624,3.0476e-13,2.4336e-13
1.2654,3.052e-13,2.4375e-13
1.2684,3.0498e-13,2.443e-13
1.2714,3.0476e-13,2.4469e-13
1.2744,3.052e-13,2.4525e-13
1.2773,3.052e-13,2.4553e-13
1.2803,3.0509e-13,2.4608e-13
1.2833,3.0553e-13,2.4653e-13
1.2863,3.0542e-13,2.4686e-13
1.2893,3.0564e-13,2.4714e-13
1.2922,3.0576e-13,2.4736e-13
1.2952,3.0531e-13,2.4819e-13
1.2982,3.0564e-13,2.4858e-13
1.3012,3.0564e-13,2.4908e-13
1.3042,3.0564e-13,2.4963e-13
1.3071,3.0598e-13,2.4974e-13
1.3101,3.0609e-13,2.5063e-13
1.3131,3.0631e-13,2.5085e-13
1.3161,3.0609e-13,2.5174e-13
1.3191,3.062e-13,2.5147e-13
1.322,3.062e-13,2.5191e-13
1.325,3.062e-13,2.5296e-13
1.328,3.0653e-13,2.5324e-13
1.331,3.0631e-13,2.5341e-13
1.334,3.0664e-13,2.5407e-13
1.3369,3.0631e-13,2.5457e-13
1.3399,3.0664e-13,2.548e-13
1.3429,3.0653e-13,2.553e-13
1.3459,3.0653e-13,2.5546e-13
1.3489,3.0675e-13,2.5596e-13
1.3519,3.0709e-13,2.5652e-13
1.3548,3.0698e-13,2.5696e-13
1.3578,3.0709e-13,2.5707e-13
1.3608,3.072e-13,2.5763e-13
1.3638,3.0709e-13,2.584e-13
1.3668,3.0709e-13,2.5857e-13
1.3697,3.0742e-13,2.5907e-13
1.3727,3.072e-13,2.5968e-13
1.3757,3.0731e-13,2.5979e-13
1.3787,3.0731e-13,2.6046e-13
1.3817,3.0753e-13,2.6062e-13
1.3846,3.0764e-13,2.6129e-13
1.3876,3.0775e-13,2.6168e-13
1.3906,3.0775e-13,2.6185e-13
1.3936,3.0775e-13,2.6223e-13
1.3966,3.0775e-13,2.6273e-13
1.3995,3.0786e-13,2.6318e-13
1.4025,3.0831e-13,2.6396e-13
1.4055,3.0798e-13,2.639e-13
1.4085,3.0842e-13,2.6468e-13
1.4115,3.0809e-13,2.6495e-13
1.4144,3.082e-13,2.6518e-13
1.4174,3.082e-13,2.6612e-13
1.4204,3.0842e-13,2.6656e-13
1.4234,3.0864e-13,2.6668e-13
1.4264,3.0864e-13,2.6723e-13
1.4293,3.0875e-13,2.6729e-13
1.4323,3.0886e-13,2.6784e-13
1.4353,3.0875e-13,2.6845e-13
1.4383,3.0898e-13,2.6856e-13
1.4413,3.0886e-13,2.6928e-13
1.4442,3.0931e-13,2.6917e-13
1.4472,3.0875e-13,2.699e-13
1.4502,3.092e-13,2.7039e-13
1.4532,3.0909e-13,2.7062e-13
1.4562,3.0898e-13,2.7117e-13
1.4592,3.0909e-13,2.7173e-13
1.4621,3.0931e-13,2.7245e-13
1.4651,3.0942e-13,2.7217e-13
1.4681,3.0964e-13,2.7289e-13
1.4711,3.0942e-13,2.7317e-13
1.4741,3.0953e-13,2.7373e-13
1.477,3.0975e-13,2.7406e-13
1.48,3.0986e-13,2.7456e-13
1.483,3.0975e-13,2.7489e-13
1.486,3.0986e-13,2.7567e-13
1.489,3.0997e-13,2.7561e-13
1.4919,3.1031e-13,2.7589e-13
1.4949,3.1031e-13,2.765e-13
1.4979,3.1009e-13,2.7711e-13
1.5009,3.1031e-13,2.7717e-13
1.5039,3.1064e-13,2.7783e-13
1.5068,3.1042e-13,2.7828e-13
1.5098,3.1064e-13,2.785e-13
1.5128,3.1031e-13,2.79e-13
1.5158,3.1075e-13,2.7944e-13
1.5188,3.1053e-13,2.8e-13
1.5217,3.1042e-13,2.8011e-13
1.5247,3.1075e-13,2.8066e-13
1.5277,3.1086e-13,2.8128e-13
1.5307,3.1108e-13,2.8139e-13
1.5337,3.1097e-13,2.8161e-13
1.5366,3.1108e-13,2.8233e-13
1.5396,3.112e-13,2.8255e-13
1.5426,3.1097e-13,2.8327e-13
1.5456,3.1131e-13,2.8333e-13
1.5486,3.1108e-13,2.8377e-13
1.5516,3.1131e-13,2.8427e-13
1.5545,3.1164e-13,2.8466e-13
1.5575,3.1164e-13,2.8477e-13
1.5605,3.1164e-13,2.8533e-13
1.5635,3.1175e-13,2.8583e-13
1.5665,3.1197e-13,2.8633e-13
1.5694,3.1164e-13,2.8672e-13
1.5724,3.1186e-13,2.8721e-13
1.5754,3.1175e-13,2.8744e-13
1.5784,3.1164e-13,2.876e-13
1.5814,3.1208e-13,2.8816e-13
1.5843,3.1197e-13,2.8855e-13
1.5873,3.1219e-13,2.8921e-13
1.5903,3.1242e-13,2.8944e-13
1.5933,3.1219e-13,2.8993e-13
1.5963,3.1275e-13,2.8999e-13
1.5992,3.1219e-13,2.906e-13
1.6022,3.1242e-13,2.9099e-13
1.6052,3.1264e-13,2.9127e-13
1.6082,3.1231e-13,2.9199e-13
1.6112,3.1242e-13,2.9216e-13
1.6141,3.1275e-13,2.9249e-13
1.6171,3.1264e-13,2.9315e-13
1.6201,3.1286e-13,2.9338e-13
1.6231,3.1308e-13,2.9399e-13
1.6261,3.1319e-13,2.9426e-13
1.629,3.1297e-13,2.9454e-13
1.632,3.1308e-13,2.9499e-13
1.635,3.133e-13,2.9526e-13
1.638,3.133e-13,2.9576e-13
1.641,3.1319e-13,2.9626e-13
1.6439,3.1364e-13,2.9649e-13
1.6469,3.1353e-13,2.9698e-13
1.6499,3.1364e-13,2.9732e-13
1.6529,3.1386e-13,2.9809e-13
1.6559,3.1386e-13,2.9815e-13
1.6589,3.1386e-13,2.9854e-13
1.6618,3.1397e-13,2.9893e-13
1.6648,3.1397e-13,2.9943e-13
1.6678,3.1419e-13,2.997e-13
1.6708,3.1386e-13,3.0032e-13
1.6738,3.1364e-13,3.0048e-13
1.6767,3.1408e-13,3.0093e-13
1.6797,3.1397e-13,3.0148e-13
1.6827,3.143e-13,3.0154e-13
1.6857,3.1453e-13,3.0209e-13
1.6887,3.143e-13,3.0259e-13
1.6916,3.1464e-13,3.0304e-13
1.6946,3.1442e-13,3.0359e-13
1.6976,3.1442e-13,3.0376e-13
1.7006,3.1442e-13,3.0426e-13
1.7036,3.1464e-13,3.0448e-13
1.7065,3.1497e-13,3.0481e-13
1.7095,3.1475e-13,3.0537e-13
1.7125,3.1464e-13,3.0559e-13
1.7155,3.1464e-13,3.0617e-13
1.7185,3.1486e-13,3.0634e-13
1.7214,3.1519e-13,3.0667e-13
1.7244,3.1508e-13,3.075e-13
1.7274,3.153e-13,3.0781e-13
1.7304,3.153e-13,3.0795e-13
1.7334,3.1519e-13,3.0848e-13
1.7363,3.1541e-13,3.0873e-13
1.7393,3.1564e-13,3.0922e-13
1.7423,3.1564e-13,3.0939e-13
1.7453,3.1541e-13,3.0992e-13
1.7483,3.1575e-13,3.1028e-13
1.7513,3.1575e-13,3.1097e-13
1.7542,3.1586e-13,3.1136e-13
1.7572,3.1586e-13,3.1161e-13
1.7602,3.1597e-13,3.1197e-13
1.7632,3.1586e-13,3.1231e-13
1.7662,3.1608e-13,3.1289e-13
1.7691,3.1597e-13,3.1333e-13
1.7721,3.1597e-13,3.135e-13
1.7751,3.1608e-13,3.1394e-13
1.7781,3.1608e-13,3.1461e-13
1.7811,3.1686e-13,3.1469e-13
1.784,3.1619e-13,3.1497e-13
1.787,3.1597e-13,3.1544e-13
1.79,3.1664e-13,3.1591e-13
1.793,3.1664e-13,3.1641e-13
1.796,3.1686e-13,3.1683e-13
1.7989,3.1675e-13,3.1702e-13
1.8019,3.1664e-13,3.1747e-13
1.8049,3.1697e-13,3.1791e-13
1.8079,3.1697e-13,3.1816e-13
1.8109,3.1686e-13,3.1863e-13
1.8138,3.1686e-13,3.1913e-13
1.8168,3.1675e-13,3.1949e-13
1.8198,3.1708e-13,3.1991e-13
1.8228,3.1686e-13,3.2022e-13
1.8258,3.1697e-13,3.2066e-13
1.8287,3.1708e-13,3.2099e-13
1.8317,3.1697e-13,3.2138e-13
1.8347,3.1752e-13,3.218e-13
1.8377,3.1763e-13,3.2199e-13
1.8407,3.173e-13,3.2258e-13
1.8436,3.173e-13,3.2291e-13
1.8466,3.1719e-13,3.2346e-13
1.8496,3.1752e-13,3.2369e-13
1.8526,3.1797e-13,3.241e-13
1.8556,3.1775e-13,3.2463e-13
1.8586,3.1808e-13,3.2505e-13
1.8615,3.1752e-13,3.2527e-13
1.8645,3.1808e-13,3.2577e-13
1.8675,3.1786e-13,3.2604e-13
1.8705,3.1819e-13,3.2635e-13
1.8735,3.1819e-13,3.2693e-13
1.8764,3.1808e-13,3.2715e-13
1.8794,3.1819e-13,3.2774e-13
1.8824,3.1786e-13,3.2799e-13
1.8854,3.1841e-13,3.2854e-13
1.8884,3.183e-13,3.2885e-13
1.8913,3.183e-13,3.2924e-13
1.8943,3.1863e-13,3.296e-13
1.8973,3.1863e-13,3.2996e-13
1.9003,3.1886e-13,3.3024e-13
1.9033,3.1863e-13,3.3087e-13
1.9062,3.1886e-13,3.3118e-13
1.9092,3.1875e-13,3.3148e-13
1.9122,3.1863e-13,3.3187e-13
1.9152,3.1908e-13,3.3237e-13
1.9182,3.1852e-13,3.3279e-13
1.9211,3.1875e-13,3.3318e-13
1.9241,3.1897e-13,3.3351e-13
1.9271,3.193e-13,3.3373e-13
1.9301,3.1886e-13,3.3454e-13
1.9331,3.193e-13,3.3465e-13
1.936,3.1919e-13,3.3507e-13
1.939,3.1908e-13,3.3565e-13
1.942,3.1908e-13,3.3598e-13
1.945,3.1952e-13,3.362e-13
1.948,3.1941e-13,3.3684e-13
1.951,3.1919e-13,3.372e-13
1.9539,3.1908e-13,3.3776e-13
1.9569,3.1952e-13,3.3787e-13
1.9599,3.1986e-13,3.3845e-13
1.9629,3.1986e-13,3.3867e-13
1.9659,3.1952e-13,3.3917e-13
1.9688,3.1963e-13,3.3942e-13
1.9718,3.1986e-13,3.3976e-13
1.9748,3.1986e-13,3.4006e-13
1.9778,3.1986e-13,3.4064e-13
1.9808,3.2008e-13,3.4109e-13
1.9837,3.1986e-13,3.415e-13
1.9867,3.1974e-13,3.4181e-13
1.9897,3.203e-13,3.4198e-13
1.9927,3.2019e-13,3.4267e-13
1.9957,3.1963e-13,3.4284e-13
1.9986,3.2019e-13,3.4348e-13
2.0016,3.2063e-13,3.4364e-13
2.0046,3.1997e-13,3.4428e-13
2.0076,3.2074e-13,3.4461e-13
2.0106,3.203e-13,3.4486e-13
2.0135,3.2074e-13,3.4545e-13
2.0165,3.2085e-13,3.4575e-13
2.0195,3.203e-13,3.4633e-13
2.0225,3.2063e-13,3.4658e-13
2.0255,3.2085e-13,3.4692e-13
2.0284,3.2097e-13,3.4725e-13
2.0314,3.2074e-13,3.4767e-13
2.0344,3.2108e-13,3.4819e-13
2.0374,3.213e-13,3.4858e-13
2.0404,3.2097e-13,3.4894e-13
2.0433,3.2108e-13,3.4936e-13
2.0463,3.2074e-13,3.4972e-13
2.0493,3.2119e-13,3.5016e-13
2.0523,3.2119e-13,3.5041e-13
2.0553,3.213e-13,3.5101e-13
2.0583,3.2108e-13,3.5119e-13
2.0612,3.2119e-13,3.5162e-13
2.0642,3.2152e-13,3.5215e-13
2.0672,3.213e-13,3.5237e-13
2.0702,3.2163e-13,3.5288e-13
2.0732,3.2174e-13,3.5319e-13
2.0761,3.2163e-13,3.5351e-13
2.0791,3.2174e-13,3.5415e-13
2.0821,3.213e-13,3.5454e-13
2.0851,3.2174e-13,3.5506e-13
2.0881,3.2163e-13,3.5534e-13
2.091,3.2152e-13,3.5565e-13
2.094,3.2163e-13,3.5635e-13
2.097,3.2163e-13,3.5646e-13
2.1,3.2196e-13,3.5684e-13
2.103,3.2163e-13,3.5716e-13
2.1059,3.2152e-13,3.5794e-13
2.1089,3.2196e-13,3.5801e-13
2.1119,3.2185e-13,3.5859e-13
2.1149,3.2196e-13,3.5898e-13
2.1179,3.223e-13,3.5931e-13
2.1208,3.223e-13,3.5953e-13
2.1238,3.2174e-13,3.6017e-13
2.1268,3.2208e-13,3.6048e-13
2.1298,3.2263e-13,3.6084e-13
2.1328,3.2196e-13,3.6132e-13
2.1357,3.2241e-13,3.6168e-13
2.1387,3.2263e-13,3.6228e-13
2.1417,3.223e-13,3.6247e-13
2.1447,3.2252e-13,3.6253e-13
2.1477,3.2285e-13,3.6338e-13
2.1507,3.2219e-13,3.6378e-13
2.1536,3.2219e-13,3.6415e-13
2.1566,3.223e-13,3.6451e-13
2.1596,3.2296e-13,3.6489e-13
2.1626,3.2274e-13,3.6525e-13
2.1656,3.2285e-13,3.6569e-13
2.1685,3.2296e-13,3.6607e-13
2.1715,3.2274e-13,3.6661e-13
2.1745,3.2296e-13,3.6697e-13
2.1775,3.2296e-13,3.6735e-13
2.1805,3.2285e-13,3.6753e-13
2.1834,3.2285e-13,3.68e-13
2.1864,3.2307e-13,3.6848e-13
2.1894,3.2263e-13,3.6902e-13
2.1924,3.233e-13,3.6933e-13
2.1954,3.2319e-13,3.6991e-13
2.1983,3.2319e-13,3.7026e-13
2.2013,3.2307e-13,3.7062e-13
2.2043,3.233e-13,3.7123e-13
2.2073,3.2296e-13,3.7131e-13
2.2103,3.2319e-13,3.7183e-13
2.2132,3.233e-13,3.7209e-13
2.2162,3.2352e-13,3.7233e-13
2.2192,3.2296e-13,3.7287e-13
2.2222,3.233e-13,3.7335e-13
2.2252,3.2352e-13,3.7406e-13
2.2281,3.233e-13,3.7406e-13
2.2311,3.2363e-13,3.7464e-13
2.2341,3.2374e-13,3.7496e-13
2.2371,3.2341e-13,3.7581e-13
2.2401,3.2374e-13,3.762e-13
2.243,3.2341e-13,3.7631e-13
2.246,3.2385e-13,3.7659e-13
2.249,3.2374e-13,3.7731e-13
2.252,3.2363e-13,3.7746e-13
2.255,3.2385e-13,3.7806e-13
2.258,3.2385e-13,3.7859e-13
2.2609,3.2396e-13,3.7889e-13
2.2639,3.2352e-13,3.7914e-13
2.2669,3.2396e-13,3.7954e-13
2.2699,3.2363e-13,3.8e-13
2.2729,3.2396e-13,3.802e-13
2.2758,3.2396e-13,3.8092e-13
2.2788,3.2374e-13,3.8117e-13
2.2818,3.2419e-13,3.8168e-13
2.2848,3.243e-13,3.8225e-13
2.2878,3.243e-13,3.8277e-13
2.2907,3.2419e-13,3.828e-13
2.2937,3.2396e-13,3.833e-13
2.2967,3.2419e-13,3.8339e-13
2.2997,3.2419e-13,3.8395e-13
2.3027,3.2407e-13,3.8442e-13
2.3056,3.2419e-13,3.8494e-13
2.3086,3.2441e-13,3.8532e-13
2.3116,3.2474e-13,3.8573e-13
2.3146,3.243e-13,3.8614e-13
2.3176,3.2441e-13,3.865e-13
2.3205,3.2474e-13,3.8698e-13
2.3235,3.2441e-13,3.8764e-13
2.3265,3.2463e-13,3.8781e-13
2.3295,3.2463e-13,3.884e-13
2.3325,3.2474e-13,3.886e-13
2.3354,3.2474e-13,3.8906e-13
2.3384,3.2463e-13,3.8961e-13
2.3414,3.2441e-13,3.8979e-13
2.3444,3.2474e-13,3.905e-13
2.3474,3.2452e-13,3.9081e-13
2.3504,3.2452e-13,3.9115e-13
2.3533,3.2474e-13,3.9175e-13
2.3563,3.2485e-13,3.9218e-13
2.3593,3.2507e-13,3.9242e-13
2.3623,3.2496e-13,3.9275e-13
2.3653,3.2507e-13,3.9295e-13
2.3682,3.2507e-13,3.9372e-13
2.3712,3.2463e-13,3.9401e-13
2.3742,3.2485e-13,3.9457e-13
2.3772,3.2496e-13,3.9482e-13
2.3802,3.2518e-13,3.9525e-13
2.3831,3.2496e-13,3.9575e-13
2.3861,3.2507e-13,3.961e-13
2.3891,3.2496e-13,3.967e-13
2.3921,3.2485e-13,3.9712e-13
2.3951,3.2485e-13,3.9767e-13
2.398,3.2518e-13,3.979e-13
2.401,3.2507e-13,3.9823e-13
2.404,3.253e-13,3.9857e-13
2.407,3.2507e-13,3.9905e-13
2.41,3.2496e-13,3.9984e-13
2.4129,3.2518e-13,4.0025e-13
2.4159,3.2496e-13,4.0047e-13
2.4189,3.253e-13,4.0089e-13
2.4219,3.2518e-13,4.0122e-13
2.4249,3.253e-13,4.0184e-13
2.4278,3.2541e-13,4.0217e-13
2.4308,3.2518e-13,4.0235e-13
2.4338,3.253e-13,4.0308e-13
2.4368,3.2518e-13,4.0346e-13
2.4398,3.2518e-13,4.0373e-13
2.4427,3.2552e-13,4.0423e-13
2.4457,3.253e-13,4.0478e-13
2.4487,3.253e-13,4.0489e-13
2.4517,3.2541e-13,4.0538e-13
2.4547,3.2518e-13,4.0603e-13
2.4577,3.253e-13,4.0633e-13
2.4606,3.2541e-13,4.0686e-13
2.4636,3.2574e-13,4.0759e-13
2.4666,3.2552e-13,4.0765e-13
2.4696,3.2574e-13,4.0785e-13
2.4726,3.2541e-13,4.0847e-13
2.4755,3.2518e-13,4.0897e-13
2.4785,3.2563e-13,4.0967e-13
2.4815,3.2552e-13,4.0987e-13
2.4845,3.2563e-13,4.1022e-13
2.4875,3.2552e-13,4.107e-13
2.4904,3.2574e-13,4.1126e-13
2.4934,3.2552e-13,4.1156e-13
2.4964,3.2596e-13,4.1212e-13
2.4994,3.2563e-13,4.1237e-13
2.5024,3.2596e-13,4.1292e-13
2.5053,3.2596e-13,4.1333e-13
2.5083,3.2585e-13,4.1356e-13
2.5113,3.2585e-13,4.142e-13
2.5143,3.2574e-13,4.1432e-13
2.5173,3.2585e-13,4.1498e-13
2.5202,3.2596e-13,4.1554e-13
2.5232,3.2563e-13,4.1568e-13
2.5262,3.2563e-13,4.1657e-13
2.5292,3.2552e-13,4.165e-13
2.5322,3.2552e-13,4.1722e-13
2.5351,3.2596e-13,4.1753e-13
2.5381,3.2563e-13,4.1798e-13
2.5411,3.2574e-13,4.1844e-13
2.5441,3.2596e-13,4.1915e-13
2.5471,3.2596e-13,4.1936e-13
2.5501,3.2585e-13,4.1996e-13
2.553,3.2596e-13,4.2001e-13
2.556,3.2552e-13,4.2034e-13
2.559,3.2607e-13,4.2111e-13
2.562,3.2552e-13,4.2133e-13
2.565,3.2607e-13,4.2203e-13
2.5679,3.2563e-13,4.2247e-13
2.5709,3.2574e-13,4.2244e-13
2.5739,3.2607e-13,4.2342e-13
2.5769,3.2596e-13,4.2373e-13
2.5799,3.2607e-13,4.2428e-13
2.5828,3.2607e-13,4.2479e-13
2.5858,3.2596e-13,4.2495e-13
2.5888,3.2618e-13,4.2522e-13
2.5918,3.2596e-13,4.2555e-13
2.5948,3.2596e-13,4.2613e-13
2.5977,3.2629e-13,4.2664e-13
2.6007,3.2563e-13,4.2703e-13
2.6037,3.2618e-13,4.2763e-13
2.6067,3.2607e-13,4.2807e-13
2.6097,3.2607e-13,4.2864e-13
2.6126,3.2641e-13,4.2899e-13
2.6156,3.2596e-13,4.2964e-13
2.6186,3.2607e-13,4.2979e-13
2.6216,3.2618e-13,4.3035e-13
2.6246,3.2629e-13,4.3066e-13
2.6275,3.2585e-13,4.3118e-13
2.6305,3.2596e-13,4.3134e-13
2.6335,3.2607e-13,4.3192e-13
2.6365,3.2585e-13,4.3228e-13
2.6395,3.2596e-13,4.329e-13
2.6424,3.2607e-13,4.331e-13
2.6454,3.2607e-13,4.3375e-13
2.6484,3.2607e-13,4.3442e-13
2.6514,3.2596e-13,4.348e-13
2.6544,3.2607e-13,4.3519e-13
2.6574,3.2629e-13,4.3588e-13
2.6603,3.2607e-13,4.3584e-13
2.6633,3.2596e-13,4.3616e-13
2.6663,3.2629e-13,4.3656e-13
2.6693,3.2641e-13,4.373e-13
2.6723,3.2629e-13,4.3795e-13
2.6752,3.2641e-13,4.3818e-13
2.6782,3.2629e-13,4.3836e-13
2.6812,3.2618e-13,4.3932e-13
2.6842,3.2618e-13,4.3961e-13
2.6872,3.2629e-13,4.3994e-13
2.6901,3.2596e-13,4.4042e-13
2.6931,3.2607e-13,4.4057e-13
2.6961,3.2618e-13,4.4159e-13
2.6991,3.2585e-13,4.4184e-13
2.7021,3.2596e-13,4.4229e-13
2.705,3.2585e-13,4.4239e-13
2.708,3.2641e-13,4.4282e-13
2.711,3.2596e-13,4.4357e-13
2.714,3.2607e-13,4.4384e-13
2.717,3.2652e-13,4.4426e-13
2.7199,3.2618e-13,4.4475e-13
2.7229,3.2607e-13,4.4541e-13
2.7259,3.2629e-13,4.4595e-13
2.7289,3.2618e-13,4.4625e-13
2.7319,3.2629e-13,4.4681e-13
2.7348,3.2618e-13,4.4695e-13
2.7378,3.2618e-13,4.475e-13
2.7408,3.2641e-13,4.4788e-13
2.7438,3.2629e-13,4.4877e-13
2.7468,3.2618e-13,4.4914e-13
2.7497,3.2652e-13,4.4961e-13
2.7527,3.2618e-13,4.4969e-13
2.7557,3.2607e-13,4.5015e-13
2.7587,3.2607e-13,4.5068e-13
2.7617,3.2629e-13,4.5133e-13
2.7647,3.2596e-13,4.5172e-13
2.7676,3.2596e-13,4.5212e-13
2.7706,3.2652e-13,4.532e-13
2.7736,3.2618e-13,4.5326e-13
2.7766,3.2618e-13,4.5339e-13
2.7796,3.2596e-13,4.5421e-13
2.7825,3.2585e-13,4.544e-13
2.7855,3.2607e-13,4.5483e-13
2.7885,3.2618e-13,4.5557e-13
2.7915,3.2629e-13,4.561e-13
2.7945,3.2652e-13,4.562e-13
2.7974,3.2607e-13,4.5632e-13
2.8004,3.2596e-13,4.5709e-13
2.8034,3.2618e-13,4.577e-13
2.8064,3.2618e-13,4.581e-13
2.8094,3.2629e-13,4.5866e-13
2.8123,3.2641e-13,4.5915e-13
2.8153,3.2596e-13,4.5948e-13
2.8183,3.2607e-13,4.6009e-13
2.8213,3.2629e-13,4.6026e-13
2.8243,3.2607e-13,4.609e-13
2.8272,3.2585e-13,4.6113e-13
2.8302,3.2618e-13,4.6178e-13
2.8332,3.2596e-13,4.6225e-13
2.8362,3.2596e-13,4.6258e-13
2.8392,3.2585e-13,4.6332e-13
2.8421,3.2607e-13,4.6352e-13
2.8451,3.2585e-13,4.6392e-13
2.8481,3.2613e-13,4.6472e-13
2.8511,3.2618e-13,4.651e-13
2.8541,3.2618e-13,4.6566e-13
2.8571,3.2574e-13,4.6568e-13
2.86,3.2596e-13,4.6631e-13
2.863,3.2585e-13,4.6693e-13
2.866,3.2613e-13,4.6693e-13
2.869,3.2596e-13,4.6749e-13
2.872,3.2618e-13,4.6797e-13
2.8749,3.2602e-13,4.6853e-13
2.8779,3.2613e-13,4.6909e-13
2.8809,3.2613e-13,4.6969e-13
2.8839,3.2591e-13,4.7011e-13
2.8869,3.2607e-13,4.7023e-13
2.8898,3.2641e-13,4.7083e-13
2.8928,3.2646e-13,4.7124e-13
2.8958,3.2591e-13,4.7172e-13
2.8988,3.2602e-13,4.7262e-13
2.9018,3.2613e-13,4.7277e-13
2.9047,3.2613e-13,4.7334e-13
2.9077,3.2541e-13,4.7352e-13
2.9107,3.2602e-13,4.7412e-13
2.9137,3.2607e-13,4.7452e-13
2.9167,3.2613e-13,4.7527e-13
2.9196,3.2607e-13,4.7565e-13
2.9226,3.2613e-13,4.7632e-13
2.9256,3.2629e-13,4.7658e-13
2.9286,3.2618e-13,4.7681e-13
2.9316,3.2591e-13,4.7733e-13
2.9345,3.2607e-13,4.7816e-13
2.9375,3.2602e-13,4.7829e-13
2.9405,3.2585e-13,4.7901e-13
2.9435,3.2613e-13,4.7912e-13
2.9465,3.2579e-13,4.7949e-13
2.9494,3.2613e-13,4.8023e-13
2.9524,3.2585e-13,4.8039e-13
2.9554,3.2563e-13,4.8085e-13
2.9584,3.2574e-13,4.818e-13
2.9614,3.2613e-13,4.8209e-13
2.9644,3.2568e-13,4.8227e-13
2.9673,3.2585e-13,4.8271e-13
2.9703,3.2618e-13,4.8356e-13
2.9733,3.2596e-13,4.8361e-13
2.9763,3.2579e-13,4.8452e-13
2.9793,3.2591e-13,4.8478e-13
2.9822,3.2579e-13,4.8517e-13
2.9852,3.2602e-13,4.86e-13
2.9882,3.2624e-13,4.8654e-13
2.9912,3.2591e-13,4.8636e-13
2.9942,3.2618e-13,4.8739e-13
2.9971,3.2602e-13,4.8754e-13
3.0001,3.2635e-13,4.8803e-13
3.0031,3.2591e-13,4.8817e-13
3.0061,3.2613e-13,4.8929e-13
3.0091,3.2618e-13,4.8982e-13
3.012,3.2607e-13,4.8996e-13
3.015,3.2618e-13,4.9045e-13
3.018,3.2585e-13,4.9112e-13
3.021,3.2591e-13,4.9158e-13
3.024,3.2624e-13,4.922e-13
3.0269,3.2563e-13,4.9231e-13
3.0299,3.2607e-13,4.932e-13
3.0329,3.2574e-13,4.9333e-13
3.0359,3.2618e-13,4.9367e-13
3.0389,3.2574e-13,4.9438e-13
3.0418,3.2574e-13,4.9458e-13
3.0448,3.2591e-13,4.9515e-13
3.0478,3.2552e-13,4.9571e-13
3.0508,3.2568e-13,4.9614e-13
3.0538,3.2563e-13,4.9631e-13
3.0568,3.2629e-13,4.9689e-13
3.0597,3.2585e-13,4.9744e-13
3.0627,3.2596e-13,4.9735e-13
3.0657,3.2607e-13,4.9839e-13
3.0687,3.2591e-13,4.9927e-13
3.0717,3.2574e-13,4.9956e-13
3.0746,3.2602e-13,4.9949e-13
3.0776,3.2574e-13,4.9992e-13
3.0806,3.2602e-13,5.0088e-13
3.0836,3.2591e-13,5.0175e-13
3.0866,3.2552e-13,5.0218e-13
3.0895,3.2579e-13,5.0204e-13
3.0925,3.2563e-13,5.0308e-13
3.0955,3.253e-13,5.0318e-13
3.0985,3.2557e-13,5.0389e-13
3.1015,3.2563e-13,5.0393e-13
3.1044,3.2602e-13,5.0483e-13
3.1074,3.2629e-13,5.0503e-13
3.1104,3.2602e-13,5.0575e-13
3.1134,3.2602e-13,5.0659e-13
3.1164,3.2585e-13,5.0626e-13
3.1193,3.2624e-13,5.0697e-13
3.1223,3.2535e-13,5.0729e-13
3.1253,3.2613e-13,5.0769e-13
3.1283,3.2596e-13,5.0833e-13
3.1313,3.2563e-13,5.0875e-13
3.1342,3.2585e-13,5.0986e-13
3.1372,3.2613e-13,5.1036e-13
3.1402,3.2557e-13,5.1049e-13
3.1432,3.2574e-13,5.1104e-13
3.1462,3.2585e-13,5.1135e-13
3.1491,3.2591e-13,5.119e-13
3.1521,3.2563e-13,5.1173e-13
3.1551,3.2535e-13,5.1231e-13
3.1581,3.2585e-13,5.1277e-13
3.1611,3.2607e-13,5.1313e-13
3.1641,3.2602e-13,5.1364e-13
3.167,3.2585e-13,5.148e-13
3.17,3.2574e-13,5.1496e-13
3.173,3.2585e-13,5.1546e-13
3.176,3.2591e-13,5.1588e-13
3.179,3.2574e-13,5.1641e-13
3.1819,3.2591e-13,5.1682e-13
3.1849,3.2591e-13,5.1681e-13
3.1879,3.2579e-13,5.1763e-13
3.1909,3.2546e-13,5.1834e-13
3.1939,3.2591e-13,5.1882e-13
3.1968,3.2613e-13,5.1935e-13
3.1998,3.2563e-13,5.1989e-13
3.2028,3.2585e-13,5.2029e-13
3.2058,3.2579e-13,5.2015e-13
3.2088,3.2596e-13,5.2086e-13
3.2117,3.2607e-13,5.2172e-13
3.2147,3.2629e-13,5.2248e-13
3.2177,3.2579e-13,5.2236e-13
3.2207,3.2618e-13,5.23e-13
3.2237,3.2607e-13,5.2361e-13
3.2266,3.2624e-13,5.2403e-13
3.2296,3.2579e-13,5.2497e-13
3.2326,3.2618e-13,5.2483e-13
3.2356,3.2602e-13,5.254e-13
3.2386,3.2602e-13,5.2593e-13
3.2415,3.2596e-13,5.2615e-13
3.2445,3.2585e-13,5.272e-13
3.2475,3.2602e-13,5.2795e-13
3.2505,3.2629e-13,5.2798e-13
3.2535,3.2641e-13,5.2844e-13
3.2565,3.2635e-13,5.2916e-13
3.2594,3.2585e-13,5.2897e-13
3.2624,3.2591e-13,5.2985e-13
3.2654,3.2585e-13,5.301e-13
3.2684,3.2613e-13,5.3074e-13
3.2714,3.2641e-13,5.3137e-13
3.2743,3.2652e-13,5.3185e-13
3.2773,3.2602e-13,5.3245e-13
3.2803,3.2679e-13,5.3252e-13
3.2833,3.2646e-13,5.3309e-13
3.2863,3.2607e-13,5.3321e-13
3.2892,3.2657e-13,5.3405e-13
3.2922,3.2596e-13,5.3445e-13
3.2952,3.2629e-13,5.3448e-13
3.2982,3.2613e-13,5.3497e-13
3.3012,3.2607e-13,5.3609e-13
3.3041,3.2652e-13,5.3646e-13
3.3071,3.2635e-13,5.3645e-13
3.3101,3.2657e-13,5.3685e-13
3.3131,3.2629e-13,5.3767e-13
3.3161,3.2641e-13,5.3844e-13
3.319,3.2707e-13,5.3907e-13
3.322,3.2624e-13,5.3903e-13
3.325,3.2702e-13,5.4e-13
3.328,3.2641e-13,5.3993e-13
3.331,3.2635e-13,5.4091e-13
3.3339,3.2635e-13,5.4079e-13
3.3369,3.2663e-13,5.4144e-13
3.3399,3.2652e-13,5.4155e-13
3.3429,3.2635e-13,5.4207e-13
3.3459,3.2696e-13,5.4304e-13
3.3488,3.2657e-13,5.4337e-13
3.3518,3.2629e-13,5.4344e-13
3.3548,3.2702e-13,5.4451e-13
3.3578,3.2685e-13,5.4451e-13
3.3608,3.2668e-13,5.4558e-13
3.3638,3.2691e-13,5.4572e-13
3.3667,3.2707e-13,5.4669e-13
3.3697,3.2685e-13,5.467e-13
3.3727,3.2685e-13,5.4692e-13
3.3757,3.2702e-13,5.4744e-13
3.3787,3.2707e-13,5.4774e-13
3.3816,3.2679e-13,5.4871e-13
3.3846,3.2696e-13,5.4862e-13
3.3876,3.2691e-13,5.4982e-13
3.3906,3.2735e-13,5.5002e-13
3.3936,3.2785e-13,5.503e-13
3.3965,3.2713e-13,5.5066e-13
3.3995,3.2702e-13,5.5102e-13
3.4025,3.2757e-13,5.5118e-13
3.4055,3.2746e-13,5.5199e-13
3.4085,3.2713e-13,5.526e-13
3.4114,3.274e-13,5.5303e-13
3.4144,3.274e-13,5.5322e-13
3.4174,3.2757e-13,5.5353e-13
3.4204,3.2763e-13,5.5421e-13
3.4234,3.2746e-13,5.5482e-13
3.4263,3.274e-13,5.5493e-13
3.4293,3.2785e-13,5.5607e-13
3.4323,3.2752e-13,5.5649e-13
3.4353,3.2802e-13,5.5735e-13
3.4383,3.2768e-13,5.5733e-13
3.4412,3.2763e-13,5.5787e-13
3.4442,3.2807e-13,5.5854e-13
3.4472,3.2774e-13,5.5841e-13
3.4502,3.2835e-13,5.5861e-13
3.4532,3.2746e-13,5.5973e-13
3.4562,3.2807e-13,5.6015e-13
3.4591,3.2796e-13,5.6093e-13
3.4621,3.2802e-13,5.6094e-13
3.4651,3.2857e-13,5.6204e-13
3.4681,3.284e-13,5.6198e-13
3.4711,3.2824e-13,5.6258e-13
3.474,3.2851e-13,5.6272e-13
3.477,3.284e-13,5.6337e-13
3.48,3.2879e-13,5.6348e-13
3.483,3.289e-13,5.6448e-13
3.486,3.2879e-13,5.647e-13
3.4889,3.2924e-13,5.6473e-13
3.4919,3.2907e-13,5.6584e-13
3.4949,3.2896e-13,5.6584e-13
3.4979,3.2868e-13,5.6613e-13
3.5009,3.2918e-13,5.6741e-13
3.5038,3.2963e-13,5.6725e-13
3.5068,3.2918e-13,5.6811e-13
3.5098,3.2929e-13,5.6839e-13
3.5128,3.2918e-13,5.6916e-13
3.5158,3.2896e-13,5.6892e-13
3.5187,3.2924e-13,5.7042e-13
3.5217,3.2901e-13,5.6959e-13
3.5247,3.2951e-13,5.7003e-13
3.5277,3.2946e-13,5.7034e-13
3.5307,3.299e-13,5.7106e-13
3.5336,3.2946e-13,5.72e-13
3.5366,3.2946e-13,5.7221e-13
3.5396,3.2974e-13,5.726e-13
3.5426,3.2996e-13,5.7283e-13
3.5456,3.3079e-13,5.7342e-13
3.5485,3.299e-13,5.7394e-13
3.5515,3.299e-13,5.7478e-13
3.5545,3.2985e-13,5.7507e-13
3.5575,3.3007e-13,5.7525e-13
3.5605,3.2957e-13,5.7561e-13
3.5635,3.3051e-13,5.7702e-13
3.5664,3.299e-13,5.7711e-13
3.5694,3.309e-13,5.7723e-13
3.5724,3.3051e-13,5.7801e-13
3.5754,3.3057e-13,5.7807e-13
3.5784,3.3079e-13,5.7866e-13
3.5813,3.3096e-13,5.7973e-13
3.5843,3.309e-13,5.7954e-13
3.5873,3.3124e-13,5.7966e-13
3.5903,3.3173e-13,5.8023e-13
3.5933,3.3157e-13,5.8065e-13
3.5962,3.3112e-13,5.813e-13
3.5992,3.3162e-13,5.8215e-13
3.6022,3.3151e-13,5.8251e-13
3.6052,3.3173e-13,5.8287e-13
3.6082,3.3146e-13,5.8376e-13
3.6111,3.3168e-13,5.8345e-13
3.6141,3.3218e-13,5.8442e-13
3.6171,3.319e-13,5.8463e-13
3.6201,3.324e-13,5.8518e-13
3.6231,3.3257e-13,5.8534e-13
3.626,3.3246e-13,5.8546e-13
3.629,3.3223e-13,5.8625e-13
3.632,3.3284e-13,5.8602e-13
3.635,3.3296e-13,5.8731e-13
3.638,3.3257e-13,5.8746e-13
3.6409,3.3329e-13,5.8774e-13
3.6439,3.3268e-13,5.8828e-13
3.6469,3.3346e-13,5.8917e-13
3.6499,3.3351e-13,5.8965e-13
3.6529,3.3334e-13,5.8974e-13
3.6559,3.334e-13,5.9011e-13
3.6588,3.3329e-13,5.9046e-13
3.6618,3.339e-13,5.9093e-13
3.6648,3.339e-13,5.9099e-13
3.6678,3.344e-13,5.9204e-13
3.6708,3.344e-13,5.9193e-13
3.6737,3.3423e-13,5.925e-13
3.6767,3.3396e-13,5.9296e-13
3.6797,3.3501e-13,5.9376e-13
3.6827,3.3523e-13,5.9444e-13
3.6857,3.3495e-13,5.9423e-13
3.6886,3.3579e-13,5.9489e-13
3.6916,3.3518e-13,5.9505e-13
3.6946,3.3501e-13,5.9494e-13
3.6976,3.3584e-13,5.9594e-13
3.7006,3.354e-13,5.9644e-13
3.7035,3.354e-13,5.9676e-13
3.7065,3.3568e-13,5.9736e-13
3.7095,3.3568e-13,5.981e-13
3.7125,3.3623e-13,5.9826e-13
3.7155,3.3601e-13,5.983e-13
3.7184,3.3662e-13,5.9933e-13
3.7214,3.3623e-13,5.9955e-13
3.7244,3.3684e-13,5.9944e-13
3.7274,3.374e-13,5.9992e-13
3.7304,3.3695e-13,6.0081e-13
3.7333,3.3695e-13,6.0148e-13
3.7363,3.3773e-13,6.0198e-13
3.7393,3.3795e-13,6.0175e-13
3.7423,3.3806e-13,6.0167e-13
3.7453,3.3734e-13,6.0237e-13
3.7482,3.384e-13,6.0282e-13
3.7512,3.3795e-13,6.0285e-13
3.7542,3.3779e-13,6.0389e-13
3.7572,3.3828e-13,6.0396e-13
3.7602,3.3895e-13,6.0463e-13
3.7632,3.3845e-13,6.0478e-13
3.7661,3.3862e-13,6.0524e-13
3.7691,3.3928e-13,6.0599e-13
3.7721,3.3917e-13,6.0585e-13
3.7751,3.394e-13,6.0618e-13
3.7781,3.3989e-13,6.0704e-13
3.781,3.3984e-13,6.0754e-13
3.784,3.3995e-13,6.0817e-13
3.787,3.3984e-13,6.0803e-13
3.79,3.4006e-13,6.0849e-13
3.793,3.4028e-13,6.0943e-13
3.7959,3.4028e-13,6.0975e-13
3.7989,3.4039e-13,6.1058e-13
3.8019,3.4128e-13,6.104e-13
3.8049,3.4139e-13,6.103e-13
3.8079,3.4139e-13,6.1051e-13
3.8108,3.415e-13,6.1129e-13
3.8138,3.4217e-13,6.1164e-13
3.8168,3.4223e-13,6.125e-13
3.8198,3.4234e-13,6.1184e-13
3.8228,3.4212e-13,6.1262e-13
3.8257,3.4289e-13,6.1338e-13
3.8287,3.4267e-13,6.1372e-13
3.8317,3.4334e-13,6.143e-13
3.8347,3.43e-13,6.1399e-13
3.8377,3.4356e-13,6.1495e-13
3.8406,3.4378e-13,6.1519e-13
3.8436,3.4384e-13,6.1576e-13
3.8466,3.4445e-13,6.162e-13
3.8496,3.4484e-13,6.1694e-13
3.8526,3.4467e-13,6.1666e-13
3.8556,3.4528e-13,6.1672e-13
3.8585,3.4489e-13,6.1713e-13
3.8615,3.4517e-13,6.1758e-13
3.8645,3.4556e-13,6.1827e-13
3.8675,3.4572e-13,6.1802e-13
3.8705,3.4611e-13,6.1895e-13
3.8734,3.4667e-13,6.1931e-13
3.8764,3.4694e-13,6.1928e-13
3.8794,3.4711e-13,6.1996e-13
3.8824,3.4689e-13,6.2125e-13
3.8854,3.4794e-13,6.2042e-13
3.8883,3.4761e-13,6.2109e-13
3.8913,3.4789e-13,6.2172e-13
3.8943,3.4833e-13,6.2224e-13
3.8973,3.4922e-13,6.2142e-13
3.9003,3.4917e-13,6.2196e-13
3.9032,3.4889e-13,6.2311e-13
3.9062,3.4939e-13,6.2275e-13
3.9092,3.4972e-13,6.2324e-13
3.9122,3.5011e-13,6.2392e-13
3.9152,3.5005e-13,6.239e-13
3.9181,3.5039e-13,6.2442e-13
3.9211,3.5077e-13,6.2556e-13
3.9241,3.5083e-13,6.2531e-13
3.9271,3.5172e-13,6.2601e-13
3.9301,3.5189e-13,6.2653e-13
3.933,3.5211e-13,6.2625e-13
3.936,3.5144e-13,6.2696e-13
3.939,3.5227e-13,6.2654e-13
3.942,3.5238e-13,6.2718e-13
3.945,3.5294e-13,6.2809e-13
3.9479,3.5288e-13,6.2858e-13
3.9509,3.5361e-13,6.2848e-13
3.9539,3.5394e-13,6.2841e-13
3.9569,3.5377e-13,6.2951e-13
3.9599,3.5411e-13,6.29e-13
3.9629,3.5494e-13,6.2933e-13
3.9658,3.5466e-13,6.3034e-13
3.9688,3.5538e-13,6.3026e-13
3.9718,3.5566e-13,6.3008e-13
3.9748,3.5577e-13,6.3084e-13
3.9778,3.5599e-13,6.3187e-13
3.9807,3.566e-13,6.327e-13
3.9837,3.5721e-13,6.3161e-13
3.9867,3.5677e-13,6.3215e-13
3.9897,3.576e-13,6.3266e-13
3.9927,3.5738e-13,6.3334e-13
3.9956,3.5866e-13,6.3292e-13
3.9986,3.5838e-13,6.3402e-13
4.0016,3.5899e-13,6.3337e-13
4.0046,3.5955e-13,6.3358e-13
4.0076,3.5971e-13,6.3535e-13
4.0105,3.601e-13,6.3471e-13
4.0135,3.6077e-13,6.3446e-13
4.0165,3.6116e-13,6.3535e-13
4.0195,3.6143e-13,6.3526e-13
4.0225,3.6138e-13,6.3684e-13
4.0254,3.6221e-13,6.3673e-13
4.0284,3.6232e-13,6.3678e-13
4.0314,3.6215e-13,6.372e-13
4.0344,3.6349e-13,6.3718e-13
4.0374,3.6354e-13,6.3709e-13
4.0403,3.6318e-13,6.3841e-13
4.0433,3.6429e-13,6.3834e-13
4.0463,3.6515e-13,6.3834e-13
4.0493,3.6493e-13,6.3868e-13
4.0523,3.6501e-13,6.3893e-13
4.0553,3.6615e-13,6.3953e-13
4.0582,3.6629e-13,6.404e-13
4.0612,3.671e-13,6.3938e-13
4.0642,3.6723e-13,6.4054e-13
4.0672,3.6735e-13,6.3974e-13
4.0702,3.6768e-13,6.4075e-13
4.0731,3.6823e-13,6.4143e-13
4.0761,3.6945e-13,6.4079e-13
4.0791,3.6934e-13,6.4174e-13
4.0821,3.6945e-13,6.412e-13
4.0851,3.6962e-13,6.426e-13
4.088,3.7045e-13,6.4172e-13
4.091,3.7081e-13,6.4199e-13
4.094,3.7123e-13,6.4311e-13
4.097,3.7198e-13,6.4279e-13
4.1,3.7215e-13,6.4336e-13
4.1029,3.7301e-13,6.4376e-13
4.1059,3.7245e-13,6.4411e-13
4.1089,3.7351e-13,6.443e-13
4.1119,3.734e-13,6.4469e-13
4.1149,3.7384e-13,6.4457e-13
4.1178,3.7526e-13,6.4475e-13
4.1208,3.7578e-13,6.4548e-13
4.1238,3.7634e-13,6.4523e-13
4.1268,3.7712e-13,6.4579e-13
4.1298,3.7734e-13,6.4621e-13
4.1327,3.7745e-13,6.4593e-13
4.1357,3.7703e-13,6.4594e-13
4.1387,3.7914e-13,6.4609e-13
4.1417,3.7989e-13,6.4679e-13
4.1447,3.7931e-13,6.4744e-13
4.1476,3.792e-13,6.4719e-13
4.1506,3.8045e-13,6.4788e-13
4.1536,3.8092e-13,6.472e-13
4.1566,3.8169e-13,6.4709e-13
4.1596,3.8153e-13,6.4859e-13
4.1626,3.8197e-13,6.4856e-13
4.1655,3.8253e-13,6.4819e-13
4.1685,3.8217e-13,6.4874e-13
4.1715,3.8522e-13,6.4901e-13
4.1745,3.8522e-13,6.4868e-13
4.1775,3.8589e-13,6.4937e-13
4.1804,3.8464e-13,6.501e-13
4.1834,3.8616e-13,6.4934e-13
4.1864,3.8622e-13,6.4926e-13
4.1894,3.8766e-13,6.5052e-13
4.1924,3.8788e-13,6.5034e-13
4.1953,3.88e-13,6.5098e-13
4.1983,3.8861e-13,6.5149e-13
4.2013,3.8972e-13,6.5124e-13
4.2043,3.8988e-13,6.5123e-13
4.2073,3.9074e-13,6.5198e-13
4.2102,3.9088e-13,6.5101e-13
4.2132,3.9113e-13,6.5158e-13
4.2162,3.9205e-13,6.5213e-13
4.2192,3.931e-13,6.5228e-13
4.2222,3.9332e-13,6.5238e-13
4.2251,3.9396e-13,6.5224e-13
4.2281,3.9466e-13,6.5274e-13
4.2311,3.9507e-13,6.5288e-13
4.2341,3.9635e-13,6.5331e-13
4.2371,3.976e-13,6.5355e-13
4.24,3.9735e-13,6.5326e-13
4.243,3.9826e-13,6.5359e-13
4.246,3.9962e-13,6.5303e-13
4.249,3.991e-13,6.532e-13
4.252,3.9999e-13,6.5485e-13
4.255,4.0074e-13,6.5405e-13
4.2579,4.0126e-13,6.5394e-13
4.2609,4.0098e-13,6.5468e-13
4.2639,4.0271e-13,6.5407e-13
4.2669,4.0207e-13,6.551e-13
4.2699,4.0379e-13,6.5528e-13
4.2728,4.0445e-13,6.5485e-13
4.2758,4.0556e-13,6.5527e-13
4.2788,4.0498e-13,6.553e-13
4.2818,4.069e-13,6.5528e-13
4.2848,4.0662e-13,6.5559e-13
4.2877,4.0676e-13,6.5624e-13
4.2907,4.0837e-13,6.5579e-13
4.2937,4.0845e-13,6.5609e-13
4.2967,4.0909e-13,6.5699e-13
4.2997,4.1128e-13,6.5586e-13
4.3026,4.1117e-13,6.5599e-13
4.3056,4.1248e-13,6.5614e-13
4.3086,4.1203e-13,6.5641e-13
4.3116,4.1395e-13,6.5668e-13
4.3146,4.1425e-13,6.5789e-13
4.3175,4.1508e-13,6.5789e-13
4.3205,4.1578e-13,6.5675e-13
4.3235,4.1619e-13,6.5789e-13
4.3265,4.1708e-13,6.5696e-13
4.3295,4.1889e-13,6.567e-13
4.3324,4.1775e-13,6.5649e-13
4.3354,4.2025e-13,6.5704e-13
4.3384,4.2036e-13,6.5749e-13
4.3414,4.208e-13,6.5756e-13
4.3444,4.2297e-13,6.5827e-13
4.3473,4.2316e-13,6.5785e-13
4.3503,4.2386e-13,6.5663e-13
4.3533,4.2522e-13,6.5717e-13
4.3563,4.2474e-13,6.5763e-13
4.3593,4.2613e-13,6.5761e-13
4.3623,4.2705e-13,6.579e-13
4.3652,4.2763e-13,6.5706e-13
4.3682,4.2796e-13,6.5803e-13
4.3712,4.3043e-13,6.576e-13
4.3742,4.3007e-13,6.5767e-13
4.3772,4.3102e-13,6.5772e-13
4.3801,4.3263e-13,6.5896e-13
4.3831,4.329e-13,6.5865e-13
4.3861,4.3401e-13,6.5779e-13
4.3891,4.3399e-13,6.5818e-13
4.3921,4.3524e-13,6.575e-13
4.395,4.3573e-13,6.5895e-13
4.398,4.3779e-13,6.5827e-13
4.401,4.3904e-13,6.5903e-13
4.404,4.3937e-13,6.5818e-13
4.407,4.4051e-13,6.5825e-13
4.4099,4.404e-13,6.5919e-13
4.4129,4.4242e-13,6.5789e-13
4.4159,4.4281e-13,6.5813e-13
4.4189,4.4342e-13,6.5867e-13
4.4219,4.4467e-13,6.5786e-13
4.4248,4.457e-13,6.5854e-13
4.4278,4.4695e-13,6.585e-13
4.4308,4.4781e-13,6.5842e-13
4.4338,4.4748e-13,6.5857e-13
4.4368,4.5022e-13,6.5822e-13
4.4397,4.5128e-13,6.5767e-13
4.4427,4.5169e-13,6.5797e-13
4.4457,4.5214e-13,6.5919e-13
4.4487,4.53e-13,6.5803e-13
4.4517,4.5455e-13,6.5831e-13
4.4547,4.5527e-13,6.5843e-13
4.4576,4.5691e-13,6.5821e-13
4.4606,4.5755e-13,6.5781e-13
4.4636,4.5761e-13,6.579e-13
4.4666,4.5952e-13,6.5892e-13
4.4696,4.5994e-13,6.5811e-13
4.4725,4.6088e-13,6.5919e-13
4.4755,4.626e-13,6.5824e-13
4.4785,4.6343e-13,6.5815e-13
4.4815,4.6468e-13,6.5777e-13
4.4845,4.6618e-13,6.5813e-13
4.4874,4.6696e-13,6.5807e-13
4.4904,4.6751e-13,6.5695e-13
4.4934,4.686e-13,6.582e-13
4.4964,4.6951e-13,6.5783e-13
4.4994,4.7068e-13,6.5797e-13
4.5023,4.7221e-13,6.5731e-13
4.5053,4.7384e-13,6.5725e-13
4.5083,4.7456e-13,6.5663e-13
4.5113,4.747e-13,6.5725e-13
4.5143,4.7704e-13,6.5756e-13
4.5172,4.7695e-13,6.5672e-13
4.5202,4.7834e-13,6.5667e-13
4.5232,4.7989e-13,6.5671e-13
4.5262,4.8092e-13,6.5635e-13
4.5292,4.8284e-13,6.5566e-13
4.5321,4.8381e-13,6.5656e-13
4.5351,4.8481e-13,6.5636e-13
4.5381,4.8639e-13,6.5545e-13
4.5411,4.8697e-13,6.5485e-13
4.5441,4.8844e-13,6.5555e-13
4.547,4.893e-13,6.5541e-13
4.55,4.9052e-13,6.5467e-13
4.553,4.9108e-13,6.5531e-13
4.556,4.9233e-13,6.5552e-13
4.559,4.9488e-13,6.5488e-13
4.562,4.9533e-13,6.5503e-13
4.5649,4.9699e-13,6.5538e-13
4.5679,4.9735e-13,6.5448e-13
4.5709,4.9954e-13,6.5416e-13
4.5739,4.9999e-13,6.5398e-13
4.5769,5.0165e-13,6.5518e-13
4.5798,5.0202e-13,6.5405e-13
4.5828,5.0429e-13,6.5385e-13
4.5858,5.0548e-13,6.5307e-13
4.5888,5.0773e-13,6.5323e-13
4.5918,5.084e-13,6.5255e-13
4.5947,5.0912e-13,6.5206e-13
4.5977,5.1129e-13,6.5198e-13
4.6007,5.1212e-13,6.522e-13
4.6037,5.1303e-13,6.5242e-13
4.6067,5.1564e-13,6.516e-13
4.6096,5.1664e-13,6.5106e-13
4.6126,5.1639e-13,6.5228e-13
4.6156,5.185e-13,6.5117e-13
4.6186,5.2025e-13,6.5027e-13
4.6216,5.2167e-13,6.5165e-13
4.6245,5.2183e-13,6.5212e-13
4.6275,5.245e-13,6.504e-13
4.6305,5.2616e-13,6.5023e-13
4.6335,5.2783e-13,6.5052e-13
4.6365,5.2858e-13,6.4891e-13
4.6394,5.3013e-13,6.4876e-13
4.6424,5.3157e-13,6.4895e-13
4.6454,5.3332e-13,6.4877e-13
4.6484,5.351e-13,6.4848e-13
4.6514,5.3682e-13,6.4865e-13
4.6544,5.3649e-13,6.4711e-13
4.6573,5.3951e-13,6.4705e-13
4.6603,5.4079e-13,6.4783e-13
4.6633,5.427e-13,6.4672e-13
4.6663,5.4351e-13,6.4748e-13
4.6693,5.4587e-13,6.4681e-13
4.6722,5.4626e-13,6.4547e-13
4.6752,5.4878e-13,6.4563e-13
4.6782,5.5014e-13,6.4524e-13
4.6812,5.5222e-13,6.4444e-13
4.6842,5.5386e-13,6.4507e-13
4.6871,5.5458e-13,6.4443e-13
4.6901,5.56e-13,6.4333e-13
4.6931,5.5772e-13,6.4296e-13
4.6961,5.583e-13,6.4321e-13
4.6991,5.6102e-13,6.4313e-13
4.702,5.6305e-13,6.4207e-13
4.705,5.6408e-13,6.4269e-13
4.708,5.6544e-13,6.4192e-13
4.711,5.6707e-13,6.4138e-13
4.714,5.6868e-13,6.4179e-13
4.7169,5.6999e-13,6.4071e-13
4.7199,5.7299e-13,6.407e-13
4.7229,5.7351e-13,6.4009e-13
4.7259,5.7518e-13,6.4005e-13
4.7289,5.7823e-13,6.3947e-13
4.7318,5.7826e-13,6.3951e-13
4.7348,5.8001e-13,6.3755e-13
4.7378,5.8228e-13,6.3714e-13
4.7408,5.845e-13,6.3777e-13
4.7438,5.862e-13,6.3741e-13
4.7467,5.8836e-13,6.3662e-13
4.7497,5.9042e-13,6.3657e-13
4.7527,5.9094e-13,6.3572e-13
4.7557,5.9319e-13,6.3507e-13
4.7587,5.9547e-13,6.3585e-13
4.7617,5.958e-13,6.3408e-13
4.7646,5.9894e-13,6.3365e-13
4.7676,5.998e-13,6.3303e-13
4.7706,6.0371e-13,6.3357e-13
4.7736,6.0402e-13,6.3297e-13
4.7766,6.0543e-13,6.3139e-13
4.7795,6.0882e-13,6.3291e-13
4.7825,6.0912e-13,6.3163e-13
4.7855,6.1198e-13,6.3047e-13
4.7885,6.1334e-13,6.3e-13
4.7915,6.1412e-13,6.2938e-13
4.7944,6.1764e-13,6.2892e-13
4.7974,6.1978e-13,6.2866e-13
4.8004,6.2081e-13,6.2814e-13
4.8034,6.2278e-13,6.2747e-13
4.8064,6.2508e-13,6.2659e-13
4.8093,6.2683e-13,6.2721e-13
4.8123,6.2944e-13,6.2527e-13
4.8153,6.318e-13,6.2394e-13
4.8183,6.338e-13,6.2408e-13
4.8213,6.3374e-13,6.2406e-13
4.8242,6.3616e-13,6.2346e-13
4.8272,6.3957e-13,6.2306e-13
4.8302,6.4249e-13,6.2185e-13
4.8332,6.4165e-13,6.2161e-13
4.8362,6.4465e-13,6.2138e-13
4.8391,6.4729e-13,6.212e-13
4.8421,6.482e-13,6.1914e-13
4.8451,6.512e-13,6.1994e-13
4.8481,6.5323e-13,6.1853e-13
4.8511,6.557e-13,6.171e-13
4.8541,6.5895e-13,6.1692e-13
4.857,6.5817e-13,6.1777e-13
4.86,6.6178e-13,6.1674e-13
4.863,6.6516e-13,6.1694e-13
4.866,6.6427e-13,6.1522e-13
4.869,6.6747e-13,6.1467e-13
4.8719,6.706e-13,6.1454e-13
4.8749,6.7374e-13,6.1422e-13
4.8779,6.7449e-13,6.1187e-13
4.8809,6.7629e-13,6.1362e-13
4.8839,6.7951e-13,6.1159e-13
4.8868,6.8104e-13,6.0957e-13
4.8898,6.8387e-13,6.1048e-13
4.8928,6.849e-13,6.0835e-13
4.8958,6.8812e-13,6.0895e-13
4.8988,6.9156e-13,6.074e-13
4.9017,6.958e-13,6.0657e-13
4.9047,6.9564e-13,6.0608e-13
4.9077,6.9994e-13,6.0508e-13
4.9107,7.0097e-13,6.0534e-13
4.9137,7.0127e-13,6.0514e-13
4.9166,7.0532e-13,6.0349e-13
4.9196,7.0519e-13,5.9978e-13
4.9226,7.091e-13,6.0072e-13
4.9256,7.1321e-13,6.0116e-13
4.9286,7.1315e-13,6.0042e-13
4.9315,7.1657e-13,5.9925e-13
4.9345,7.1904e-13,5.9915e-13
4.9375,7.2214e-13,5.9728e-13
4.9405,7.2362e-13,5.9619e-13
4.9435,7.2603e-13,5.962e-13
4.9464,7.2817e-13,5.9561e-13
4.9494,7.3219e-13,5.9359e-13
4.9524,7.3316e-13,5.9278e-13
4.9554,7.3477e-13,5.9345e-13
4.9584,7.3838e-13,5.922e-13
4.9614,7.4254e-13,5.9131e-13
4.9643,7.4649e-13,5.8956e-13
4.9673,7.4771e-13,5.8987e-13
4.9703,7.5087e-13,5.8805e-13
4.9733,7.5265e-13,5.8811e-13
4.9763,7.5581e-13,5.8802e-13
4.9792,7.5973e-13,5.8656e-13
4.9822,7.5967e-13,5.8498e-13
4.9852,7.6519e-13,5.8382e-13
4.9882,7.6464e-13,5.8304e-13
4.9912,7.6791e-13,5.828e-13
4.9941,7.7013e-13,5.8092e-13
4.9971,7.7266e-13,5.8057e-13
5.0001,7.7535e-13,5.8024e-13
5.0031,7.7818e-13,5.8013e-13
5.0061,7.8187e-13,5.7782e-13
5.009,7.8429e-13,5.7672e-13
5.012,7.8648e-13,5.7643e-13
5.015,7.8998e-13,5.7436e-13
5.018,7.9139e-13,5.7376e-13
5.021,7.9683e-13,5.7327e-13
5.0239,7.995e-13,5.7234e-13
5.0269,8.0322e-13,5.6959e-13
5.0299,8.0427e-13,5.7093e-13
5.0329,8.0802e-13,5.699e-13
5.0359,8.1116e-13,5.6773e-13
5.0388,8.1166e-13,5.6766e-13
5.0418,8.1662e-13,5.6568e-13
5.0448,8.1762e-13,5.6496e-13
5.0478,8.2193e-13,5.6212e-13
5.0508,8.252e-13,5.6301e-13
5.0538,8.2945e-13,5.6091e-13
5.0567,8.305e-13,5.6313e-13
5.0597,8.3344e-13,5.5961e-13
5.0627,8.3708e-13,5.5818e-13
5.0657,8.4097e-13,5.561e-13
5.0687,8.4219e-13,5.5597e-13
5.0716,8.471e-13,5.5675e-13
5.0746,8.4741e-13,5.542e-13
5.0776,8.5357e-13,5.5123e-13
5.0806,8.5726e-13,5.5018e-13
5.0836,8.5967e-13,5.4933e-13
5.0865,8.6192e-13,5.4883e-13
5.0895,8.6553e-13,5.4789e-13
5.0925,8.6872e-13,5.4685e-13
5.0955,8.72e-13,5.4609e-13
5.0985,8.7536e-13,5.4388e-13
5.1014,8.7833e-13,5.4284e-13
5.1044,8.8071e-13,5.4073e-13
5.1074,8.8499e-13,5.4125e-13
5.1104,8.8826e-13,5.384e-13
5.1134,8.897e-13,5.3839e-13
5.1163,8.9259e-13,5.3859e-13
5.1193,8.9659e-13,5.3583e-13
5.1223,9.0009e-13,5.3348e-13
5.1253,9.0608e-13,5.3398e-13
5.1283,9.0447e-13,5.3139e-13
5.1312,9.1221e-13,5.3095e-13
5.1342,9.143e-13,5.295e-13
5.1372,9.1666e-13,5.2808e-13
5.1402,9.1954e-13,5.2804e-13
5.1432,9.2393e-13,5.2621e-13
5.1461,9.2834e-13,5.2509e-13
5.1491,9.3256e-13,5.235e-13
5.1521,9.3464e-13,5.2201e-13
5.1551,9.413e-13,5.197e-13
5.1581,9.4105e-13,5.183e-13
5.1611,9.4477e-13,5.1878e-13
5.164,9.4891e-13,5.1715e-13
5.167,9.529e-13,5.148e-13
5.17,9.5596e-13,5.1421e-13
5.173,9.6029e-13,5.1185e-13
5.176,9.6376e-13,5.1224e-13
5.1789,9.6875e-13,5.0884e-13
5.1819,9.7047e-13,5.0769e-13
5.1849,9.7578e-13,5.0581e-13
5.1879,9.7788e-13,5.0605e-13
5.1909,9.8296e-13,5.0463e-13
5.1938,9.8696e-13,5.0175e-13
5.1968,9.8788e-13,5.014e-13
5.1998,9.9193e-13,5.0071e-13
5.2028,9.9709e-13,4.9873e-13
5.2058,1.0016e-12,4.9796e-13
5.2087,1.0046e-12,4.9398e-13
5.2117,1.0077e-12,4.9327e-13
5.2147,1.0113e-12,4.9185e-13
5.2177,1.0179e-12,4.9237e-13
5.2207,1.0203e-12,4.9033e-13
5.2236,1.024e-12,4.8812e-13
5.2266,1.03e-12,4.8651e-13
5.2296,1.0316e-12,4.8682e-13
5.2326,1.0369e-12,4.8472e-13
5.2356,1.0413e-12,4.8313e-13
5.2385,1.0458e-12,4.8113e-13
5.2415,1.0477e-12,4.7895e-13
5.2445,1.0522e-12,4.7776e-13
5.2475,1.056e-12,4.7526e-13
5.2505,1.061e-12,4.7299e-13
5.2535,1.0636e-12,4.7267e-13
5.2564,1.0695e-12,4.6983e-13
5.2594,1.0747e-12,4.6932e-13
5.2624,1.0765e-12,4.6708e-13
5.2654,1.081e-12,4.6545e-13
5.2684,1.0849e-12,4.6268e-13
5.2713,1.0895e-12,4.6366e-13
5.2743,1.095e-12,4.602e-13
5.2773,1.0969e-12,4.5758e-13
5.2803,1.1029e-12,4.5826e-13
5.2833,1.1066e-12,4.5585e-13
5.2862,1.1109e-12,4.5326e-13
5.2892,1.1141e-12,4.5269e-13
5.2922,1.1216e-12,4.5031e-13
5.2952,1.1261e-12,4.4773e-13
5.2982,1.1291e-12,4.4693e-13
5.3011,1.1339e-12,4.4441e-13
5.3041,1.1377e-12,4.4401e-13
5.3071,1.142e-12,4.4253e-13
5.3101,1.1476e-12,4.3864e-13
5.3131,1.151e-12,4.3838e-13
5.316,1.1559e-12,4.3617e-13
5.319,1.1605e-12,4.3377e-13
5.322,1.1658e-12,4.328e-13
5.325,1.1694e-12,4.3105e-13
5.328,1.1738e-12,4.2947e-13
5.3309,1.1786e-12,4.2504e-13
5.3339,1.1834e-12,4.248e-13
5.3369,1.1864e-12,4.2218e-13
5.3399,1.1919e-12,4.2099e-13
5.3429,1.1974e-12,4.1835e-13
5.3458,1.201e-12,4.1534e-13
5.3488,1.2072e-12,4.1615e-13
5.3518,1.2134e-12,4.1318e-13
5.3548,1.2159e-12,4.1131e-13
5.3578,1.2206e-12,4.1034e-13
5.3608,1.2271e-12,4.0878e-13
5.3637,1.2314e-12,4.0374e-13
5.3667,1.237e-12,4.0308e-13
5.3697,1.2403e-12,4.0246e-13
5.3727,1.2475e-12,3.9987e-13
5.3757,1.2523e-12,3.9802e-13
5.3786,1.2549e-12,3.948e-13
5.3816,1.2632e-12,3.9348e-13
5.3846,1.2663e-12,3.9211e-13
5.3876,1.2706e-12,3.8869e-13
5.3906,1.275e-12,3.8638e-13
5.3935,1.2778e-12,3.8395e-13
5.3965,1.2872e-12,3.8384e-13
5.3995,1.293e-12,3.8039e-13
5.4025,1.2966e-12,3.7971e-13
5.4055,1.3022e-12,3.7787e-13
5.4084,1.3057e-12,3.7584e-13
5.4114,1.3129e-12,3.717e-13
5.4144,1.3183e-12,3.7027e-13
5.4174,1.3236e-12,3.6763e-13
5.4204,1.3266e-12,3.6573e-13
5.4233,1.3339e-12,3.6468e-13
5.4263,1.339e-12,3.6088e-13
5.4293,1.3452e-12,3.5867e-13
5.4323,1.3508e-12,3.5729e-13
5.4353,1.3565e-12,3.5561e-13
5.4382,1.3623e-12,3.5244e-13
5.4412,1.3669e-12,3.4917e-13
5.4442,1.3717e-12,3.4844e-13
5.4472,1.3781e-12,3.4584e-13
5.4502,1.3817e-12,3.4349e-13
5.4532,1.3892e-12,3.4185e-13
5.4561,1.3914e-12,3.3831e-13
5.4591,1.4011e-12,3.3511e-13
5.4621,1.4073e-12,3.344e-13
5.4651,1.4119e-12,3.2997e-13
5.4681,1.418e-12,3.2975e-13
5.471,1.4201e-12,3.2623e-13
5.474,1.4267e-12,3.2643e-13
5.477,1.4325e-12,3.2059e-13
5.48,1.437e-12,3.1816e-13
5.483,1.4436e-12,3.1653e-13
5.4859,1.4489e-12,3.1413e-13
5.4889,1.4583e-12,3.1204e-13
5.4919,1.4622e-12,3.0815e-13
5.4949,1.4697e-12,3.0605e-13
5.4979,1.4744e-12,3.0433e-13
5.5008,1.4805e-12,3.0109e-13
5.5038,1.4839e-12,3.002e-13
5.5068,1.492e-12,2.9716e-13
5.5098,1.4973e-12,2.9628e-13
5.5128,1.5023e-12,2.9015e-13
5.5157,1.5103e-12,2.8928e-13
5.5187,1.5147e-12,2.8654e-13
5.5217,1.5223e-12,2.8332e-13
5.5247,1.5304e-12,2.8229e-13
5.5277,1.5337e-12,2.7902e-13
5.5306,1.5423e-12,2.754e-13
5.5336,1.5463e-12,2.73e-13
5.5366,1.554e-12,2.7062e-13
5.5396,1.561e-12,2.6776e-13
5.5426,1.5646e-12,2.6434e-13
5.5455,1.5707e-12,2.6432e-13
5.5485,1.5795e-12,2.6129e-13
5.5515,1.5844e-12,2.5796e-13
5.5545,1.5934e-12,2.5541e-13
5.5575,1.5982e-12,2.5186e-13
5.5605,1.6032e-12,2.4895e-13
5.5634,1.6116e-12,2.472e-13
5.5664,1.6195e-12,2.429e-13
5.5694,1.6264e-12,2.3978e-13
5.5724,1.6318e-12,2.3833e-13
5.5754,1.6386e-12,2.3522e-13
5.5783,1.6464e-12,2.3254e-13
5.5813,1.6528e-12,2.2932e-13
5.5843,1.6566e-12,2.2567e-13
5.5873,1.6655e-12,2.2375e-13
5.5903,1.6732e-12,2.2065e-13
5.5932,1.6786e-12,2.1691e-13
5.5962,1.6847e-12,2.1351e-13
5.5992,1.6935e-12,2.1192e-13
5.6022,1.699e-12,2.0907e-13
5.6052,1.7077e-12,2.0714e-13
5.6081,1.7141e-12,2.0357e-13
5.6111,1.7204e-12,2.0057e-13
5.6141,1.7273e-12,1.9681e-13
5.6171,1.7355e-12,1.9429e-13
5.6201,1.7417e-12,1.8993e-13
5.623,1.7518e-12,1.8858e-13
5.626,1.7557e-12,1.8518e-13
5.629,1.7642e-12,1.8263e-13
5.632,1.7708e-12,1.761e-13
5.635,1.7783e-12,1.7689e-13
5.6379,1.7837e-12,1.7141e-13
5.6409,1.792e-12,1.6951e-13
5.6439,1.8012e-12,1.6761e-13
5.6469,1.8048e-12,1.6408e-13
5.6499,1.8132e-12,1.605e-13
5.6529,1.8233e-12,1.5672e-13
5.6558,1.827e-12,1.5261e-13
5.6588,1.8395e-12,1.4867e-13
5.6618,1.8443e-12,1.4592e-13
5.6648,1.8506e-12,1.4518e-13
5.6678,1.8574e-12,1.3897e-13
5.6707,1.8647e-12,1.368e-13
5.6737,1.8742e-12,1.3469e-13
5.6767,1.8821e-12,1.3117e-13
5.6797,1.8938e-12,1.2756e-13
5.6827,1.8979e-12,1.2177e-13
5.6856,1.9081e-12,1.1904e-13
5.6886,1.9133e-12,1.1572e-13
5.6916,1.9234e-12,1.1233e-13
5.6946,1.9291e-12,1.1079e-13
5.6976,1.9352e-12,1.0614e-13
5.7005,1.9461e-12,1.0385e-13
5.7035,1.9515e-12,9.9801e-14
5.7065,1.96e-12,9.5973e-14
5.7095,1.9697e-12,9.2782e-14
5.7125,1.9781e-12,9.0343e-14
5.7154,1.9852e-12,8.7226e-14
5.7184,1.9958e-12,8.0613e-14
5.7214,2.0026e-12,7.9246e-14
5.7244,2.01e-12,7.4357e-14
5.7274,2.0189e-12,7.0486e-14
5.7303,2.0255e-12,6.8836e-14
5.7333,2.0354e-12,6.0793e-14
5.7363,2.0437e-12,5.9931e-14
5.7393,2.0531e-12,5.6398e-14
5.7423,2.0618e-12,5.5319e-14
5.7452,2.0692e-12,5.0807e-14
5.7482,2.076e-12,4.6824e-14
5.7512,2.0835e-12,4.4884e-14
5.7542,2.0938e-12,3.866e-14
5.7572,2.1003e-12,3.4552e-14
5.7602,2.1108e-12,3.0516e-14
5.7631,2.1213e-12,2.5556e-14
5.7661,2.1317e-12,2.429e-14
5.7691,2.138e-12,2.043e-14
5.7721,2.1479e-12,1.448e-14
5.7751,2.1571e-12,1.151e-14
5.778,2.1639e-12,8.5539e-15
5.781,2.1763e-12,6.7134e-16
5.784,2.181e-12,1.9377e-15
5.787,2.1911e-12,4.3819e-15
5.79,2.1992e-12,8.2486e-15
5.7929,2.2105e-12,1.2349e-14
5.7959,2.2188e-12,1.4086e-14
5.7989,2.2274e-12,2.0952e-14
5.8019,2.2359e-12,2.3872e-14
5.8049,2.247e-12,2.7943e-14
5.8078,2.2562e-12,3.0691e-14
5.8108,2.264e-12,3.4117e-14
5.8138,2.275e-12,3.9472e-14
5.8168,2.2819e-12,4.3625e-14
5.8198,2.2926e-12,4.9599e-14
5.8227,2.3017e-12,5.2599e-14
5.8257,2.3101e-12,5.615e-14
5.8287,2.3201e-12,5.7664e-14
5.8317,2.3329e-12,6.0724e-14
5.8347,2.3398e-12,6.9781e-14
5.8376,2.347e-12,7.0591e-14
5.8406,2.3614e-12,7.5863e-14
5.8436,2.3714e-12,8.1338e-14
5.8466,2.38e-12,8.5062e-14
5.8496,2.3893e-12,8.9906e-14
5.8526,2.3993e-12,9.5137e-14
5.8555,2.4125e-12,9.5424e-14
5.8585,2.4209e-12,1.0397e-13
5.8615,2.4277e-12,1.0668e-13
5.8645,2.4412e-12,1.1136e-13
5.8675,2.4463e-12,1.1725e-13
5.8704,2.4593e-12,1.2153e-13
5.8734,2.4694e-12,1.2642e-13
5.8764,2.4814e-12,1.2295e-13
5.8794,2.4886e-12,1.3272e-13
5.8824,2.4955e-12,1.3748e-13
5.8853,2.5085e-12,1.3921e-13
5.8883,2.5202e-12,1.4429e-13
5.8913,2.5278e-12,1.4878e-13
5.8943,2.5401e-12,1.5599e-13
5.8973,2.5511e-12,1.5952e-13
5.9002,2.5646e-12,1.6258e-13
5.9032,2.5706e-12,1.6797e-13
5.9062,2.5792e-12,1.7678e-13
5.9092,2.5917e-12,1.7779e-13
5.9122,2.6035e-12,1.8143e-13
5.9151,2.6121e-12,1.8604e-13
5.9181,2.6236e-12,1.905e-13
5.9211,2.6339e-12,1.9731e-13
5.9241,2.6439e-12,1.9802e-13
5.9271,2.6539e-12,2.0193e-13
5.93,2.6667e-12,2.0791e-13
5.933,2.6808e-12,2.1507e-13
5.936,2.6913e-12,2.186e-13
5.939,2.7024e-12,2.2493e-13
5.942,2.7123e-12,2.2877e-13
5.9449,2.7212e-12,2.3553e-13
5.9479,2.7332e-12,2.3905e-13
5.9509,2.7439e-12,2.4196e-13
5.9539,2.756e-12,2.4839e-13
5.9569,2.7687e-12,2.545e-13
5.9599,2.7828e-12,2.6122e-13
5.9628,2.7895e-12,2.6317e-13
5.9658,2.803e-12,2.6818e-13
5.9688,2.8133e-12,2.7407e-13
5.9718,2.8269e-12,2.7876e-13
5.9748,2.8342e-12,2.8145e-13
5.9777,2.8446e-12,2.9007e-13
5.9807,2.8613e-12,2.9534e-13
5.9837,2.8713e-12,2.985e-13
5.9867,2.8841e-12,3.0675e-13
5.9897,2.8939e-12,3.097e-13
5.9926,2.9073e-12,3.1195e-13
5.9956,2.9194e-12,3.1931e-13
5.9986,2.9345e-12,3.2288e-13
6.0016,2.9394e-12,3.31e-13
6.0046,2.9562e-12,3.3643e-13
6.0075,2.9657e-12,3.4102e-13
6.0105,2.9802e-12,3.465e-13
6.0135,2.9926e-12,3.5048e-13
6.0165,3.0026e-12,3.5678e-13
6.0195,3.0154e-12,3.621e-13
6.0224,3.0278e-12,3.6583e-13
6.0254,3.0392e-12,3.736e-13
6.0284,3.0568e-12,3.7584e-13
6.0314,3.0617e-12,3.8671e-13
6.0344,3.0775e-12,3.9021e-13
6.0373,3.0893e-12,3.9586e-13
6.0403,3.107e-12,3.9861e-13
6.0433,3.1199e-12,4.0811e-13
6.0463,3.1301e-12,4.1186e-13
6.0493,3.141e-12,4.2108e-13
6.0523,3.1512e-12,4.2203e-13
6.0552,3.1668e-12,4.2692e-13
6.0582,3.1772e-12,4.3598e-13
6.0612,3.1923e-12,4.4373e-13
6.0642,3.2072e-12,4.4523e-13
6.0672,3.218e-12,4.4898e-13
6.0701,3.2333e-12,4.5728e-13
6.0731,3.2452e-12,4.5925e-13
6.0761,3.2568e-12,4.6647e-13
6.0791,3.2726e-12,4.7224e-13
6.0821,3.2855e-12,4.8007e-13
6.085,3.298e-12,4.8269e-13
6.088,3.3118e-12,4.9304e-13
6.091,3.3271e-12,4.9354e-13
6.094,3.3412e-12,5.0183e-13
6.097,3.3521e-12,5.0949e-13
6.0999,3.3653e-12,5.1461e-13
6.1029,3.3792e-12,5.1786e-13
6.1059,3.393e-12,5.2839e-13
6.1089,3.4092e-12,5.3326e-13
6.1119,3.423e-12,5.3682e-13
6.1148,3.4334e-12,5.4527e-13
6.1178,3.4496e-12,5.5119e-13
6.1208,3.4641e-12,5.5957e-13
6.1238,3.4819e-12,5.6363e-13
6.1268,3.4893e-12,5.6804e-13
6.1297,3.5068e-12,5.7424e-13
6.1327,3.52e-12,5.7932e-13
6.1357,3.532e-12,5.8771e-13
6.1387,3.5458e-12,5.9594e-13
6.1417,3.5643e-12,5.97e-13
6.1446,3.5767e-12,6.0743e-13
6.1476,3.5915e-12,6.1511e-13
6.1506,3.6079e-12,6.1669e-13
6.1536,3.6224e-12,6.2331e-13
6.1566,3.6389e-12,6.2993e-13
6.1596,3.6528e-12,6.3565e-13
6.1625,3.6653e-12,6.447e-13
6.1655,3.6828e-12,6.4439e-13
6.1685,3.6941e-12,6.5783e-13
6.1715,3.7106e-12,6.6411e-13
6.1745,3.7242e-12,6.656e-13
6.1774,3.7398e-12,6.7784e-13
6.1804,3.7561e-12,6.841e-13
6.1834,3.7727e-12,6.8802e-13
6.1864,3.7867e-12,6.9444e-13
6.1894,3.8021e-12,7.0065e-13
6.1923,3.8191e-12,7.1293e-13
6.1953,3.835e-12,7.1503e-13
6.1983,3.8458e-12,7.2143e-13
6.2013,3.8687e-12,7.2809e-13
6.2043,3.8785e-12,7.343e-13
6.2072,3.8952e-12,7.4455e-13
6.2102,3.9081e-12,7.4939e-13
6.2132,3.9259e-12,7.562e-13
6.2162,3.9411e-12,7.6562e-13
6.2192,3.9631e-12,7.6941e-13
6.2221,3.979e-12,7.7738e-13
6.2251,3.9871e-12,7.8696e-13
6.2281,4.0065e-12,7.8788e-13
6.2311,4.0241e-12,7.9688e-13
6.2341,4.037e-12,8.0727e-13
6.237,4.0558e-12,8.1269e-13
6.24,4.0694e-12,8.1976e-13
6.243,4.091e-12,8.2551e-13
6.246,4.1063e-12,8.3109e-13
6.249,4.12e-12,8.4312e-13
6.252,4.1419e-12,8.4469e-13
6.2549,4.1562e-12,8.5265e-13
6.2579,4.1705e-12,8.5693e-13
6.2609,4.1862e-12,8.7309e-13
6.2639,4.2093e-12,8.7649e-13
6.2669,4.2221e-12,8.826e-13
6.2698,4.2376e-12,8.9061e-13
6.2728,4.2536e-12,8.9911e-13
6.2758,4.2707e-12,9.0646e-13
6.2788,4.2889e-12,9.124e-13
6.2818,4.3099e-12,9.1659e-13
6.2847,4.3264e-12,9.2735e-13
6.2877,4.3425e-12,9.3488e-13
6.2907,4.3561e-12,9.4077e-13
6.2937,4.3785e-12,9.5105e-13
6.2967,4.3932e-12,9.5297e-13
6.2996,4.4123e-12,9.6673e-13
6.3026,4.4278e-12,9.7192e-13
6.3056,4.447e-12,9.7871e-13
6.3086,4.4653e-12,9.8999e-13
6.3116,4.4847e-12,9.9836e-13
6.3145,4.5016e-12,1.0012e-12
6.3175,4.5189e-12,1.0111e-12
6.3205,4.5369e-12,1.0211e-12
6.3235,4.555e-12,1.0269e-12
6.3265,4.5729e-12,1.0326e-12
6.3294,4.5944e-12,1.0418e-12
6.3324,4.6149e-12,1.0472e-12
6.3354,4.6338e-12,1.058e-12
6.3384,4.6461e-12,1.067e-12
6.3414,4.6677e-12,1.0754e-12
6.3443,4.6853e-12,1.0844e-12
6.3473,4.7011e-12,1.0903e-12
6.3503,4.7228e-12,1.0967e-12
6.3533,4.7399e-12,1.1043e-12
6.3563,4.7561e-12,1.1162e-12
6.3593,4.7771e-12,1.1243e-12
6.3622,4.7931e-12,1.1365e-12
6.3652,4.8107e-12,1.1442e-12
6.3682,4.8355e-12,1.1475e-12
6.3712,4.8554e-12,1.151e-12
6.3742,4.8751e-12,1.1609e-12
6.3771,4.8909e-12,1.1726e-12
6.3801,4.9158e-12,1.1769e-12
6.3831,4.9319e-12,1.1896e-12
6.3861,4.9518e-12,1.2009e-12
6.3891,4.97e-12,1.1991e-12
6.392,4.9915e-12,1.2125e-12
6.395,5.0164e-12,1.2206e-12
6.398,5.0382e-12,1.2307e-12
6.401,5.0545e-12,1.2404e-12
6.404,5.0749e-12,1.2466e-12
6.4069,5.0908e-12,1.2554e-12
6.4099,5.1139e-12,1.2616e-12
6.4129,5.1332e-12,1.2778e-12
6.4159,5.1521e-12,1.2803e-12
6.4189,5.1709e-12,1.2958e-12
6.4218,5.1906e-12,1.2965e-12
6.4248,5.2102e-12,1.3099e-12
6.4278,5.2342e-12,1.315e-12
6.4308,5.2567e-12,1.3287e-12
6.4338,5.2791e-12,1.331e-12
6.4367,5.2964e-12,1.3448e-12
6.4397,5.3175e-12,1.3566e-12
6.4427,5.339e-12,1.3623e-12
6.4457,5.3617e-12,1.3734e-12
6.4487,5.3795e-12,1.3778e-12
6.4517,5.4021e-12,1.3895e-12
6.4546,5.4239e-12,1.3988e-12
6.4576,5.4487e-12,1.4078e-12
6.4606,5.4699e-12,1.4104e-12
6.4636,5.4848e-12,1.4258e-12
6.4666,5.5105e-12,1.4393e-12
6.4695,5.5358e-12,1.4447e-12
6.4725,5.555e-12,1.4532e-12
6.4755,5.577e-12,1.4627e-12
6.4785,5.5991e-12,1.4689e-12
6.4815,5.6199e-12,1.4846e-12
6.4844,5.6403e-12,1.4901e-12
6.4874,5.6615e-12,1.4973e-12
6.4904,5.6952e-12,1.5086e-12
6.4934,5.7132e-12,1.5186e-12
6.4964,5.7388e-12,1.5245e-12
6.4993,5.7583e-12,1.5431e-12
6.5023,5.7787e-12,1.547e-12
6.5053,5.8005e-12,1.5573e-12
6.5083,5.8208e-12,1.5715e-12
6.5113,5.8468e-12,1.5793e-12
6.5142,5.8696e-12,1.5838e-12
6.5172,5.8926e-12,1.6004e-12
6.5202,5.9147e-12,1.6064e-12
6.5232,5.9434e-12,1.6129e-12
6.5262,5.9645e-12,1.6265e-12
6.5291,5.9907e-12,1.6318e-12
6.5321,6.0131e-12,1.6481e-12
6.5351,6.0296e-12,1.6559e-12
6.5381,6.0525e-12,1.6652e-12
6.5411,6.0806e-12,1.6722e-12
6.544,6.1111e-12,1.6879e-12
6.547,6.1272e-12,1.6974e-12
6.55,6.1587e-12,1.7052e-12
6.553,6.1763e-12,1.7207e-12
6.556,6.1982e-12,1.7257e-12
6.559,6.2289e-12,1.7414e-12
6.5619,6.2476e-12,1.7467e-12
6.5649,6.2766e-12,1.7514e-12
6.5679,6.2992e-12,1.7704e-12
6.5709,6.3189e-12,1.7749e-12
6.5739,6.3496e-12,1.7897e-12
6.5768,6.3701e-12,1.8005e-12
6.5798,6.3949e-12,1.8028e-12
6.5828,6.4218e-12,1.8135e-12
6.5858,6.445e-12,1.826e-12
6.5888,6.4709e-12,1.8409e-12
6.5917,6.4988e-12,1.852e-12
6.5947,6.5197e-12,1.8592e-12
6.5977,6.5531e-12,1.8746e-12
6.6007,6.5777e-12,1.8804e-12
6.6037,6.5962e-12,1.8917e-12
6.6066,6.626e-12,1.9005e-12
6.6096,6.6524e-12,1.9123e-12
6.6126,6.6793e-12,1.9285e-12
6.6156,6.7101e-12,1.9329e-12
6.6186,6.7342e-12,1.9473e-12
6.6215,6.7542e-12,1.958e-12
6.6245,6.7862e-12,1.9703e-12
6.6275,6.8016e-12,1.9811e-12
6.6305,6.8368e-12,1.9889e-12
6.6335,6.8685e-12,2.0015e-12
6.6364,6.8878e-12,2.0168e-12
6.6394,6.9158e-12,2.0279e-12
6.6424,6.9473e-12,2.0342e-12
6.6454,6.9696e-12,2.0452e-12
6.6484,6.995e-12,2.0587e-12
6.6514,7.0212e-12,2.0694e-12
6.6543,7.0568e-12,2.0784e-12
6.6573,7.0771e-12,2.0904e-12
6.6603,7.1045e-12,2.1041e-12
6.6633,7.1374e-12,2.1132e-12
6.6663,7.1516e-12,2.1302e-12
6.6692,7.1862e-12,2.1387e-12
6.6722,7.2181e-12,2.1456e-12
6.6752,7.2455e-12,2.1578e-12
6.6782,7.2713e-12,2.173e-12
6.6812,7.302e-12,2.1878e-12
6.6841,7.3272e-12,2.2009e-12
6.6871,7.3552e-12,2.2083e-12
6.6901,7.3871e-12,2.2217e-12
6.6931,7.4135e-12,2.2281e-12
6.6961,7.4432e-12,2.2409e-12
6.699,7.4681e-12,2.2551e-12
6.702,7.5017e-12,2.2665e-12
6.705,7.5309e-12,2.2736e-12
6.708,7.5573e-12,2.296e-12
6.711,7.588e-12,2.3061e-12
6.7139,7.6193e-12,2.326e-12
6.7169,7.6449e-12,2.3298e-12
6.7199,7.6749e-12,2.3399e-12
6.7229,7.7059e-12,2.3464e-12
6.7259,7.7287e-12,2.3672e-12
6.7288,7.7625e-12,2.3694e-12
6.7318,7.7907e-12,2.3867e-12
6.7348,7.8192e-12,2.3986e-12
6.7378,7.8577e-12,2.4162e-12
6.7408,7.8746e-12,2.4231e-12
6.7437,7.9138e-12,2.4372e-12
6.7467,7.9421e-12,2.4501e-12
6.7497,7.9727e-12,2.4672e-12
6.7527,8.0055e-12,2.4747e-12
6.7557,8.0378e-12,2.4905e-12
6.7587,8.0677e-12,2.4982e-12
6.7616,8.095e-12,2.514e-12
6.7646,8.1305e-12,2.5286e-12
6.7676,8.159e-12,2.5389e-12
6.7706,8.186e-12,2.5517e-12
6.7736,8.2238e-12,2.5714e-12
6.7765,8.2545e-12,2.5792e-12
6.7795,8.2828e-12,2.5902e-12
6.7825,8.3168e-12,2.5979e-12
6.7855,8.3484e-12,2.6089e-12
6.7885,8.378e-12,2.6294e-12
6.7914,8.4106e-12,2.6341e-12
6.7944,8.4424e-12,2.6545e-12
6.7974,8.4812e-12,2.6655e-12
6.8004,8.5048e-12,2.6733e-12
6.8034,8.5435e-12,2.6948e-12
6.8063,8.5814e-12,2.7087e-12
6.8093,8.6166e-12,2.7223e-12
6.8123,8.6423e-12,2.7362e-12
6.8153,8.6678e-12,2.7545e-12
6.8183,8.7105e-12,2.7576e-12
6.8212,8.7365e-12,2.777e-12
6.8242,8.7771e-12,2.7848e-12
6.8272,8.8085e-12,2.8042e-12
6.8302,8.8432e-12,2.8145e-12
6.8332,8.8715e-12,2.8282e-12
6.8361,8.9102e-12,2.838e-12
6.8391,8.9369e-12,2.8596e-12
6.8421,8.9774e-12,2.8708e-12
6.8451,9.0097e-12,2.8902e-12
6.8481,9.0443e-12,2.9025e-12
6.8511,9.0764e-12,2.9116e-12
6.854,9.1073e-12,2.9248e-12
6.857,9.1517e-12,2.9441e-12
6.86,9.1801e-12,2.9512e-12
6.863,9.2097e-12,2.9667e-12
6.866,9.247e-12,2.9894e-12
6.8689,9.2917e-12,3.0039e-12
6.8719,9.32e-12,3.017e-12
6.8749,9.3555e-12,3.024e-12
6.8779,9.3929e-12,3.0386e-12
6.8809,9.426e-12,3.0507e-12
6.8838,9.4534e-12,3.0663e-12
6.8868,9.4968e-12,3.0769e-12
6.8898,9.5397e-12,3.0964e-12
6.8928,9.5663e-12,3.1064e-12
6.8958,9.606e-12,3.1363e-12
6.8987,9.6509e-12,3.1416e-12
6.9017,9.6755e-12,3.1551e-12
6.9047,9.7186e-12,3.1741e-12
6.9077,9.7581e-12,3.1896e-12
6.9107,9.7977e-12,3.2028e-12
6.9136,9.8279e-12,3.2142e-12
6.9166,9.866e-12,3.232e-12
6.9196,9.8975e-12,3.2506e-12
6.9226,9.9449e-12,3.2708e-12
6.9256,9.9819e-12,3.2785e-12
6.9285,1.0014e-11,3.2955e-12
6.9315,1.0049e-11,3.3037e-12
6.9345,1.0087e-11,3.328e-12
6.9375,1.0127e-11,3.3327e-12
6.9405,1.017e-11,3.349e-12
6.9434,1.02e-11,3.3753e-12
6.9464,1.0242e-11,3.3794e-12
6.9494,1.0283e-11,3.3973e-12
6.9524,1.0318e-11,3.4122e-12
6.9554,1.0356e-11,3.432e-12
6.9584,1.0396e-11,3.4366e-12
6.9613,1.0436e-11,3.4556e-12
6.9643,1.0476e-11,3.4792e-12
6.9673,1.0517e-11,3.4918e-12
6.9703,1.0555e-11,3.5073e-12
6.9733,1.0596e-11,3.5201e-12
6.9762,1.0626e-11,3.5377e-12
6.9792,1.0674e-11,3.5533e-12
6.9822,1.0717e-11,3.5714e-12
6.9852,1.0753e-11,3.5872e-12
6.9882,1.0787e-11,3.6062e-12
6.9911,1.0828e-11,3.6212e-12
6.9941,1.0874e-11,3.6276e-12
6.9971,1.0913e-11,3.6564e-12
7.0001,1.0952e-11,3.6657e-12
7.0031,1.0992e-11,3.6862e-12
7.006,1.1039e-11,3.7006e-12
7.009,1.1071e-11,3.7178e-12
7.012,1.1112e-11,3.7379e-12
7.015,1.116e-11,3.7539e-12
7.018,1.1201e-11,3.774e-12
7.0209,1.1236e-11,3.7778e-12
7.0239,1.1284e-11,3.7956e-12
7.0269,1.133e-11,3.8101e-12
7.0299,1.1378e-11,3.831e-12
7.0329,1.1409e-11,3.8472e-12
7.0358,1.145e-11,3.8635e-12
7.0388,1.1492e-11,3.8758e-12
7.0418,1.1534e-11,3.9062e-12
7.0448,1.1578e-11,3.915e-12
7.0478,1.1623e-11,3.9398e-12
7.0508,1.1674e-11,3.9484e-12
7.0537,1.1703e-11,3.9632e-12
7.0567,1.1757e-11,3.9841e-12
7.0597,1.18e-11,4.0028e-12
7.0627,1.1844e-11,4.022e-12
7.0657,1.1888e-11,4.0397e-12
7.0686,1.1928e-11,4.0486e-12
7.0716,1.1974e-11,4.0717e-12
7.0746,1.2024e-11,4.0814e-12
7.0776,1.2065e-11,4.1084e-12
7.0806,1.211e-11,4.1234e-12
7.0835,1.2157e-11,4.1403e-12
7.0865,1.2196e-11,4.1506e-12
7.0895,1.2245e-11,4.1771e-12
7.0925,1.2286e-11,4.194e-12
7.0955,1.2332e-11,4.2073e-12
7.0984,1.2371e-11,4.2228e-12
7.1014,1.2423e-11,4.251e-12
7.1044,1.2473e-11,4.2605e-12
7.1074,1.2517e-11,4.2754e-12
7.1104,1.2564e-11,4.2935e-12
7.1133,1.2612e-11,4.32e-12
7.1163,1.2657e-11,4.344e-12
7.1193,1.27e-11,4.3584e-12
7.1223,1.2752e-11,4.3804e-12
7.1253,1.2798e-11,4.3883e-12
7.1282,1.284e-11,4.4113e-12
7.1312,1.2892e-11,4.4285e-12
7.1342,1.2934e-11,4.4458e-12
7.1372,1.2986e-11,4.4633e-12
7.1402,1.3037e-11,4.4875e-12
7.1431,1.308e-11,4.5083e-12
7.1461,1.3134e-11,4.5245e-12
7.1491,1.3181e-11,4.5441e-12
7.1521,1.3222e-11,4.5572e-12
7.1551,1.3278e-11,4.575e-12
7.1581,1.3315e-11,4.5986e-12
7.161,1.3371e-11,4.6259e-12
7.164,1.3416e-11,4.6391e-12
7.167,1.3464e-11,4.6573e-12
7.17,1.3518e-11,4.6721e-12
7.173,1.3568e-11,4.689e-12
7.1759,1.3628e-11,4.7049e-12
7.1789,1.3674e-11,4.7294e-12
7.1819,1.3722e-11,4.7436e-12
7.1849,1.3775e-11,4.7735e-12
7.1879,1.3813e-11,4.7853e-12
7.1908,1.3868e-11,4.805e-12
7.1938,1.3922e-11,4.8245e-12
7.1968,1.3968e-11,4.837e-12
7.1998,1.4023e-11,4.8651e-12
7.2028,1.4072e-11,4.8764e-12
7.2057,1.4132e-11,4.901e-12
7.2087,1.4186e-11,4.9332e-12
7.2117,1.4235e-11,4.9521e-12
7.2147,1.4277e-11,4.968e-12
7.2177,1.4333e-11,4.9806e-12
7.2206,1.4384e-11,4.9963e-12
7.2236,1.4451e-11,5.019e-12
7.2266,1.448e-11,5.0526e-12
7.2296,1.4545e-11,5.0628e-12
7.2326,1.4592e-11,5.0871e-12
7.2355,1.4648e-11,5.0985e-12
7.2385,1.4696e-11,5.1244e-12
7.2415,1.4749e-11,5.1485e-12
7.2445,1.4799e-11,5.1646e-12
7.2475,1.4853e-11,5.1931e-12
7.2505,1.4914e-11,5.2051e-12
7.2534,1.4975e-11,5.226e-12
7.2564,1.5014e-11,5.2472e-12
7.2594,1.5074e-11,5.2667e-12
7.2624,1.5124e-11,5.294e-12
7.2654,1.5183e-11,5.3119e-12
7.2683,1.5246e-11,5.3402e-12
7.2713,1.5302e-11,5.352e-12
7.2743,1.535e-11,5.3792e-12
7.2773,1.5409e-11,5.399e-12
7.2803,1.5467e-11,5.4136e-12
7.2832,1.552e-11,5.4435e-12
7.2862,1.5575e-11,5.4536e-12
7.2892,1.5635e-11,5.4753e-12
7.2922,1.5686e-11,5.503e-12
7.2952,1.5744e-11,5.5244e-12
7.2981,1.5806e-11,5.5444e-12
7.3011,1.5865e-11,5.5669e-12
7.3041,1.5915e-11,5.5921e-12
7.3071,1.5974e-11,5.6132e-12
7.3101,1.6042e-11,5.628e-12
7.313,1.6096e-11,5.6559e-12
7.316,1.6149e-11,5.6741e-12
7.319,1.6202e-11,5.703e-12
7.322,1.6256e-11,5.714e-12
7.325,1.6328e-11,5.7455e-12
7.3279,1.6388e-11,5.7565e-12
7.3309,1.644e-11,5.8e-12
7.3339,1.649e-11,5.8001e-12
7.3369,1.6571e-11,5.8491e-12
7.3399,1.6628e-11,5.8694e-12
7.3428,1.669e-11,5.8732e-12
7.3458,1.6738e-11,5.8929e-12
7.3488,1.6798e-11,5.9287e-12
7.3518,1.6863e-11,5.9466e-12
7.3548,1.6919e-11,5.9658e-12
7.3578,1.6981e-11,5.9775e-12
7.3607,1.7047e-11,6.0192e-12
7.3637,1.7103e-11,6.0335e-12
7.3667,1.716e-11,6.0549e-12
7.3697,1.7233e-11,6.082e-12
7.3727,1.7293e-11,6.0926e-12
7.3756,1.7352e-11,6.1302e-12
7.3786,1.7411e-11,6.1539e-12
7.3816,1.7476e-11,6.1762e-12
7.3846,1.754e-11,6.1962e-12
7.3876,1.7602e-11,6.2126e-12
7.3905,1.7666e-11,6.2503e-12
7.3935,1.7734e-11,6.2485e-12
7.3965,1.7784e-11,6.2855e-12
7.3995,1.7854e-11,6.324e-12
7.4025,1.793e-11,6.3388e-12
7.4054,1.7981e-11,6.3729e-12
7.4084,1.8042e-11,6.3841e-12
7.4114,1.8116e-11,6.4237e-12
7.4144,1.8178e-11,6.4427e-12
7.4174,1.8245e-11,6.4496e-12
7.4203,1.8299e-11,6.4855e-12
7.4233,1.8382e-11,6.506e-12
7.4263,1.8437e-11,6.5369e-12
7.4293,1.8497e-11,6.563e-12
7.4323,1.8579e-11,6.5629e-12
7.4352,1.8645e-11,6.6173e-12
7.4382,1.8707e-11,6.6302e-12
7.4412,1.876e-11,6.6499e-12
7.4442,1.8838e-11,6.6787e-12
7.4472,1.89e-11,6.6951e-12
7.4502,1.8971e-11,6.7411e-12
7.4531,1.9044e-11,6.7412e-12
7.4561,1.9105e-11,6.7808e-12
7.4591,1.9174e-11,6.8094e-12
7.4621,1.9231e-11,6.8232e-12
7.4651,1.9304e-11,6.8516e-12
7.468,1.937e-11,6.8763e-12
7.471,1.9446e-11,6.9069e-12
7.474,1.9497e-11,6.9324e-12
7.477,1.9566e-11,6.9557e-12
7.48,1.9645e-11,6.9692e-12
7.4829,1.9729e-11,7.007e-12
7.4859,1.9783e-11,7.0298e-12
7.4889,1.9865e-11,7.0626e-12
7.4919,1.993e-11,7.0713e-12
7.4949,2.0005e-11,7.1083e-12
7.4978,2.008e-11,7.1418e-12
7.5008,2.0154e-11,7.1754e-12
7.5038,2.0215e-11,7.1846e-12
7.5068,2.0298e-11,7.2122e-12
7.5098,2.0352e-11,7.2395e-12
7.5127,2.0434e-11,7.2607e-12
7.5157,2.0495e-11,7.2897e-12
7.5187,2.0575e-11,7.3073e-12
7.5217,2.0646e-11,7.3367e-12
7.5247,2.0736e-11,7.3506e-12
7.5276,2.0798e-11,7.393e-12
7.5306,2.0883e-11,7.4139e-12
7.5336,2.0947e-11,7.4463e-12
7.5366,2.1022e-11,7.4714e-12
7.5396,2.1078e-11,7.4986e-12
7.5425,2.1156e-11,7.5333e-12
7.5455,2.1234e-11,7.542e-12
7.5485,2.1318e-11,7.5664e-12
7.5515,2.1391e-11,7.602e-12
7.5545,2.1464e-11,7.6341e-12
7.5575,2.1545e-11,7.6667e-12
7.5604,2.1614e-11,7.6953e-12
7.5634,2.1684e-11,7.7243e-12
7.5664,2.1758e-11,7.7299e-12
7.5694,2.1839e-11,7.7795e-12
7.5724,2.1915e-11,7.7939e-12
7.5753,2.1999e-11,7.8319e-12
7.5783,2.2059e-11,7.8665e-12
7.5813,2.2134e-11,7.8766e-12
7.5843,2.2226e-11,7.8978e-12
7.5873,2.2297e-11,7.9451e-12
7.5902,2.2382e-11,7.9637e-12
7.5932,2.246e-11,7.9855e-12
7.5962,2.2544e-11,8.0393e-12
7.5992,2.2616e-11,8.0545e-12
7.6022,2.2703e-11,8.0797e-12
7.6051,2.2783e-11,8.1106e-12
7.6081,2.2861e-11,8.1313e-12
7.6111,2.295e-11,8.1601e-12
7.6141,2.3003e-11,8.1938e-12
7.6171,2.3099e-11,8.2296e-12
7.62,2.3184e-11,8.2357e-12
7.623,2.3263e-11,8.2708e-12
7.626,2.3346e-11,8.3047e-12
7.629,2.343e-11,8.3349e-12
7.632,2.3502e-11,8.359e-12
7.6349,2.3584e-11,8.3882e-12
7.6379,2.3665e-11,8.4236e-12
7.6409,2.3746e-11,8.4551e-12
7.6439,2.3833e-11,8.4817e-12
7.6469,2.3911e-11,8.5182e-12
7.6498,2.3985e-11,8.5371e-12
7.6528,2.4081e-11,8.5765e-12
7.6558,2.4168e-11,8.6027e-12
7.6588,2.4248e-11,8.6261e-12
7.6618,2.4326e-11,8.6695e-12
7.6648,2.4409e-11,8.7029e-12
7.6677,2.4493e-11,8.7267e-12
7.6707,2.4584e-11,8.7509e-12
7.6737,2.4664e-11,8.7754e-12
7.6767,2.4751e-11,8.8117e-12
7.6797,2.4827e-11,8.8263e-12
7.6826,2.4903e-11,8.8603e-12
7.6856,2.5008e-11,8.9083e-12
7.6886,2.5096e-11,8.9352e-12
7.6916,2.5187e-11,8.9538e-12
7.6946,2.5268e-11,8.9833e-12
7.6975,2.5349e-11,9.001e-12
7.7005,2.5454e-11,9.0448e-12
7.7035,2.5545e-11,9.0951e-12
7.7065,2.5638e-11,9.1119e-12
7.7095,2.5696e-11,9.1356e-12
7.7124,2.58e-11,9.168e-12
7.7154,2.5883e-11,9.202e-12
7.7184,2.5989e-11,9.2455e-12
7.7214,2.6085e-11,9.2643e-12
7.7244,2.6158e-11,9.3008e-12
7.7273,2.6239e-11,9.331e-12
7.7303,2.635e-11,9.3803e-12
7.7333,2.6427e-11,9.4024e-12
7.7363,2.6528e-11,9.425e-12
7.7393,2.6615e-11,9.4506e-12
7.7422,2.6706e-11,9.4866e-12
7.7452,2.6811e-11,9.5218e-12
7.7482,2.6888e-11,9.559e-12
7.7512,2.698e-11,9.5747e-12
7.7542,2.7073e-11,9.6212e-12
7.7572,2.7159e-11,9.6571e-12
7.7601,2.7263e-11,9.6742e-12
7.7631,2.736e-11,9.716e-12
7.7661,2.7445e-11,9.745e-12
7.7691,2.7557e-11,9.7622e-12
7.7721,2.7632e-11,9.8232e-12
7.775,2.7728e-11,9.8457e-12
7.778,2.7818e-11,9.8789e-12
7.781,2.7921e-11,9.9116e-12
7.784,2.8015e-11,9.9643e-12
7.787,2.8109e-11,9.979e-12
7.7899,2.8212e-11,1.0016e-11
7.7929,2.8312e-11,1.0053e-11
7.7959,2.8402e-11,1.0077e-11
7.7989,2.8516e-11,1.0107e-11
7.8019,2.8604e-11,1.0144e-11
7.8048,2.8718e-11,1.0187e-11
7.8078,2.8805e-11,1.0211e-11
7.8108,2.8891e-11,1.0255e-11
7.8138,2.8996e-11,1.0286e-11
7.8168,2.9098e-11,1.0315e-11
7.8197,2.9179e-11,1.0356e-11
7.8227,2.9283e-11,1.038e-11
7.8257,2.9409e-11,1.0409e-11
7.8287,2.9492e-11,1.0451e-11
7.8317,2.9591e-11,1.049e-11
7.8346,2.9691e-11,1.0539e-11
7.8376,2.9789e-11,1.0537e-11
7.8406,2.9889e-11,1.0596e-11
7.8436,3.0002e-11,1.0633e-11
7.8466,3.0094e-11,1.0659e-11
7.8495,3.0189e-11,1.0695e-11
7.8525,3.0301e-11,1.0732e-11
7.8555,3.0412e-11,1.0775e-11
7.8585,3.0498e-11,1.0786e-11
7.8615,3.0626e-11,1.0829e-11
7.8645,3.0719e-11,1.0867e-11
7.8674,3.0817e-11,1.0886e-11
7.8704,3.0943e-11,1.0938e-11
7.8734,3.102e-11,1.0964e-11
7.8764,3.1127e-11,1.1024e-11
7.8794,3.1247e-11,1.1047e-11
7.8823,3.1347e-11,1.1081e-11
7.8853,3.1448e-11,1.1107e-11
7.8883,3.1557e-11,1.1147e-11
7.8913,3.1664e-11,1.1168e-11
7.8943,3.1768e-11,1.1232e-11
7.8972,3.1886e-11,1.1266e-11
7.9002,3.1987e-11,1.1306e-11
7.9032,3.21e-11,1.1339e-11
7.9062,3.2204e-11,1.1377e-11
7.9092,3.2325e-11,1.1417e-11
7.9121,3.2436e-11,1.1436e-11
7.9151,3.2559e-11,1.1482e-11
7.9181,3.2656e-11,1.1517e-11
7.9211,3.2757e-11,1.1557e-11
7.9241,3.2882e-11,1.1595e-11
7.927,3.2979e-11,1.1636e-11
7.93,3.3096e-11,1.1666e-11
7.933,3.3207e-11,1.1691e-11
7.936,3.3332e-11,1.1736e-11
7.939,3.342e-11,1.1773e-11
7.9419,3.3563e-11,1.1828e-11
7.9449,3.3679e-11,1.1848e-11
7.9479,3.3787e-11,1.1888e-11
7.9509,3.3895e-11,1.1911e-11
7.9539,3.3987e-11,1.1958e-11
7.9569,3.4118e-11,1.1985e-11
7.9598,3.4234e-11,1.2046e-11
7.9628,3.4342e-11,1.209e-11
7.9658,3.4457e-11,1.2115e-11
7.9688,3.4584e-11,1.2161e-11
7.9718,3.4688e-11,1.2194e-11
7.9747,3.4832e-11,1.2249e-11
7.9777,3.4926e-11,1.2278e-11
7.9807,3.5052e-11,1.2295e-11
7.9837,3.516e-11,1.2346e-11
7.9867,3.5271e-11,1.2377e-11
7.9896,3.5398e-11,1.2424e-11
7.9926,3.5507e-11,1.2457e-11
7.9956,3.5635e-11,1.2495e-11
7.9986,3.574e-11,1.2527e-11
8.0016,3.5883e-11,1.2574e-11
8.0045,3.5993e-11,1.2615e-11
8.0075,3.6115e-11,1.2648e-11
8.0105,3.6247e-11,1.2702e-11
8.0135,3.6388e-11,1.2734e-11
8.0165,3.6481e-11,1.2763e-11
8.0194,3.6617e-11,1.2821e-11
8.0224,3.6722e-11,1.2855e-11
8.0254,3.6848e-11,1.2897e-11
8.0284,3.6973e-11,1.2944e-11
8.0314,3.7078e-11,1.2984e-11
8.0343,3.7234e-11,1.3026e-11
8.0373,3.7351e-11,1.307e-11
8.0403,3.7467e-11,1.3118e-11
8.0433,3.761e-11,1.315e-11
8.0463,3.7725e-11,1.3171e-11
8.0492,3.7826e-11,1.3213e-11
8.0522,3.7971e-11,1.3246e-11
8.0552,3.8093e-11,1.3309e-11
8.0582,3.8199e-11,1.3327e-11
8.0612,3.8378e-11,1.3391e-11
8.0642,3.8494e-11,1.3431e-11
8.0671,3.8613e-11,1.3471e-11
8.0701,3.8736e-11,1.3515e-11
8.0731,3.8886e-11,1.3554e-11
8.0761,3.9008e-11,1.3612e-11
8.0791,3.9139e-11,1.3636e-11
8.082,3.9264e-11,1.3666e-11
8.085,3.9396e-11,1.3725e-11
8.088,3.9533e-11,1.3757e-11
8.091,3.9675e-11,1.3827e-11
8.094,3.9789e-11,1.3858e-11
8.0969,3.9914e-11,1.3859e-11
8.0999,4.0053e-11,1.394e-11
8.1029,4.0171e-11,1.3981e-11
8.1059,4.0293e-11,1.3998e-11
8.1089,4.0445e-11,1.4047e-11
8.1118,4.0593e-11,1.412e-11
8.1148,4.0713e-11,1.4156e-11
8.1178,4.0846e-11,1.4188e-11
8.1208,4.0973e-11,1.422e-11
8.1238,4.1104e-11,1.4288e-11
8.1267,4.1255e-11,1.4332e-11
8.1297,4.1387e-11,1.4349e-11
8.1327,4.1525e-11,1.4415e-11
8.1357,4.1661e-11,1.4443e-11
8.1387,4.1788e-11,1.4492e-11
8.1416,4.1933e-11,1.4535e-11
8.1446,4.2057e-11,1.4606e-11
8.1476,4.2216e-11,1.4622e-11
8.1506,4.2366e-11,1.4668e-11
8.1536,4.2489e-11,1.4708e-11
8.1566,4.2632e-11,1.4754e-11
8.1595,4.2777e-11,1.4827e-11
8.1625,4.2953e-11,1.4876e-11
8.1655,4.3081e-11,1.4881e-11
8.1685,4.3197e-11,1.4907e-11
8.1715,4.3332e-11,1.4992e-11
8.1744,4.3479e-11,1.5024e-11
8.1774,4.3619e-11,1.507e-11
8.1804,4.3764e-11,1.5124e-11
8.1834,4.3923e-11,1.5171e-11
8.1864,4.4069e-11,1.5219e-11
8.1893,4.4202e-11,1.5256e-11
8.1923,4.4357e-11,1.5314e-11
8.1953,4.4506e-11,1.5354e-11
8.1983,4.4648e-11,1.5392e-11
8.2013,4.4807e-11,1.5429e-11
8.2042,4.4909e-11,1.5495e-11
8.2072,4.5097e-11,1.5517e-11
8.2102,4.5247e-11,1.5582e-11
8.2132,4.5383e-11,1.5606e-11
8.2162,4.5543e-11,1.5653e-11
8.2191,4.5686e-11,1.5699e-11
8.2221,4.5853e-11,1.5775e-11
8.2251,4.5978e-11,1.5843e-11
8.2281,4.6156e-11,1.585e-11
8.2311,4.6281e-11,1.5905e-11
8.234,4.6443e-11,1.5942e-11
8.237,4.6599e-11,1.5996e-11
8.24,4.6757e-11,1.6046e-11
8.243,4.6916e-11,1.609e-11
8.246,4.709e-11,1.6149e-11
8.2489,4.7187e-11,1.6178e-11
8.2519,4.7357e-11,1.6217e-11
8.2549,4.7522e-11,1.6287e-11
8.2579,4.7636e-11,1.633e-11
8.2609,4.7833e-11,1.6378e-11
8.2639,4.797e-11,1.6422e-11
8.2668,4.8148e-11,1.6475e-11
8.2698,4.8301e-11,1.6514e-11
8.2728,4.8457e-11,1.6589e-11
8.2758,4.8575e-11,1.662e-11
8.2788,4.8777e-11,1.6669e-11
8.2817,4.8908e-11,1.6703e-11
8.2847,4.9099e-11,1.6767e-11
8.2877,4.9233e-11,1.6789e-11
8.2907,4.9387e-11,1.6875e-11
8.2937,4.9568e-11,1.6917e-11
8.2966,4.9748e-11,1.6932e-11
8.2996,4.9894e-11,1.7014e-11
8.3026,5.0069e-11,1.7051e-11
8.3056,5.0224e-11,1.7121e-11
8.3086,5.0375e-11,1.7151e-11
8.3115,5.0502e-11,1.721e-11
8.3145,5.0755e-11,1.7258e-11
8.3175,5.0852e-11,1.73e-11
8.3205,5.1061e-11,1.7319e-11
8.3235,5.1199e-11,1.74e-11
8.3264,5.1351e-11,1.7442e-11
8.3294,5.1558e-11,1.7499e-11
8.3324,5.1725e-11,1.7544e-11
8.3354,5.1872e-11,1.7628e-11
8.3384,5.2018e-11,1.7643e-11
8.3413,5.2238e-11,1.7695e-11
8.3443,5.239e-11,1.7756e-11
8.3473,5.2567e-11,1.7795e-11
8.3503,5.2724e-11,1.7847e-11
8.3533,5.2857e-11,1.7933e-11
8.3563,5.3058e-11,1.795e-11
8.3592,5.3226e-11,1.8029e-11
8.3622,5.341e-11,1.8075e-11
8.3652,5.3568e-11,1.8133e-11
8.3682,5.3767e-11,1.8176e-11
8.3712,5.3943e-11,1.8247e-11
8.3741,5.4117e-11,1.8264e-11
8.3771,5.4294e-11,1.8341e-11
8.3801,5.4471e-11,1.8354e-11
8.3831,5.4629e-11,1.8423e-11
8.3861,5.4796e-11,1.848e-11
8.389,5.5e-11,1.8523e-11
8.392,5.5161e-11,1.8594e-11
8.395,5.5337e-11,1.8653e-11
8.398,5.5527e-11,1.8669e-11
8.401,5.571e-11,1.8725e-11
8.4039,5.5878e-11,1.8789e-11
8.4069,5.606e-11,1.886e-11
8.4099,5.6209e-11,1.8904e-11
8.4129,5.6429e-11,1.8965e-11
8.4159,5.6597e-11,1.8996e-11
8.4188,5.6779e-11,1.9058e-11
8.4218,5.7014e-11,1.9122e-11
8.4248,5.7129e-11,1.9148e-11
8.4278,5.7314e-11,1.9251e-11
8.4308,5.7498e-11,1.9305e-11
8.4337,5.7701e-11,1.9355e-11
8.4367,5.7863e-11,1.9389e-11
8.4397,5.807e-11,1.9424e-11
8.4427,5.8249e-11,1.9463e-11
8.4457,5.8402e-11,1.9576e-11
8.4486,5.8671e-11,1.9617e-11
8.4516,5.8835e-11,1.967e-11
8.4546,5.9031e-11,1.9733e-11
8.4576,5.9183e-11,1.9774e-11
8.4606,5.9389e-11,1.9824e-11
8.4636,5.9572e-11,1.99e-11
8.4665,5.9804e-11,1.9948e-11
8.4695,5.9963e-11,1.9974e-11
8.4725,6.0143e-11,2.0041e-11
8.4755,6.0397e-11,2.0102e-11
8.4785,6.0554e-11,2.0161e-11
8.4814,6.0737e-11,2.0213e-11
8.4844,6.0972e-11,2.0261e-11
8.4874,6.1142e-11,2.0362e-11
8.4904,6.1337e-11,2.0419e-11
8.4934,6.1532e-11,2.0478e-11
8.4963,6.1731e-11,2.0501e-11
8.4993,6.1923e-11,2.0555e-11
8.5023,6.2128e-11,2.0622e-11
8.5053,6.2341e-11,2.0683e-11
8.5083,6.2515e-11,2.0726e-11
8.5112,6.2689e-11,2.0832e-11
8.5142,6.293e-11,2.0853e-11
8.5172,6.3123e-11,2.0896e-11
8.5202,6.3355e-11,2.0951e-11
8.5232,6.3484e-11,2.1018e-11
8.5261,6.3697e-11,2.1051e-11
8.5291,6.3923e-11,2.1122e-11
8.5321,6.4133e-11,2.12e-11
8.5351,6.4329e-11,2.1237e-11
8.5381,6.4511e-11,2.1297e-11
8.541,6.4748e-11,2.1356e-11
8.544,6.4905e-11,2.1447e-11
8.547,6.5144e-11,2.1474e-11
8.55,6.5332e-11,2.1507e-11
8.553,6.5574e-11,2.1594e-11
8.556,6.5786e-11,2.1661e-11
8.5589,6.5979e-11,2.1716e-11
8.5619,6.6202e-11,2.1752e-11
8.5649,6.6373e-11,2.1889e-11
8.5679,6.6627e-11,2.1929e-11
8.5709,6.6811e-11,2.1967e-11
8.5738,6.7014e-11,2.2016e-11
8.5768,6.7277e-11,2.2093e-11
8.5798,6.7452e-11,2.215e-11
8.5828,6.768e-11,2.221e-11
8.5858,6.7915e-11,2.2279e-11
8.5887,6.8112e-11,2.2335e-11
8.5917,6.8331e-11,2.2378e-11
8.5947,6.8571e-11,2.2414e-11
8.5977,6.8763e-11,2.2545e-11
8.6007,6.8967e-11,2.2552e-11
8.6036,6.9202e-11,2.2662e-11
8.6066,6.9415e-11,2.2698e-11
8.6096,6.9609e-11,2.2736e-11
8.6126,6.9879e-11,2.2806e-11
8.6156,7.0062e-11,2.2892e-11
8.6185,7.0281e-11,2.2921e-11
8.6215,7.0488e-11,2.3e-11
8.6245,7.0743e-11,2.3059e-11
8.6275,7.0953e-11,2.3112e-11
8.6305,7.1207e-11,2.3175e-11
8.6334,7.1421e-11,2.3277e-11
8.6364,7.1609e-11,2.3303e-11
8.6394,7.185e-11,2.3339e-11
8.6424,7.2063e-11,2.3419e-11
8.6454,7.2283e-11,2.347e-11
8.6483,7.2565e-11,2.3557e-11
8.6513,7.2761e-11,2.3624e-11
8.6543,7.3022e-11,2.3704e-11
8.6573,7.322e-11,2.3763e-11
8.6603,7.3438e-11,2.3805e-11
8.6633,7.3721e-11,2.3853e-11
8.6662,7.3936e-11,2.3942e-11
8.6692,7.4209e-11,2.3972e-11
8.6722,7.4381e-11,2.4068e-11
8.6752,7.4629e-11,2.4078e-11
8.6782,7.4869e-11,2.4183e-11
8.6811,7.5095e-11,2.4232e-11
8.6841,7.5339e-11,2.432e-11
8.6871,7.5576e-11,2.4378e-11
8.6901,7.5787e-11,2.4442e-11
8.6931,7.6054e-11,2.4509e-11
8.696,7.6301e-11,2.4574e-11
8.699,7.6538e-11,2.462e-11
8.702,7.6749e-11,2.4708e-11
8.705,7.6983e-11,2.478e-11
8.708,7.722e-11,2.4844e-11
8.7109,7.752e-11,2.4918e-11
8.7139,7.7745e-11,2.4983e-11
8.7169,7.795e-11,2.5058e-11
8.7199,7.8231e-11,2.5096e-11
8.7229,7.8469e-11,2.5197e-11
8.7258,7.8698e-11,2.5245e-11
8.7288,7.8981e-11,2.5322e-11
8.7318,7.9205e-11,2.5348e-11
8.7348,7.9463e-11,2.5449e-11
8.7378,7.9709e-11,2.5522e-11
8.7407,7.9931e-11,2.556e-11
8.7437,8.0215e-11,2.5653e-11
8.7467,8.0462e-11,2.5725e-11
8.7497,8.0706e-11,2.5763e-11
8.7527,8.0962e-11,2.5853e-11
8.7557,8.1204e-11,2.5904e-11
8.7586,8.1442e-11,2.5969e-11
8.7616,8.1697e-11,2.5997e-11
8.7646,8.1958e-11,2.6106e-11
8.7676,8.2241e-11,2.6179e-11
8.7706,8.2498e-11,2.6221e-11
8.7735,8.2754e-11,2.6323e-11
8.7765,8.2969e-11,2.6413e-11
8.7795,8.3245e-11,2.6438e-11
8.7825,8.3519e-11,2.653e-11
8.7855,8.3785e-11,2.6582e-11
8.7884,8.405e-11,2.6645e-11
8.7914,8.4332e-11,2.6699e-11
8.7944,8.4587e-11,2.6818e-11
8.7974,8.4814e-11,2.6872e-11
8.8004,8.5103e-11,2.6949e-11
8.8033,8.5358e-11,2.6989e-11
8.8063,8.5639e-11,2.7083e-11
8.8093,8.5893e-11,2.7155e-11
8.8123,8.6147e-11,2.7231e-11
8.8153,8.6458e-11,2.7304e-11
8.8182,8.6658e-11,2.7364e-11
8.8212,8.6918e-11,2.7453e-11
8.8242,8.7237e-11,2.7481e-11
8.8272,8.7497e-11,2.7571e-11
8.8302,8.7785e-11,2.7638e-11
8.8331,8.8035e-11,2.7727e-11
8.8361,8.8285e-11,2.7776e-11
8.8391,8.8582e-11,2.7813e-11
8.8421,8.8895e-11,2.7933e-11
8.8451,8.9118e-11,2.8005e-11
8.848,8.9452e-11,2.8059e-11
8.851,8.9681e-11,2.8142e-11
8.854,8.9922e-11,2.8217e-11
8.857,9.0247e-11,2.8282e-11
8.86,9.0473e-11,2.8365e-11
8.863,9.0794e-11,2.8436e-11
8.8659,9.1036e-11,2.8533e-11
8.8689,9.1367e-11,2.859e-11
8.8719,9.1635e-11,2.8614e-11
8.8749,9.1949e-11,2.8672e-11
8.8779,9.2247e-11,2.8812e-11
8.8808,9.2471e-11,2.8882e-11
8.8838,9.2779e-11,2.8991e-11
8.8868,9.3047e-11,2.9002e-11
8.8898,9.3355e-11,2.9086e-11
8.8928,9.3689e-11,2.9129e-11
8.8957,9.3895e-11,2.9226e-11
8.8987,9.4236e-11,2.9274e-11
8.9017,9.454e-11,2.9384e-11
8.9047,9.4781e-11,2.9475e-11
8.9077,9.5074e-11,2.9518e-11
8.9106,9.538e-11,2.9578e-11
8.9136,9.5746e-11,2.9659e-11
8.9166,9.5992e-11,2.9776e-11
8.9196,9.6279e-11,2.9817e-11
8.9226,9.659e-11,2.9883e-11
8.9255,9.6887e-11,2.9985e-11
8.9285,9.7154e-11,2.9997e-11
8.9315,9.7487e-11,3.0104e-11
8.9345,9.776e-11,3.0203e-11
8.9375,9.8098e-11,3.0294e-11
8.9404,9.8359e-11,3.0376e-11
8.9434,9.8641e-11,3.0442e-11
8.9464,9.8966e-11,3.0465e-11
8.9494,9.9237e-11,3.0553e-11
8.9524,9.9584e-11,3.0651e-11
8.9554,9.9826e-11,3.0703e-11
8.9583,1.0022e-10,3.0856e-11
8.9613,1.0048e-10,3.0847e-11
8.9643,1.0076e-10,3.0974e-11
8.9673,1.0106e-10,3.1069e-11
8.9703,1.0146e-10,3.1108e-11
8.9732,1.0174e-10,3.1211e-11
8.9762,1.0207e-10,3.1267e-11
8.9792,1.0235e-10,3.1316e-11
8.9822,1.0268e-10,3.1447e-11
8.9852,1.0301e-10,3.1449e-11
8.9881,1.0324e-10,3.1545e-11
8.9911,1.0359e-10,3.1616e-11
8.9941,1.0399e-10,3.172e-11
8.9971,1.0428e-10,3.1789e-11
9.0001,1.046e-10,3.1872e-11
9.003,1.0488e-10,3.2007e-11
9.006,1.0525e-10,3.2053e-11
9.009,1.0556e-10,3.2138e-11
9.012,1.0589e-10,3.2232e-11
9.015,1.0617e-10,3.2306e-11
9.0179,1.0643e-10,3.2373e-11
9.0209,1.0679e-10,3.2431e-11
9.0239,1.071e-10,3.2527e-11
9.0269,1.0751e-10,3.2604e-11
9.0299,1.078e-10,3.2682e-11
9.0328,1.0811e-10,3.2773e-11
9.0358,1.0852e-10,3.2842e-11
9.0388,1.088e-10,3.2918e-11
9.0418,1.0911e-10,3.299e-11
9.0448,1.0945e-10,3.3125e-11
9.0477,1.0978e-10,3.3178e-11
9.0507,1.1014e-10,3.3269e-11
9.0537,1.1045e-10,3.3298e-11
9.0567,1.1082e-10,3.339e-11
9.0597,1.1113e-10,3.3519e-11
9.0627,1.1148e-10,3.3542e-11
9.0656,1.1182e-10,3.3603e-11
9.0686,1.1218e-10,3.37e-11
9.0716,1.1244e-10,3.387e-11
9.0746,1.1285e-10,3.3883e-11
9.0776,1.1313e-10,3.4035e-11
9.0805,1.1357e-10,3.4056e-11
9.0835,1.1391e-10,3.4113e-11
9.0865,1.1429e-10,3.427e-11
9.0895,1.1456e-10,3.4344e-11
9.0925,1.149e-10,3.4384e-11
9.0954,1.1522e-10,3.4553e-11
9.0984,1.1558e-10,3.4561e-11
9.1014,1.1594e-10,3.4643e-11
9.1044,1.1633e-10,3.4748e-11
9.1074,1.1666e-10,3.4816e-11
9.1103,1.1699e-10,3.4965e-11
9.1133,1.1739e-10,3.4988e-11
9.1163,1.1772e-10,3.5079e-11
9.1193,1.1807e-10,3.5135e-11
9.1223,1.1845e-10,3.5256e-11
9.1252,1.1879e-10,3.5361e-11
9.1282,1.1915e-10,3.5401e-11
9.1312,1.1955e-10,3.546e-11
9.1342,1.1984e-10,3.5524e-11
9.1372,1.2024e-10,3.5605e-11
9.1401,1.2057e-10,3.5751e-11
9.1431,1.2094e-10,3.5837e-11
9.1461,1.2139e-10,3.5902e-11
9.1491,1.2175e-10,3.6059e-11
9.1521,1.2207e-10,3.6094e-11
9.1551,1.2242e-10,3.6211e-11
9.158,1.2284e-10,3.6304e-11
9.161,1.2321e-10,3.6371e-11
9.164,1.235e-10,3.6448e-11
9.167,1.2389e-10,3.6483e-11
9.17,1.2426e-10,3.6567e-11
9.1729,1.2474e-10,3.6716e-11
9.1759,1.251e-10,3.6758e-11
9.1789,1.2544e-10,3.6841e-11
9.1819,1.2577e-10,3.6996e-11
9.1849,1.262e-10,3.7053e-11
9.1878,1.2654e-10,3.7113e-11
9.1908,1.2693e-10,3.7322e-11
9.1938,1.2731e-10,3.7363e-11
9.1968,1.2774e-10,3.7381e-11
9.1998,1.2809e-10,3.7466e-11
9.2027,1.2847e-10,3.7584e-11
9.2057,1.288e-10,3.7655e-11
9.2087,1.2925e-10,3.775e-11
9.2117,1.296e-10,3.7789e-11
9.2147,1.2999e-10,3.7893e-11
9.2176,1.3045e-10,3.8014e-11
9.2206,1.3076e-10,3.8081e-11
9.2236,1.3122e-10,3.8197e-11
9.2266,1.3155e-10,3.8253e-11
9.2296,1.3203e-10,3.8323e-11
9.2325,1.3235e-10,3.8487e-11
9.2355,1.3276e-10,3.8536e-11
9.2385,1.333e-10,3.8646e-11
9.2415,1.3353e-10,3.8654e-11
9.2445,1.3394e-10,3.8878e-11
9.2474,1.3444e-10,3.8924e-11
9.2504,1.3473e-10,3.9032e-11
9.2534,1.352e-10,3.9097e-11
9.2564,1.3563e-10,3.9162e-11
9.2594,1.3598e-10,3.9288e-11
9.2624,1.364e-10,3.9342e-11
9.2653,1.3685e-10,3.9511e-11
9.2683,1.372e-10,3.9573e-11
9.2713,1.376e-10,3.9636e-11
9.2743,1.3804e-10,3.9765e-11
9.2773,1.3841e-10,3.9821e-11
9.2802,1.3883e-10,3.9942e-11
9.2832,1.3927e-10,4.002e-11
9.2862,1.3972e-10,4.0108e-11
9.2892,1.4007e-10,4.017e-11
9.2922,1.4054e-10,4.0301e-11
9.2951,1.4089e-10,4.0385e-11
9.2981,1.4133e-10,4.0449e-11
9.3011,1.4177e-10,4.0571e-11
9.3041,1.4224e-10,4.0615e-11
9.3071,1.4262e-10,4.0752e-11
9.31,1.4312e-10,4.089e-11
9.313,1.4346e-10,4.0866e-11
9.316,1.4392e-10,4.0984e-11
9.319,1.4433e-10,4.1141e-11
9.322,1.4479e-10,4.1226e-11
9.3249,1.4516e-10,4.1383e-11
9.3279,1.456e-10,4.141e-11
9.3309,1.4606e-10,4.151e-11
9.3339,1.4645e-10,4.1623e-11
9.3369,1.4693e-10,4.1742e-11
9.3398,1.4743e-10,4.1746e-11
9.3428,1.4777e-10,4.1913e-11
9.3458,1.482e-10,4.1922e-11
9.3488,1.4865e-10,4.2052e-11
9.3518,1.4917e-10,4.2179e-11
9.3548,1.4958e-10,4.2277e-11
9.3577,1.5009e-10,4.2367e-11
9.3607,1.5046e-10,4.2449e-11
9.3637,1.5091e-10,4.2572e-11
9.3667,1.5137e-10,4.2648e-11
9.3697,1.5177e-10,4.273e-11
9.3726,1.5226e-10,4.2722e-11
9.3756,1.5272e-10,4.2904e-11
9.3786,1.5316e-10,4.3012e-11
9.3816,1.5365e-10,4.3099e-11
9.3846,1.5399e-10,4.3232e-11
9.3875,1.5446e-10,4.3294e-11
9.3905,1.5499e-10,4.3428e-11
9.3935,1.5552e-10,4.3513e-11
9.3965,1.5593e-10,4.3588e-11
9.3995,1.5635e-10,4.3699e-11
9.4024,1.5679e-10,4.3793e-11
9.4054,1.5727e-10,4.3898e-11
9.4084,1.5779e-10,4.396e-11
9.4114,1.5819e-10,4.415e-11
9.4144,1.5872e-10,4.4236e-11
9.4173,1.5913e-10,4.4307e-11
9.4203,1.5964e-10,4.4462e-11
9.4233,1.6013e-10,4.4464e-11
9.4263,1.6059e-10,4.4536e-11
9.4293,1.611e-10,4.4624e-11
9.4322,1.6152e-10,4.4778e-11
9.4352,1.6203e-10,4.4866e-11
9.4382,1.6251e-10,4.4991e-11
9.4412,1.6299e-10,4.5055e-11
9.4442,1.6341e-10,4.5153e-11
9.4471,1.6384e-10,4.5241e-11
9.4501,1.6436e-10,4.5392e-11
9.4531,1.6497e-10,4.5457e-11
9.4561,1.6534e-10,4.5532e-11
9.4591,1.6584e-10,4.569e-11
9.4621,1.6637e-10,4.5797e-11
9.465,1.6691e-10,4.588e-11
9.468,1.6741e-10,4.5993e-11
9.471,1.6785e-10,4.6028e-11
9.474,1.6828e-10,4.6192e-11
9.477,1.6879e-10,4.6324e-11
9.4799,1.6931e-10,4.64e-11
9.4829,1.6978e-10,4.6415e-11
9.4859,1.7036e-10,4.6618e-11
9.4889,1.7083e-10,4.6695e-11
9.4919,1.713e-10,4.686e-11
9.4948,1.718e-10,4.6917e-11
9.4978,1.7235e-10,4.7019e-11
9.5008,1.7282e-10,4.7127e-11
9.5038,1.7335e-10,4.7221e-11
9.5068,1.7384e-10,4.7326e-11
9.5097,1.7442e-10,4.741e-11
9.5127,1.7484e-10,4.7487e-11
9.5157,1.7534e-10,4.7629e-11
9.5187,1.7584e-10,4.7721e-11
9.5217,1.7639e-10,4.7825e-11
9.5246,1.7698e-10,4.7982e-11
9.5276,1.7746e-10,4.8046e-11
9.5306,1.7799e-10,4.809e-11
9.5336,1.7845e-10,4.8265e-11
9.5366,1.7898e-10,4.8361e-11
9.5395,1.7953e-10,4.8469e-11
9.5425,1.8003e-10,4.8584e-11
9.5455,1.8059e-10,4.8624e-11
9.5485,1.8107e-10,4.8845e-11
9.5515,1.8166e-10,4.8821e-11
9.5545,1.8222e-10,4.8959e-11
9.5574,1.8271e-10,4.9109e-11
9.5604,1.8326e-10,4.9208e-11
9.5634,1.8376e-10,4.9346e-11
9.5664,1.8428e-10,4.9371e-11
9.5694,1.8485e-10,4.9454e-11
9.5723,1.8533e-10,4.9553e-11
9.5753,1.8592e-10,4.9709e-11
9.5783,1.8644e-10,4.9798e-11
9.5813,1.8701e-10,4.9878e-11
9.5843,1.8751e-10,5.0065e-11
9.5872,1.8806e-10,5.0121e-11
9.5902,1.886e-10,5.0316e-11
9.5932,1.8915e-10,5.0307e-11
9.5962,1.898e-10,5.0471e-11
9.5992,1.9033e-10,5.0604e-11
9.6021,1.9096e-10,5.0724e-11
9.6051,1.9143e-10,5.0729e-11
9.6081,1.92e-10,5.0873e-11
9.6111,1.9251e-10,5.0964e-11
9.6141,1.9305e-10,5.1007e-11
9.617,1.9359e-10,5.1186e-11
9.62,1.9419e-10,5.1312e-11
9.623,1.948e-10,5.1459e-11
9.626,1.9531e-10,5.1495e-11
9.629,1.9582e-10,5.1698e-11
9.6319,1.9642e-10,5.1699e-11
9.6349,1.9707e-10,5.1889e-11
9.6379,1.9761e-10,5.2048e-11
9.6409,1.9822e-10,5.2073e-11
9.6439,1.9877e-10,5.2121e-11
9.6468,1.9933e-10,5.2269e-11
9.6498,1.9999e-10,5.2405e-11
9.6528,2.0055e-10,5.2603e-11
9.6558,2.01e-10,5.2715e-11
9.6588,2.0166e-10,5.2629e-11
9.6618,2.0222e-10,5.2776e-11
9.6647,2.028e-10,5.299e-11
9.6677,2.034e-10,5.315e-11
9.6707,2.0405e-10,5.3259e-11
9.6737,2.0471e-10,5.3295e-11
9.6767,2.0522e-10,5.3481e-11
9.6796,2.0577e-10,5.3563e-11
9.6826,2.064e-10,5.3616e-11
9.6856,2.0695e-10,5.3773e-11
9.6886,2.0759e-10,5.3822e-11
9.6916,2.0821e-10,5.3982e-11
9.6945,2.0882e-10,5.4094e-11
9.6975,2.0945e-10,5.4208e-11
9.7005,2.0993e-10,5.4377e-11
9.7035,2.1061e-10,5.4448e-11
9.7065,2.1125e-10,5.4451e-11
9.7094,2.1178e-10,5.4613e-11
9.7124,2.1249e-10,5.4783e-11
9.7154,2.1306e-10,5.4832e-11
9.7184,2.137e-10,5.4974e-11
9.7214,2.1436e-10,5.5025e-11
9.7243,2.1497e-10,5.5189e-11
9.7273,2.1563e-10,5.529e-11
9.7303,2.162e-10,5.5495e-11
9.7333,2.1678e-10,5.5619e-11
9.7363,2.1739e-10,5.5639e-11
9.7392,2.1798e-10,5.58e-11
9.7422,2.1864e-10,5.5891e-11
9.7452,2.1937e-10,5.6018e-11
9.7482,2.1993e-10,5.6245e-11
9.7512,2.2066e-10,5.6232e-11
9.7542,2.212e-10,5.637e-11
9.7571,2.2185e-10,5.6438e-11
9.7601,2.2245e-10,5.6455e-11
9.7631,2.231e-10,5.6637e-11
9.7661,2.2379e-10,5.6759e-11
9.7691,2.2443e-10,5.6881e-11
9.772,2.2497e-10,5.7001e-11
9.775,2.2566e-10,5.7104e-11
9.778,2.2633e-10,5.7228e-11
9.781,2.2696e-10,5.7407e-11
9.784,2.2763e-10,5.753e-11
9.7869,2.2827e-10,5.7494e-11
9.7899,2.2895e-10,5.7758e-11
9.7929,2.2965e-10,5.7979e-11
9.7959,2.3038e-10,5.7862e-11
9.7989,2.3095e-10,5.8026e-11
9.8018,2.3162e-10,5.8269e-11
9.8048,2.3216e-10,5.832e-11
9.8078,2.3288e-10,5.8431e-11
9.8108,2.3349e-10,5.8533e-11
9.8138,2.3425e-10,5.8637e-11
9.8167,2.3489e-10,5.8768e-11
9.8197,2.3556e-10,5.8962e-11
9.8227,2.3631e-10,5.907e-11
9.8257,2.3701e-10,5.904e-11
9.8287,2.3769e-10,5.9185e-11
9.8316,2.382e-10,5.9332e-11
9.8346,2.3911e-10,5.9505e-11
9.8376,2.3976e-10,5.9643e-11
9.8406,2.4042e-10,5.9824e-11
9.8436,2.4101e-10,5.9867e-11
9.8465,2.4168e-10,5.9975e-11
9.8495,2.4247e-10,6.0198e-11
9.8525,2.4305e-10,6.0179e-11
9.8555,2.4371e-10,6.0443e-11
9.8585,2.446e-10,6.0516e-11
9.8615,2.4531e-10,6.0624e-11
9.8644,2.4596e-10,6.0513e-11
9.8674,2.4671e-10,6.0804e-11
9.8704,2.4728e-10,6.0879e-11
9.8734,2.4802e-10,6.1074e-11
9.8764,2.4881e-10,6.1111e-11
9.8793,2.4937e-10,6.1212e-11
9.8823,2.5011e-10,6.1377e-11
9.8853,2.5095e-10,6.1601e-11
9.8883,2.5169e-10,6.1691e-11
9.8913,2.5235e-10,6.1665e-11
9.8942,2.531e-10,6.1881e-11
9.8972,2.538e-10,6.1898e-11
9.9002,2.5451e-10,6.2168e-11
9.9032,2.5531e-10,6.2217e-11
9.9062,2.5591e-10,6.2364e-11
9.9091,2.5672e-10,6.2421e-11
9.9121,2.5742e-10,6.2543e-11
9.9151,2.5816e-10,6.2776e-11
9.9181,2.5885e-10,6.2864e-11
9.9211,2.5964e-10,6.2982e-11
9.924,2.6018e-10,6.3114e-11
9.927,2.6102e-10,6.3263e-11
9.93,2.6187e-10,6.3326e-11
9.933,2.6259e-10,6.3413e-11
9.936,2.6344e-10,6.358e-11
9.9389,2.6412e-10,6.3597e-11
9.9419,2.6472e-10,6.3791e-11
9.9449,2.6559e-10,6.3875e-11
9.9479,2.6638e-10,6.4082e-11
9.9509,2.6714e-10,6.4128e-11
9.9539,2.6782e-10,6.4466e-11
9.9568,2.6855e-10,6.436e-11
9.9598,2.6936e-10,6.4553e-11
9.9628,2.7001e-10,6.4623e-11
9.9658,2.7091e-10,6.4795e-11
9.9688,2.7159e-10,6.4916e-11
9.9717,2.7247e-10,6.5064e-11
9.9747,2.7326e-10,6.5121e-11
9.9777,2.739e-10,6.5319e-11
9.9807,2.7474e-10,6.5375e-11
9.9837,2.7545e-10,6.5398e-11
9.9866,2.763e-10,6.559e-11
9.9896,2.7701e-10,6.5742e-11
9.9926,2.7785e-10,6.5864e-11
9.9956,2.7865e-10,6.6009e-11
9.9986,2.7943e-10,6.63e-11
10.002,2.802e-10,6.6278e-11
10.005,2.811e-10,6.6322e-11
10.008,2.8181e-10,6.6489e-11
10.01,2.8258e-10,6.6632e-11
10.013,2.8346e-10,6.6745e-11
10.016,2.8431e-10,6.6868e-11
10.019,2.8512e-10,6.6937e-11
10.022,2.8588e-10,6.711e-11
10.025,2.8658e-10,6.7319e-11
10.028,2.8751e-10,6.7456e-11
10.031,2.8828e-10,6.7516e-11
10.034,2.8908e-10,6.7642e-11
10.037,2.8995e-10,6.7729e-11
10.04,2.9068e-10,6.8118e-11
10.043,2.9147e-10,6.7998e-11
10.046,2.9231e-10,6.8159e-11
10.049,2.9308e-10,6.8413e-11
10.052,2.9402e-10,6.8312e-11
10.055,2.9495e-10,6.8618e-11
10.058,2.9576e-10,6.8592e-11
10.061,2.9643e-10,6.8844e-11
10.064,2.9726e-10,6.8789e-11
10.067,2.9822e-10,6.8939e-11
10.07,2.9909e-10,6.9127e-11
10.073,2.9989e-10,6.9327e-11
10.076,3.0079e-10,6.9476e-11
10.079,3.0149e-10,6.9494e-11
10.082,3.0241e-10,6.9584e-11
10.085,3.032e-10,6.9929e-11
10.088,3.042e-10,6.985e-11
10.091,3.0496e-10,7.0018e-11
10.094,3.0584e-10,7.007e-11
10.097,3.0659e-10,7.0339e-11
10.1,3.075e-10,7.0493e-11
10.103,3.084e-10,7.0602e-11
10.106,3.0921e-10,7.0734e-11
10.109,3.1015e-10,7.0776e-11
10.112,3.1103e-10,7.0961e-11
10.115,3.1192e-10,7.1065e-11
10.118,3.129e-10,7.1252e-11
10.121,3.1365e-10,7.1298e-11
10.124,3.1449e-10,7.1477e-11
10.127,3.1542e-10,7.1634e-11
10.13,3.1636e-10,7.1592e-11
10.133,3.1713e-10,7.1982e-11
10.136,3.1803e-10,7.2024e-11
10.139,3.1903e-10,7.2174e-11
10.142,3.1978e-10,7.226e-11
10.145,3.2073e-10,7.2366e-11
10.148,3.2172e-10,7.2505e-11
10.151,3.2252e-10,7.2605e-11
10.154,3.2348e-10,7.2709e-11
10.157,3.2448e-10,7.2782e-11
10.16,3.2523e-10,7.2991e-11
10.162,3.2622e-10,7.315e-11
10.165,3.2712e-10,7.3227e-11
10.168,3.2801e-10,7.3266e-11
10.171,3.2893e-10,7.351e-11
10.174,3.2984e-10,7.3485e-11
10.177,3.3083e-10,7.3732e-11
10.18,3.3162e-10,7.3883e-11
10.183,3.3258e-10,7.4068e-11
10.186,3.3348e-10,7.4125e-11
10.189,3.3446e-10,7.433e-11
10.192,3.3538e-10,7.4413e-11
10.195,3.3632e-10,7.4536e-11
10.198,3.3716e-10,7.4718e-11
10.201,3.3812e-10,7.4829e-11
10.204,3.3915e-10,7.4997e-11
10.207,3.4006e-10,7.5098e-11
10.21,3.4105e-10,7.5192e-11
10.213,3.4202e-10,7.526e-11
10.216,3.4294e-10,7.5459e-11
10.219,3.4383e-10,7.5651e-11
10.222,3.4479e-10,7.569e-11
10.225,3.4578e-10,7.6069e-11
10.228,3.467e-10,7.6159e-11
10.231,3.4769e-10,7.6056e-11
10.234,3.4876e-10,7.6384e-11
10.237,3.4961e-10,7.6309e-11
10.24,3.5069e-10,7.6537e-11
10.243,3.5168e-10,7.6682e-11
10.246,3.5256e-10,7.6653e-11
10.249,3.536e-10,7.6894e-11
10.252,3.5454e-10,7.7135e-11
10.255,3.5556e-10,7.7323e-11
10.258,3.5657e-10,7.7175e-11
10.261,3.5748e-10,7.757e-11
10.264,3.5854e-10,7.7488e-11
10.267,3.5956e-10,7.7752e-11
10.27,3.6049e-10,7.7824e-11
10.273,3.6142e-10,7.8098e-11
10.276,3.6269e-10,7.8127e-11
10.279,3.6356e-10,7.8145e-11
10.282,3.6462e-10,7.8335e-11
10.285,3.6556e-10,7.8526e-11
10.288,3.6663e-10,7.8707e-11
10.291,3.6757e-10,7.8719e-11
10.294,3.6861e-10,7.8831e-11
10.297,3.6961e-10,7.9057e-11
10.3,3.7076e-10,7.9185e-11
10.303,3.7162e-10,7.9213e-11
10.306,3.7275e-10,7.9387e-11
10.309,3.7379e-10,7.952e-11
10.312,3.7479e-10,7.9758e-11
10.315,3.7578e-10,7.97e-11
10.317,3.7693e-10,7.9957e-11
10.32,3.7791e-10,8.015e-11
10.323,3.7894e-10,8.0244e-11
10.326,3.7995e-10,8.0351e-11
10.329,3.8113e-10,8.0508e-11
10.332,3.8209e-10,8.0611e-11
10.335,3.8323e-10,8.0693e-11
10.338,3.8414e-10,8.0712e-11
10.341,3.8527e-10,8.1016e-11
10.344,3.8644e-10,8.1188e-11
10.347,3.8755e-10,8.1242e-11
10.35,3.8843e-10,8.1483e-11
10.353,3.8948e-10,8.15e-11
10.356,3.9076e-10,8.165e-11
10.359,3.916e-10,8.1746e-11
10.362,3.928e-10,8.1853e-11
10.365,3.9389e-10,8.2101e-11
10.368,3.9493e-10,8.2236e-11
10.371,3.961e-10,8.2408e-11
10.374,3.9725e-10,8.2413e-11
10.377,3.9818e-10,8.265e-11
10.38,3.9924e-10,8.2715e-11
10.383,4.0043e-10,8.2807e-11
10.386,4.0166e-10,8.2995e-11
10.389,4.0255e-10,8.2958e-11
10.392,4.0368e-10,8.3371e-11
10.395,4.0497e-10,8.3448e-11
10.398,4.0586e-10,8.3462e-11
10.401,4.0724e-10,8.3698e-11
10.404,4.0814e-10,8.381e-11
10.407,4.0913e-10,8.3935e-11
10.41,4.1059e-10,8.4302e-11
10.413,4.1157e-10,8.4221e-11
10.416,4.1255e-10,8.4356e-11
10.419,4.1387e-10,8.4451e-11
10.422,4.1496e-10,8.4739e-11
10.425,4.1598e-10,8.4855e-11
10.428,4.1741e-10,8.4724e-11
10.431,4.1844e-10,8.4838e-11
10.434,4.1958e-10,8.5001e-11
10.437,4.2076e-10,8.5571e-11
10.44,4.2184e-10,8.538e-11
10.443,4.231e-10,8.5525e-11
10.446,4.2414e-10,8.5581e-11
10.449,4.2532e-10,8.5634e-11
10.452,4.2656e-10,8.6036e-11
10.455,4.2774e-10,8.6066e-11
10.458,4.2892e-10,8.6255e-11
10.461,4.3009e-10,8.6379e-11
10.464,4.3124e-10,8.6275e-11
10.467,4.3251e-10,8.6465e-11
10.469,4.3371e-10,8.6751e-11
10.472,4.3486e-10,8.6732e-11
10.475,4.3603e-10,8.6955e-11
10.478,4.3725e-10,8.7235e-11
10.481,4.3848e-10,8.7216e-11
10.484,4.3969e-10,8.7394e-11
10.487,4.4081e-10,8.7486e-11
10.49,4.4183e-10,8.7716e-11
10.493,4.433e-10,8.7956e-11
10.496,4.4433e-10,8.8035e-11
10.499,4.4558e-10,8.8015e-11
10.502,4.4679e-10,8.8175e-11
10.505,4.4823e-10,8.8247e-11
10.508,4.4924e-10,8.8426e-11
10.511,4.5075e-10,8.8627e-11
10.514,4.5165e-10,8.8771e-11
10.517,4.5286e-10,8.8959e-11
10.52,4.543e-10,8.921e-11
10.523,4.5536e-10,8.9148e-11
10.526,4.5651e-10,8.9205e-11
10.529,4.5794e-10,8.9378e-11
10.532,4.5929e-10,8.9525e-11
10.535,4.6036e-10,8.9644e-11
10.538,4.6163e-10,9.006e-11
10.541,4.631e-10,8.9899e-11
10.544,4.6433e-10,9.005e-11
10.547,4.6552e-10,9.0059e-11
10.55,4.669e-10,9.0368e-11
10.553,4.6818e-10,9.0507e-11
10.556,4.6942e-10,9.056e-11
10.559,4.706e-10,9.0692e-11
10.562,4.7176e-10,9.0929e-11
10.565,4.7317e-10,9.1031e-11
10.568,4.7451e-10,9.097e-11
10.571,4.7585e-10,9.1371e-11
10.574,4.7722e-10,9.1432e-11
10.577,4.7846e-10,9.1332e-11
10.58,4.7968e-10,9.1715e-11
10.583,4.8103e-10,9.1718e-11
10.586,4.8259e-10,9.1958e-11
10.589,4.8362e-10,9.2009e-11
10.592,4.8485e-10,9.2183e-11
10.595,4.8626e-10,9.2225e-11
10.598,4.8768e-10,9.2625e-11
10.601,4.8876e-10,9.2751e-11
10.604,4.902e-10,9.2659e-11
10.607,4.9164e-10,9.28e-11
10.61,4.9282e-10,9.3123e-11
10.613,4.9427e-10,9.3075e-11
10.616,4.9564e-10,9.3267e-11
10.619,4.9677e-10,9.354e-11
10.622,4.9815e-10,9.3618e-11
10.624,4.9951e-10,9.374e-11
10.627,5.0115e-10,9.3645e-11
10.63,5.0233e-10,9.3928e-11
10.633,5.0363e-10,9.4105e-11
10.636,5.0485e-10,9.4298e-11
10.639,5.0642e-10,9.4246e-11
10.642,5.0773e-10,9.4369e-11
10.645,5.0943e-10,9.4648e-11
10.648,5.1036e-10,9.4696e-11
10.651,5.118e-10,9.4722e-11
10.654,5.1332e-10,9.503e-11
10.657,5.1465e-10,9.5114e-11
10.66,5.1597e-10,9.5247e-11
10.663,5.1746e-10,9.5455e-11
10.666,5.1886e-10,9.5575e-11
10.669,5.2022e-10,9.5857e-11
10.672,5.2196e-10,9.5722e-11
10.675,5.2318e-10,9.5914e-11
10.678,5.2454e-10,9.6203e-11
10.681,5.2602e-10,9.6158e-11
10.684,5.2741e-10,9.6399e-11
10.687,5.2874e-10,9.6472e-11
10.69,5.305e-10,9.6393e-11
10.693,5.3161e-10,9.6812e-11
10.696,5.3336e-10,9.6567e-11
10.699,5.3454e-10,9.7106e-11
10.702,5.3602e-10,9.7065e-11
10.705,5.3735e-10,9.7337e-11
10.708,5.3873e-10,9.733e-11
10.711,5.4049e-10,9.7337e-11
10.714,5.4191e-10,9.7672e-11
10.717,5.4345e-10,9.7632e-11
10.72,5.4469e-10,9.7492e-11
10.723,5.4629e-10,9.8146e-11
10.726,5.4772e-10,9.8317e-11
10.729,5.4927e-10,9.8428e-11
10.732,5.5063e-10,9.8316e-11
10.735,5.5213e-10,9.8569e-11
10.738,5.5349e-10,9.862e-11
10.741,5.551e-10,9.8688e-11
10.744,5.5676e-10,9.8761e-11
10.747,5.5803e-10,9.8943e-11
10.75,5.5939e-10,9.9206e-11
10.753,5.6118e-10,9.9203e-11
10.756,5.6273e-10,9.9209e-11
10.759,5.6403e-10,9.9552e-11
10.762,5.6563e-10,9.9795e-11
10.765,5.6741e-10,9.9772e-11
10.768,5.6868e-10,9.9951e-11
10.771,5.701e-10,1.0003e-10
10.774,5.7175e-10,1.0026e-10
10.776,5.7308e-10,1.0032e-10
10.779,5.7479e-10,1.0042e-10
10.782,5.7624e-10,1.0077e-10
10.785,5.7808e-10,1.0065e-10
10.788,5.7942e-10,1.0097e-10
10.791,5.8087e-10,1.0099e-10
10.794,5.824e-10,1.0114e-10
10.797,5.8425e-10,1.0117e-10
10.8,5.8578e-10,1.0144e-10
10.803,5.8735e-10,1.0129e-10
10.806,5.8892e-10,1.0156e-10
10.809,5.9048e-10,1.0187e-10
10.812,5.9189e-10,1.0188e-10
10.815,5.9347e-10,1.0196e-10
10.818,5.9514e-10,1.0209e-10
10.821,5.969e-10,1.0199e-10
10.824,5.9858e-10,1.0229e-10
10.827,5.9995e-10,1.0249e-10
10.83,6.0164e-10,1.0253e-10
10.833,6.0323e-10,1.0284e-10
10.836,6.0484e-10,1.028e-10
10.839,6.0633e-10,1.0294e-10
10.842,6.0783e-10,1.0309e-10
10.845,6.0977e-10,1.0334e-10
10.848,6.1134e-10,1.0308e-10
10.851,6.1328e-10,1.0368e-10
10.854,6.1465e-10,1.0364e-10
10.857,6.1613e-10,1.0359e-10
10.86,6.1786e-10,1.0362e-10
10.863,6.1954e-10,1.0382e-10
10.866,6.2122e-10,1.0432e-10
10.869,6.2306e-10,1.0414e-10
10.872,6.2445e-10,1.0424e-10
10.875,6.2612e-10,1.0438e-10
10.878,6.2791e-10,1.0456e-10
10.881,6.297e-10,1.0463e-10
10.884,6.3131e-10,1.0491e-10
10.887,6.3283e-10,1.0498e-10
10.89,6.3463e-10,1.0517e-10
10.893,6.3634e-10,1.0528e-10
10.896,6.3821e-10,1.0528e-10
10.899,6.3968e-10,1.0557e-10
10.902,6.415e-10,1.0565e-10
10.905,6.4298e-10,1.0568e-10
10.908,6.4512e-10,1.0539e-10
10.911,6.4693e-10,1.0579e-10
10.914,6.4849e-10,1.0587e-10
10.917,6.5002e-10,1.0643e-10
10.92,6.518e-10,1.0633e-10
10.923,6.5379e-10,1.0627e-10
10.926,6.5517e-10,1.0648e-10
10.929,6.5686e-10,1.0643e-10
10.931,6.5853e-10,1.0675e-10
10.934,6.6071e-10,1.0675e-10
10.937,6.6236e-10,1.07e-10
10.94,6.6413e-10,1.0708e-10
10.943,6.6571e-10,1.071e-10
10.946,6.6754e-10,1.0725e-10
10.949,6.6933e-10,1.0742e-10
10.952,6.7113e-10,1.0761e-10
10.955,6.7288e-10,1.0794e-10
10.958,6.7468e-10,1.0801e-10
10.961,6.762e-10,1.0809e-10
10.964,6.7836e-10,1.0802e-10
10.967,6.8002e-10,1.0832e-10
10.97,6.8183e-10,1.0853e-10
10.973,6.8377e-10,1.0826e-10
10.976,6.8559e-10,1.0831e-10
10.979,6.874e-10,1.0854e-10
10.982,6.8918e-10,1.0883e-10
10.985,6.9111e-10,1.0866e-10
10.988,6.9278e-10,1.0897e-10
10.991,6.9493e-10,1.0891e-10
10.994,6.9642e-10,1.0911e-10
10.997,6.9848e-10,1.0924e-10
11,7.0025e-10,1.0939e-10
11.003,7.0197e-10,1.0927e-10
11.006,7.0387e-10,1.0958e-10
11.009,7.0583e-10,1.0973e-10
11.012,7.0765e-10,1.0988e-10
11.015,7.0933e-10,1.0978e-10
11.018,7.1131e-10,1.1033e-10
11.021,7.13e-10,1.1014e-10
11.024,7.1512e-10,1.1015e-10
11.027,7.1696e-10,1.1045e-10
11.03,7.1913e-10,1.104e-10
11.033,7.209e-10,1.1058e-10
11.036,7.227e-10,1.1074e-10
11.039,7.248e-10,1.1067e-10
11.042,7.2659e-10,1.1089e-10
11.045,7.2853e-10,1.108e-10
11.048,7.3055e-10,1.1132e-10
11.051,7.3234e-10,1.1144e-10
11.054,7.3458e-10,1.1129e-10
11.057,7.3629e-10,1.1139e-10
11.06,7.3807e-10,1.1173e-10
11.063,7.4036e-10,1.1176e-10
11.066,7.4194e-10,1.1194e-10
11.069,7.4432e-10,1.1201e-10
11.072,7.4608e-10,1.1214e-10
11.075,7.4816e-10,1.1229e-10
11.078,7.5023e-10,1.1231e-10
11.081,7.5222e-10,1.1234e-10
11.083,7.5412e-10,1.1221e-10
11.086,7.5625e-10,1.125e-10
11.089,7.5815e-10,1.1252e-10
11.092,7.5985e-10,1.1269e-10
11.095,7.6205e-10,1.1275e-10
11.098,7.6421e-10,1.1284e-10
11.101,7.6605e-10,1.1306e-10
11.104,7.6791e-10,1.1333e-10
11.107,7.706e-10,1.1314e-10
11.11,7.7234e-10,1.1345e-10
11.113,7.7396e-10,1.1345e-10
11.116,7.7637e-10,1.1337e-10
11.119,7.7843e-10,1.1324e-10
11.122,7.8014e-10,1.1367e-10
11.125,7.8264e-10,1.137e-10
11.128,7.8417e-10,1.1383e-10
11.131,7.8639e-10,1.1393e-10
11.134,7.8837e-10,1.1406e-10
11.137,7.9088e-10,1.1421e-10
11.14,7.9246e-10,1.1465e-10
11.143,7.9489e-10,1.1444e-10
11.146,7.9675e-10,1.1429e-10
11.149,7.9907e-10,1.1468e-10
11.152,8.0099e-10,1.145e-10
11.155,8.0304e-10,1.1461e-10
11.158,8.0491e-10,1.1502e-10
11.161,8.0718e-10,1.1507e-10
11.164,8.0922e-10,1.151e-10
11.167,8.1165e-10,1.1505e-10
11.17,8.1354e-10,1.1549e-10
11.173,8.1581e-10,1.1519e-10
11.176,8.1809e-10,1.1498e-10
11.179,8.2018e-10,1.157e-10
11.182,8.2237e-10,1.1595e-10
11.185,8.2467e-10,1.1593e-10
11.188,8.2695e-10,1.163e-10
11.191,8.2865e-10,1.1598e-10
11.194,8.3107e-10,1.1631e-10
11.197,8.3326e-10,1.1618e-10
11.2,8.354e-10,1.1627e-10
11.203,8.3734e-10,1.1591e-10
11.206,8.3961e-10,1.1629e-10
11.209,8.4185e-10,1.1601e-10
11.212,8.4418e-10,1.1645e-10
11.215,8.4624e-10,1.1609e-10
11.218,8.4835e-10,1.1656e-10
11.221,8.5061e-10,1.1657e-10
11.224,8.5306e-10,1.166e-10
11.227,8.5524e-10,1.1647e-10
11.23,8.5734e-10,1.1685e-10
11.233,8.5946e-10,1.1707e-10
11.236,8.6166e-10,1.1709e-10
11.238,8.6432e-10,1.1721e-10
11.241,8.6633e-10,1.1684e-10
11.244,8.6848e-10,1.1739e-10
11.247,8.7076e-10,1.1731e-10
11.25,8.7344e-10,1.1715e-10
11.253,8.7557e-10,1.178e-10
11.256,8.7781e-10,1.1781e-10
11.259,8.8009e-10,1.1753e-10
11.262,8.8254e-10,1.1771e-10
11.265,8.8474e-10,1.1801e-10
11.268,8.8703e-10,1.1782e-10
11.271,8.8946e-10,1.1811e-10
11.274,8.9119e-10,1.1805e-10
11.277,8.9339e-10,1.1842e-10
11.28,8.9675e-10,1.1828e-10
11.283,8.986e-10,1.1847e-10
11.286,9.0163e-10,1.1845e-10
11.289,9.0325e-10,1.1818e-10
11.292,9.0539e-10,1.1865e-10
11.295,9.0846e-10,1.1818e-10
11.298,9.1051e-10,1.1844e-10
11.301,9.1275e-10,1.187e-10
11.304,9.1542e-10,1.1907e-10
11.307,9.1745e-10,1.1949e-10
11.31,9.2022e-10,1.1905e-10
11.313,9.2198e-10,1.1902e-10
11.316,9.2436e-10,1.1916e-10
11.319,9.2719e-10,1.1893e-10
11.322,9.291e-10,1.1922e-10
11.325,9.3201e-10,1.1965e-10
11.328,9.3423e-10,1.193e-10
11.331,9.3675e-10,1.1943e-10
11.334,9.3946e-10,1.1956e-10
11.337,9.4078e-10,1.1955e-10
11.34,9.4412e-10,1.1971e-10
11.343,9.4676e-10,1.1941e-10
11.346,9.4905e-10,1.1936e-10
11.349,9.5168e-10,1.1999e-10
11.352,9.5384e-10,1.2014e-10
11.355,9.5626e-10,1.2009e-10
11.358,9.5921e-10,1.1994e-10
11.361,9.6157e-10,1.2001e-10
11.364,9.6417e-10,1.2003e-10
11.367,9.66e-10,1.2054e-10
11.37,9.6856e-10,1.1993e-10
11.373,9.7143e-10,1.1997e-10
11.376,9.7385e-10,1.2009e-10
11.379,9.7656e-10,1.2047e-10
11.382,9.7906e-10,1.2051e-10
11.385,9.8139e-10,1.2053e-10
11.388,9.8405e-10,1.2078e-10
11.39,9.8666e-10,1.2067e-10
11.393,9.8899e-10,1.207e-10
11.396,9.9223e-10,1.2075e-10
11.399,9.9452e-10,1.2116e-10
11.402,9.9673e-10,1.211e-10
11.405,9.9946e-10,1.2108e-10
11.408,1.0024e-09,1.2094e-10
11.411,1.0048e-09,1.2138e-10
11.414,1.0074e-09,1.2124e-10
11.417,1.0102e-09,1.2141e-10
11.42,1.0125e-09,1.2108e-10
11.423,1.0154e-09,1.2134e-10
11.426,1.0179e-09,1.212e-10
11.429,1.0204e-09,1.2131e-10
11.432,1.0231e-09,1.2144e-10
11.435,1.0252e-09,1.2102e-10
11.438,1.0289e-09,1.2104e-10
11.441,1.0311e-09,1.2126e-10
11.444,1.0334e-09,1.214e-10
11.447,1.0361e-09,1.2177e-10
11.45,1.0389e-09,1.2177e-10
11.453,1.0419e-09,1.2141e-10
11.456,1.0444e-09,1.2136e-10
11.459,1.0472e-09,1.2168e-10
11.462,1.0499e-09,1.2178e-10
11.465,1.0526e-09,1.2164e-10
11.468,1.0553e-09,1.211e-10
11.471,1.0581e-09,1.2151e-10
11.474,1.0607e-09,1.2219e-10
11.477,1.0635e-09,1.2154e-10
11.48,1.0661e-09,1.219e-10
11.483,1.0693e-09,1.2176e-10
11.486,1.0714e-09,1.2165e-10
11.489,1.0743e-09,1.2144e-10
11.492,1.0771e-09,1.218e-10
11.495,1.0798e-09,1.2177e-10
11.498,1.0827e-09,1.2179e-10
11.501,1.0855e-09,1.2233e-10
11.504,1.0887e-09,1.2204e-10
11.507,1.091e-09,1.2181e-10
11.51,1.0941e-09,1.2168e-10
11.513,1.0967e-09,1.2219e-10
11.516,1.0996e-09,1.2222e-10
11.519,1.102e-09,1.2242e-10
11.522,1.1052e-09,1.2198e-10
11.525,1.1082e-09,1.2201e-10
11.528,1.1105e-09,1.2187e-10
11.531,1.1138e-09,1.2228e-10
11.534,1.1166e-09,1.218e-10
11.537,1.1197e-09,1.2249e-10
11.54,1.1228e-09,1.2208e-10
11.543,1.1256e-09,1.2199e-10
11.545,1.1281e-09,1.2206e-10
11.548,1.1313e-09,1.2239e-10
11.551,1.1339e-09,1.2197e-10
11.554,1.1371e-09,1.2192e-10
11.557,1.1399e-09,1.2237e-10
11.56,1.1428e-09,1.2265e-10
11.563,1.1458e-09,1.2212e-10
11.566,1.149e-09,1.2213e-10
11.569,1.1518e-09,1.2171e-10
11.572,1.155e-09,1.2215e-10
11.575,1.1574e-09,1.2227e-10
11.578,1.1608e-09,1.2205e-10
11.581,1.1636e-09,1.2222e-10
11.584,1.1666e-09,1.2258e-10
11.587,1.1695e-09,1.2254e-10
11.59,1.1727e-09,1.2244e-10
11.593,1.1756e-09,1.2257e-10
11.596,1.1787e-09,1.2221e-10
11.599,1.1819e-09,1.216e-10
11.602,1.1853e-09,1.2132e-10
11.605,1.1873e-09,1.222e-10
11.608,1.1908e-09,1.2279e-10
11.611,1.1935e-09,1.2278e-10
11.614,1.1966e-09,1.2221e-10
11.617,1.1997e-09,1.2197e-10
11.62,1.2028e-09,1.2221e-10
11.623,1.206e-09,1.2197e-10
11.626,1.2092e-09,1.2262e-10
11.629,1.2126e-09,1.2227e-10
11.632,1.2156e-09,1.2248e-10
11.635,1.2184e-09,1.2216e-10
11.638,1.2214e-09,1.2217e-10
11.641,1.2246e-09,1.223e-10
11.644,1.2279e-09,1.222e-10
11.647,1.2311e-09,1.223e-10
11.65,1.2342e-09,1.2194e-10
11.653,1.237e-09,1.2205e-10
11.656,1.2404e-09,1.2231e-10
11.659,1.2437e-09,1.2237e-10
11.662,1.2469e-09,1.2197e-10
11.665,1.2503e-09,1.2188e-10
11.668,1.2525e-09,1.221e-10
11.671,1.2563e-09,1.2171e-10
11.674,1.2595e-09,1.2127e-10
11.677,1.2632e-09,1.2188e-10
11.68,1.2662e-09,1.2142e-10
11.683,1.2689e-09,1.2185e-10
11.686,1.2723e-09,1.218e-10
11.689,1.2753e-09,1.218e-10
11.692,1.2792e-09,1.2186e-10
11.695,1.2822e-09,1.2151e-10
11.697,1.2856e-09,1.2122e-10
11.7,1.2886e-09,1.2174e-10
11.703,1.292e-09,1.2116e-10
11.706,1.2948e-09,1.2095e-10
11.709,1.2985e-09,1.2099e-10
11.712,1.3015e-09,1.2101e-10
11.715,1.3045e-09,1.2103e-10
11.718,1.3084e-09,1.2109e-10
11.721,1.3115e-09,1.2118e-10
11.724,1.3149e-09,1.208e-10
11.727,1.3184e-09,1.2064e-10
11.73,1.3221e-09,1.2118e-10
11.733,1.3254e-09,1.2101e-10
11.736,1.3284e-09,1.2104e-10
11.739,1.3322e-09,1.207e-10
11.742,1.3351e-09,1.2053e-10
11.745,1.3384e-09,1.2117e-10
11.748,1.3417e-09,1.2061e-10
11.751,1.3457e-09,1.2041e-10
11.754,1.349e-09,1.2022e-10
11.757,1.3521e-09,1.2032e-10
11.76,1.3559e-09,1.2006e-10
11.763,1.3596e-09,1.2e-10
11.766,1.3628e-09,1.2048e-10
11.769,1.3658e-09,1.1941e-10
11.772,1.3693e-09,1.1948e-10
11.775,1.3726e-09,1.1935e-10
11.778,1.3764e-09,1.202e-10
11.781,1.3799e-09,1.1967e-10
11.784,1.3835e-09,1.1964e-10
11.787,1.3872e-09,1.198e-10
11.79,1.3908e-09,1.1967e-10
11.793,1.3944e-09,1.1926e-10
11.796,1.3977e-09,1.1957e-10
11.799,1.4011e-09,1.1915e-10
11.802,1.4047e-09,1.1911e-10
11.805,1.4084e-09,1.1912e-10
11.808,1.4116e-09,1.1866e-10
11.811,1.415e-09,1.1873e-10
11.814,1.4193e-09,1.1879e-10
11.817,1.4227e-09,1.1844e-10
11.82,1.4263e-09,1.1876e-10
11.823,1.4301e-09,1.1826e-10
11.826,1.4335e-09,1.1866e-10
11.829,1.437e-09,1.1805e-10
11.832,1.441e-09,1.1836e-10
11.835,1.444e-09,1.1815e-10
11.838,1.4482e-09,1.1791e-10
11.841,1.4518e-09,1.1764e-10
11.844,1.4554e-09,1.1723e-10
11.847,1.4588e-09,1.18e-10
11.85,1.4622e-09,1.1792e-10
11.852,1.4665e-09,1.1772e-10
11.855,1.4704e-09,1.1712e-10
11.858,1.4732e-09,1.1682e-10
11.861,1.4774e-09,1.166e-10
11.864,1.4815e-09,1.1645e-10
11.867,1.4852e-09,1.1704e-10
11.87,1.4885e-09,1.1662e-10
11.873,1.492e-09,1.1654e-10
11.876,1.4962e-09,1.1701e-10
11.879,1.4991e-09,1.1625e-10
11.882,1.5037e-09,1.1655e-10
11.885,1.5077e-09,1.158e-10
11.888,1.5112e-09,1.1564e-10
11.891,1.5147e-09,1.1579e-10
11.894,1.519e-09,1.1553e-10
11.897,1.5233e-09,1.1564e-10
11.9,1.5264e-09,1.155e-10
11.903,1.5305e-09,1.1513e-10
11.906,1.5344e-09,1.1513e-10
11.909,1.538e-09,1.1475e-10
11.912,1.5421e-09,1.1489e-10
11.915,1.5464e-09,1.1428e-10
11.918,1.5492e-09,1.1442e-10
11.921,1.5534e-09,1.1477e-10
11.924,1.5573e-09,1.15e-10
11.927,1.5611e-09,1.1469e-10
11.93,1.5663e-09,1.1427e-10
11.933,1.5704e-09,1.1413e-10
11.936,1.5734e-09,1.1341e-10
11.939,1.5774e-09,1.1307e-10
11.942,1.5815e-09,1.1386e-10
11.945,1.5844e-09,1.1322e-10
11.948,1.5886e-09,1.131e-10
11.951,1.5933e-09,1.1309e-10
11.954,1.5972e-09,1.1316e-10
11.957,1.6013e-09,1.1316e-10
11.96,1.605e-09,1.1228e-10
11.963,1.6089e-09,1.1183e-10
11.966,1.613e-09,1.1193e-10
11.969,1.6178e-09,1.1131e-10
11.972,1.6219e-09,1.1197e-10
11.975,1.6264e-09,1.1168e-10
11.978,1.63e-09,1.112e-10
11.981,1.6338e-09,1.1095e-10
11.984,1.6378e-09,1.107e-10
11.987,1.6419e-09,1.1076e-10
11.99,1.646e-09,1.0995e-10
11.993,1.6496e-09,1.1146e-10
11.996,1.6536e-09,1.1052e-10
11.999,1.6588e-09,1.1013e-10
12.002,1.6628e-09,1.1028e-10
12.005,1.6669e-09,1.096e-10
12.007,1.6707e-09,1.1049e-10
12.01,1.6749e-09,1.0969e-10
12.013,1.6788e-09,1.0961e-10
12.016,1.6844e-09,1.086e-10
12.019,1.6884e-09,1.0855e-10
12.022,1.6921e-09,1.0874e-10
12.025,1.6962e-09,1.0832e-10
12.028,1.7008e-09,1.0836e-10
12.031,1.7056e-09,1.0819e-10
12.034,1.709e-09,1.0718e-10
12.037,1.7131e-09,1.0688e-10
12.04,1.7181e-09,1.0613e-10
12.043,1.7219e-09,1.073e-10
12.046,1.726e-09,1.0751e-10
12.049,1.7313e-09,1.0549e-10
12.052,1.7356e-09,1.064e-10
12.055,1.7396e-09,1.0678e-10
12.058,1.7443e-09,1.0506e-10
12.061,1.7482e-09,1.0591e-10
12.064,1.7531e-09,1.0528e-10
12.067,1.7569e-09,1.0512e-10
12.07,1.7611e-09,1.0421e-10
12.073,1.7647e-09,1.0485e-10
12.076,1.7694e-09,1.0395e-10
12.079,1.7738e-09,1.0329e-10
12.082,1.7789e-09,1.0327e-10
12.085,1.7829e-09,1.0341e-10
12.088,1.7881e-09,1.0377e-10
12.091,1.792e-09,1.0268e-10
12.094,1.7966e-09,1.0254e-10
12.097,1.8016e-09,1.0176e-10
12.1,1.8063e-09,1.0261e-10
12.103,1.81e-09,1.0232e-10
12.106,1.815e-09,1.0266e-10
12.109,1.8196e-09,1.0261e-10
12.112,1.8237e-09,1.0189e-10
12.115,1.8281e-09,1.0065e-10
12.118,1.8333e-09,1.0018e-10
12.121,1.837e-09,1.0003e-10
12.124,1.8417e-09,9.8784e-11
12.127,1.8458e-09,1.0038e-10
12.13,1.8516e-09,9.9633e-11
12.133,1.8557e-09,9.8394e-11
12.136,1.8599e-09,9.8553e-11
12.139,1.8652e-09,9.9195e-11
12.142,1.8696e-09,9.8878e-11
12.145,1.8739e-09,9.8649e-11
12.148,1.8787e-09,9.6771e-11
12.151,1.8836e-09,9.7737e-11
12.154,1.8887e-09,9.7077e-11
12.157,1.8919e-09,9.6995e-11
12.159,1.8971e-09,9.6624e-11
12.162,1.902e-09,9.6033e-11
12.165,1.9074e-09,9.6377e-11
12.168,1.9113e-09,9.5129e-11
12.171,1.9167e-09,9.602e-11
12.174,1.9216e-09,9.4849e-11
12.177,1.9257e-09,9.5037e-11
12.18,1.9315e-09,9.4421e-11
12.183,1.9354e-09,9.4262e-11
12.186,1.9404e-09,9.3717e-11
12.189,1.9457e-09,9.3717e-11
12.192,1.9505e-09,9.2125e-11
12.195,1.956e-09,9.2538e-11
12.198,1.9598e-09,9.2147e-11
12.201,1.9653e-09,9.193e-11
12.204,1.9703e-09,9.1642e-11
12.207,1.9746e-09,9.1511e-11
12.21,1.9792e-09,9.1618e-11
12.213,1.9848e-09,9.041e-11
12.216,1.9888e-09,9.0334e-11
12.219,1.994e-09,8.963e-11
12.222,1.9987e-09,8.9084e-11
12.225,2.0037e-09,8.8985e-11
12.228,2.0089e-09,8.8826e-11
12.231,2.0144e-09,8.7775e-11
12.234,2.0198e-09,8.8395e-11
12.237,2.0246e-09,8.7929e-11
12.24,2.0299e-09,8.6439e-11
12.243,2.0339e-09,8.6734e-11
12.246,2.0389e-09,8.6135e-11
12.249,2.0438e-09,8.5801e-11
12.252,2.0493e-09,8.4279e-11
12.255,2.0538e-09,8.4898e-11
12.258,2.0587e-09,8.4207e-11
12.261,2.0646e-09,8.4107e-11
12.264,2.0691e-09,8.3678e-11
12.267,2.0737e-09,8.4256e-11
12.27,2.0786e-09,8.3139e-11
12.273,2.0848e-09,8.194e-11
12.276,2.0898e-09,8.1809e-11
12.279,2.0946e-09,8.2197e-11
12.282,2.1004e-09,8.0458e-11
12.285,2.1057e-09,8.1774e-11
12.288,2.1111e-09,7.9389e-11
12.291,2.1147e-09,7.9932e-11
12.294,2.1209e-09,7.9867e-11
12.297,2.126e-09,7.9994e-11
12.3,2.1321e-09,7.9144e-11
12.303,2.1371e-09,7.8374e-11
12.306,2.1424e-09,7.858e-11
12.309,2.1466e-09,7.7159e-11
12.312,2.153e-09,7.7068e-11
12.314,2.1585e-09,7.6204e-11
12.317,2.1644e-09,7.6122e-11
12.32,2.1699e-09,7.4921e-11
12.323,2.174e-09,7.4394e-11
12.326,2.1789e-09,7.4913e-11
12.329,2.1848e-09,7.3274e-11
12.332,2.1896e-09,7.3371e-11
12.335,2.1949e-09,7.3958e-11
12.338,2.2006e-09,7.3512e-11
12.341,2.2063e-09,7.1647e-11
12.344,2.212e-09,7.245e-11
12.347,2.2175e-09,7.1202e-11
12.35,2.2223e-09,7.0707e-11
12.353,2.2284e-09,7.1231e-11
12.356,2.2342e-09,7.0607e-11
12.359,2.2391e-09,6.9125e-11
12.362,2.2441e-09,6.9342e-11
12.365,2.25e-09,6.7951e-11
12.368,2.2564e-09,6.8552e-11
12.371,2.2611e-09,6.8237e-11
12.374,2.2664e-09,6.7834e-11
12.377,2.273e-09,6.7168e-11
12.38,2.2774e-09,6.6366e-11
12.383,2.2842e-09,6.609e-11
12.386,2.2895e-09,6.5373e-11
12.389,2.294e-09,6.5372e-11
12.392,2.3009e-09,6.3541e-11
12.395,2.306e-09,6.1668e-11
12.398,2.312e-09,6.2649e-11
12.401,2.3182e-09,6.3068e-11
12.404,2.323e-09,6.173e-11
12.407,2.3282e-09,6.1076e-11
12.41,2.335e-09,6.1026e-11
12.413,2.3402e-09,5.9746e-11
12.416,2.3473e-09,5.9454e-11
12.419,2.3511e-09,5.9378e-11
12.422,2.357e-09,5.9533e-11
12.425,2.3631e-09,5.7443e-11
12.428,2.369e-09,5.6808e-11
12.431,2.3755e-09,5.6689e-11
12.434,2.38e-09,5.6369e-11
12.437,2.387e-09,5.6388e-11
12.44,2.3921e-09,5.5507e-11
12.443,2.3994e-09,5.3909e-11
12.446,2.4033e-09,5.3959e-11
12.449,2.4094e-09,5.3448e-11
12.452,2.4163e-09,5.2656e-11
12.455,2.4212e-09,5.2787e-11
12.458,2.4266e-09,5.2097e-11
12.461,2.4346e-09,5.0778e-11
12.464,2.4397e-09,5.0271e-11
12.466,2.4458e-09,5.0444e-11
12.469,2.451e-09,4.8712e-11
12.472,2.4567e-09,4.9437e-11
12.475,2.4641e-09,4.7129e-11
12.478,2.4702e-09,4.782e-11
12.481,2.4761e-09,4.7356e-11
12.484,2.4818e-09,4.547e-11
12.487,2.4879e-09,4.5681e-11
12.49,2.494e-09,4.4482e-11
12.493,2.4992e-09,4.4461e-11
12.496,2.5058e-09,4.3824e-11
12.499,2.5112e-09,4.2885e-11
12.502,2.5184e-09,4.101e-11
12.505,2.5244e-09,4.1321e-11
12.508,2.5299e-09,4.1224e-11
12.511,2.5363e-09,3.8808e-11
12.514,2.5427e-09,3.873e-11
12.517,2.5493e-09,3.8235e-11
12.52,2.5545e-09,3.7965e-11
12.523,2.5614e-09,3.8052e-11
12.526,2.568e-09,3.6373e-11
12.529,2.5734e-09,3.6706e-11
12.532,2.5813e-09,3.4638e-11
12.535,2.5865e-09,3.5143e-11
12.538,2.5926e-09,3.3739e-11
12.541,2.5993e-09,3.3396e-11
12.544,2.6047e-09,3.2557e-11
12.547,2.6125e-09,3.22e-11
12.55,2.6185e-09,3.1069e-11
12.553,2.6239e-09,3.14e-11
12.556,2.6317e-09,2.9817e-11
12.559,2.6388e-09,2.8256e-11
12.562,2.6439e-09,2.8451e-11
12.565,2.6517e-09,2.6786e-11
12.568,2.6565e-09,2.6482e-11
12.571,2.6634e-09,2.4928e-11
12.574,2.6701e-09,2.5464e-11
12.577,2.6758e-09,2.5489e-11
12.58,2.6821e-09,2.5713e-11
12.583,2.6884e-09,2.3077e-11
12.586,2.6951e-09,2.2997e-11
12.589,2.7016e-09,2.2734e-11
12.592,2.7078e-09,2.0418e-11
12.595,2.7151e-09,2.1282e-11
12.598,2.7221e-09,1.9052e-11
12.601,2.7287e-09,1.8785e-11
12.604,2.7355e-09,1.6244e-11
12.607,2.7409e-09,1.8705e-11
12.61,2.7494e-09,1.6734e-11
12.613,2.7557e-09,1.6077e-11
12.616,2.7621e-09,1.3379e-11
12.619,2.7699e-09,1.377e-11
12.621,2.7751e-09,1.3575e-11
12.624,2.7821e-09,1.2677e-11
12.627,2.7874e-09,1.2324e-11
12.63,2.796e-09,1.0124e-11
12.633,2.8035e-09,8.7103e-12
12.636,2.8094e-09,7.8934e-12
12.639,2.8163e-09,7.4677e-12
12.642,2.8236e-09,5.8783e-12
12.645,2.8297e-09,6.788e-12
12.648,2.8374e-09,3.7955e-12
12.651,2.8443e-09,2.8774e-12
12.654,2.8512e-09,4.45e-12
12.657,2.8562e-09,3.0504e-12
12.66,2.8646e-09,1.8942e-12
12.663,2.8705e-09,1.3165e-12
12.666,2.8783e-09,2.2613e-13
12.669,2.8854e-09,4.0743e-13
12.672,2.8913e-09,1.5919e-12
12.675,2.8969e-09,4.0038e-12
12.678,2.9068e-09,3.9221e-12
12.681,2.9109e-09,3.822e-12
12.684,2.9218e-09,6.4153e-12
12.687,2.9273e-09,7.2657e-12
12.69,2.9339e-09,6.3522e-12
12.693,2.9413e-09,7.152e-12
12.696,2.949e-09,6.6944e-12
12.699,2.9572e-09,1.2489e-11
12.702,2.9628e-09,1.1617e-11
12.705,2.9691e-09,1.267e-11
12.708,2.9764e-09,1.1753e-11
12.711,2.9849e-09,1.3432e-11
12.714,2.9926e-09,1.2573e-11
12.717,2.999e-09,1.507e-11
12.72,3.0073e-09,1.7549e-11
12.723,3.014e-09,1.9328e-11
12.726,3.019e-09,1.7831e-11
12.729,3.028e-09,2.0802e-11
12.732,3.0351e-09,2.0865e-11
12.735,3.0427e-09,2.4095e-11
12.738,3.0509e-09,2.3444e-11
12.741,3.0594e-09,2.5739e-11
12.744,3.0654e-09,2.4978e-11
12.747,3.0729e-09,2.7051e-11
12.75,3.0798e-09,2.8128e-11
12.753,3.0871e-09,2.8014e-11
12.756,3.0965e-09,3.1628e-11
12.759,3.101e-09,3.1163e-11
12.762,3.1096e-09,3.1562e-11
12.765,3.1178e-09,3.2062e-11
12.768,3.1248e-09,3.5099e-11
12.771,3.1319e-09,3.3897e-11
12.773,3.1394e-09,3.7131e-11
12.776,3.1455e-09,3.4819e-11
12.779,3.1556e-09,3.7549e-11
12.782,3.1612e-09,4.0612e-11
12.785,3.1689e-09,4.1438e-11
12.788,3.1772e-09,4.1313e-11
12.791,3.1846e-09,4.2969e-11
12.794,3.193e-09,4.2047e-11
12.797,3.1993e-09,4.5174e-11
12.8,3.2083e-09,4.68e-11
12.803,3.2161e-09,4.6784e-11
12.806,3.225e-09,4.84e-11
12.809,3.231e-09,4.8976e-11
12.812,3.2381e-09,5.0257e-11
12.815,3.2462e-09,5.4227e-11
12.818,3.2539e-09,5.3491e-11
12.821,3.2616e-09,5.3724e-11
12.824,3.2684e-09,5.2634e-11
12.827,3.2771e-09,5.5894e-11
12.83,3.2863e-09,5.7362e-11
12.833,3.2939e-09,5.8193e-11
12.836,3.3023e-09,5.9602e-11
12.839,3.309e-09,5.9322e-11
12.842,3.3182e-09,6.1097e-11
12.845,3.3268e-09,6.2945e-11
12.848,3.334e-09,6.3285e-11
12.851,3.3419e-09,6.4979e-11
12.854,3.3514e-09,6.6836e-11
12.857,3.3555e-09,6.6956e-11
12.86,3.3641e-09,6.9115e-11
12.863,3.3735e-09,7.0779e-11
12.866,3.382e-09,7.2934e-11
12.869,3.3886e-09,7.2605e-11
12.872,3.3974e-09,7.52e-11
12.875,3.406e-09,7.3645e-11
12.878,3.4141e-09,7.7347e-11
12.881,3.4223e-09,7.9287e-11
12.884,3.4314e-09,7.9711e-11
12.887,3.4387e-09,8.0627e-11
12.89,3.4451e-09,8.2279e-11
12.893,3.455e-09,8.2319e-11
12.896,3.4644e-09,8.4131e-11
12.899,3.4723e-09,8.5255e-11
12.902,3.48e-09,8.8367e-11
12.905,3.4886e-09,8.7706e-11
12.908,3.4957e-09,8.9749e-11
12.911,3.5064e-09,9.1468e-11
12.914,3.5144e-09,9.3224e-11
12.917,3.5226e-09,9.1361e-11
12.92,3.531e-09,9.4098e-11
12.923,3.5394e-09,9.6775e-11
12.926,3.5453e-09,9.6447e-11
12.928,3.555e-09,9.8331e-11
12.931,3.5647e-09,9.9552e-11
12.934,3.5717e-09,1.0274e-10
12.937,3.5808e-09,1.0251e-10
12.94,3.5895e-09,1.0639e-10
12.943,3.5966e-09,1.0697e-10
12.946,3.6056e-09,1.0767e-10
12.949,3.6153e-09,1.0733e-10
12.952,3.623e-09,1.0859e-10
12.955,3.6331e-09,1.1189e-10
12.958,3.6426e-09,1.1158e-10
12.961,3.6502e-09,1.138e-10
12.964,3.6608e-09,1.1692e-10
12.967,3.6686e-09,1.1779e-10
12.97,3.6759e-09,1.1829e-10
12.973,3.6843e-09,1.2006e-10
12.976,3.6922e-09,1.2224e-10
12.979,3.7012e-09,1.2402e-10
12.982,3.7106e-09,1.2499e-10
12.985,3.718e-09,1.2693e-10
12.988,3.7283e-09,1.2882e-10
12.991,3.738e-09,1.2884e-10
12.994,3.7459e-09,1.3317e-10
12.997,3.7564e-09,1.317e-10
13,3.7647e-09,1.3331e-10
13.003,3.7741e-09,1.3637e-10
13.006,3.783e-09,1.3711e-10
13.009,3.7936e-09,1.4027e-10
13.012,3.8008e-09,1.4257e-10
13.015,3.8091e-09,1.4236e-10
13.018,3.8181e-09,1.4387e-10
13.021,3.8272e-09,1.4446e-10
13.024,3.8369e-09,1.4636e-10
13.027,3.8475e-09,1.4696e-10
13.03,3.8553e-09,1.5031e-10
13.033,3.8638e-09,1.4967e-10
13.036,3.8757e-09,1.5244e-10
13.039,3.8834e-09,1.5524e-10
13.042,3.8902e-09,1.5678e-10
13.045,3.9008e-09,1.5898e-10
13.048,3.9107e-09,1.5935e-10
13.051,3.919e-09,1.6108e-10
13.054,3.93e-09,1.6269e-10
13.057,3.9391e-09,1.6399e-10
13.06,3.9479e-09,1.6569e-10
13.063,3.957e-09,1.671e-10
13.066,3.9661e-09,1.6948e-10
13.069,3.9759e-09,1.7331e-10
13.072,3.984e-09,1.71e-10
13.075,3.9955e-09,1.7537e-10
13.078,4.005e-09,1.7554e-10
13.08,4.0139e-09,1.765e-10
13.083,4.0251e-09,1.804e-10
13.086,4.0321e-09,1.8233e-10
13.089,4.0435e-09,1.8441e-10
13.092,4.0525e-09,1.8401e-10
13.095,4.0604e-09,1.8675e-10
13.098,4.0722e-09,1.8881e-10
13.101,4.0824e-09,1.8997e-10
13.104,4.0916e-09,1.9291e-10
13.107,4.0993e-09,1.9477e-10
13.11,4.109e-09,1.955e-10
13.113,4.1191e-09,1.9967e-10
13.116,4.1288e-09,2.0047e-10
13.119,4.1387e-09,2.0176e-10
13.122,4.1504e-09,2.0253e-10
13.125,4.16e-09,2.0494e-10
13.128,4.168e-09,2.0673e-10
13.131,4.1788e-09,2.0779e-10
13.134,4.1884e-09,2.099e-10
13.137,4.1956e-09,2.1199e-10
13.14,4.2094e-09,2.1442e-10
13.143,4.2175e-09,2.1568e-10
13.146,4.2298e-09,2.1936e-10
13.149,4.2382e-09,2.1992e-10
13.152,4.2488e-09,2.2198e-10
13.155,4.2583e-09,2.2353e-10
13.158,4.2688e-09,2.2502e-10
13.161,4.2766e-09,2.2771e-10
13.164,4.2887e-09,2.2912e-10
13.167,4.2969e-09,2.3334e-10
13.17,4.3077e-09,2.3344e-10
13.173,4.3181e-09,2.3615e-10
13.176,4.3266e-09,2.3664e-10
13.179,4.3386e-09,2.3986e-10
13.182,4.3478e-09,2.4036e-10
13.185,4.3595e-09,2.4478e-10
13.188,4.3705e-09,2.4683e-10
13.191,4.3793e-09,2.4828e-10
13.194,4.3924e-09,2.4973e-10
13.197,4.4001e-09,2.5075e-10
13.2,4.4109e-09,2.55e-10
13.203,4.4213e-09,2.5612e-10
13.206,4.4307e-09,2.6001e-10
13.209,4.4425e-09,2.5934e-10
13.212,4.4524e-09,2.6319e-10
13.215,4.4627e-09,2.644e-10
13.218,4.4741e-09,2.6686e-10
13.221,4.4849e-09,2.6781e-10
13.224,4.4965e-09,2.6966e-10
13.227,4.5065e-09,2.7278e-10
13.23,4.5166e-09,2.7565e-10
13.233,4.5278e-09,2.7922e-10
13.235,4.5392e-09,2.7832e-10
13.238,4.5481e-09,2.8173e-10
13.241,4.5588e-09,2.8395e-10
13.244,4.5691e-09,2.8644e-10
13.247,4.5795e-09,2.8635e-10
13.25,4.5908e-09,2.9068e-10
13.253,4.6027e-09,2.9313e-10
13.256,4.6107e-09,2.9511e-10
13.259,4.6247e-09,2.9631e-10
13.262,4.6346e-09,3.0011e-10
13.265,4.6438e-09,3.025e-10
13.268,4.6557e-09,3.0363e-10
13.271,4.6652e-09,3.073e-10
13.274,4.6775e-09,3.1029e-10
13.277,4.6876e-09,3.1188e-10
13.28,4.7001e-09,3.1263e-10
13.283,4.7114e-09,3.1151e-10
13.286,4.72e-09,3.1822e-10
13.289,4.7309e-09,3.2076e-10
13.292,4.7438e-09,3.2037e-10
13.295,4.7561e-09,3.2733e-10
13.298,4.764e-09,3.2706e-10
13.301,4.7771e-09,3.3181e-10
13.304,4.7891e-09,3.3119e-10
13.307,4.7979e-09,3.3464e-10
13.31,4.8104e-09,3.3615e-10
13.313,4.8211e-09,3.4174e-10
13.316,4.8341e-09,3.4193e-10
13.319,4.8446e-09,3.4524e-10
13.322,4.8559e-09,3.473e-10
13.325,4.8683e-09,3.5202e-10
13.328,4.8791e-09,3.5086e-10
13.331,4.8902e-09,3.5448e-10
13.334,4.9045e-09,3.5909e-10
13.337,4.9136e-09,3.605e-10
13.34,4.9239e-09,3.6153e-10
13.343,4.9351e-09,3.6382e-10
13.346,4.9476e-09,3.6575e-10
13.349,4.9619e-09,3.687e-10
13.352,4.968e-09,3.7086e-10
13.355,4.9803e-09,3.7434e-10
13.358,4.9933e-09,3.7567e-10
13.361,5.0033e-09,3.8048e-10
13.364,5.0173e-09,3.8104e-10
13.367,5.0319e-09,3.8625e-10
13.37,5.0424e-09,3.8786e-10
13.373,5.0522e-09,3.8923e-10
13.376,5.0625e-09,3.9153e-10
13.379,5.0761e-09,3.9759e-10
13.382,5.0911e-09,3.9794e-10
13.385,5.0981e-09,4.032e-10
13.387,5.1149e-09,4.0236e-10
13.39,5.1246e-09,4.0632e-10
13.393,5.1359e-09,4.0937e-10
13.396,5.1524e-09,4.1466e-10
13.399,5.1582e-09,4.1487e-10
13.402,5.174e-09,4.1911e-10
13.405,5.1826e-09,4.1904e-10
13.408,5.1971e-09,4.2514e-10
13.411,5.2146e-09,4.249e-10
13.414,5.2206e-09,4.29e-10
13.417,5.2364e-09,4.338e-10
13.42,5.245e-09,4.3624e-10
13.423,5.256e-09,4.3728e-10
13.426,5.2655e-09,4.4086e-10
13.429,5.2814e-09,4.3927e-10
13.432,5.2977e-09,4.4384e-10
13.435,5.3073e-09,4.4706e-10
13.438,5.3163e-09,4.5103e-10
13.441,5.3294e-09,4.5405e-10
13.444,5.3449e-09,4.6137e-10
13.447,5.3534e-09,4.6125e-10
13.45,5.3673e-09,4.6493e-10
13.453,5.3795e-09,4.6438e-10
13.456,5.3926e-09,4.673e-10
13.459,5.402e-09,4.7184e-10
13.462,5.417e-09,4.7356e-10
13.465,5.4336e-09,4.7535e-10
13.468,5.4435e-09,4.7938e-10
13.471,5.4524e-09,4.8035e-10
13.474,5.4687e-09,4.8679e-10
13.477,5.4794e-09,4.9092e-10
13.48,5.4924e-09,4.9326e-10
13.483,5.505e-09,4.9287e-10
13.486,5.5157e-09,4.9987e-10
13.489,5.5335e-09,5.0168e-10
13.492,5.54e-09,5.0311e-10
13.495,5.5549e-09,5.0861e-10
13.498,5.5713e-09,5.1129e-10
13.501,5.5824e-09,5.1634e-10
13.504,5.5954e-09,5.2051e-10
13.507,5.6079e-09,5.2254e-10
13.51,5.6238e-09,5.2295e-10
13.513,5.633e-09,5.2598e-10
13.516,5.6473e-09,5.2867e-10
13.519,5.6592e-09,5.3223e-10
13.522,5.6731e-09,5.3792e-10
13.525,5.6888e-09,5.3954e-10
13.528,5.7011e-09,5.4082e-10
13.531,5.7159e-09,5.4682e-10
13.534,5.7303e-09,5.5302e-10
13.537,5.739e-09,5.5131e-10
13.54,5.7537e-09,5.5497e-10
13.542,5.7687e-09,5.6097e-10
13.545,5.7826e-09,5.6516e-10
13.548,5.7899e-09,5.6699e-10
13.551,5.8093e-09,5.6734e-10
13.554,5.8234e-09,5.7598e-10
13.557,5.8343e-09,5.7537e-10
13.56,5.8485e-09,5.7975e-10
13.563,5.8619e-09,5.8416e-10
13.566,5.8755e-09,5.8133e-10
13.569,5.887e-09,5.9295e-10
13.572,5.8992e-09,5.967e-10
13.575,5.9132e-09,5.983e-10
13.578,5.9282e-09,6.0222e-10
13.581,5.9461e-09,6.0384e-10
13.584,5.9569e-09,6.0644e-10
13.587,5.9716e-09,6.1089e-10
13.59,5.9856e-09,6.1231e-10
13.593,5.9984e-09,6.1865e-10
13.596,6.0088e-09,6.1894e-10
13.599,6.0256e-09,6.2276e-10
13.602,6.0378e-09,6.2774e-10
13.605,6.0518e-09,6.3083e-10
13.608,6.0681e-09,6.3685e-10
13.611,6.0813e-09,6.405e-10
13.614,6.0947e-09,6.4274e-10
13.617,6.1106e-09,6.4459e-10
13.62,6.1256e-09,6.4963e-10
13.623,6.1352e-09,6.5631e-10
13.626,6.1534e-09,6.5535e-10
13.629,6.1652e-09,6.5945e-10
13.632,6.1814e-09,6.6272e-10
13.635,6.1933e-09,6.6704e-10
13.638,6.2092e-09,6.7523e-10
13.641,6.2236e-09,6.7619e-10
13.644,6.235e-09,6.8046e-10
13.647,6.2492e-09,6.8297e-10
13.65,6.2684e-09,6.8668e-10
13.653,6.2789e-09,6.8855e-10
13.656,6.2973e-09,6.9594e-10
13.659,6.3109e-09,6.9854e-10
13.662,6.326e-09,7.0455e-10
13.665,6.3384e-09,7.1005e-10
13.668,6.357e-09,7.0866e-10
13.671,6.3685e-09,7.155e-10
13.674,6.385e-09,7.1878e-10
13.677,6.3933e-09,7.2306e-10
13.68,6.4101e-09,7.2965e-10
13.683,6.428e-09,7.3066e-10
13.686,6.4384e-09,7.3576e-10
13.689,6.4562e-09,7.3766e-10
13.692,6.4705e-09,7.4505e-10
13.694,6.4873e-09,7.4615e-10
13.697,6.5003e-09,7.4817e-10
13.7,6.5145e-09,7.5565e-10
13.703,6.5293e-09,7.6051e-10
13.706,6.544e-09,7.6219e-10
13.709,6.5606e-09,7.6886e-10
13.712,6.577e-09,7.6985e-10
13.715,6.5911e-09,7.7387e-10
13.718,6.6045e-09,7.7641e-10
13.721,6.6202e-09,7.8353e-10
13.724,6.6386e-09,7.8706e-10
13.727,6.6519e-09,7.9508e-10
13.73,6.6685e-09,7.9372e-10
13.733,6.684e-09,8.0095e-10
13.736,6.6946e-09,8.0547e-10
13.739,6.7115e-09,8.1069e-10
13.742,6.727e-09,8.1359e-10
13.745,6.7429e-09,8.1975e-10
13.748,6.7585e-09,8.2146e-10
13.751,6.7765e-09,8.2505e-10
13.754,6.7872e-09,8.3284e-10
13.757,6.8035e-09,8.3326e-10
13.76,6.8214e-09,8.3656e-10
13.763,6.8348e-09,8.4493e-10
13.766,6.8522e-09,8.4894e-10
13.769,6.8673e-09,8.5624e-10
13.772,6.8805e-09,8.5945e-10
13.775,6.9021e-09,8.6431e-10
13.778,6.9142e-09,8.6908e-10
13.781,6.9321e-09,8.7108e-10
13.784,6.9458e-09,8.7615e-10
13.787,6.9571e-09,8.7984e-10
13.79,6.9772e-09,8.8274e-10
13.793,6.9914e-09,8.8503e-10
13.796,7.0074e-09,8.9526e-10
13.799,7.0237e-09,8.9938e-10
13.802,7.0422e-09,9.0311e-10
13.805,7.0579e-09,9.0559e-10
13.808,7.0719e-09,9.1485e-10
13.811,7.0901e-09,9.1322e-10
13.814,7.1045e-09,9.2188e-10
13.817,7.1198e-09,9.2651e-10
13.82,7.1358e-09,9.3145e-10
13.823,7.1543e-09,9.3701e-10
13.826,7.1686e-09,9.3987e-10
13.829,7.1875e-09,9.4355e-10
13.832,7.2e-09,9.5319e-10
13.835,7.2197e-09,9.5657e-10
13.838,7.2355e-09,9.651e-10
13.841,7.2555e-09,9.647e-10
13.844,7.2687e-09,9.6915e-10
13.847,7.2834e-09,9.7223e-10
13.849,7.3034e-09,9.7966e-10
13.852,7.318e-09,9.8437e-10
13.855,7.3374e-09,9.9085e-10
13.858,7.3506e-09,9.9801e-10
13.861,7.3696e-09,9.9812e-10
13.864,7.3871e-09,1.0054e-09
13.867,7.4018e-09,1.0111e-09
13.87,7.4206e-09,1.0128e-09
13.873,7.4373e-09,1.022e-09
13.876,7.4505e-09,1.0195e-09
13.879,7.4701e-09,1.0279e-09
13.882,7.4874e-09,1.0329e-09
13.885,7.5036e-09,1.0385e-09
13.888,7.518e-09,1.0453e-09
13.891,7.5389e-09,1.0506e-09
13.894,7.5592e-09,1.0517e-09
13.897,7.5724e-09,1.0546e-09
13.9,7.5935e-09,1.0671e-09
13.903,7.6097e-09,1.0692e-09
13.906,7.6241e-09,1.0731e-09
13.909,7.6409e-09,1.0835e-09
13.912,7.6625e-09,1.0869e-09
13.915,7.6735e-09,1.0905e-09
13.918,7.6908e-09,1.0942e-09
13.921,7.7064e-09,1.1042e-09
13.924,7.7291e-09,1.1097e-09
13.927,7.7461e-09,1.1155e-09
13.93,7.759e-09,1.1207e-09
13.933,7.7813e-09,1.125e-09
13.936,7.8011e-09,1.1337e-09
13.939,7.815e-09,1.1384e-09
13.942,7.8345e-09,1.1375e-09
13.945,7.8504e-09,1.145e-09
13.948,7.8663e-09,1.1527e-09
13.951,7.887e-09,1.156e-09
13.954,7.9038e-09,1.1632e-09
13.957,7.9176e-09,1.1637e-09
13.96,7.9409e-09,1.1729e-09
13.963,7.9565e-09,1.1793e-09
13.966,7.9724e-09,1.1846e-09
13.969,7.9924e-09,1.1929e-09
13.972,8.0095e-09,1.1967e-09
13.975,8.0328e-09,1.202e-09
13.978,8.0455e-09,1.2087e-09
13.981,8.0713e-09,1.2166e-09
13.984,8.0795e-09,1.2224e-09
13.987,8.0998e-09,1.227e-09
13.99,8.1165e-09,1.2341e-09
13.993,8.1337e-09,1.2347e-09
13.996,8.1578e-09,1.2422e-09
13.999,8.1784e-09,1.2467e-09
14.002,8.1958e-09,1.2581e-09
14.004,8.2128e-09,1.2604e-09
14.007,8.2282e-09,1.2677e-09
14.01,8.2528e-09,1.2679e-09
14.013,8.2626e-09,1.2783e-09
14.016,8.2851e-09,1.2898e-09
14.019,8.3062e-09,1.2927e-09
14.022,8.3278e-09,1.2957e-09
14.025,8.344e-09,1.3022e-09
14.028,8.3622e-09,1.3089e-09
14.031,8.3795e-09,1.3115e-09
14.034,8.3971e-09,1.3238e-09
14.037,8.4145e-09,1.324e-09
14.04,8.4333e-09,1.3378e-09
14.043,8.4548e-09,1.3419e-09
14.046,8.4759e-09,1.3448e-09
14.049,8.4932e-09,1.356e-09
14.052,8.5094e-09,1.3592e-09
14.055,8.5348e-09,1.3643e-09
14.058,8.5543e-09,1.3678e-09
14.061,8.5746e-09,1.3724e-09
14.064,8.5939e-09,1.3808e-09
14.067,8.6068e-09,1.3909e-09
14.07,8.6307e-09,1.3948e-09
14.073,8.6503e-09,1.4061e-09
14.076,8.6686e-09,1.4162e-09
14.079,8.6888e-09,1.4144e-09
14.082,8.709e-09,1.4252e-09
14.085,8.7275e-09,1.4321e-09
14.088,8.7436e-09,1.4398e-09
14.091,8.769e-09,1.442e-09
14.094,8.7914e-09,1.4513e-09
14.097,8.8096e-09,1.4512e-09
14.1,8.8217e-09,1.462e-09
14.103,8.8411e-09,1.4758e-09
14.106,8.8653e-09,1.4744e-09
14.109,8.8883e-09,1.4897e-09
14.112,8.9027e-09,1.4937e-09
14.115,8.9268e-09,1.4997e-09
14.118,8.9545e-09,1.5087e-09
14.121,8.9674e-09,1.511e-09
14.124,8.9861e-09,1.5176e-09
14.127,8.9997e-09,1.5239e-09
14.13,9.0222e-09,1.5297e-09
14.133,9.0502e-09,1.5422e-09
14.136,9.0649e-09,1.5408e-09
14.139,9.0825e-09,1.5532e-09
14.142,9.1021e-09,1.5606e-09
14.145,9.1265e-09,1.5653e-09
14.148,9.1516e-09,1.5705e-09
14.151,9.1699e-09,1.5798e-09
14.154,9.1797e-09,1.5895e-09
14.156,9.2092e-09,1.5889e-09
14.159,9.2249e-09,1.6018e-09
14.162,9.2451e-09,1.6088e-09
14.165,9.2704e-09,1.6108e-09
14.168,9.2959e-09,1.6246e-09
14.171,9.3109e-09,1.6335e-09
14.174,9.33e-09,1.6478e-09
14.177,9.356e-09,1.6376e-09
14.18,9.3686e-09,1.6552e-09
14.183,9.3995e-09,1.66e-09
14.186,9.4133e-09,1.664e-09
14.189,9.4321e-09,1.6781e-09
14.192,9.456e-09,1.6785e-09
14.195,9.4771e-09,1.6908e-09
14.198,9.5024e-09,1.6962e-09
14.201,9.5146e-09,1.7036e-09
14.204,9.5429e-09,1.7123e-09
14.207,9.5627e-09,1.7129e-09
14.21,9.5896e-09,1.7234e-09
14.213,9.6086e-09,1.7309e-09
14.216,9.6259e-09,1.7401e-09
14.219,9.6473e-09,1.7442e-09
14.222,9.6682e-09,1.7545e-09
14.225,9.6932e-09,1.7599e-09
14.228,9.7113e-09,1.7685e-09
14.231,9.7424e-09,1.7766e-09
14.234,9.7499e-09,1.7853e-09
14.237,9.7694e-09,1.795e-09
14.24,9.7948e-09,1.8021e-09
14.243,9.8309e-09,1.8164e-09
14.246,9.8403e-09,1.8195e-09
14.249,9.8675e-09,1.8279e-09
14.252,9.8909e-09,1.8392e-09
14.255,9.9116e-09,1.8518e-09
14.258,9.9329e-09,1.848e-09
14.261,9.9468e-09,1.8577e-09
14.264,9.9739e-09,1.8661e-09
14.267,9.9924e-09,1.8745e-09
14.27,1.0013e-08,1.8941e-09
14.273,1.0042e-08,1.89e-09
14.276,1.006e-08,1.9031e-09
14.279,1.009e-08,1.9132e-09
14.282,1.0112e-08,1.919e-09
14.285,1.0134e-08,1.9186e-09
14.288,1.0152e-08,1.9369e-09
14.291,1.0173e-08,1.9415e-09
14.294,1.0191e-08,1.9521e-09
14.297,1.0219e-08,1.9561e-09
14.3,1.0241e-08,1.9684e-09
14.303,1.0261e-08,1.9796e-09
14.306,1.0293e-08,1.9792e-09
14.309,1.0316e-08,1.9877e-09
14.311,1.0333e-08,2.0045e-09
14.314,1.0356e-08,2.0063e-09
14.317,1.0383e-08,2.0155e-09
14.32,1.0403e-08,2.0297e-09
14.323,1.0433e-08,2.029e-09
14.326,1.0448e-08,2.0457e-09
14.329,1.0477e-08,2.053e-09
14.332,1.0497e-08,2.0664e-09
14.335,1.052e-08,2.0642e-09
14.338,1.0547e-08,2.0833e-09
14.341,1.057e-08,2.0909e-09
14.344,1.0588e-08,2.0938e-09
14.347,1.0609e-08,2.103e-09
14.35,1.0639e-08,2.1115e-09
14.353,1.0658e-08,2.127e-09
14.356,1.0685e-08,2.1344e-09
14.359,1.0707e-08,2.1475e-09
14.362,1.0733e-08,2.1622e-09
14.365,1.075e-08,2.1693e-09
14.368,1.078e-08,2.1758e-09
14.371,1.0802e-08,2.1852e-09
14.374,1.083e-08,2.1937e-09
14.377,1.085e-08,2.2003e-09
14.38,1.0872e-08,2.208e-09
14.383,1.0902e-08,2.2221e-09
14.386,1.0926e-08,2.2296e-09
14.389,1.095e-08,2.2349e-09
14.392,1.0976e-08,2.2462e-09
14.395,1.0989e-08,2.2542e-09
14.398,1.1019e-08,2.2629e-09
14.401,1.1045e-08,2.2728e-09
14.404,1.1066e-08,2.284e-09
14.407,1.1091e-08,2.2934e-09
14.41,1.1114e-08,2.3056e-09
14.413,1.1142e-08,2.3092e-09
14.416,1.1168e-08,2.319e-09
14.419,1.1185e-08,2.3272e-09
14.422,1.1218e-08,2.3456e-09
14.425,1.1236e-08,2.3515e-09
14.428,1.1263e-08,2.3558e-09
14.431,1.1283e-08,2.3669e-09
14.434,1.1317e-08,2.3722e-09
14.437,1.1342e-08,2.3808e-09
14.44,1.1362e-08,2.3959e-09
14.443,1.1393e-08,2.411e-09
14.446,1.1406e-08,2.4204e-09
14.449,1.1436e-08,2.4355e-09
14.452,1.1462e-08,2.4424e-09
14.455,1.1484e-08,2.452e-09
14.458,1.1512e-08,2.4605e-09
14.461,1.1541e-08,2.4688e-09
14.463,1.1564e-08,2.4839e-09
14.466,1.1586e-08,2.4879e-09
14.469,1.1611e-08,2.4992e-09
14.472,1.1639e-08,2.5108e-09
14.475,1.1662e-08,2.5263e-09
14.478,1.169e-08,2.5317e-09
14.481,1.171e-08,2.5424e-09
14.484,1.1737e-08,2.5555e-09
14.487,1.1767e-08,2.5613e-09
14.49,1.1792e-08,2.5744e-09
14.493,1.182e-08,2.5845e-09
14.496,1.185e-08,2.6014e-09
14.499,1.1878e-08,2.6048e-09
14.502,1.1896e-08,2.6176e-09
14.505,1.1926e-08,2.6309e-09
14.508,1.194e-08,2.6365e-09
14.511,1.1973e-08,2.6549e-09
14.514,1.1994e-08,2.6609e-09
14.517,1.2029e-08,2.6762e-09
14.52,1.2055e-08,2.6834e-09
14.523,1.2081e-08,2.688e-09
14.526,1.2105e-08,2.7024e-09
14.529,1.2133e-08,2.7182e-09
14.532,1.2157e-08,2.7278e-09
14.535,1.2192e-08,2.7318e-09
14.538,1.2215e-08,2.7537e-09
14.541,1.2236e-08,2.7551e-09
14.544,1.2259e-08,2.7649e-09
14.547,1.2286e-08,2.7785e-09
14.55,1.2319e-08,2.7945e-09
14.553,1.2341e-08,2.8025e-09
14.556,1.2379e-08,2.8226e-09
14.559,1.2393e-08,2.819e-09
14.562,1.2416e-08,2.8372e-09
14.565,1.2449e-08,2.8476e-09
14.568,1.2475e-08,2.8522e-09
14.571,1.2508e-08,2.8765e-09
14.574,1.2529e-08,2.8906e-09
14.577,1.2562e-08,2.8857e-09
14.58,1.2585e-08,2.9005e-09
14.583,1.2615e-08,2.9161e-09
14.586,1.2642e-08,2.9256e-09
14.589,1.2673e-08,2.9384e-09
14.592,1.2701e-08,2.9512e-09
14.595,1.2728e-08,2.9616e-09
14.598,1.2758e-08,2.9775e-09
14.601,1.2775e-08,2.9862e-09
14.604,1.2809e-08,2.9975e-09
14.607,1.2842e-08,3.0104e-09
14.61,1.2865e-08,3.0285e-09
14.613,1.2892e-08,3.0408e-09
14.616,1.2916e-08,3.0513e-09
14.618,1.2943e-08,3.0561e-09
14.621,1.2977e-08,3.0726e-09
14.624,1.3007e-08,3.0879e-09
14.627,1.3027e-08,3.0944e-09
14.63,1.3061e-08,3.1057e-09
14.633,1.3094e-08,3.1202e-09
14.636,1.3119e-08,3.1323e-09
14.639,1.3146e-08,3.147e-09
14.642,1.3176e-08,3.1533e-09
14.645,1.3203e-08,3.1812e-09
14.648,1.3225e-08,3.1849e-09
14.651,1.3265e-08,3.201e-09
14.654,1.3295e-08,3.2083e-09
14.657,1.3324e-08,3.2237e-09
14.66,1.3344e-08,3.2318e-09
14.663,1.3379e-08,3.2448e-09
14.666,1.3409e-08,3.2566e-09
14.669,1.3438e-08,3.2771e-09
14.672,1.3465e-08,3.2822e-09
14.675,1.3498e-08,3.3e-09
14.678,1.3524e-08,3.3089e-09
14.681,1.3561e-08,3.3168e-09
14.684,1.3589e-08,3.3414e-09
14.687,1.3615e-08,3.349e-09
14.69,1.3641e-08,3.3666e-09
14.693,1.3664e-08,3.3779e-09
14.696,1.3697e-08,3.3908e-09
14.699,1.3727e-08,3.4045e-09
14.702,1.3757e-08,3.408e-09
14.705,1.3786e-08,3.4225e-09
14.708,1.3822e-08,3.4465e-09
14.711,1.385e-08,3.4564e-09
14.714,1.3876e-08,3.4682e-09
14.717,1.3916e-08,3.4777e-09
14.72,1.3942e-08,3.4953e-09
14.723,1.3969e-08,3.5173e-09
14.726,1.4001e-08,3.5276e-09
14.729,1.4036e-08,3.5403e-09
14.732,1.4067e-08,3.5509e-09
14.735,1.4078e-08,3.5694e-09
14.738,1.4121e-08,3.572e-09
14.741,1.4149e-08,3.5956e-09
14.744,1.4191e-08,3.6019e-09
14.747,1.422e-08,3.6241e-09
14.75,1.4245e-08,3.632e-09
14.753,1.4269e-08,3.6474e-09
14.756,1.4313e-08,3.6747e-09
14.759,1.4322e-08,3.684e-09
14.762,1.4365e-08,3.69e-09
14.765,1.4401e-08,3.711e-09
14.768,1.4425e-08,3.7171e-09
14.77,1.446e-08,3.7344e-09
14.773,1.4482e-08,3.7521e-09
14.776,1.4529e-08,3.7566e-09
14.779,1.4554e-08,3.7779e-09
14.782,1.458e-08,3.7871e-09
14.785,1.4618e-08,3.812e-09
14.788,1.4649e-08,3.8215e-09
14.791,1.468e-08,3.8387e-09
14.794,1.4701e-08,3.8598e-09
14.797,1.4738e-08,3.8604e-09
14.8,1.4774e-08,3.8847e-09
14.803,1.4795e-08,3.8858e-09
14.806,1.4838e-08,3.9119e-09
14.809,1.4872e-08,3.9267e-09
14.812,1.4896e-08,3.9338e-09
14.815,1.4928e-08,3.9636e-09
14.818,1.4962e-08,3.9767e-09
14.821,1.4996e-08,3.9857e-09
14.824,1.5029e-08,3.9931e-09
14.827,1.5056e-08,4.0156e-09
14.83,1.5089e-08,4.0304e-09
14.833,1.5123e-08,4.0349e-09
14.836,1.5148e-08,4.0686e-09
14.839,1.5183e-08,4.0791e-09
14.842,1.5233e-08,4.095e-09
14.845,1.5251e-08,4.1048e-09
14.848,1.5284e-08,4.1243e-09
14.851,1.5324e-08,4.1486e-09
14.854,1.5347e-08,4.1539e-09
14.857,1.5389e-08,4.1653e-09
14.86,1.541e-08,4.187e-09
14.863,1.5441e-08,4.215e-09
14.866,1.5474e-08,4.2136e-09
14.869,1.551e-08,4.2215e-09
14.872,1.5554e-08,4.2393e-09
14.875,1.5576e-08,4.258e-09
14.878,1.5617e-08,4.2952e-09
14.881,1.5655e-08,4.3124e-09
14.884,1.5681e-08,4.3174e-09
14.887,1.5719e-08,4.3358e-09
14.89,1.5754e-08,4.3507e-09
14.893,1.5775e-08,4.3633e-09
14.896,1.5828e-08,4.3879e-09
14.899,1.5854e-08,4.401e-09
14.902,1.5884e-08,4.4063e-09
14.905,1.5917e-08,4.4212e-09
14.908,1.5968e-08,4.4388e-09
14.911,1.5988e-08,4.4555e-09
14.914,1.6025e-08,4.4918e-09
14.917,1.6057e-08,4.4909e-09
14.92,1.6093e-08,4.5091e-09
14.923,1.6112e-08,4.5255e-09
14.925,1.6165e-08,4.5489e-09
14.928,1.621e-08,4.5468e-09
14.931,1.6238e-08,4.5764e-09
14.934,1.6252e-08,4.5907e-09
14.937,1.6288e-08,4.5994e-09
14.94,1.6324e-08,4.6379e-09
14.943,1.6352e-08,4.6467e-09
14.946,1.6393e-08,4.6751e-09
14.949,1.6436e-08,4.6758e-09
14.952,1.6465e-08,4.7088e-09
14.955,1.6499e-08,4.7166e-09
14.958,1.6547e-08,4.7352e-09
14.961,1.657e-08,4.7492e-09
14.964,1.6603e-08,4.7561e-09
14.967,1.6654e-08,4.7795e-09
14.97,1.6675e-08,4.8e-09
14.973,1.6718e-08,4.8137e-09
14.976,1.6757e-08,4.8477e-09
14.979,1.6777e-08,4.8628e-09
14.982,1.6832e-08,4.8761e-09
14.985,1.6869e-08,4.8997e-09
14.988,1.6901e-08,4.9169e-09
14.991,1.6933e-08,4.928e-09
14.994,1.6959e-08,4.955e-09
14.997,1.7014e-08,4.9659e-09
15,1.7027e-08,4.9831e-09


==> quad_sing_err_logfunc.tex <==
0,8.771e-13
0.001001,7.6841e-13
0.002002,6.6584e-13
0.003003,5.6937e-13
0.004004,4.7885e-13
0.005005,3.9307e-13
0.006006,3.1308e-13
0.007007,2.3783e-13
0.008008,1.6731e-13
0.009009,1.0151e-13
0.01001,3.9996e-14
0.011011,1.725e-14
0.012012,7.0987e-14
0.013013,1.2091e-13
0.014014,1.6702e-13
0.015015,2.1007e-13
0.016016,2.4962e-13
0.017017,2.8642e-13
0.018018,3.2001e-13
0.019019,3.5117e-13
0.02002,3.7942e-13
0.021021,4.0524e-13
0.022022,4.2907e-13
0.023023,4.5031e-13
0.024024,4.6926e-13
0.025025,4.8637e-13
0.026026,5.0151e-13
0.027027,5.1481e-13
0.028028,5.2689e-13
0.029029,5.3669e-13
0.03003,5.4541e-13
0.031031,5.5261e-13
0.032032,5.5813e-13
0.033033,5.6243e-13
0.034034,5.6628e-13
0.035035,5.6829e-13
0.036036,5.6938e-13
0.037037,5.6925e-13
0.038038,5.6882e-13
0.039039,5.6686e-13
0.04004,5.6445e-13
0.041041,5.6111e-13
0.042042,5.5717e-13
0.043043,5.5261e-13
0.044044,5.4744e-13
0.045045,5.4121e-13
0.046046,5.3497e-13
0.047047,5.2797e-13
0.048048,5.2097e-13
0.049049,5.132e-13
0.05005,5.0528e-13
0.051051,4.9675e-13
0.052052,4.8791e-13
0.053053,4.7861e-13
0.054054,4.6947e-13
0.055055,4.6017e-13
0.056056,4.5026e-13
0.057057,4.405e-13
0.058058,4.3059e-13
0.059059,4.2006e-13
0.06006,4.0984e-13
0.061061,3.9962e-13
0.062062,3.8909e-13
0.063063,3.7825e-13
0.064064,3.6787e-13
0.065065,3.5719e-13
0.066066,3.4666e-13
0.067067,3.3612e-13
0.068068,3.2574e-13
0.069069,3.1489e-13
0.07007,3.0436e-13
0.071071,2.9366e-13
0.072072,2.8327e-13
0.073073,2.7273e-13
0.074074,2.6249e-13
0.075075,2.524e-13
0.076076,2.4216e-13
0.077077,2.3207e-13
0.078078,2.2214e-13
0.079079,2.122e-13
0.08008,2.0272e-13
0.081081,1.9308e-13
0.082082,1.8375e-13
0.083083,1.7411e-13
0.084084,1.6508e-13
0.085085,1.559e-13
0.086086,1.4671e-13
0.087087,1.3814e-13
0.088088,1.2926e-13
0.089089,1.2069e-13
0.09009,1.1257e-13
0.091091,1.043e-13
0.092092,9.6025e-14
0.093093,8.8057e-14
0.094094,8.0088e-14
0.095095,7.2577e-14
0.096096,6.5065e-14
0.097097,5.7705e-14
0.098098,5.0651e-14
0.099099,4.3441e-14
0.1001,3.6384e-14
0.1011,2.9786e-14
0.1021,2.3033e-14
0.1031,1.6739e-14
0.1041,1.0444e-14
0.10511,4.3008e-15
0.10611,1.8434e-15
0.10711,7.6817e-15
0.10811,1.3521e-14
0.10911,1.9208e-14
0.11011,2.4743e-14
0.11111,2.9818e-14
0.11211,3.5048e-14
0.11311,4.0279e-14
0.11411,4.5204e-14
0.11512,5.0129e-14
0.11612,5.4595e-14
0.11712,5.9216e-14
0.11812,6.3376e-14
0.11912,6.7691e-14
0.12012,7.2161e-14
0.12112,7.6016e-14
0.12212,8.0027e-14
0.12312,8.3731e-14
0.12412,8.7743e-14
0.12513,9.1141e-14
0.12613,9.4385e-14
0.12713,9.7631e-14
0.12813,1.0088e-13
0.12913,1.0412e-13
0.13013,1.0722e-13
0.13113,1.1e-13
0.13213,1.1295e-13
0.13313,1.1543e-13
0.13413,1.1822e-13
0.13514,1.2085e-13
0.13614,1.2333e-13
0.13714,1.2566e-13
0.13814,1.2784e-13
0.13914,1.2986e-13
0.14014,1.3204e-13
0.14114,1.3406e-13
0.14214,1.3593e-13
0.14314,1.378e-13
0.14414,1.3951e-13
0.14515,1.4123e-13
0.14615,1.4295e-13
0.14715,1.4436e-13
0.14815,1.4607e-13
0.14915,1.4748e-13
0.15015,1.4889e-13
0.15115,1.4984e-13
0.15215,1.511e-13
0.15315,1.5205e-13
0.15415,1.533e-13
0.15516,1.5456e-13
0.15616,1.552e-13
0.15716,1.5646e-13
0.15816,1.5726e-13
0.15916,1.5774e-13
0.16016,1.5869e-13
0.16116,1.5933e-13
0.16216,1.6013e-13
0.16316,1.6062e-13
0.16416,1.6111e-13
0.16517,1.6159e-13
0.16617,1.6193e-13
0.16717,1.6257e-13
0.16817,1.629e-13
0.16917,1.6324e-13
0.17017,1.6342e-13
0.17117,1.6406e-13
0.17217,1.6393e-13
0.17317,1.6426e-13
0.17417,1.6444e-13
0.17518,1.6447e-13
0.17618,1.6465e-13
0.17718,1.6436e-13
0.17818,1.6439e-13
0.17918,1.6488e-13
0.18018,1.6444e-13
0.18118,1.6431e-13
0.18218,1.6449e-13
0.18318,1.6405e-13
0.18418,1.6407e-13
0.18519,1.6394e-13
0.18619,1.6366e-13
0.18719,1.6353e-13
0.18819,1.6309e-13
0.18919,1.6312e-13
0.19019,1.6221e-13
0.19119,1.6239e-13
0.19219,1.6226e-13
0.19319,1.6166e-13
0.19419,1.6138e-13
0.1952,1.6094e-13
0.1962,1.6081e-13
0.1972,1.6021e-13
0.1982,1.5977e-13
0.1992,1.5917e-13
0.2002,1.5905e-13
0.2012,1.5845e-13
0.2022,1.5816e-13
0.2032,1.5741e-13
0.2042,1.5712e-13
0.20521,1.5668e-13
0.20621,1.5624e-13
0.20721,1.5564e-13
0.20821,1.552e-13
0.20921,1.5445e-13
0.21021,1.5401e-13
0.21121,1.5341e-13
0.21221,1.5281e-13
0.21321,1.5221e-13
0.21421,1.5161e-13
0.21522,1.5133e-13
0.21622,1.5057e-13
0.21722,1.4982e-13
0.21822,1.4906e-13
0.21922,1.4878e-13
0.22022,1.4802e-13
0.22122,1.4742e-13
0.22222,1.4698e-13
0.22322,1.4622e-13
0.22422,1.4562e-13
0.22523,1.4487e-13
0.22623,1.4427e-13
0.22723,1.4351e-13
0.22823,1.4307e-13
0.22923,1.4278e-13
0.23023,1.4202e-13
0.23123,1.4142e-13
0.23223,1.4066e-13
0.23323,1.4006e-13
0.23423,1.3899e-13
0.23524,1.387e-13
0.23624,1.381e-13
0.23724,1.3718e-13
0.23824,1.369e-13
0.23924,1.3629e-13
0.24024,1.3553e-13
0.24124,1.3509e-13
0.24224,1.3448e-13
0.24324,1.3388e-13
0.24424,1.3328e-13
0.24525,1.3268e-13
0.24625,1.3176e-13
0.24725,1.3147e-13
0.24825,1.3086e-13
0.24925,1.3026e-13
0.25025,1.2966e-13
0.25125,1.2905e-13
0.25225,1.2829e-13
0.25325,1.2768e-13
0.25425,1.2708e-13
0.25526,1.2632e-13
0.25626,1.2587e-13
0.25726,1.2542e-13
0.25826,1.2481e-13
0.25926,1.2405e-13
0.26026,1.236e-13
0.26126,1.2315e-13
0.26226,1.2239e-13
0.26326,1.221e-13
0.26426,1.2118e-13
0.26527,1.2073e-13
0.26627,1.2028e-13
0.26727,1.1951e-13
0.26827,1.1938e-13
0.26927,1.1877e-13
0.27027,1.18e-13
0.27127,1.1755e-13
0.27227,1.1726e-13
0.27327,1.1649e-13
0.27427,1.1604e-13
0.27528,1.1543e-13
0.27628,1.1514e-13
0.27728,1.1469e-13
0.27828,1.1392e-13
0.27928,1.1347e-13
0.28028,1.1302e-13
0.28128,1.1241e-13
0.28228,1.1195e-13
0.28328,1.1166e-13
0.28428,1.1105e-13
0.28529,1.106e-13
0.28629,1.103e-13
0.28729,1.1001e-13
0.28829,1.094e-13
0.28929,1.0878e-13
0.29029,1.0849e-13
0.29129,1.0819e-13
0.29229,1.0758e-13
0.29329,1.0697e-13
0.29429,1.0683e-13
0.2953,1.0622e-13
0.2963,1.0592e-13
0.2973,1.0563e-13
0.2983,1.0517e-13
0.2993,1.044e-13
0.3003,1.0426e-13
0.3013,1.0397e-13
0.3023,1.0367e-13
0.3033,1.0306e-13
0.3043,1.0292e-13
0.30531,1.023e-13
0.30631,1.0201e-13
0.30731,1.0187e-13
0.30831,1.0157e-13
0.30931,1.0096e-13
0.31031,1.005e-13
0.31131,1.0036e-13
0.31231,9.9903e-14
0.31331,9.9447e-14
0.31431,9.9307e-14
0.31532,9.9168e-14
0.31632,9.8552e-14
0.31732,9.8413e-14
0.31832,9.8114e-14
0.31932,9.7816e-14
0.32032,9.7676e-14
0.32132,9.7377e-14
0.32232,9.6919e-14
0.32332,9.678e-14
0.32432,9.6481e-14
0.32533,9.6182e-14
0.32633,9.5882e-14
0.32733,9.5583e-14
0.32833,9.5284e-14
0.32933,9.5143e-14
0.33033,9.4844e-14
0.33133,9.4703e-14
0.33233,9.4563e-14
0.33333,9.4104e-14
0.33433,9.4282e-14
0.33534,9.3663e-14
0.33634,9.3522e-14
0.33734,9.3382e-14
0.33834,9.3081e-14
0.33934,9.2781e-14
0.34034,9.264e-14
0.34134,9.2499e-14
0.34234,9.2199e-14
0.34334,9.2058e-14
0.34434,9.1916e-14
0.34535,9.1775e-14
0.34635,9.1314e-14
0.34735,9.1493e-14
0.34835,9.1192e-14
0.34935,9.0891e-14
0.35035,9.0909e-14
0.35135,9.0608e-14
0.35235,9.0306e-14
0.35335,9.0325e-14
0.35435,9.0183e-14
0.35536,8.9881e-14
0.35636,8.974e-14
0.35736,8.9758e-14
0.35836,8.9616e-14
0.35936,8.9314e-14
0.36036,8.9012e-14
0.36136,8.9191e-14
0.36236,8.9049e-14
0.36336,8.9067e-14
0.36436,8.8765e-14
0.36537,8.8783e-14
0.36637,8.8962e-14
0.36737,8.8659e-14
0.36837,8.8678e-14
0.36937,8.8375e-14
0.37037,8.8393e-14
0.37137,8.809e-14
0.37237,8.8109e-14
0.37337,8.7966e-14
0.37437,8.8146e-14
0.37538,8.8003e-14
0.37638,8.7539e-14
0.37738,8.7557e-14
0.37838,8.7575e-14
0.37938,8.7594e-14
0.38038,8.7612e-14
0.38138,8.7631e-14
0.38238,8.7649e-14
0.38338,8.7345e-14
0.38438,8.7202e-14
0.38539,8.7382e-14
0.38639,8.74e-14
0.38739,8.7096e-14
0.38839,8.7276e-14
0.38939,8.7133e-14
0.39039,8.7151e-14
0.39139,8.717e-14
0.39239,8.7188e-14
0.39339,8.7045e-14
0.39439,8.7225e-14
0.3954,8.7082e-14
0.3964,8.6777e-14
0.3974,8.7119e-14
0.3984,8.6976e-14
0.3994,8.6994e-14
0.4004,8.7175e-14
0.4014,8.6708e-14
0.4024,8.7212e-14
0.4034,8.7068e-14
0.4044,8.7087e-14
0.40541,8.6944e-14
0.40641,8.7124e-14
0.40741,8.7143e-14
0.40841,8.7161e-14
0.40941,8.718e-14
0.41041,8.7199e-14
0.41141,8.7217e-14
0.41241,8.7236e-14
0.41341,8.7417e-14
0.41441,8.7436e-14
0.41542,8.7292e-14
0.41642,8.7311e-14
0.41742,8.7654e-14
0.41842,8.7348e-14
0.41942,8.7529e-14
0.42042,8.7548e-14
0.42142,8.7567e-14
0.42242,8.7748e-14
0.42342,8.7767e-14
0.42442,8.7786e-14
0.42543,8.7805e-14
0.42643,8.7661e-14
0.42743,8.7843e-14
0.42843,8.8187e-14
0.42943,8.8043e-14
0.43043,8.8062e-14
0.43143,8.8407e-14
0.43243,8.8426e-14
0.43343,8.8282e-14
0.43443,8.8301e-14
0.43544,8.8484e-14
0.43644,8.8666e-14
0.43744,8.8685e-14
0.43844,8.8704e-14
0.43944,8.8886e-14
0.44044,8.9069e-14
0.44144,8.9251e-14
0.44244,8.9107e-14
0.44344,8.9127e-14
0.44444,8.9146e-14
0.44545,8.9492e-14
0.44645,8.9348e-14
0.44745,8.9858e-14
0.44845,8.9877e-14
0.44945,8.9897e-14
0.45045,8.9753e-14
0.45145,9.0099e-14
0.45245,9.0283e-14
0.45345,9.0139e-14
0.45445,9.0486e-14
0.45546,9.0342e-14
0.45646,9.0689e-14
0.45746,9.0709e-14
0.45846,9.0892e-14
0.45946,9.0748e-14
0.46046,9.1096e-14
0.46146,9.1115e-14
0.46246,9.1135e-14
0.46346,9.1483e-14
0.46446,9.1503e-14
0.46547,9.1851e-14
0.46647,9.1871e-14
0.46747,9.1727e-14
0.46847,9.1912e-14
0.46947,9.226e-14
0.47047,9.228e-14
0.47147,9.23e-14
0.47247,9.2649e-14
0.47347,9.2834e-14
0.47447,9.3019e-14
0.47548,9.3203e-14
0.47648,9.2895e-14
0.47748,9.3409e-14
0.47848,9.3429e-14
0.47948,9.345e-14
0.48048,9.3635e-14
0.48148,9.382e-14
0.48248,9.3841e-14
0.48348,9.4191e-14
0.48448,9.4211e-14
0.48549,9.4562e-14
0.48649,9.4582e-14
0.48749,9.4768e-14
0.48849,9.4954e-14
0.48949,9.5304e-14
0.49049,9.549e-14
0.49149,9.5346e-14
0.49249,9.5367e-14
0.49349,9.5718e-14
0.49449,9.574e-14
0.4955,9.5926e-14
0.4965,9.6112e-14
0.4975,9.6464e-14
0.4985,9.6815e-14
0.4995,9.6506e-14
0.5005,9.6858e-14
0.5015,9.7045e-14
0.5025,9.6901e-14
0.5035,9.7253e-14
0.5045,9.7771e-14
0.50551,9.7792e-14
0.50651,9.7649e-14
0.50751,9.8001e-14
0.50851,9.8189e-14
0.50951,9.8376e-14
0.51051,9.8398e-14
0.51151,9.8751e-14
0.51251,9.8607e-14
0.51351,9.8795e-14
0.51451,9.948e-14
0.51552,9.9336e-14
0.51652,9.9358e-14
0.51752,9.9546e-14
0.51852,1.0007e-13
0.51952,1.0009e-13
0.52052,1.0028e-13
0.52152,1.003e-13
0.52252,1.0049e-13
0.52352,1.0084e-13
0.52452,1.0086e-13
0.52553,1.0122e-13
0.52653,1.0124e-13
0.52753,1.0143e-13
0.52853,1.0178e-13
0.52953,1.0181e-13
0.53053,1.0216e-13
0.53153,1.0235e-13
0.53253,1.0254e-13
0.53353,1.0273e-13
0.53453,1.0259e-13
0.53554,1.0328e-13
0.53654,1.033e-13
0.53754,1.0349e-13
0.53854,1.0368e-13
0.53954,1.037e-13
0.54054,1.0406e-13
0.54154,1.0425e-13
0.54254,1.0444e-13
0.54354,1.0463e-13
0.54454,1.0465e-13
0.54555,1.0501e-13
0.54655,1.0503e-13
0.54755,1.0522e-13
0.54855,1.0558e-13
0.54955,1.0594e-13
0.55055,1.0596e-13
0.55155,1.0632e-13
0.55255,1.0634e-13
0.55355,1.067e-13
0.55455,1.0689e-13
0.55556,1.0708e-13
0.55656,1.0727e-13
0.55756,1.073e-13
0.55856,1.0782e-13
0.55956,1.0768e-13
0.56056,1.0787e-13
0.56156,1.0823e-13
0.56256,1.0809e-13
0.56356,1.0828e-13
0.56456,1.0864e-13
0.56557,1.0883e-13
0.56657,1.0936e-13
0.56757,1.0905e-13
0.56857,1.0957e-13
0.56957,1.0993e-13
0.57057,1.0979e-13
0.57157,1.0982e-13
0.57257,1.1018e-13
0.57357,1.1087e-13
0.57457,1.1073e-13
0.57558,1.1109e-13
0.57658,1.1095e-13
0.57758,1.1131e-13
0.57858,1.1133e-13
0.57958,1.1169e-13
0.58058,1.1206e-13
0.58158,1.1208e-13
0.58258,1.1244e-13
0.58358,1.128e-13
0.58458,1.13e-13
0.58559,1.1285e-13
0.58659,1.1338e-13
0.58759,1.1358e-13
0.58859,1.136e-13
0.58959,1.138e-13
0.59059,1.1399e-13
0.59159,1.1435e-13
0.59259,1.1472e-13
0.59359,1.1491e-13
0.59459,1.1511e-13
0.5956,1.1513e-13
0.5966,1.155e-13
0.5976,1.1569e-13
0.5986,1.1555e-13
0.5996,1.1591e-13
0.6006,1.1627e-13
0.6016,1.1613e-13
0.6026,1.1666e-13
0.6036,1.1686e-13
0.6046,1.1705e-13
0.60561,1.1708e-13
0.60661,1.1745e-13
0.60761,1.1747e-13
0.60861,1.1784e-13
0.60961,1.1786e-13
0.61061,1.1823e-13
0.61161,1.1842e-13
0.61261,1.1862e-13
0.61361,1.1865e-13
0.61461,1.1901e-13
0.61562,1.1921e-13
0.61662,1.1974e-13
0.61762,1.1977e-13
0.61862,1.198e-13
0.61962,1.2016e-13
0.62062,1.2019e-13
0.62162,1.209e-13
0.62262,1.2109e-13
0.62362,1.2061e-13
0.62462,1.2115e-13
0.62563,1.2117e-13
0.62663,1.2154e-13
0.62763,1.2174e-13
0.62863,1.2176e-13
0.62963,1.223e-13
0.63063,1.225e-13
0.63163,1.2253e-13
0.63263,1.2307e-13
0.63363,1.2326e-13
0.63463,1.2329e-13
0.63564,1.2366e-13
0.63664,1.2369e-13
0.63764,1.2405e-13
0.63864,1.2425e-13
0.63964,1.2428e-13
0.64064,1.2448e-13
0.64164,1.2468e-13
0.64264,1.2522e-13
0.64364,1.249e-13
0.64464,1.2561e-13
0.64565,1.253e-13
0.64665,1.2567e-13
0.64765,1.2604e-13
0.64865,1.2641e-13
0.64965,1.2661e-13
0.65065,1.2681e-13
0.65165,1.2718e-13
0.65265,1.2703e-13
0.65365,1.2723e-13
0.65465,1.2795e-13
0.65566,1.2763e-13
0.65666,1.2817e-13
0.65766,1.2837e-13
0.65866,1.284e-13
0.65966,1.2877e-13
0.66066,1.2897e-13
0.66166,1.2935e-13
0.66266,1.2937e-13
0.66366,1.2992e-13
0.66466,1.2995e-13
0.66567,1.2998e-13
0.66667,1.3035e-13
0.66767,1.3055e-13
0.66867,1.3058e-13
0.66967,1.3095e-13
0.67067,1.3115e-13
0.67167,1.3118e-13
0.67267,1.3155e-13
0.67367,1.3158e-13
0.67467,1.3213e-13
0.67568,1.3233e-13
0.67668,1.3253e-13
0.67768,1.3273e-13
0.67868,1.3276e-13
0.67968,1.3331e-13
0.68068,1.3316e-13
0.68168,1.3336e-13
0.68268,1.3391e-13
0.68368,1.3394e-13
0.68468,1.3431e-13
0.68569,1.3434e-13
0.68669,1.3455e-13
0.68769,1.3492e-13
0.68869,1.353e-13
0.68969,1.355e-13
0.69069,1.3536e-13
0.69169,1.3556e-13
0.69269,1.3611e-13
0.69369,1.3596e-13
0.69469,1.3634e-13
0.6957,1.3671e-13
0.6967,1.3674e-13
0.6977,1.3678e-13
0.6987,1.3715e-13
0.6997,1.3787e-13
0.7007,1.379e-13
0.7017,1.3776e-13
0.7027,1.3796e-13
0.7037,1.3834e-13
0.7047,1.3854e-13
0.70571,1.3909e-13
0.70671,1.3895e-13
0.70771,1.3916e-13
0.70871,1.3936e-13
0.70971,1.3991e-13
0.71071,1.3994e-13
0.71171,1.4015e-13
0.71271,1.4035e-13
0.71371,1.4073e-13
0.71471,1.4076e-13
0.71572,1.4079e-13
0.71672,1.4117e-13
0.71772,1.4137e-13
0.71872,1.4192e-13
0.71972,1.4213e-13
0.72072,1.4233e-13
0.72172,1.4271e-13
0.72272,1.4257e-13
0.72372,1.4312e-13
0.72472,1.4316e-13
0.72573,1.4353e-13
0.72673,1.4322e-13
0.72773,1.4377e-13
0.72873,1.4398e-13
0.72973,1.4401e-13
0.73073,1.4456e-13
0.73173,1.4442e-13
0.73273,1.448e-13
0.73373,1.4483e-13
0.73473,1.4521e-13
0.73574,1.4542e-13
0.73674,1.4563e-13
0.73774,1.4583e-13
0.73874,1.4604e-13
0.73974,1.4659e-13
0.74074,1.468e-13
0.74174,1.4683e-13
0.74274,1.4687e-13
0.74374,1.4742e-13
0.74474,1.478e-13
0.74575,1.4766e-13
0.74675,1.4804e-13
0.74775,1.4825e-13
0.74875,1.4846e-13
0.74975,1.4884e-13
0.75075,1.4905e-13
0.75175,1.4908e-13
0.75275,1.4964e-13
0.75375,1.495e-13
0.75475,1.497e-13
0.75576,1.5009e-13
0.75676,1.5029e-13
0.75776,1.505e-13
0.75876,1.5089e-13
0.75976,1.5092e-13
0.76076,1.5113e-13
0.76176,1.5134e-13
0.76276,1.5172e-13
0.76376,1.521e-13
0.76476,1.5214e-13
0.76577,1.5252e-13
0.76677,1.5255e-13
0.76777,1.5294e-13
0.76877,1.5315e-13
0.76977,1.5301e-13
0.77077,1.5357e-13
0.77177,1.5377e-13
0.77277,1.5416e-13
0.77377,1.5419e-13
0.77477,1.5423e-13
0.77578,1.5461e-13
0.77678,1.55e-13
0.77778,1.5503e-13
0.77878,1.5524e-13
0.77978,1.558e-13
0.78078,1.5584e-13
0.78178,1.5622e-13
0.78278,1.5626e-13
0.78378,1.5629e-13
0.78478,1.5668e-13
0.78579,1.5707e-13
0.78679,1.5728e-13
0.78779,1.5749e-13
0.78879,1.5787e-13
0.78979,1.5791e-13
0.79079,1.5812e-13
0.79179,1.5833e-13
0.79279,1.5836e-13
0.79379,1.5893e-13
0.79479,1.5914e-13
0.7958,1.5953e-13
0.7968,1.5956e-13
0.7978,1.5995e-13
0.7988,1.5998e-13
0.7998,1.6002e-13
0.8008,1.6076e-13
0.8018,1.608e-13
0.8028,1.6083e-13
0.8038,1.614e-13
0.8048,1.6161e-13
0.80581,1.6182e-13
0.80681,1.6203e-13
0.80781,1.6207e-13
0.80881,1.6246e-13
0.80981,1.6249e-13
0.81081,1.6306e-13
0.81181,1.6292e-13
0.81281,1.6295e-13
0.81381,1.637e-13
0.81481,1.6373e-13
0.81582,1.6412e-13
0.81682,1.6434e-13
0.81782,1.6455e-13
0.81882,1.6459e-13
0.81982,1.6515e-13
0.82082,1.6519e-13
0.82182,1.6523e-13
0.82282,1.6544e-13
0.82382,1.6601e-13
0.82482,1.6622e-13
0.82583,1.6661e-13
0.82683,1.6665e-13
0.82783,1.6686e-13
0.82883,1.6708e-13
0.82983,1.6747e-13
0.83083,1.6733e-13
0.83183,1.6772e-13
0.83283,1.6811e-13
0.83383,1.6833e-13
0.83483,1.6854e-13
0.83584,1.6893e-13
0.83684,1.6915e-13
0.83784,1.6918e-13
0.83884,1.6958e-13
0.83984,1.6979e-13
0.84084,1.7001e-13
0.84184,1.704e-13
0.84284,1.7044e-13
0.84384,1.7047e-13
0.84484,1.7122e-13
0.84585,1.7108e-13
0.84685,1.7148e-13
0.84785,1.7151e-13
0.84885,1.7173e-13
0.84985,1.7212e-13
0.85085,1.7252e-13
0.85185,1.7238e-13
0.85285,1.7295e-13
0.85385,1.7281e-13
0.85485,1.7338e-13
0.85586,1.736e-13
0.85686,1.7381e-13
0.85786,1.7385e-13
0.85886,1.7407e-13
0.85986,1.7464e-13
0.86086,1.7504e-13
0.86186,1.749e-13
0.86286,1.7511e-13
0.86386,1.7551e-13
0.86486,1.7591e-13
0.86587,1.7612e-13
0.86687,1.7616e-13
0.86787,1.7638e-13
0.86887,1.7677e-13
0.86987,1.7681e-13
0.87087,1.7739e-13
0.87187,1.7761e-13
0.87287,1.7764e-13
0.87387,1.7786e-13
0.87487,1.7826e-13
0.87588,1.7812e-13
0.87688,1.7852e-13
0.87788,1.7855e-13
0.87888,1.7913e-13
0.87988,1.7953e-13
0.88088,1.7993e-13
0.88188,1.7997e-13
0.88288,1.8018e-13
0.88388,1.8022e-13
0.88488,1.808e-13
0.88589,1.8102e-13
0.88689,1.8124e-13
0.88789,1.8146e-13
0.88889,1.8186e-13
0.88989,1.8172e-13
0.89089,1.8193e-13
0.89189,1.8233e-13
0.89289,1.8237e-13
0.89389,1.8295e-13
0.89489,1.8317e-13
0.8959,1.8339e-13
0.8969,1.8361e-13
0.8979,1.8365e-13
0.8989,1.8405e-13
0.8999,1.8409e-13
0.9009,1.8449e-13
0.9019,1.8471e-13
0.9029,1.8511e-13
0.9039,1.8515e-13
0.9049,1.8555e-13
0.90591,1.8613e-13
0.90691,1.8617e-13
0.90791,1.8621e-13
0.90891,1.8661e-13
0.90991,1.8683e-13
0.91091,1.8705e-13
0.91191,1.8746e-13
0.91291,1.8713e-13
0.91391,1.8772e-13
0.91491,1.8794e-13
0.91592,1.8816e-13
0.91692,1.8838e-13
0.91792,1.8878e-13
0.91892,1.89e-13
0.91992,1.8886e-13
0.92092,1.8945e-13
0.92192,1.8985e-13
0.92292,1.8989e-13
0.92392,1.9029e-13
0.92492,1.9052e-13
0.92593,1.9056e-13
0.92693,1.9096e-13
0.92793,1.91e-13
0.92893,1.9158e-13
0.92993,1.9144e-13
0.93093,1.9185e-13
0.93193,1.9225e-13
0.93293,1.9247e-13
0.93393,1.9252e-13
0.93493,1.931e-13
0.93594,1.9296e-13
0.93694,1.9318e-13
0.93794,1.9322e-13
0.93894,1.9363e-13
0.93994,1.9422e-13
0.94094,1.9444e-13
0.94194,1.9466e-13
0.94294,1.9452e-13
0.94394,1.9511e-13
0.94494,1.9515e-13
0.94595,1.9537e-13
0.94695,1.9578e-13
0.94795,1.9582e-13
0.94895,1.9641e-13
0.94995,1.9645e-13
0.95095,1.9649e-13
0.95195,1.969e-13
0.95295,1.9712e-13
0.95395,1.9735e-13
0.95495,1.9739e-13
0.95596,1.9816e-13
0.95696,1.9802e-13
0.95796,1.9843e-13
0.95896,1.9883e-13
0.95996,1.9906e-13
0.96096,1.991e-13
0.96196,1.9932e-13
0.96296,1.9973e-13
0.96396,1.9977e-13
0.96496,2e-13
0.96597,2.0022e-13
0.96697,2.0045e-13
0.96797,2.0067e-13
0.96897,2.009e-13
0.96997,2.0131e-13
0.97097,2.0153e-13
0.97197,2.0194e-13
0.97297,2.0162e-13
0.97397,2.0221e-13
0.97497,2.0243e-13
0.97598,2.0266e-13
0.97698,2.0307e-13
0.97798,2.0293e-13
0.97898,2.0334e-13
0.97998,2.032e-13
0.98098,2.0397e-13
0.98198,2.042e-13
0.98298,2.0424e-13
0.98398,2.0465e-13
0.98498,2.047e-13
0.98599,2.0492e-13
0.98699,2.0515e-13
0.98799,2.0538e-13
0.98899,2.0542e-13
0.98999,2.0583e-13
0.99099,2.0606e-13
0.99199,2.0628e-13
0.99299,2.0651e-13
0.99399,2.0692e-13
0.99499,2.0715e-13
0.996,2.0756e-13
0.997,2.0742e-13
0.998,2.0783e-13
0.999,2.0806e-13
1,2.081e-13


==> quad_sing_errors.tex <==
1e-05,2.395e-07,3.7642e-05,0.00010023,0.00041356
1e-06,3.6829e-08,7.6524e-06,4.2376e-06,1.9428e-05
1e-07,1.946e-09,3.356e-07,3.5978e-07,1.9028e-06
1e-08,6.851e-10,5.0883e-08,5.3778e-08,3.2778e-07
1e-09,1.3953e-10,8.6784e-10,3.4518e-10,2.6788e-09
1e-10,8.0976e-11,1.1999e-11,6.1445e-11,2.3367e-10


==> quad_sing_errors_use_exact_int.tex <==
1e-05,1.0847e-06,7.1095e-06,7.198e-05,0.00033946
1e-06,1.1692e-07,7.6094e-06,2.6336e-07,3.762e-06
1e-07,7.9964e-10,1.4252e-08,3.1313e-08,2.0269e-07
1e-08,4.6237e-11,2.0927e-09,3.1095e-09,1.8167e-08
1e-09,6.7052e-12,6.4082e-11,4.5092e-10,2.954e-09
1e-10,1.22e-12,5.0069e-12,5.3592e-11,3.9149e-10


==> quad_sing_poles.tex <==
0.3795,1.9572
0.3795,-1.9572
-0.67031,1.1624
-0.67031,-1.1624
0.55695,0.89459
0.55695,-0.89459
0.84355,0.86239
0.84355,-0.86239
0.95167,0.55577
0.95167,-0.55577
1.0574,0.43361
1.0574,-0.43361
1.1487,0.32797
1.1487,-0.32797
1.2628,0
1.2497,0.1092
1.2497,-0.1092
1.2108,0.21878
1.2108,-0.21878
-0.3151,0
-0.11144,0
-0.046991,0
-0.020945,0
-0.0095706,0
-0.0044262,0
-0.0020564,0
-0.00095484,0
-0.00044136,0
-0.00020261,0
-9.2401e-05,0
-4.196e-05,0
-1.8988e-05,0
-8.5306e-06,0
-3.7752e-06,0
-1.6326e-06,0
-6.8802e-07,0
-2.8509e-07,0
-1.1895e-07,0
-5.1352e-08,0
5.782e-08,0
-2.3113e-08,0
-1.0676e-08,0
-4.9081e-09,0
-2.147e-09,0
-8.2294e-10,0
-2.2881e-10,0
-2.481e-11,0


==> quad_sing_sum_wghts.tex <==
1e-05,1
1e-06,1.0842
1e-07,1
1e-08,1.0264
1e-09,1.0002
1e-10,1.0146


==> quad_sing_sum_wghts_use_exact_int.tex <==
1e-05,3.2025
1e-06,2.936
1e-07,1.3545
1e-08,1.5522
1e-09,1.3816
1e-10,1.3036


==> quad_sing_supp_exact_int.tex <==
1e-08
1
0.0021526
0.90328
0.12074
0.98392
1.3901e-06
0.68039
3.1091e-05
0.37217
0.95405
0.01879
0.81051
0.00029576
7.1969e-08
0.2296
0.55002
0.99448
3.7276e-06
0.0068486
0.8637
1.3895e-07
0.054593
8.1562e-05
0.74511
1.3895e-08
0.93406
0.29785
7.5574e-06
0.00069196
0.47065
7.1969e-07
0.97194
0.03325
2.6827e-08
0.62083
0.08587
0.00015591
0.0042528
0.83775
5.1795e-07
0.17447
1.3626e-05
0.99805
3.7276e-08
0.42381
0.011682


==> quad_sing_wghts.tex <==
1e-08,0.00010921
1.9088e-08,-0.00035799
5.2719e-08,0.00053886
3.0465e-07,-0.00086964
1.3901e-06,0.0014833
4.4984e-06,-0.0013294
3.4693e-05,0.00093582
0.00025413,-0.00092251
0.00096194,0.0039218
0.0026114,-0.0027194
0.0062409,0.01333
0.012646,-0.0045857
0.02254,0.027973
0.056174,0.036229
0.083944,0.02357
0.11648,0.03631
0.15513,0.047584
0.2055,0.045743
0.25626,0.063512
0.32666,0.071687
0.39877,0.074761
0.47598,0.077467
0.55158,0.074519
0.62661,0.075053
0.69783,0.06413
0.74757,0.037058
0.78838,0.046933
0.82266,0.016705
0.84894,0.042046
0.89068,0.037931
0.92339,0.027912
0.94753,0.020534
0.96481,0.014593
0.97709,0.0096189
0.98599,0.0095978
0.99529,0.0076895
1,0.0013108


==> quad_sum_wghts.tex <==
1e-05,1
1e-06,1.0469
1e-07,1.0144
1e-08,1
1e-09,1
1e-10,1.0496


==> quad_sum_wghts_use_exact_int.tex <==
1e-05,2.4098
1e-06,5.8119
1e-07,3.0774
1e-08,1.9188
1e-09,1.7138
1e-10,1.7392


==> quad_supp_exact_int.tex <==
1
0.00054058
0.093872
0.93146
0.74818
3.7276e-08
0.0093978
0.98483
0.44809
1.3895e-06
0.84835
1.6686e-05
0.23085
0.61751
8.3034e-05
1e-08
0.0031956
0.96406
0.039654
0.33519
1.9307e-07
0.89174
3.5545e-06
0.15142
0.00022747
0.69123
0.020213
1.3895e-08
0.52999
3.7276e-07
0.9951
0.001238
7.1969e-06
0.80214
0.062478
3.5643e-05
5.1795e-08
0.388
0.0055824
0.94858
7.1969e-07
0.18966
7.1969e-08
0.00015017


==> quad_wghts.tex <==
1e-08,0.00056197
1.8874e-08,-0.0023997
3.5622e-08,0.0030729
1.269e-07,-0.0019793
8.5317e-07,0.0013543
9.8735e-06,-0.0020729
3.9494e-05,0.0031739
0.00023705,-0.0059249
0.00055528,0.0088088
0.0015667,-0.0043837
0.0056293,0.014942
0.010266,-0.0083965
0.019252,0.025146
0.04265,0.020488
0.068065,0.033043
0.10362,0.040939
0.16147,0.074555
0.24179,0.076296
0.29263,0.035666
0.34531,0.063459
0.40552,0.056237
0.45841,0.058383
0.53501,0.089738
0.62391,0.083014
0.69529,0.06038
0.75226,0.056185
0.80539,0.048468
0.8506,0.04344
0.89291,0.040904
0.93225,0.038132
0.94844,-0.0039272
0.96312,0.028902
0.98467,0.01484
0.99497,0.0073433
1,0.0016114


==> time_mLf.tex <==
2,0.828144
4,0.830153
6,0.805735
8,0.842653


==> time_paaa.tex <==
1,0.161692
2,0.590216
3,2.084436
4,4.197974
5,8.711397
6,14.423735
7,40.220558
8,45.133596
9,55.284441
10,64.232641
11,109.717166
12,124.762401
13,139.517301
14,147.178594
15,171.495153
16,182.735669
17,189.425051
18,195.60406
19,205.953439
20,209.620523
21,213.56083
22,233.239731
23,284.319266
24,301.953842
25,332.89819


==> time_qraaa.tex <==
3,0.198567
10,0.167276
15,0.205343
18,0.195937
25,0.221713

